Toward a Theory of Cyber Attacks

We provide a general methodology for analyzing defender-attacker based "games" in which we model such games as Markov models and introduce a capacity region to analyze how defensive and adversarial strategies impact security. Such a framework allows us to analyze under what kind of conditions we can prove statements (about an attack objective $k$) of the form "if the attacker has a time budget $T_{bud}$, then the probability that the attacker can reach an attack objective $\geq k$ is at most $poly(T_{bud})negl(k)$". We are interested in such rigorous cryptographic security guarantees (that describe worst-case guarantees) as these shed light on the requirements of a defender's strategy for preventing more and more the progress of an attack, in terms of the "learning rate" of a defender's strategy. We explain the damage an attacker can achieve by a "containment parameter" describing the maximally reached attack objective within a specific time window.

==> General_paper_S&P_Eprint/sections/SecAnalysis.tex <==
\subsection{Adversarial Containment} \label{AC-AC}

The goal of the adversary is to reach a winning state $(k,l)$ for some $l\geq 0$ within a limited time budget $T_{bud}$ in which $k$ represents the attack objective which is defined based on various attack scenarios\footnote{For instance, $k$ could be the total number of nodes the adversary wishes to compromise before using the collective of these nodes in the next attack phases (e.g., botnet applications).}, and time budget $T_{bud}$ expresses the number of transitions in the Markov model, i.e., the total number of adversarial moves.  

The objective of the defender is to learn more and more regarding the attack technologies (e.g., malicious attack payloads),  in order to be able to recognize and halt future moves by the attacker. That is, the defender hopes to push level $l$ -- the number of so far discovered adversarial moves-- higher and higher, leading to a higher probability $f(l)$ of successfully detecting and filtering a next adversarial action. The ultimate goal of the defender is to have a good enough learning mechanism in place such that the probability of reaching $k$ is negligible in $k$ (i.e., exponentially small in $k$) and only polynomial in $T_{bud}$. In other words, the adversary cannot reach a winning state in practice.

We define $w(k,T_{bud})$ as the probability of the adversary to reach a state $(k,l)$ for some $l\geq 0$ within time budget $T_{bud}$. In the next subsections we analyze this probability. We assume a parameter $p=p_i$ for all $i$, i.e., we simply give the adversary the advantage of using $p=\sup_i p_i$ instead of the smaller individual $p_i$ values. % and discuss the role of the $p_i$ in Section \ref{AC-role}. 
We want to find a tight upper bound and determine for which model parameters $\gamma$, $h$, $p$, and learning rate $f(l)$ the upper bound proves the desired asymptotic 
\begin{equation} w(k,T_{bud})=poly(T_{bud}) negl(k). \label{eq:as} \end{equation} 
 We notice that in this case, even though the adversary cannot reach a large $k$ because $w(k,T_{bud})$ is negligible in $k$, the adversary may reach a (much) smaller $k$. We are interested in the order of magnitude of this value as a sub-objective the adversary is able to reach. For this reason, we define $k_c$ as the solution of
$$ w(k_c, T_{bud}) =1/2.$$
For instance,  $k_c$ could reflect the order of magnitude of the number of compromised nodes to which the adversary is {\em contained}. By using $w(k,T_{bud})=poly(T_{bud}) negl(k)$ we can show\footnote{This implies that with significant probability the adversary can reach an attack objective at most $O(\log T_{bud})$ (e.g., compromising at most $O(\log T_{bud})$ nodes). Therefore, if the adversary would not have the advantage of using $p=\sup_i p_i$, then it would (compromise less nodes and) only use parameters $p_0, \ldots, p_{O(\log T_{bud})}$ in the Markov game. If these first few $p_i$ values do not differ much, then a constant $p$ becomes a realistic assumption which does not give the adversary that much advantage.}   `{\em containment parameter}' $k_c= O(\log T_{bud})$. 

Our analysis will show that for a stagnating learning rate (i.e., $1-f(l)$ remains larger than some constant $\tau>0$) the adversary cannot be contained ($w(k,T_{bud})$ does not follow the desired asymptotic). For a learning rate $f(l)\geq 1-O(1/l^2)$ which approaches $1$ fast enough, we are able to prove the desired asymptotic.
We also develop tight lower and upper bounds on $w(k,T_{bud})$ and show an efficient algorithm which is able to compute these bounds with $O(k\cdot T_{bud})$ complexity.
%  The next section evaluates other learning rates by using a dynamic programming approach developed in Section \ref{AC-dp}. 

%The proofs of each of the theorems will be available in an extended eprint.

\subsection{Time budget measured in real time}\label{Real_Time}

 We first discuss the effect of translating the time budget $T_{bud}$, measured in Markov model transitions, to a time budget which is measured in real time (seconds) as this makes sense in practice. If the adversary wins as soon as $k$ nodes are compromised and if each Markov model transition takes $\Delta$ seconds, then at most $k$ moves can be made by each of the compromised nodes {\em in parallel} in $\Delta$ seconds. With a time budget of $T$ seconds, this implies $T_{bud}\leq T k/\Delta$. This means that the desired asymptotic (\ref{eq:as}) translates into
$$ w(k,T_{bud})\leq poly(T k/ \Delta) negl(k).$$
This is $poly(T)negl(k)$ and again implies that in practice the adversary cannot reach $k$ since the probability of reaching $k$ is negligible in $k$ and only polynomial in the physical time budget $T$. 

%\emph{TO DO: COST, US dollars, How should we think of attack objective k and not only in the form of compromised nodes}
In some scenarios each adversarial move costs a certain amount, say $C$ USD, for example due to having to  rent a virtual machine in order to remotely launch or execute an attack move. In such a case the time budget $T_{bud}$, measured in Markov model transitions, directly translates into $C\cdot T_{bud}$, the amount of USD the adversary is restricted to. Such conversion allows one to reason about economically constrained adversaries.

\subsection{Stagnating learning rate} \label{stagnating}

Suppose that the learning rate stagnates in that $1-f(l)\geq \tau$ for some $\tau>0$. This means that $f(l)\leq 1-\tau$ and as a result at least a fraction $\tau$ goes undetected. 

\begin{theorem}[Stagnating learning rate]\label{Theo.stag}
	The attacker's probability $w(k,T_{bud})$ of winning   a game in which the defender's learning rate stagnates in that $1-f(l)\geq \tau$ is given by 
	\begin{equation}
w(k,T_{bud})% = [1-(1-\tau p)^{T_{bud}/k}]^{k} 
\geq 1-k(1-\tau p)^{T_{bud}/k}.
	\end{equation}
\end{theorem}

%\begin{corollary}
	For a stagnating learning rate, the attacker almost always wins the security game, i.e., $w(k, T_{bud})\approx 1$ even for relatively small time budgets $T_{bud}=c\cdot k$ for some multiplicative factor $c\geq 1$. This is because $1-w(k,T_{bud}) \leq k(1-\tau p)^{T_{bud}/k}$ is exponentially small in $T_{bud}/k=c$. 
%\end{corollary}
%This shows that $w(k, T_{bud})\approx 1$ for relatively small $T_{bud}$ because $1-w(k,T_{bud}) \leq k(m_1+m_4)^{T_{bud}/k}$ which is exponentially small in $T_{bud}$. 

%For example, $T_{bud}=lambda k ln k$ to get >=1- x^{-lambda} for some small x
% REAL TIME: Use f_i/(i+1) in the formula -- i.e. sum f_i/(i+1) is real time, take f_i = T_real / ln k, hence T_real = lambda (ln k)^2 is sufficient
In order to have the desired asymptotics (\ref{eq:as}), the learning rate should not stagnate, i.e., we need $1-f(l)\rightarrow 0$ for $l\rightarrow \infty$.

\subsection{Formula for $w(k,T_{bud})$}

The theorem below characterizes $w(k,T_{bud})$ in a closed form expression. In the next subsection, we show that neglecting the sum over $T$ of $B$ values leads to tight upper and lower bounds. The remaining sum over $A$ values turns out to correspond to a simpler Markov model which can be used to compute this sum in $O(k\cdot T_{bud})$ time using dynamic programming.

\begin{theorem}[Closed Form Winning Probability]\label{closedw}
The probability $w(k, T_{bud})$ of winning is equal to
$$\sum_{L=0}^{T_{bud}-1}\sum_{B=0}^{\min\{L,(k-1)\}}
  \frac{m_2(L)+m_3(L)}{1-m_1(L)} \cdot A 
 \cdot \sum_{T=0}^{(T_{bud}-1)-[(k-1)+L-B]} B $$
 with $A$ and $B$ substituted by
 \begin{eqnarray*}
 A &=&
 \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ \label{p-a}
					\sum_{l=1}^{L}b_l=B}}
\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg) \\
&& \cdot \sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\ \label{p-b}
					\sum_{l=0}^{L}(g_l-1)=(k-1)-B}}
  \prod_{l=0}^{L} \bigg( \frac{m_2(l)}{1-m_1(l)}\bigg)^{g_l-1} \mbox{, and } \\
  B &=&	\sum_{\substack{t_0,\dots,t_L s.t.\\ \label{p-c}
					\sum_{l=0}^{L}t_l=T}}
	\prod_{l=0}^{L}			{t_l+g_l-1 \choose t_l}
 m_1(l)^{t_l}(1-m_1(l))^{g_l}.
  \end{eqnarray*}
\end{theorem}

\subsection{Upper and Lower Bounds on $w(k, T_{bud})$} \label{AC-dp}

In the notation of Theorem \ref{closedw}, we define $\bar{w}$ as 
	\begin{eqnarray}
	\bar{w}(k,T_{bud}) % &=& (\ref{w-a}) \nonumber \\
	&=&
	\sum_{L=0}^{T_{bud}-1}\sum_{B=0}^{\min\{L,(k-1)\}} \frac{m_2(L)+m_3(L)}{1-m_1(L)}\cdot A. % (\ref{p-a})\cdot (\ref{p-b}).
	\label{UB}
	\end{eqnarray}

\begin{theorem}[Upper and Lower Bounds on $w$]\label{Theo.wbar}
	 For $v\geq k$, we have
	\begin{equation}
	 \bar{w}(k,T_{bud}/v)\cdot (1- (k + \frac{T_{bud}}{v}) (1-\gamma)^{\frac{v}{k}}) \leq w(k,T_{bud}) \leq \bar{w}(k,T_{bud}). \label{LB}
	\end{equation}
\end{theorem}

%By noticing that (\ref{w-b}) for $T_{bud}=\infty$ is equal to 1, a straightforward upper bound on $w(k,T_{bud})$ is given by just formula (\ref{w-a}): We have $w(k,T_{bud})$ is at most equal to 


%By using a proof strategy similar to the one used in Section \ref{stagnating} 

%We may lower bound (\ref{w-b}) as follows.
% For $v\leq T_{bud}/(L+1)$, we can show that
% {\footnotesize
%$$ (\ref{w-b}) \geq 1- \sum_{l=0}^{(T_{bud}/v)-1} k \cdot m_1(l)^{v/k}\geq 1- T_{bud} \frac{k}{v} (1-\gamma)^{\frac{v}{k}},$$
%}
%where the first inequality follows from a proof strategy similar to the one used in Section \ref{stagnating}, and the second inequality follows from $m_1(l)\leq 1-\gamma$.
%This lower bound on (\ref{w-b})  is independent of any of the other summing variables used in (\ref{w-a}) but requires $L< T_{bud}/v$. By restricting $L$ to be $<T_{bud}/v$ in (\ref{w-a}) (i.e., we substitute $T_{bud}$ by $T_{bud}/v$) we obtain a lower bound on $w(k,T_{bud})$:
%\begin{equation} w(k,T_{bud}) \geq \bar{w}(k,T_{bud}/v)\cdot (1- T_{bud} \frac{k}{v} (1-\gamma)^{\frac{v}{k}}). 
%\label{LB}
%\end{equation}
In particular for $v= k \ln ((T_{bud}+k)/\epsilon) / \ln (1/(1-\gamma))$, we have $w(k,T_{bud}) \geq \bar{w}(k,T_{bud}/v)\cdot (1-\epsilon)$. 
%
Upper bound  (\ref{UB}) proves that if $\bar{w}(k,T_{bud})$ has the desired complexity, i.e., $\bar{w}(k,T_{bud})=poly(T_{bud}) negl(k)$, then $w(k,T_{bud})$ inherits this desired asymptotics. And vice versa, the lower bound in (\ref{LB}) for the special choice of $v$ proves that if $w(k,T_{bud})$ has desired asymptotics $w(k,T_{bud})=poly(T_{bud}) negl(k)$, then also $\bar{w}(k,T_{bud}) \leq w(k, T_{bud}\cdot v)/(1-\epsilon) = poly(T_{bud} \cdot v)\cdot negl(k) = poly(T_{bud})negl(k)$. We conclude that in order to find out which learning rates lead to the desired asymptotics  for the defender, we only need to study which learning rates lead to $\bar{w}(k,T_{bud})=poly(T_{bud})negl(k)$.

The advantage of studying $\bar{w}(k,T_{bud})$ is having eliminated expression $B$ in Theorem \ref{closedw} which represents the effect of self-loops (and turns out to be very inefficient to evaluate as an exact expression). Probability $\bar{w}(k,T_{bud})$ corresponds to a Markov model without any self-loops and with horizontal transition probabilities $m_2(l)/(1-m_1(l))=(1-\gamma)\alpha(l)$, diagonal transition probabilities $m_3(l)/(1-m_1(l))=\gamma \alpha(l)$, and vertical transition probabilities $m_4(l)/(1-m_1(l))=1-\alpha(l)$, where 

\begin{equation} \alpha(l) = \frac{p(1-f(l))}{\gamma + (1-\gamma)(p+h)(1-f(l))}. \label{eq-alpha} \end{equation}


 Algorithm \ref{alg:wbar}  depicts how $\bar{w}(k,T_{bud})$ can be computed in $O(k\cdot T_{bud})$ time using dynamic programming -- and this is what we use in section \ref{AC-Param} to evaluate $\bar{w}(k,T_{bud})$ for different learning rates.
 
%\begin{algorithm}
%	\caption{$\bar{w}$ Computation}
%	\label{alg:wbar}
%	\begin{algorithmic}[1]
%		\Function{$\bar{w}$}{$k,T_{bud}$}
%		\State{$pr \gets zeros(k-1,T_{bud}-1)$}
%		\State{$pr[0,0]\gets 1$}
%		\For{$i\gets 0,T_{bud}-1$}
%		\If{$i != 0$}
%		\State{$pr[0,i]\gets(1-\alpha(i-1,a))pr[0,i-1]$}
%		\EndIf
%		\For{$j \gets 1,k-1$}
%		\If{$i==0$}\State{$pr[j,i]\gets [(1-\gamma)\alpha(0,a)]^{j}$}
%		\Else \State{$pr[j,i]\gets (1 - \gamma)\alpha(i,a)pr[j-1,i] + \gamma \alpha(i - 1,a) pr[j-1,i-1] + (
%			1 - \alpha(i - 1,a))pr[j,i-1]$}
%		\EndIf
%		\EndFor
%		\EndFor
%		%\State {$A \gets pr[k-1,...]$}
%		\State{$\bar{w}\gets 0$}
%		\For{$i\gets 0,T_{bud}-1$}
%		\State{$\bar{w} \gets \bar{w}+\alpha(i,a)pr[k-1,i]$}
%		\EndFor
%		\State \textbf{return}{$~\bar{w}$}
%		\EndFunction
%		\Statex
%		\Function{$\alpha$}{$l,a$}
%		\State \textbf{return}{$~(l+1)^{-a}$}
%		\EndFunction
%	\end{algorithmic}
%\end{algorithm}

\begin{algorithm}
	\caption{$\bar{w}$ Computation}
	\label{alg:wbar}
	\begin{algorithmic}[1]
		\Function{$\bar{w}$}{$k,T_{bud}$}
		\State{$pr \gets zeros(k-1,T_{bud}-1)$}
		\State{$pr[0,0]\gets 1$}
		\For{$i\gets 0,T_{bud}-1$}
		\If{$i != 0$}
		\State{$pr[0,i]\gets(1-\alpha(i-1))pr[0,i-1]$}
		\EndIf
		\For{$j \gets 1,k-1$}
		\If{$i==0$}\State{$pr[j,i]\gets [(1-\gamma)\alpha(0)]^{j}$}
		\Else \State{$pr[j,i]\gets (1 - \gamma)\alpha(i)pr[j-1,i] + \gamma \alpha(i - 1) pr[j-1,i-1] + (
			1 - \alpha(i - 1))pr[j,i-1]$}
		\EndIf
		\EndFor
		\EndFor
		%\State {$A \gets pr[k-1,...]$}
		\State{$\bar{w}\gets 0$}
		\For{$i\gets 0,T_{bud}-1$}
		\State{$\bar{w} \gets \bar{w}+\alpha(i)pr[k-1,i]$}
		\EndFor
		\State \textbf{return}{$~\bar{w}$}
		\EndFunction
	\end{algorithmic}
\end{algorithm}

\subsection{Analyzing Learning Rate $f(l)=1-\frac{d}{(l+2)^2}$}

We further upper bound $\bar{w}(k, T_{bud})$ in the next theorem which shows 
 that small enough learning rates $f(l)\geq 1- d/(l+2)^2$ will attain our desired asymptotic (as explained as a consequence after the theorem).
In Section \ref{AC-phase}  we will discuss what happens if there is an initial period during which the adversary already starts making progress in the game (e.g., compromising nodes) without the defender being aware or not having learned anything. For example, $f(l)=0$ for $l\leq L^*$ and $f(l)\geq 1-\frac{d}{(l-L^*)^2}$ for $l>L^*$. Here,  $L^*$ represents this initial period; only after a sufficient level $L^*$ is reached, i.e., a sufficient number of attack samples (e.g., malware payloads) have been collected, the learning rate increases.

\begin{theorem}[Upper Bound on $\bar{w}$]\label{Theo.wbarUB}
Assume that there exists a $d\geq 0$ such that 
$1-f(l)\leq d$ for all $l\geq 0$, or 
%for some small $d$. 
equivalently, $\beta(l)=\sqrt{\frac{1-f(l)}{d}}\leq 1$ for all $l\geq 0$. 
Let $\theta\geq (1-\gamma)/\gamma$. Then, 
%{\footnotesize
%	$$\beta(l)=\sqrt{\frac{1-f(l)}{d}}\leq 1,$$
%}. 
%$\forall \theta$ such that $(1-\gamma)/\gamma\leq \theta$ we have
		\begin{eqnarray*}
		\bar{w}(k,T_{bud})
		% &\leq &\nonumber
		%\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k-1}(1+\frac{1}{\theta})\frac{\beta(L)^2}{1-\beta(L)}\prod_{l=0}^{L-1} \frac{1+\beta(l)/\theta}{1-\beta(l)}\\
		&\leq&  	(1+\theta^{-1}) \sum_{L=0}^{T_{bud}-1} [\theta p d]^{k} \prod_{l=0}^{L} \left(1+ (1+\theta^{-1})\frac{\beta(l)}{1-\beta(l)}\right).
		\end{eqnarray*}

Let 
$$ c =\int_{l=0}^{T_{bud}-1} \frac{\beta(l)}{1-\beta(l)} dl +  \frac{\beta(0)}{1-\beta(0)}.$$
Then, minimizing the above upper bound with respect to $\theta$ proves
$$ c\leq \frac{1-\gamma}{\gamma} k \ \  \Rightarrow  \  \  \bar{w}(k,T_{bud})\leq  (1-\gamma)^{-1}  T_{bud} e^{(1-\gamma)^{-1} c} [\frac{1-\gamma}{\gamma}pd]^{k} .$$
Applying this statement for 
$$ 1-f(l) \leq \frac{d}{(l+2)^2}$$
gives
\begin{eqnarray*}
	&& T_{bud} \leq e^{-1+k (1-\gamma)/\gamma }  \\
	&& \hspace{1cm} \Rightarrow  \  \ \bar{w}(k,T_{bud}) \leq 
\frac{e^{1/(1-\gamma)}}{1-\gamma} \cdot T_{bud}^{1+1/(1-\gamma)} \cdot  [\frac{1-\gamma}{\gamma}pd]^{k} .
\end{eqnarray*}
\end{theorem}

For $f(l)\geq 1-\frac{d}{(l+2)^2}$ with $d<\frac{\gamma}{p(1-\gamma)}$, the theorem shows that if $T_{bud}< exp(k)$, then $w(k,T_{bud})\leq \bar{w}(k,T_{bud})= poly(T_{bud})negl(k)$ satisfying the desired asymptotics. % (if $T_{bud}=exp(k)$, then indeed  $w(k,T_{bud})=  poly(T_{bud})negl(k)= O(1)$).
%Since adversaries are interested in reaching large $k$,  condition $T_{bud} \leq e^{-1+k (1-\gamma)/\gamma }$ is met in practice.
 For analyzing other learning rates, the more  general upper bound of the theorem can be used.


\subsection{Delayed learning} \label{AC-phase}

In practice, learning only starts after seeing a sufficient number of attack samples. That is, $f(l)=0$ for $l< L^*$ for some $L^*$ after which $f(l)$ starts to converge to $1$. What would be the attacker state in the game during this initial phase, where no learning takes place (for instance, how many nodes will be compromised)? 

\begin{theorem}[Delayed learning]\label{Theo.delay} Suppose $f(l)=0$ for $l< L^*$.
	Define $u(k^*,L^*)$ as the probability  that $L^*$ is reached by a state $(i,L^*)$ with $i\leq k^*$, where we give the adversary the advantage of an unlimited time budget. Then, for $k^*\geq L^*+1$,
	$$ u(k^*,L^*) \geq 1- L^* [\frac{(1-\gamma)p}{1-(1-\gamma)(1-(p+h))}]^{\frac{k^*-1}{L^*}}. $$
	%	\bigg(1-(\frac{m_2}{1-m_1})^{k^*/L^*}\bigg)^{L^*}\geq 1- L^*\bigg(\frac{m_2}{1-m_1}\bigg)^{k^*/L^*}$$

Let $w'(k,T_{bud})$  correspond to learning rate $f(l+L^*)$ as a function of $l$ (e.g., $1-f(l+L^*)\leq \frac{d}{(l+2)^2}$). Then, for $k^*\geq L^*+1$,
\begin{equation} w(k,T_{bud})\leq (1- u(k^*,L^*)) + w'(k-k^*,T_{bud}),\label{eqdelayed} \end{equation}
where $1-u(k^*, L^*)$ is the probability that  $>k^*$ is achieved during the initial phase and where $ w'(k-k^*,T_{bud})$ is the probability that another $k-k^*$ progressive adversarial moves happen after the initial phase with time budget $T_{bud}$. 
\end{theorem}

The lower bound on $u(k^*,L^*)$ can be further simplified by using $p\leq 1-h$ which implies 
$$  u(k^*,L^*) \geq 1- L^* [(1-\gamma)(1-h)]^{\frac{k^*-1}{L^*}}. $$



%is 
%\begin{equation}\label{eq.delta.1}
%\leq (L^*+1)[(1-\gamma)(1-h)]^{\frac{k^*-1}{L^*+1}} + \bar{w}(k-k^*,T_{bud}), 
%\end{equation}

%where $\bar{w}$ can be computed through simulation or $\bar{w}$ has the special form as derived for $(1-f(x)) = \frac{d}{(1+x)^2}$.

%We define $u(k^*,L^*)$ as the probability  that $L^*$ is reached by a state $(i,L^*)$ with $i\leq k^*$, where we give the adversary the advantage of an unlimited time budget in this initial phase.
%By using similar proof strategies as the ones used before, we can prove that  
%{\footnotesize
%$$ u(k^*,L^*) \geq \bigg(1-(\frac{m_2}{1-m_1})^{k^*/L^*}\bigg)^{L^*}\geq 1- L^*\bigg(\frac{m_2}{1-m_1}\bigg)^{k^*/L^*}$$
%}
%We notice that $p\leq 1-h$ implies $m_2/(1-m_1)\leq (1-\gamma)(1-h)$.

Since $1-u(k^*,L^*)$ is exponentially small in $k^*/L^*$, this shows that very likely $k^* = O(L^*)$. This makes common sense because initially, every adversarial move has a significant probability of success since the defender's knowledge of the attack is very limited in the beginning (the attack is still unknown to the defender, in other words, no valid attack signature is formed yet). 
%Overall the adversary will reach $k$ with probability at most
%$$1-u(k^*,L^*) + w(k-k^*,T_{bud}).$$
%where $1-u(k^*, L^*)$ is the probability that  $>k^*$ nodes are compromised during the intial phase and where $ w(k-k^*,T_{bud})$ is the probability that another $k-k^*$ nodes are compromised after the initial phase with time budget $T_{bud}$. 
%The containment parameter (see Section \ref{AC-AC}) $k_c(L^*)$ as a function of $L^*$ turns out to be approximately $k_c(L^*)\approx k_c(0)\cdot L^*$. 
%TO DO Next subsection shows $L^*\ln L^*$ dependence ---
If we achieve desired asymptotic (\ref{eq:as}) for $w'(k,T_{bud})$, then the resulting containment parameter for $w(k,T_{bud})$ (see Section \ref{AC-AC}) is $k_c=O(L^* + \log T_{bud})$. It is very important for the defender to keep $L^*$ small. A larger $L^*$ leads to a longer initial phase during which the adversary keeps on making progressive moves of the order of $O(L^*)$.  

\subsection{Capacity Region}

In this subsection, we show that as a result of our analysis we are able to prove statements like the one in the following definition which defines a `capacity region' of combinations of parameters defining the adversarial time budget, the probability of winning, and $k$ which characterizes what it means to be in a winning state. The definition describes what was previously called `desired asymptotics' since a {\em non-empty} capacity region shows that an exponentially small probability of winning $O(2^{-s})$  is achieved if $k=O(s + \log T_{bud})$ implying that the probability of winning is $poly(T_{bud})negl(k)$.

%TO DO Relationship to `desired asymptotics'.

\begin{definition} Suppose there exist vectors $\boldsymbol{\delta}$, $\boldsymbol{\mu}$, $\boldsymbol{\xi}$, and the all-one vector ${\bf 1}$, such that, for all $k\geq 0$ (characterizing a winning state for the adversary) and for all $s\geq 0$ and $t\geq 0$ satisfying
$$ s\boldsymbol{\delta} + t \boldsymbol{\mu} \leq k {\bf 1} + \boldsymbol{\xi},$$
 we have the following security guarantee: If the attacker has a time budget $\leq 2^t$, then his probability of reaching a winning state is at most $\leq 2^{-s}$. 
 
 We say that $(\boldsymbol{\delta}, \boldsymbol{\mu},  \boldsymbol{\xi})$ describes a capacity region for $\{(s,t) \ : \ s,t\geq 0\}$. Its definition implies that for a fixed $k$ and time budget $2^t$, the probability of winning is at most $\leq 2^{-s(k,t)}$, where
 \begin{equation} s(k,t)= \max\{ s\geq 0 \ : \  s\boldsymbol{\delta} + t \boldsymbol{\mu} \leq k {\bf 1} + \boldsymbol{\xi} \}. \label{eqcapreg} \end{equation}
 Similarly, for a  time budget $2^t$, the probability of winning is $\leq 2^{-s}$ if  a winning state is characterized by some $k\geq k(s,t)$, where
 \begin{equation} k(s,t)= \min\{ k\geq 0 \ : \  s\boldsymbol{\delta} + t \boldsymbol{\mu} \leq k {\bf 1} + \boldsymbol{\xi} \}. \label{eqcapreg2} \end{equation}
 \end{definition}
 
This definition generalizes the definition of security capacity used in MTD games \cite{saeed2016markov} where only a single equation of the form $s+t\leq \delta \cdot k$ needs to be satisfied and where $\delta$ is defined as the ``security capacity''. The definition of capacity region may be of interest for other more general defender-adversarial games where a Markov model is used to characterize defender and adversarial moves.\footnote{A more general definition which captures  winning states  characterized by parameter vectors ${\bf k}$, rather than a single $k$, can also be formulated.}

%and where winning states are characterized by parameter vectors ${\bf k}$ (rather than a single $k$)  -- with in the definition of a corresponding capacity region $\boldsymbol{\delta}$ represents a matrix (and $k\boldsymbol{\delta}$ is replaced by ${\bf k} \cdot \boldsymbol{\delta}$).

The definition of capacity region is of interest for a couple of reasons. First, it clearly describes the limitation of the adversary: 
The capacity region explicitly characterizes the probability of winning as a function of $t$ and $k$, see (\ref{eqcapreg}). In practice, the attacker's time budget is $\leq 2^t$, limited to some ``small'' $t$, e.g., $t=80, 128$, and using such a fixed $t$ makes the probability of winning only a function of $k$. 
 % In addition  that the adversary wants to affect a  ``large'' number of nodes -- or, equivalenty, $k$ is, say $\geq 1000$. Then, the capacity region characterizes the probablity of winning explicitely as a function of $t$ and $k$, see (\ref{eqcapreg}).

Second, the capacity region can also be used to compute the containment parameter $k_c$, defined as the solution  $k(s,t)$ in (\ref{eqcapreg2}) where $s$ is set to $s=1$ which corresponds to a probability of winning equal to $1/2$. This allows us to understand how 
$$k_c=k(1,t)=O(t)=O(\ln T_{bud})$$ depends on the parameters that describe the overall Markov model.

Third, the definition allows us to trivially compose capacity regions of Markov models corresponding to different learning rates. For instance, in practice, an attacker may use several exploits or attack vectors and use each attack vector to advance its footprint and increase the number of compromised nodes. For each attack vector $i$, the defender develops a learning rate $f_i(l)$. In essence, the defender plays individual games with each attack vector, and the adversary wins the overall game if the individual games lead to $k_i$ compromised nodes such that $k=\sum_i k_i$. The following theorem makes this argument precise.

\begin{theorem} Let $f_i(l)$, $1\leq i\leq a$, be learning rates corresponding to Markov models describing different defender-adversary games that are played simultaneously. Let  $k_i(s,t)$ for the $i$-th game  be defined as in (\ref{eqcapreg2}). Let $T_{bud}\leq 2^t$ be the overall time budget of the adversary. Then the probability of reaching a state with $k_i(s+\ln a,t)$ compromised nodes in the $i$-th game is at most $\leq 2^{-(s+\ln a)}=2^{-s}/a$. Since the transition probabilities in each of the Markov models are independent from the number of compromised nodes, the probability of reaching $k=\sum_{i=1}^a k_i(s+\ln a,t)$ is at most
$$\leq 1- \prod_{i=1}^a (1-2^{-s}/a)\leq 2^{-s}.$$
\end{theorem}

Notice that for $a$ simultaneous adversarial games an exponentially small probability of winning $O(2^{-s})$  is achieved for $k=O(s + \ln a + \ln T_{bud})$. In this parallel game, if the time budget is measured in real time $T$, then (as before) $T_{bud}\leq Tk/\Delta$ for  $k=\sum_{i=1}^a k_i(s+\ln a,t)$ and we require $T\leq \frac{\Delta}{k} 2^{t}$. As a final note,  $k=\sum_{i=1}^a k_i(s+\ln a,t)$ is dominated by  $\max_{i=1}^a k_i(s+\ln a,t) \geq k/a$. In other words, the attacker keeps on searching for an attack vector which can be used to achieve a large fraction\footnote{Due to the defender either starting learning after a too long initial period or, once learning starts,  not learning fast enough (in order to attain the desired asymptotic).} of the desired $k$, and the defender tries to learn how to recognize attack vectors as fast as possible in order to contain these sufficiently.

%This shows that the order of used exploits does not matter; the attacker is in search of finding one exploit leading to a large containment parameter due to the defender either starting learning after a too long initial period or, once learning starts,  not learning fast enough (in order to attain the desired asymptotic).

%The attacker wants to compromise $k$ nodes. TO DO Say $a$ attack vectors with learning rates $f_a(l)$ and capacity regions ... Just concatenate all equations, divide $k$ in each by $k/a$, and use $s+\ln a$. Or use $k_a$ and have their sum equal to $k$ -- this is better -- add in definition of min $k$ for a given $2^t$ and $2^{-s}$ and this also directly relates to the containment parameter. THEOREM

As an example of  a capacity region, we translate Theorem \ref{Theo.wbarUB} for $1-f(l) \leq \frac{d}{(l+2)^2}$ in terms of a capacity region: 

\begin{corollary} \label{crcor}
For learning rate  $1-f(l) \leq \frac{d}{(l+2)^2}$ we have a capacity region $(\boldsymbol{\delta}, \boldsymbol{\mu},  \boldsymbol{\xi})$ defined by 2-dimensional vectors
\begin{eqnarray*}
\boldsymbol{\delta} &=& (0, q \ln 2), \mbox{ where } q = \left[ \ln(\frac{\gamma}{pd(1-\gamma)})\right]^{-1}, \\
\boldsymbol{\mu} &=& (\frac{\gamma \ln 2}{1-\gamma}, q (\ln 2)(1+\frac{1}{1-\gamma})), \\
\boldsymbol{\xi} &=& (-\frac{\gamma}{1-\gamma}, q(-\frac{1}{1-\gamma} + \ln \frac{1}{1-\gamma}).
\end{eqnarray*}
\end{corollary}

%We have the security guarantee
%\begin{equation}
% T_{bud} \leq e^{-1+k (1-\gamma)/\gamma } \ \ \Rightarrow  \  \ \bar{w}(k,T_{bud}) \leq 
%\frac{e^{1/(1-\gamma)}}{1-\gamma} \cdot T_{bud}^{1+1/(1-\gamma)} \cdot  [\frac{1-\gamma}{\gamma}pd]^{k} .
%\label{eqimpl}
%\end{equation}
%If 
%\begin{eqnarray}
%2^t &\leq & e^{-1+k (1-\gamma)/\gamma }, \mbox{ and} \label{crex}  \\
%2^{-s} &\geq& \frac{e^{1/(1-\gamma)}}{1-\gamma} \cdot (2^t)^{1+1/(1-\gamma)} \cdot  [\frac{1-\gamma}{\gamma}pd]^{k} , \nonumber
%\end{eqnarray}
%then $T_{bud}\leq 2^t$ implies the condition on the left hand side of the implication in (\ref{eqimpl}), hence,
%\begin{eqnarray*}
%\bar{w}(k,T_{bud}) &\leq & \frac{e^{1/(1-\gamma)}}{1-\gamma} \cdot T_{bud}^{1+1/(1-\gamma)} \cdot  [\frac{1-\gamma}{\gamma}pd]^{k} \\
%&\leq & \frac{e^{1/(1-\gamma)}}{1-\gamma} \cdot (2^t)^{1+1/(1-\gamma)} \cdot  [\frac{1-\gamma}{\gamma}pd]^{k} \\
%&\leq & 2^{-s}.
%\end{eqnarray*}
%This shows that the capacity region is characterized by (\ref{crex}), or equivalently after taking logarithms, assuming $\frac{pd(1-\gamma}{\gamma}<1$, and reordering terms, $\boldsymbol{\delta}$, $\boldsymbol{\mu}$, and $\boldsymbol{\xi}$ are given by 2-dimensional vectors
%\begin{eqnarray*}
%\boldsymbol{\delta} &=& (0, q \ln 2), \mbox{ where } q = \left[ \ln(\frac{\gamma}{pd(1-\gamma)})\right]^{-1}, \\
%\boldsymbol{\mu} &=& (\frac{\gamma \ln 2}{1-\gamma}, q (\ln 2)(1+\frac{1}{1-\gamma})), \\
%\boldsymbol{\xi} &=& (-\frac{\gamma}{1-\gamma}, q(-\frac{1}{1-\gamma} + \ln \frac{1}{1-\gamma}).
%\end{eqnarray*}

%TO DO -- Make this a theorem -- Substitute $k^*=k'+L^*+1$ and consider two cases $k'=0$ or $k'>0$ for a given $s$.

As a second example of working with capacity regions, we translate (\ref{eqdelayed}) in Theorem \ref{Theo.delay} for delayed learning:
%Finally, delayed learning shows that for all $k^*\geq L^*+1$,
%\begin{eqnarray*}
% w(k,T_{bud}) &\leq& (1- u(k^*,L^*)) + w'(k-k^*,T_{bud}) \\
 %&\leq&  L^* [\frac{(1-\gamma)p}{1-(1-\gamma)(1-(p+h))}]^{\frac{k^*-1}{L^*}} + w'(k-k^*,T_{bud}).
 %\end{eqnarray*}
 %This translates into the following lemma.
 
\begin{corollary} \label{lemdel} Suppose $f(l)=0$ for $l<L^*$ and let $(\boldsymbol{\delta}', \boldsymbol{\mu}',  \boldsymbol{\xi}')$ be the capacity region corresponding to learning rate $f(l+L^*)$ as a function of $l$. Suppose that
$$z= \left[ \ln(\frac{1-(1-\gamma)(1-(p+h))}{(1-\gamma)p})\right]^{-1}\geq 0.$$
%(which is small for small $(1-\gamma)p$).
Then, first,
 for all $s\geq \max\{0, 1/{z\ln 2} - {\ln (2L^*)}{\ln 2} \}$ and $t\geq 0$ satisfying
$$ s[\boldsymbol{\delta}'+  L^* (\ln 2) z {\bf 1}]
 + t \boldsymbol{\mu}' \leq k {\bf 1} + [\boldsymbol{\xi}' -\boldsymbol{\delta}' + ( L^* (\ln 2L^*) z -1){\bf 1}] $$
and, second, for all\footnote{Notice that  $1/{z\ln 2} - {\ln (2L^*)}{\ln 2}\geq 0$ if and only if $L^*\leq \frac{1}{2}e^{1/z}= \frac{1-(1-\gamma)(1-(p+h))}{2(1-\gamma)p}$, which is large  for small $(1-\gamma)p$.} $0\leq s\leq  1/{z\ln 2} - {\ln (2L^*)}{\ln 2}$ and $t\geq 0$ satisfying
$$ s\boldsymbol{\delta}' + t \boldsymbol{\mu}' \leq k {\bf 1} + [\boldsymbol{\xi}' -\boldsymbol{\delta}' - (L^*+1){\bf 1}],$$
 we have the following security guarantee: If the attacker has a time budget $\leq 2^t$, then his probability of reaching a winning state is at most $\leq 2^{-s}$. 
\end{corollary}

The corollary confirms that the containment parameter for delayed learning (for both cases) is 
$k_c = O(L^* + \log T_{bud})$.



%As a next example, 

\subsection{Parametric analysis of Learning Rate $f(l)=1-\frac{d}{(l+2)^a}$}\label{AC-Param}

In this subsection, we use Algorithm \ref{alg:wbar} to evaluate $\bar{w}(k,T_{bud})$ based on different learning rates and $T_{bud}=10,000$ logical timesteps. Fig. \ref{fig.wbar} depicts $\bar{w}(k,T_{bud})$ as a function of $k$ for several $\gamma$ and  several learning rates of the form $\alpha(l)= (l+1)^{-a}$. As it can be seen from this plot, a proper defense mechanism (with sufficiently fast converging learning rates and large enough $\gamma$ values) substantially decreases the adversary's chances of making progress in the game. 
 
% This plot shows the importance of having a proper defense learning mechanism in order to be able to contain the adversary. Clearly, $k$ remains small $<100$ with high probability for sufficiently fast converging learning rates and large enough $\gamma$.
 Fig. \ref{fig.kc} depicts how the containment parameter $k_c$ (computed using $\bar{w}(k,T_{bud})$) depends on $\alpha(l)= (l+1)^{-a}$. For $a\geq 0.9$, $k_c\leq 20$ is very small making it impossible for the adversary to reach high-value attack objectives (e.g., total number of infected nodes in a malware propagation game).
 
 \begin{figure*}%[h!]
 	\begin{center}
 		\scalebox{0.65}
 		{\includegraphics{figure2k50_gammaED}}
 		\caption{$\bar{w}(k,T_{bud})$ based on different values of $\gamma$ and learning functions $\alpha(l) = (l+1)^{-a}$ where $T_{bud} = 10,000$ logical timesteps}
 		\label{fig.wbar}
 	\end{center}
 \end{figure*}
 
 \begin{figure}%[h!]
 	\begin{center}
 		\scalebox{0.43}
 		{\includegraphics{kc-eps-converted-to.pdf}}
 		\caption{$k_c$ for different classes of learning functions $\alpha(l) = (l+1)^{-a}$ where $T_{bud} = 10,000$ logical timesteps}
 		\label{fig.kc}
 	\end{center}
 \end{figure}
 
 Fig. \ref{fig.roleOfp} depicts the chances of attack prosperity in two different cases $p=0.1$, and $p =1.0$ (see (\ref{eq-alpha})) while $\gamma = 0.5$ meaning that half of the adversarial moves will be observed by the defender at the network levels (i.e., will be marked as suspicious on the flow classifier). 
% In the same figure, $p =1$ represents the case of the strongest adversary equipped with a precompiled list of vulnerable nodes, i.e., a hitlist, meaning that it does not require to probe the network environment which gives the defender the minimum number of malware samples. Notice that in this case, at each time step, the adversary only hits a vulnerable node ($p=1, h= 0$). Even for such a strong adversary, the simulation shows that with a proper learning rate mechanism in place, chances of constructing a botnet for the attacker are minimal.
\begin{figure}%[h!]
 	\begin{center}
 		\scalebox{0.43}
 		{\includegraphics{figureP_hitlist}}
 		\caption{$\bar{w}(k,10000)$ for two cases $p=0.1$, and $p=1.0$ with $\gamma=0.5$ and learning function $1-f(l) = (l+1)^{-a}$ where $a=0.6$ and $a=1$ respectively.}
 		\label{fig.roleOfp}
 	\end{center}
 \end{figure}
 %\begin{algorithm}
 %	\caption{$\bar{w}$ Computation}
 %	\label{alg:wbar}
 %	\begin{algorithmic}[1]
 %		\Function{$\bar{w}$}{$k,l,\gamma$}
 %		\State {$A \gets prob(k-1,l,\gamma)[k-1,...]$}
 %		\State{$\bar{w}\gets 0$}
 %		\For{$i\gets 0,l$}
 %		\State{$\bar{w} \gets \bar{w}+\alpha(i)A[i]$}
 %		\EndFor{;}
 %		\Return{$\bar{w}$;}
 %		\EndFunction
 %		\Statex
 %		\Function{$prob$}{$k,l,\gamma$}
 %		\State{$pr \gets zeros[k,l]$}
 %		\For{$i\gets 0,l$}
 %		\If{$i == 0$}\State{$pr[0,i]\gets 1$}
 %		\Else \State{$pr[0,i]\gets(1-\alpha(i-1))pr[0,i-1]$}
 %		\EndIf
 %		\For{$j \gets 1,k$}
 %		\If{$i==0$}\State{$pr[j,i]\gets [(1-\gamma)\alpha(0)]^{j}$}
 %		\Else \State{$pr[j,i]\gets (1 - \gamma)\alpha(i)pr[j-1,i] + \gamma \alpha(i - 1) pr[j-1,i-1] + (
 %			1 - \alpha(i - 1))pr[j,i-1]$}
 %		\EndIf
 %		\EndFor
 %		\EndFor{;}
 %		\Return{$pr$;}
 %		\EndFunction
 %		\Statex
 %		\Function{$\alpha$}{$l,a$}
 %		\Return{$(l+1)^{-a}$}
 %		\EndFunction
 %	\end{algorithmic}
 %\end{algorithm}
 
 The impact of delayed learning on the adversarial containment parameter $k_c$  is shown in Fig. \ref{fig.delayed} for two different cases. In the first scenario, the learning starts immediately (with no delay, i.e.,  $L^{*}=0$), and in the second case, the learning commences after missing the first 100 attack samples (i.e., $L^*=100$). 
 
 %means_a0 = (100, 29, 11)
 %means_a1 = (300, 228, 210)
 \begin{figure}%[h!]
 	\begin{center}
 		\scalebox{0.43}
 		{\includegraphics{delayedLearning}}
 		\caption{The impact of delayed learning on $k_c$ for different classes of learning functions $\alpha(l) = (l+1)^{-a}$ where $T_{bud} = 10,000$ logical timesteps}
 		\label{fig.delayed}
 	\end{center}
 \end{figure}
 
%%%%%%%%%% PROOF BELOW %%%%%%%%%%%%%

%The probability that $L^*$ is reached by a state $(i,L^*)$ with $i\leq k^*$ is equal to the probability of reaching a state $(i,L^*-1)$  and leaving it by a diagonal or vertical transition to $(i+1,L^*)$ or $(i,L^*)$. Let us denote this probability by $u(k^*,L^*)$, where we give the adversary the advantage of an unlimited time budget in this initial phase:
%{\footnotesize
%\begin{eqnarray}\label{eq.k}
%&& u(k^*,L^*) \nonumber \\
%&\geq& \sum_{k=0}^{k^{*}-1} p(k,L^{*}-1,\infty)(\frac{m_4(L^*-1)}{1-m_1(L^*-1)}+\frac{m_3(L^*-1)}{1-m_1(L^*-1)}) \nonumber \\
%&=&  \sum_{B=0}^{L^*-1}\sum_{k=B+1}^{k^{*}}(\ref{p-a})(\ref{p-b})\frac{m_3(L^*-1)+m_4(L^*-1)}{1-m_1(L^*-1)}, \nonumber
%\end{eqnarray}
%}
%where $L$ is substituted by $L^*-1$ in (\ref{p-a}) and (\ref{p-b}).
%Notice that $m_1$, $m_2$, $m_3$, and $m_4$ do not depend on $l$ because $f(l)=0$ during the initial phase. By using the proof strategy of Section \ref{stagnating} we can derive
%{\footnotesize
%$$ \sum_{k=B+1}^{k^*} (\ref{p-b}) \geq \bigg( \frac{1-m_1}{m_3+m_4}\bigg)^{L^*} \cdot \bigg( 1- \bigg(\frac{m_2}{1-m_1}\bigg)^{(k^*-1-B)/L^*+1}\bigg)^{L^*}.
%$$
%}
%This is further lower bounded by $B\leq L^*-1$ to
%{\footnotesize
%$$ \sum_{k=B+1}^{k^*} (\ref{p-b}) \geq \bigg( \frac{1-m_1}{m_3+m_4}\bigg)^{L^*} \cdot \bigg( 1- \bigg(\frac{m_2}{1-m_1}\bigg)^{k^*/L^*}\bigg)^{L^*},
%$$
%}
%which is independent of $B$ and the $b_{l+1}$ in (\ref{p-a}). Now we derive
%{\footnotesize
%\begin{eqnarray*}
%&& \sum_{B=0}^{L^*-1}(\ref{p-a})\frac{m_3(L^*-1)+m_4(L^*-1)}{1-m_1(L^*-1)}  = \\  
%&&	{ \sum_{b_1,\dots,b_L^*\in\{0,1\}}\prod_{l=0}^{L^*-2} \bigg( b_{l+1}\frac{m_3}{1-m_1} + (1-b_{l+1})\frac{m_4}{1-m_1} \bigg)\frac{m_3+m_4}{1-m_1}
%}\\
%&& =\bigg( \frac{m_3+m_4}{1-m_1} \bigg)^{L^*}.
%\end{eqnarray*}
%}
%Combining the above formulas yields
%{\footnotesize
%$$ u(k^*,L^*) \geq \bigg(1-(\frac{m_2}{1-m_1})^{k^*/L^*}\bigg)^{L^*}\geq 1- L^*\bigg(\frac{m_2}{1-m_1}\bigg)^{k^*/L^*}$$
%}
%Since $1-u(k^*,L^*)$ is exponentially small in $k^*/L^*$, this shows that very likely $k^* = O(L^*)$. This makes common sense because initially every malicious payload has a significant probability of compromising a node.

%Suppose that after the initial phase learning takes place according to $1-f(l)\leq \frac{d}{(l-L^*+2)^2}$ for $l\geq L^*$, see previous subsection. Then, overall the adversary will reach $k$ with probability at most
%$$1-u(k^*,L^*) + w(k-k^*,T_{bud}).$$
%where $1-u(k^*, L^*)$ is the probability that $>k^*$ nodes are compromised during the intial phase and where $ w(k-k^*,T_{bud})$ is the probability that another $k-k^*$ nodes are compromised after the initial phase with time budget $T_{bud}$.
%We notice that the upper bound of $1-u(k^*,L^*)$ has the form $C_1 e^{-\alpha_1 k^*}$ and the upper bound of $w(k-k^*,T_{bud})$ has the form $C_2e^{-\alpha_2 (k-k^*)}$. As a lemma we can prove that if we minimize $C_1 e^{-\alpha_1 k^*}+C_2e^{-\alpha_2 (k-k^*)}$ over $k^*$, then we obtain the minimal value 
%{\footnotesize
%$$e^{-\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2} k }\cdot \bigg(\frac{C_1}{\alpha_2}\bigg)^{\frac{\alpha_2}{\alpha_1+\alpha_2}}
%\cdot \bigg(\frac{C_2}{\alpha_1}\bigg)^{\frac{\alpha_1}{\alpha_1+\alpha_2}}\cdot (\alpha_1+\alpha_2).$$
%}
%Hence, the exponential dependency on $k^*$ is given by $e^{-\frac{\alpha_1\alpha_2}{\alpha_1+\alpha_2} k }\leq e^{-\min\{\alpha_1, \alpha_2\} k/2 }$ and is mostly characterized by the smaller value of $\alpha_1$ and $\alpha_2$. E.g., if we take $d=\gamma$ in $1-f(l)\leq \frac{d}{(l-L^*+2)^2}$ for $l\geq L^*$, then $e^{-\alpha_2}\approx e^{-\alpha_1 L^*}$ for large $p$ ($p$ is controlled by the adversary). As a consequence, the `containment parameter' $k_c(L^*)$ as a function of $L^*$ is approximately $k_c(L^*)\approx k_c(0)\cdot L^*$. It is obviously important to keep $L^*$ small. A larger $L^*$ leads to a longer initial phase during which the adversary keeps on compromising $O(L^*)$ nodes.

%%%%%%%%%% END PROOF and extra writing %%%%%%%%%%%%%%%%%%%%%%

%\subsection{Role of $p$} \label{AC-role}

%TO DO Rewrite and in part merge with the security capacity section

%In our analysis we assume $p=p_i$ for a fixed parameter $p$. If the $p_i$ vary, then we can give the adversary the advantage of $p= \sup_i p_i$ in our analysis. Notice that during an initial phase where no learning takes place  $u(k^*,L^*) \geq 1 - L^*((1-\gamma)(1-h))^{k^*/L^*}$ which is independent of $p$. Also, for learning after such an initial phase, our  general bound (\ref{eq.conditions})  with maximum $p=1-h$ shows that the effect of a larger overall $p$ does not change the asymptotic behavior of  desired learning rates (i.e., learning rates that achieve the desired asymptotic of $w(k,T_{bud})$). As a consequence the asymptotic behavior of  containment parameter $k_c$ is independent of $p$. Of course, a concrete small $p$ does have a huge impact and will make $k_c$ small as well.

%TO DO Connection Lemma 1-- possibly push this to a comment after lemma 1 ----
%Consider the case of an adversary who starts with a first exploit for some $p_1$ and compromises $k_c^1$ nodes. After noticing being contained to $k^1_c$ compromised nodes, the attacker continues with  these  nodes  to compromise more nodes by using a second exploit associated to some $p_2$, etc. (see Section \ref{subsec.gameExtentions}).  For each exploit, transition probabilities in our Markov model do not depend on $i$; they only depend on $p_j$ (for the $j$-th used exploit), $h$, $\gamma$, and the learning rate $f(l)$; our analysis applies for each exploit individually showing that the second and generally $j$th exploit only adds another $k^j_c$ compromised nodes. So, the overall containment parameter is equal to the aggregate $\sum_j k^j_c$ which is largely independent of the $p_j$ (in the way discussed above). This shows that the order of used exploits does not matter; the attacker is in search of finding one exploit leading to a large containment parameter due to the defender either starting learning after a too long initial period or, once learning starts,  not learning fast enough (in order to attain the desired asymptotic).

%Now consider the case of host based cleaning of nodes (see Section \ref{subsec.gameExtentions}), which is  modeled by multiplying $p_i$ with $1-f_h(i)$ for some host based `cleaning rate' function $f_h(.)$. We notice that for $1-f_h(i)\geq \tau$ for some $\tau>0$ the above analysis shows that the resulting containment parameter has asymptotic behavior independent of $p_i(1-f_h(i))$. In other words a stagnating cleaning rate has little effect. On the other hand if $1-f_h(i) \rightarrow 0$ for $i\rightarrow \infty$, then cleaning will have a major influence since $p_i(1-f_h(i))\rightarrow 0$. We leave a detailed analysis for future work.






==> General_paper_S&P_Eprint/sections/bg.tex <==
Modeling cyber attacks as a game between a defender and an attacker is a classical research problem. Here, we review some of the research that has been done in this area which we find the most relevant (current state-of-the-art) and connected to this presented work. 

The intrusion detection problem in heterogeneous networks consisting of nodes with various security assets is studied in \cite{chen2009game}. The expected behaviors of rational attackers in addition to the optimal defender strategy are derived by formulating the attacker-defender interaction as a non-cooperative game. The paper concludes that sufficient resources for monitoring the environment and proper system configuration at the defender side are two necessary conditions of efficiently protecting the network. Similarly, the interaction of players is modeled as a general-sum stochastic game in \cite{lye2005game} in which Lye and Wing studied three different attack-response scenarios including defacing a website, stealing confidential data, and launching a Denial of Service (DoS) attack. The authors though left the richer and more complex scenarios for future works including a more capable defender with a more extensive action set for attack detection and prevention purposes. Such a stronger defender could potentially lure the attacker and learn the attack technology by setting up defensive agents such as honeypots within the environment. Carroll and Grosu \cite{carroll2011game} consider such stronger defense strategies, i.e., taking advantage of camouflage techniques (e.g., disguising a regular system as a honeypot or vice versa) by investigating the effects of deception on players' interaction using a signaling game. 

Motivated by the rise of advanced persistent threats, van Dijk \textit{et al.} \cite{van2013flipit} introduced the {F{\footnotesize{LIP}}}{I{\footnotesize{T}}} game to model the interaction of two players competing in a race of maximizing the amount of time each is in control of a shared computing resource while minimizing their total cost (associated with each player move). Strongly dominant strategies for both players (if there exist such strategies) are determined based on different employed attack strategies. Also, they provided general guidance on how and when to implement a cost-effective defense strategy.

Valizadeh \textit{et al.} \cite{saeed2016markov} introduced the concept of ``security capacity'' as a metric for gauging the effectiveness of an MTD strategy. The interactions of attacker and defender in dynamic environments\footnote{Those with changing system configurations and therefore attack surfaces} is modeled by probabilistic algorithms and characterized by a Markov chain. In particular, they showed how the probability of a successful adversary defeating an MTD strategy is related to the amount of time/cost spent by the adversary. The relationship between the attack success probability and the time it takes to reach the attack objectives (i.e., the winning state for the adversary) is then translated into the security capacity concept:  ``the security capacity of an  MTD game (a defense system) is at least $c$ if the probability that the attacker wins in the first $T = 2^t$ time steps is $\leq 2^{-s}$ for all $t+s = c$''. 
Connell  \textit{et al.} \cite{connell2018performance} used a similar approach as \cite{saeed2016markov} to model the attacker-defender interactions via a Markov chain in dynamic environments. In particular, a quantitative analytic model is proposed for evaluating the performance of MTD schemes, and the availability of resources in the environment and a method is recommended for maximizing a utility function that takes the tradeoffs between security and performance into consideration.

For a review of existing game-theory based solutions for network security problems see \cite{liang2013game,manshaei2013game}. For instance, Liang \textit{et al.} \cite{liang2013game} summarized the presented game models' application scenarios (both cooperative and non-cooperative games) under two categories: attack-defense analysis, and security measurement. Manshaei \textit{et al.} \cite{manshaei2013game} however, surveyed the use of game theory in addressing diverse forms of privacy and security problems in mobile and network applications. The studied works are organized in six main categories: physical and MAC layer security, security of self-organizing networks, intrusion detection systems, anonymity and privacy, network security economics, and cryptography.

%Unlike game-theory based models which try to determine the best decision for the defender(s) based on the predicted actions of the attacker(s) (in every possible scenario), ...



==> General_paper_S&P_Eprint/sections/case_study.tex <==
In this section, we walk through two examples of attack-defense games as case studies to show how real-world cyber attack scenarios can be translated into our presented framework. Their security analsyis is worked out in the appendix.

\subsection{Malware propagation and Botnet construction} \label{CS1}

 Consider a statically addressed network of size $\mathcal{N}$ in which a fraction of the hosts $\mathcal{K}$ suffers from a zero-day vulnerability only known to an adversary. The attacker's objective is to locate such hosts in the network, based on a target discovery strategy $\sigma$ (e.g., a random scan scheme, or a hitlist) associated with a probability $p_i$, and infect them during the Window of Vulnerability (WoV) time as the number of vulnerable systems is not yet shrunken to insignificance and the attacker’s exploit is useful in this period. The game starts with one infected machine as the ``Patient Zero''. The attacker desires to take control of at least $k$ out of $\mathcal{K}$ vulnerable hosts, meaning that the winning state for the adversary is defined as $(i,l)=(k,*)$. 
In the meantime, the defender’s objective is to generate an attack signature to be able to filter next adversarial attack traffic (see Fig. \ref{fig.ids_scenario}). The defender’s knowledge of the attack can be increased in two manners: (1) if an adversary agent hits a honeypot with probability $h$ (assuming that there exist in total $\mathcal{H}$ honeypots in the environment, therefore, $h =\mathcal{H}/\mathcal{N}$ for a memoryless blind scan strategy), or (2) if the attack traffic is correctly labeled as suspicious on the network (classifier) level with probability $\gamma$ \footnote{This is a typical architecture in automatic signature generation schemes (e.g., see \cite{kim2004autograph,newsome2005polygraph,li2006hamsa,tang2011signature}).}. In either of these cases, the defender’s detection rate $f(l)$ in which $l$ is the number of so far collected attack samples will be enhanced. This function represents the probability that given $l$ samples so far, the system detects a new incoming malicious packet and filters it on the fly. We also consider a skillful attacker (for instance taking advantage of a polymorphic worm) as defined in previous sections, and therefore, having only a few attack samples is not enough for signature generation.

\begin{algorithm}%[h]
	\caption{Malware propagation game simulator}
	\label{alg:sim}
	\begin{algorithmic}[1]
		\Function{Simulator}{$\mathcal{N,K,H},k,\sigma,\varepsilon,\gamma,f(.),\vartheta$}
		\State {$\mathcal{I} = \emptyset$; $l = 0$;}
		\State {droppingOut = False};
		\State {winningState = False};
		\While {not droppingOut and not winningState}
%		\State {targetHost $\xleftarrow[\text{}]{\text{\$}} probe(\mathcal{N}\setminus \mathcal{I})$};
	\State {targetHost $\xleftarrow[\text{}]{p_i} probe(\mathcal{N},\sigma)$};
		\State {filtered,sampled $\xleftarrow[\text{}]{f(l),\gamma}$$transmit$($\varepsilon$,targetHost)};
		\If {(not filtered and targetHost $\in \mathcal{H}$) or sampled} \label{alg.def_start}
		\State{$l\pluseq 1$};
		\State {update $f(l)$};
		\If {$f(l) \geq 1-\vartheta$}
		\State {Output \textit{"Game is finished. Attacker dropped out! Defender won!"}};
		\State {droppingOut = True};
		\EndIf 
		\EndIf \label{alg.def_end}
		\If {targetHost $\in \mathcal{K}$ and not filtered}
		\State $\mathcal{I} = \mathcal{I}~ \cup$ targetHost;
		\If {$|\mathcal{I}| \geq k$}
		\State {Output \textit{"Game is finished. Adversary won!"}};
		\State {winningState = True};
		\EndIf 
		\EndIf
		\EndWhile
		\EndFunction
	\end{algorithmic}
\end{algorithm}

The system state $(i,l)$ represents the total number of infected machines and the total number of captured attack traffic (i.e., malware samples) so far by the defense system. The attacker's view of the system state will change if an agent's effort in infecting a new node is successful (or if it possibly loses its control over an agent).
The defender's view gets updated as a consequence of discovering an adversarial move (i.e., an attack/malware sample). 
Algorithm \ref{alg:sim} shows the above description of the game in which the game simulator takes $\mathcal{N,K,H},k$, and an adversarial target discovery strategy $\sigma$ and an exploit $\varepsilon$, in addition to the detection probability $f(l)$, the sampling rate $\gamma$, and an acceptable ``threshold'' $1-\vartheta$ as the input and outputs if the attacker wins the game. The termination rule is whether the attacker compromises its desired number of hosts $k$ or if the attacker decides not to play anymore\footnote{For instance, the attacker concludes that not enough gain can be made in a reasonable time because of not being able to make a progressive move in the game due to defender's high-value detection rates that keep on improving.}, that is $f(l) \geq 1-\vartheta$. Note that the transmit method returns a tuple, i.e., if the transmitted packet by the attacker got filtered by IDPS or got sampled at the flow classifier level.


%%%%%%%%%%%%%%%%%%%%%%%%%%% Detailed scenario 1; malware propagation
%Consider a statically addressed network of size $\mathcal{N}$ in which a fraction of the hosts $\mathcal{K}$ suffers from a zero-day vulnerability only known to the adversary. The attacker's objective is to locate such hosts in the network, based on a target discovery strategy (e.g., a random scan scheme, a hitlist, etc) associated with a probability $p_i$, and infect them during the Window of Vulnerability (WoV) time as the number of vulnerable systems is not yet shrunken to insignificance and the attacker’s exploit is effective in this period. The game starts with one infected machine as the ``Patient Zero''. The attacker desires to take control of at least $k$ out of $K$ vulnerable hosts, meaning that the winning state for the adversary is defined as $(i=k,*)$. In the meantime, the defender monitors the network via an inline network intrusion detection and prevention system. In addition, defense agents $H$ (e.g., honeypots, host-based intrusion detection systems) are distributed in the environment as well. Hence, the defender is capable of preventing the attack progress (halting an adversarial move) via common schemes such as session snipping, in addition to dropping/rejecting suspicious network activities, and altering and sanitizing the malicious content within a packet with some probability $f(l)$, in which $l$ is the number of so far collected attack samples. These attack samples are provided to the defender through traffic analysis tools (e.g., a ) classifier engine (dealing with a copy of traffic) for the purpose of suspicious flow detection, or the defense agents such as honeypots implemented in the network\footnote{This is a very common architecture in automatic signature generation schemes (e.g., see \cite{kim2004autograph,newsome2005polygraph,li2006hamsa,tang2011signature})}. The function $f$ value can be updated in two different manners: $(1)$ if an adversary's agent hits a honeypot with probability $h = H/N$; or $(2)$ if the packet will be correctly labled as suspicious at the flow classifier level with probability $\gamma$. Notice that the adversary's chance of making a progressive move in the future time steps decreases as the $f$ function's value increases over time. 
%
%For a \emph{skillful} adversary leveraging different evasion techniques and being capable of sneaking through the defensive system, signature generation is not a rudimentary task meaning that only a few attack/malware samples are not enough for the purpose of signature generation. For instance, a polymorphic or metamorphic worm (in contrast with monomorphic malware) will disclose minimum information by encrypting the content and obfuscating the instruction sequences for each connection respectively. Such a skillful attacker can minimize the information leakage to the defender, or in other words maximizing its cost (e.g., time),  for the suspicious traffic flow detection, signature generation, malware analysis, and reverse engineering processes.
%
%At each timestep, the attacker tries to locate a vulnerable node in the network, based on its target discovery strategy (e.g., a random scan scheme, a hitlist, etc). The attackers move might bring to a halt with probability $f(l)$ (based on current attack signature), if not it has the chance of hitting a vulnerable node with some probability $p_i$, or hitting a defense agent with probability $h=H/N$ or hitting a regular host with probability $1-p_i-h$. Moreover, the attacker's move might be observer via the defenders traffic analysis tool.
%For simplisity, we model the classifer as a probabilistic sampling process \cite{sperotto2010overview} in which each incoming adversarial packet is sampled with probability $\gamma$. Note that $\gamma$ reflects the classifier's accuracy in which it is the probability that an incoming packet will be marked as suspicious traffic conditioned on the fact that it is indeed malicious. In addition, there exist $\mathcal{H}$ honeypots implemented in the network as the electronic decoys for the purpose of attack information gathering. The attack information (i.e., packet payload samples) from the honeypots and the flow classifier is given to the signature generator engine for the purpose of signature generation. The generated signatures then are used for the inline packet filtering by the IDPS (see Fig. \ref{fig.ids_scenario}).
%
%
%
%%Nevertheless, we give the defender the opportunity to learn from the adversarial moves and actions. 
%%The idea is that in the early phases of an epidemic, the defender's knowledge of the attack, i.e., a valid signature, is limited (almost non-existent). As the game proceeds, and by witnessing enough number of attack samples, the defender's detection rate increases by improvements in the quality of signatures it has for that specific class of malware.
%%In order to study the learning rate of a signature generation algorithm or the time that the system is finally trained
%%and is able to detect the adversary's actions with probability almost $1$, we consider a cumulative time-varying function $0\leq f\mytiny{(}.\mytiny{)} \leq 1$ as the detection rate, which is a function of the total number of times an adversary agent's activity is captured or in other words, an attack sample is given to the signature generator engine. 
%%The idea is the more samples\footnote{Byte pattern or binary representation of the malware} are given to the defender, the more accurate would be the signatures which immediately reflects in the detection rate which is used by the system to filter potential future malicious traffic. 
%This function's value can be updated in two different manners: $(1)$ if an adversary's agent hits a honeypot with probability $h = H/N$; or $(2)$ if the packet will be correctly labled as suspicious at the flow classifier level with probability $\gamma$. Notice that the adversary's chance of making a progressive move in the future time steps decreases as the $f$ function's value increases over time. In these cases, $f$ will be updated by one factor meaning that some information is leaked about the malware components or the attack technology to the defender where it can take the defender one step closer to understanding the attack signature thoroughly (see lines \ref{alg.def_start} to \ref{alg.def_end} of Algorithm \ref{alg:sim}). This function represents the probability that given $l$ samples so far, the system detects a new incoming malicious packet and filters it on the fly.
%
%The system state $(i,l)$ represents the total number of infected machines and the total number of captured attack traffic (i.e., malware samples) so far by the defense system. The attacker's view of the system state will change if an agent's effort in infecting a new node is successful (or if it possibly loses its control over an agent).
%The defender's view gets updated as a consequence of discovering an adversarial move (i.e., an attack/malware sample). This increasing knowledge of the attack technology enables the defender to correctly detect and halt a new incoming malicious packet with some probability $f\mytiny{(}.\mytiny{)}$ (true positive). It is also possible that the system fails in detecting a malicious packet (or it falsely labels it as benign) with probability $1-f\mytiny{(}.\mytiny{)}$ (false negative). Note that we do not care about the occurrence of false positives (categorizing a benign activity as malicious or abnormal), as they only play a role in the system performance and the defender's detection cost meaning that such incidents do not change the security state of the system (neither the attacker's nor the defender's view). 
%
%%\begin{figure}%[h!]
%%	\begin{center}
%%		\scalebox{0.60}
%%		{\includegraphics{IDPS_detectionSchemeFull.pdf}}
%%		\caption{Defense system architecture}
%%		\label{fig.ids_scenario}
%%	\end{center}
%%\end{figure}
%
%
%Algorithm \ref{alg:sim} shows the above description of the game in which the game simulator takes $\mathcal{N,K,H},k$, and an adversarial exploit $\varepsilon$, in addition to the detection probability $f\mytiny{(}.\mytiny{)}$, the sampling rate $\gamma$, and an acceptable ``threshold'' $1-\tau$ as the input and outputs who wins the game. The termination rule is whether the attacker compromises its desired number of hosts $k$ or if the defender decides if its attack signatures' quality is good enough for malicious traffic detection and filtering, that is $f\mytiny{(}.\mytiny{)} \geq 1-\tau$. Note that the transmit method returns a tuple, i.e., if the transmitted packet by the attacker got filtered by IDPS or got sampled at the flow classifier level. In section \ref{sec:secAna.sim}, we investigate the role of convergence rate of $f(.)$ and the acceptable thresholds for the defender in order to be able to win the game. It turns out that for a  stagnating learning rate  $f\mytiny{(}.\mytiny{)} = 1-\tau$, for some $\tau>0$, the adversary will always win. So, claiming to be victorious as a defender in line 12 is premature.
%%%%%%%%%%%%%%%%%%%%%%%%%%% END OF Detailed scenario 1; malware propagation

\subsection{A Moving Target Defense Game}  \label{CS2}
As another example, we consider the ``Multiple-Target Hiding'' (MTH) game introduced in \cite{saeed2016markov} with minor modifications to the game. In the MTH game studied in \cite{saeed2016markov}, the adversary is interacting with a probabilistic defender taking advantage of a moving target defense strategy in which it reallocates/shuffles its resources at each time step of the game with some probability $\lambda$ (for instance, consider an IP hopping strategy). In order to win the game, the adversary needs to locate $k$ out of $\mathcal{K}$ sensitive targets/resources distributed in the environment while there exist in total $\mathcal{N}$ ``locations''. The defender moves by reallocating a target causing the attacker to redo its search for the locations. The attacker moves by selecting one of the $\mathcal{N}$ possible locations and examining whether it corresponds to one of the targets or not. Notice that MTD strategies are usually costly for the defender as they have an immediate impact on the availability of the resources and system performance. Therefore, instead of a randomized defense strategy (i.e., a probabilistic move at each time step), we consider that the defender issues a move if the number of observed adversarial actions reaches a threshold $L^*$ based on which an attack detection signal is being generated. 

\begin{algorithm}%[h]
	\caption{MTD  game simulator}
	\label{alg:MTDsim}
	\begin{algorithmic}[1]
		\Function{Simulator}{$\mathcal{N,K,H},k,\sigma,\gamma,L^*$}
		\State {$\mathcal{I} = \emptyset$; $l = 0$;}
		\State {reallocateResources = False};
		\State {winningState = False};
		\While {not reallocateResources and not winningState}
%		\State {observed,targetHost $\xleftarrow[\text{}]{(\gamma,h),\$} locate(\mathcal{N}\setminus \mathcal{I})$};
		\State {observed,targetHost $\xleftarrow[\text{}]{(\gamma,h),p_i} locate(\mathcal{N},\sigma)$};
		\If {observed} \label{alg:MTDsim.def_observe}
		\State{$l\pluseq 1$};
%		\State {update $f(l)$};
%		\If {$f(l) \geq f(L^*)$}
		\If {$l \geq L^*$}
		\State {reallocateResources = True};
		\State {$\mathcal{I} = \emptyset$};
		\State {Output \textit{"Game is finished. Defender won!"}};
		\EndIf 
		\EndIf \label{alg:MTDsim.def_end}
		\If {targetHost $\in \mathcal{K}$}
		\State $\mathcal{I} = \mathcal{I}~ \cup$ targetHost;
		\If {$|\mathcal{I}| \geq k$}
		\State {winningState = True};
		\State {Output \textit{"Game is finished. Adversary won!"}};
		\EndIf 
		\EndIf
		\EndWhile
		\EndFunction
	\end{algorithmic}
\end{algorithm}


The system state $(i,l)$ represents the total number of located target machines by the attacker and the total number of recognized adversarial moves so far by the defender. The attacker's view of the system state will change if it successfully finds a sensitive target based on its target discovery strategy $\sigma$, while the defender's view gets updated as a consequence of discovering an adversarial move (whether on network levels with probability $\gamma$ or on host levels with probability $h$ via a defense agent). 
Algorithm \ref{alg:sim} shows the above description of the game in which the game simulator takes $\mathcal{N,K,H},k$, and an adversarial target discovery strategy $\sigma$, in addition to the sampling rate $\gamma$, and a ``threshold'' $L^*$ as the input and outputs if the attacker wins the game. The termination rule is whether the attacker finds its desired number of sensitive targets $k$ or if the defender reallocates its resources as it discovers enough amount of attack evidence.

%\subsection{A Game of sneaky Defender}  \label{CS3}
%
%In this example, we consider a sneaky defender in which it already knows the attacker and its current attack methodology (e.g., it already has the attack signature), but if it brings all the adversarial moves to a halt (for instance, filtering the attack traffic), the attacker recognizes that its attack vector and methodology is known to the defender and it will, therefore, invest on finding a new attack vector not known to the defender. In this regard, the defender prefers to keep the attacker busy before . To mitigate the attack damage, the defender can lead the attack traffic to non-sensitive targets (for instance an electronic decoy such as a honeypot). However, in order to not to make the attacker suspicious, it will let the attacker proceed with its attack objective (for instance directing the attack traffic to sensitive targets). The defender's objective is to keep the adversary busy before the attack objective is satisfied within $T_{bud}$ (denoting the attacker's resources invested in the attack, e.g., time, USD).

==> General_paper_S&P_Eprint/sections/conclusion.tex <==
%\noindent
%Note that the analysis presented in this work can be applied to specific architectures and IDPS types by considering related parameters. For instance, if we are dealing with a network-based architecture with \emph{inline} sensor deployment, the IDPS can potentially halt attacks by blocking network traffic since this traffic is passing through the system. On the other hand, a passive sensor deployment, which deals with copies of actual network traffic by means of spanning ports or network taps or even IDS load balancers, usually provide a narrower detection, smaller detection accuracy. Therefore, by choosing the framework parameters finely tuned, one can capture the specfic scenario under study.
%With respect to our framework, considering the preventing capabilities of IDPS, we implicitly are dealing with an inline implementation, since passive architecture does not provide such features inherently. 
This presented work is an attempt at constructing a theory of security and developing a general framework for modeling cyber attacks prevalent today, including opportunistic, targeted and multi-stage attacks while taking practical constraints and observations into consideration. 
To this end, we have modeled the interactions of an adversary (and possibly its agents) with a defensive system during the lifecycle of an attack as an incremental online learning game. In comparison with the available works in this area, which are too simple, specific and static to be used in almost any practical situation, our presented framework, to the best of our knowledge, is the most comprehensive and realistic one which can be used to represent the dynamic interplay between the attacker and the defender. Unlike most of the available research in this area which ignores entirely one player's actions and strategies (usually the defender), we have shown how the game evolves by taking both parties set of available actions and strategies into consideration. More specifically, instead of considering a ``dummy defender'' in our modeling, we gave it the opportunity to learn regarding the attack technology incrementally. As time elapses, and the defender captures more attack samples, it can reach better detection rates and accuracy. This learning rate indeed reflects into higher quality attack signatures and detection rates which can be used to bring a next adversarial move to a halt and hence to contain the adversary meaning that the adversary's probability of making a progressive move in the game decreases consequently.

%We revisit the spread of malware phenomenon from a completely new perspective and we walk through the example of malware propagation and botnet construction.
%Although the self-propagating class of malware might seem to be an \emph{old}\footnote{The Morris worm was the first computer worm released on the Internet on Nov. 1988, almost three decades ago.} type of a threat due to the decline in the ``worm-like'' common vulnerabilities exposures (CVEs) \cite{cisco:Misc},  the rise of self-propagating ransomware (e.g., the WannaCry cryptoworm) and the highly sophisticated malware such as Stuxnet worm attest that the network vector is one of the few attack vectors which is capable of passing the test of time. 
%Taking advantage of the network vector and releasing the malware in a worm-like fashion, meaning that the malware is equipped with a self-propagating functionality, can provide the attackers a more potent malware which is capable of causing widespread damage.
%This means that the security community and professionals need to take the self-propagating class of malware more serious to first better understand such malware lifecycle and then to be able to come up with feasible solutions to tackle this problem.




%One flew over the botmaster's network, i.e., the botnet, answers the question of  ``\emph{how does the malware spread and why do we see exponential growth in the number of botnets found in the wild?}''. 
By focusing on the most significant and tangible aspects of sophisticated cyber attacks i.e., (1) the amount of time it takes for the adversary to accomplish its mission and (2) the success probabilities of fulfilling the attack objectives, we were able to study under which circumstances the defense system can provide an effective response that makes the probability of  reaching an attack objective $k$ to be $poly(T_{bud})negl(k)$ in which $T_{bud}$ is the attacker time budget. This led us to the definition of a \emph{security capacity region} as a metric for gauging a defensive system’s efficiency from a security perspective. In particular, we show that a stagnating learning rate allows the attacker to win meaning that being able to reach its attack objective within a limited budget (e.g., time, US dollars), whether it is constructing a botnet of any specific size or locating information on a distributed number of nodes. The defender cannot wait for too long learning about a used attack vector/exploit, and once learning starts it must continue learning with an associated detection probability converging fast enough to $1$. Our security analysis gives precise recommendations for the defender, i.e.,  $1-f(l)\leq O(l^{-a})$ for some $a \geq 2$ with a proof for $a=2$ in our framework. The attacker needs to find just one attack vector/exploit for which the defender is too slow to react or too slow in learning. 



%By focusing on the most important and tangible aspects of sophisticated cyber attacks: (1) the amount of time it takes for the adversary to accomplish its mission and (2) the success probabilities of fulfilling the attack objectives we translated attacker-defender interactions into a well-defined game so that we are able to provide rigorous cryptographic security gurantees for a system given both players' tactics and strategies. We generalize the basic notion of computational security of a cryptographic scheme \cite{lindell2014introduction} to a \emph{system} which must be defended and introduce a \emph{computationally secure system} in which a ``given (\emph{system}) is $(T_{bud},k,\epsilon)$\emph{-secure} (for $T_{bud},k > 0$, and $\epsilon \leq 1$), if every adversary playing for the time budget at most $T_{bud}$ succeeds in breaking\footnote{The notion of breaking the system however could mean different in different scenarios.} the (\emph{system}), in other words, reaching the attack objective $k$, with probability at most $\epsilon$''.  We study under which circumstances the defense system provides an effective response that makes $\epsilon = poly(T_{bud})negl(k)$.

An essential venue of future work is to estimate the learning rate $f(l)$ based on the number of observed malicious acts given a ``worst-case adversary''. Our framework lays the foundation for such work and allows to give a worst-case probabilistic bound on the maximal reached attack objective based on the estimated $f(l)$. This, in turn, will give guidance to the defender in how to allocate its resources. In addition, we notice that the learning rate might not always be positive, for instance, when dealing with a \emph{delusive} adversary who maliciously engineers the training data to prevent a learner from generating an accurate classifier, even if the training data is correctly labeled \cite{newsome2006paragraph}. Therefore, in case of noise injection attacks, such as deliberately crafted attack samples to mislead the defender's learning engine, and in general a delusive adversary, the learning engine's false positive rates should be taken into consideration, and we leave this problem for future studies.

%Although we walk through the example of malware propagation and botnet construction, the strength of our framework is that it not only can be used for malware (e.g., a worm/bot) propagation modeling, but also it can be used to model the dynamic nature of most network security games. It is general enough to potentially capture other possible scenarios such as APT, hitlist worms \cite{antonatos2007defending}, and MTD strategies \cite{saeed2016markov}. We believe our study can provide network security researchers and architects valuable lessons and more robust understandings of both attack and defense technologies concerning malware with a broad audience. Besides, with the advent of software-defined networking (SDN) in which the entire network infrastructure can be controlled from a centralized software controller, new generations of traditional cyber defense technologies (e.g., HPs, IDPSes, firewalls, etc.), which are more capable, scalable and secure, are already being introduced.
%This could be a new opportunity and a fresh start to fight against the botnet phenomenon or the spreading of the malware in general.

%By modeling the learning rate of the defender as a function $f\mytiny{(}l\mytiny{)}$ (which is the probability of detecting and filtering a next malicious payload) where $l$ represents the number of malicious payloads for a specific exploit so far collected, we presented the following results:
%\begin{itemize}
%	\item If $f\mytiny{(}l\mytiny{)}$ does not converge to $1$, then we call such a learning rate stagnating and the adversary is able to reach his goal of $k$ compromised nodes within $poly(k)$ time budget.
%	\item If $f\mytiny{(}l\mytiny{)}\rightarrow 1$ and more specifically $1-f\mytiny{(}l\mytiny{)} = O(l^{-2})$, then the probability of the adversary affecting $k$ nodes (i.e., the probability of winning) is proven to be polynomial in the attacker's time budget and negligible in $k$. Numerical analysis shows that this property is even satisfied for $1-f\mytiny{(}l\mytiny{)} = O(l^{-???})$.
%	\item The above results hold for time budget measured in logical Markov model transitions or real time (seconds), and also hold for learning rates that remain equal to $f(l)=0$ until a certain number $l=L^*$ malicious payloads have been collected after which learning starts.
%	\item The presented adversarial/defender game in terms of a Markov model is general and fits most practical scenarios as our extensive overview shows.
%\end{itemize}
%The adversary may not reach his goal of $k$ compromised nodes, but will reach a much smaller number $k_c$ compromised nodes of the order $O(L^* \log T_{bud})$, where $T_{bud}$ is the attacker's time budget, for $1-f(l) \rightarrow 0$. We conclude that at a meta level the adversary needs to find  one exploit for which the defender cannot find a fast enough increasing learning rate and the defender needs to have a learning system/methodology in place which should be able to reach fast enough learning rates for any possible exploit. In practice infrastructures are being compromised and this means that, as given by our general framework, its thorough analysis, and numerical analysis, effort is needed in order to understand associated learning rates and why these are $\leq 1-O(l^{-???})$ or have $L^*=O(k)$ (i.e., learning starts too late).

%We believe our study can provide network security researchers, system architects, and administrators an intuitive overview and a more robust understanding of how large-scale self-propagating malware could behave in the wild and how effective current security solutions are when it comes to fighting against such malware. This type of work can be very beneficial especially with the advent of software-defined networking (SDN) in which the entire network infrastructure can be controlled from a centralized software controller, new generations of traditional cyber defense technologies (e.g., HPs, IDPSs, firewalls, etc.), which are more capable, scalable and secure, are already being introduced \cite{giotis2014combining,zanna2014adaptive,hu2014flowguard,han2016honeymix,fan2017novel,jin2018snapshotter,mehdi2011revisiting}. 

%Although we walk through the example of malware propagation and botnet construction, the strength of our framework is that it not only can be used for malware (e.g., a worm/bot) propagation modeling, but also it can be used to model the dynamic nature of most network security games. It is general enough to potentially capture other possible scenarios such as APT, hitlist worms \cite{antonatos2007defending}, and MTD strategies \cite{saeed2016markov}. We believe our study can provide network security researchers and architects valuable lessons and more robust understandings of both attack and defense technologies concerning malware with a broad audience. Besides, with the advent of software-defined networking (SDN) in which the entire network infrastructure can be controlled from a centralized software controller, new generations of traditional cyber defense technologies (e.g., HPs, IDPSes, firewalls, etc.), which are more capable, scalable and secure, are already being introduced.
%This could be a new opportunity and a fresh start to fight against the botnet phenomenon or the spreading of the malware in general.

%\cite{giotis2014combining,zanna2014adaptive,hu2014flowguard,han2016honeymix,fan2017novel,jin2018snapshotter,mehdi2011revisiting}

%\textbf{Acknowledgements.}  [Redacted for anonymity during review process]

% As another example, \cite{nobakht2016host} proposes an SDN-enabled host-based intrusion detection and mitigation framework called IoT-IDM to protect IoT devices deployed in a smart home along the same lines of \cite{mehdi2011revisiting} which revisits traffic anomaly detection using SDN in a small network. However, before a complete transfer, such defensive tools and technologies' effectiveness should be studied effectively from a security standpoint.

==> General_paper_S&P_Eprint/sections/game.tex <==
In this section, we introduce a general network security game based on the interactions between an adversary, its agents (e.g., bots controlled by a botmaster), and a defender who is equipped with a logically centralized defense system\footnote{For instance, network/host-based intrusion detection and prevention systems, honeypots, etc. One motivation for our work is the advent of Software-Defined Networking (SDN) in which the entire network infrastructure can be controlled from a centralized software controller.} implemented in the network. We explain how this game can be directly mapped to an equivalent Markov model and in the next section, we provide the security analysis for this Markov model as well as presenting compelling interpretations of the role of both players' strategies in their probability of winning the introduced game. 
%An upper bound on the adversary's probability of success is derived. In addition, the security capacity of the defense strategies (more specifically, any automatic signature generation scheme) is defined and calculated to gauge the effectiveness of the defense system.
%\footnote{Also referred to as the attacker or the intruder}

%To create a realistic mathematical model, we make reasonable simplified assumptions from both attack and defense perspectives. This is due to the significant level of freedom in attack design and technology and the complexity and diversity of defense mechanisms and systems.
%As there is a significant level of freedom in malware design (specifically malware with a broad audience e.g., worms and bots) \cite{wagner2003experiences}, in addition to complexity and diversity of such malware defense mechanisms (specifically IDPS and HPs) in order to create a realistic mathematical model which could be used to predict the behavior of such malware, we have to let go of some attack/defense details. 
%For instance, from the adversarial perspective, we do not mind the nature of vulnerabilities exploited by the adversary to compromise a system. Similarly, malware's host-level activities are not in the interest of this work. Such behaviors could be different for various malware (e.g., staying dormant for a specific time or immediately initiate malware operations). 
%Moreover, we provide the analysis for a random scanning strategy as the malware target discovery scheme and give general guidance on how the proposed model can capture other types of scanning methods including the hitlist strategy (see section \ref{AC-role}).








%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%From the defensive perspective, we encounter the same challenge as before. 
%For instance, when it comes to evaluating a defense system's efficiency (especially an IDPS), the accuracy, performance, completeness, fault tolerance, and timeliness properties should be taken into considerations as the top five criteria \cite{debar2000introduction}. However, for this study, we believe considering all the playing factors in modeling such systems makes the model excessively complicated (and possibly inaccurate). For this reason, we mainly focus on \emph{security-related} concerns and specifications, i.e., the accuracy and completeness (dealing with false alarms and detection rates) of the system. This means the ability of the system in detecting malicious behaviors and parties in the environment, and taking effective actions to foil such incidents, regardless of its architecture, used methods, or its impact on the system performance.
%Therefore, assuming that the non-security related traits are ideal (e.g., no latency, high performance, unlimited bandwidth and fault tolerance), we are dealing with a defense system which is neither entirely accurate nor complete, as every information technology system suffers from security shortcomings and deficiencies.

%In this regard, we consider a general system state $(i,l)$ which only captures the security-related parameters. From the adversary's perspective, its view of the system state will change if only it makes a progressive move in the game. 
%For instance, a bot herder's successful effort in infecting a new node or if it possibly loses its control over an agent. 

%We consider a detection function at the network level for the defender meaning that it can correctly detect a malicious packet with probability $f\mytiny{(}.\mytiny{)}$ (true positive) and with $1-f\mytiny{(}.\mytiny{)}$ it fails to detect such packet, or it falsely labels that as benign (false negative). Hence, the defender's view gets updated as a consequence of detecting an adversarial move (i.e., a malware sample) and an increase in its detection accuracy. Note that we do not care about the occurrence of false positives (categorizing a benign activity as malicious or abnormal), as they only play a role in the system performance and the defender's detection cost meaning that such incidents do not change the security state of the system (neither the attacker's nor the defender's view). 
%The defender's view gets updated as a consequence of discovering an adversarial move (i.e., an attack sample). This increasing knowledge of the attack technology enables the defender to correctly detect and halt a new incoming malicious action with some probability $f\mytiny{(}.\mytiny{)}$ (true positive). It is also possible that the system fails in detecting an adversarial move (or it falsely labels it as benign) with probability $1-f\mytiny{(}.\mytiny{)}$ (false negative). Note that we do not care about the occurrence of false positives (categorizing a benign activity as malicious or abnormal), as they only play a role in the system performance and the defender's detection cost meaning that such incidents do not change the security state of the system (neither the attacker's nor the defender's view). 
%The defender's view gets updated as a consequence of detecting an adversarial move (i.e., attack/malware samples denoted by l). This update immediately reflects into the system's probability of halting next incoming malicious traffic. By denoting this probability as f, the system is capable of correctly detecting and halting a malicious packet with $f(l)$ (true positive) and with 1- f, it fails to detect such malicious packets (false negative).

%We notice that in many attacker-defender based games the interplay of the players could be summarized in one of the following states: (1) The attacker might have a fruitless effort, meaning that no progress in the game, but it got lucky and no information was leaked to the defender.
%(2) As a result of adversary's action, it might make a progress in the game meaning that getting one step closer to its final attack objective without revealing/leaking any information regarding the attack technology to the defender. This move is an ideal and perfect move for the attacker. However, it is also possible that (3) in spite of making progress in the game, the defender observes that adversarial moves meaning that both players get one step closer to their objective. And finally, (4) there might be the case in which the attacker gains nothing after its move but the defender observes the attack as a result of attack information leakage during the adversarial move.


\subsection{The Game of Consequences}

\noindent
{\bf [Game Setup]}
In almost any sophisticated and persistent cyber attack, the adversary continues the attack until its attack objective is satisfied. However, due to the incomplete and imperfect information of the players (in this case the attacker), and the probabilistic nature of an attack's success rates, the attacker's objective usually cannot be achieved in only a few numbers of moves/attempts. Adding a defender to this picture leads to an unceasing game unless the attacker decides not to play anymore (i.e., dropping out of the game, whether the attack objective is satisfied or the chances of making a progressive move become overwhelmingly small). We model the interactions of players in such scenarios as a stochastic game. 

To create a realistic mathematical model, we make reasonable simplified assumptions from both attack and defense perspectives. This is due to the significant level of freedom in attack design and technology and the complexity and diversity of defense mechanisms and systems.
For instance, when it comes to evaluating a defense system's efficiency (especially an IDPS), the accuracy, performance, completeness, fault tolerance, and timeliness properties should be taken into considerations as the top five criteria \cite{debar2000introduction}. However, for this study, we believe considering all the playing factors in modeling such systems makes the model excessively complicated (and possibly inaccurate). For this reason, we mainly focus on \emph{security-related} concerns and specifications, i.e., the accuracy and completeness (dealing with false alarms and detection rates) of the system. This means the ability of the system in detecting malicious behaviors and parties in the environment, and taking effective actions to foil such incidents, regardless of its architecture, used methods, or its impact on the system performance.
Therefore, assuming that the non-security related traits are ideal (e.g., no latency, high performance, unlimited bandwidth, and fault tolerance), we are dealing with a defense system which is neither entirely accurate nor complete, as every information technology system suffers from security shortcomings and deficiencies.

In this regard, we consider a general system state $(i,l)$ which only captures the security-related parameters. The players start the game at the state $(i=0,l=0)$ in which it represents the inauguration of the attack and the zero-knowledge of the defender regarding the attack technology at time zero. From the adversary's perspective, its view of the system state $i$ will change if only it makes a progressive move in the game. On the other hand, by noticing that any adversarial move (whether fruitful or fruitless) can potentially be observed and captured by the defender (for instance via the defense system's agents and sensors implemented in the environment), we model the defender as an incremental online learning process\footnote{Another motivation for this work is the introduction and widespread embrace of Automated machine learning (AutoML) which provides the opportunity for automatic (and possibly distributed) attack learning, detection, and prevention.}, meaning that
%However, the game setup and settings, highly dependent on the system parameters and are application dependent.
the defender's view $l$ gets updated as a consequence of discovering an adversarial move (i.e., an attack sample). This increasing knowledge of the attack technology enables the defender to correctly detect and halt a new incoming malicious action with some probability $f(l)$ (true positive). It is also possible that the system fails in detecting an adversarial move (or it falsely labels it as benign) with probability $1-f(l)$ (false negative). Note that we do not care about the occurrence of false positives (categorizing a benign activity as malicious or abnormal), as they only play a role in the system performance and the defender's detection cost meaning that such incidents do not change the security state of the system (neither the attacker's nor the defender's view). 

%The players start the game at the state $(k=0,l=0)$ in which it resembles the inauguration of the attack and the zero-knowledge of the defender regarding the attack technology at time $0$. 
%The attacker's objective is to reach a winning state of the form $(k, *)$ within a limited time budget $T_{bud}$. We emphasize that $k$ or in the other words the attack objective differ from scenario to scenario. For instance, a malware propagator or a botmaster desires to push $k$ as high as possible\footnote{Or at least \%5 of the total number of vulnerable hosts, as \cite{provos2004virtual} shows via simulation that in order to have hopes that no more than \%50 of the total vulnerable hosts ever become infected, patching process must begin before \%5 of such population become ever infected}. On the contrary, in an advanced persistent threat, the attacker might prefer to stop playing in a much smaller $k$ to minimize the attack detection probability. An adversary trying to access distributed information on a set of nodes within the network might want to stop the attack as soon as its mission is accomplished. As another example, to construct a hitlist, the attacker will terminate its reconnaissance after the compiled list of vulnerable nodes is constructed.

%Consider a statically addressed network of size $\mathcal{N}$. We assume that a fraction of the hosts $\mathcal{K}$ suffer from a zero-day vulnerability only known to the adversary. The adversary's objective is to locate such hosts in the network and infect them immediately while there exists an opponent player who can observe attacker's activities and learn from them to halt its next actions. 

\noindent
{\bf [Attacker]} 
%The game starts with one infected machine as the ``Patient Zero''. The attacker desires to take control of at least $k$ out of $K$ vulnerable hosts in the network. A few motivations for the adversary include worm propagation, constructing a botnet, or accessing distributed information on a set of nodes within the network. Note that from a practical perspective, $k$ can also represent \%5 of the total number of vulnerable hosts, as \cite{provos2004virtual} shows via simulation that in order to have hopes that no more than \%50 of the total vulnerable hosts ever become infected, patching process must begin before \%5 of such population become ever infected (i.e., the attacker must infect at least $k=0.05K$ nodes before a cure is found or in other words, the defender must learn a high-quality signature before more than \%5 of $K$ get infected).
The attacker's objective is to reach a winning state of the form $(k, *)$ within a limited time budget $T_{bud}$. We emphasize that $k$ or in other words the attack objective differs from scenario to scenario. For instance, a malware propagator or a botmaster desires to push $k$ (in this case, the total number of infected nodes) as high as possible\footnote{Or at least 5\% of the total number of vulnerable hosts, as \cite{provos2004virtual} shows via simulation that in order to have hopes that no more than 50\% of the total vulnerable hosts ever become infected, patching process must begin before 5\% of such population become ever infected.}. On the contrary, in an advanced persistent threat, the attacker might prefer to stop playing after reaching a much smaller $k$ to minimize the attack detection probability since once the target machine has been identified, the attacker should use as few infections as possible to decrease the chance of exposing the operation. An adversary trying to access distributed information on a set of nodes within the network terminates the attack as soon as its mission is accomplished. In a similar fashion, to construct a hitlist, the attacker will conclude its reconnaissance after a compiled list of vulnerable nodes is constructed.


%For APT attack, to the opposite, the less machine controlled the better. When the target machine has been identified, the attacker should take as few infections as possible to decrease the chance of exposing the operation.

%To reach the winning state, at any time step, the attacker issues a move which can potentially lead to an incremental progress in the game meaning that getting one step closer to the final attack objective. We assign a success probability $p_i$ to each adversarial move at any given state of the game. 
%This probability indeed depicts the attack (atomic move) success probability as a function of attack strategy without taking the effect of the defender's tactics and actions impact on the attacker move into consideration. This enables us to represent the adversarial move in a single transition in the Markov model which will be explained in section \ref{ss.markovModel}. 

To reach the winning state, at any time step, the attacker issues a move associated with a success probability $p$ (purely depends on attack strategy and not the defender's maneuvering) that can potentially lead to incremental progress in the game, i.e.,  getting one step closer to the final attack objective  $(i = i +1)$. This enables us to represent the adversarial move in a single transition in the Markov model which will be explained in section \ref{ss.markovModel}. For generality, we consider a state-dependent success probability, i.e., $p_i$, since, intuitively, there could be cases in which the chances of making a progressive move depends on the current state of the attacker in the game. For instance, consider an attacker who is trying to locate vulnerable nodes within an address space of size $N$, while $i$ out of $K$ vulnerable hosts are already found, this means that the probability of hitting a new vulnerable node is $p_i = (K-i)/(N-i)$. Also, we assume the adversary is aware of its current state in the game $i$ in $(i,l)$ for some $l \geq 0$ but it does not know the defender's knowledge of the attack expressed as $l$.

%We assume that each adversarial move, regardless of how skillful the adversary is, the actions that need to be taken by an adversary in each cycle of a cyber attack's life inevitably involves abnormal and suspicious activities on both host and network levels. 

%Based on this definition of an adversarial move, an attacker agent's endeavor to infect a new node for sure includes an attack sample. In addition, we assume the adversary is given the knowledge if its current state in the game $(k,)$ but he does not know the $l$. unusual port usage \cite{inoue2009automated} and internals such as irregular system call sequences \cite{kolosnjaji2016deep}

Moreover, we assume that at each time step, the interaction of the attacker (or an attacker agent) with the system which is encapsulated as an adversarial move, can potentially leak some information to the defender (if observed) regarding the attack technology and methodology. This is because regardless of the mastery and skillfulness of an attacker, its taken actions during any phase of the attack, inevitably lead to abnormal and suspicious incidents and events on both host and network levels. Hence, almost all security tools and technologies rely on the existence of such attack signal indicators for detection and prevention purposes. For instance, unusual port usage \cite{inoue2009automated}, irregular system call sequences \cite{kolosnjaji2016deep}, and the occurrence of pointer value corruption on a host’s process memory \cite{liang2005fast} are amongst a few events that can happen as a result of adversarial moves on host levels.  On the network levels, such conducts include but are not limited to an increase in the network latency, high bandwidth usage, suspicious traffic on exotic ports, irregular scan activity, simultaneous identical domain name system (DNS) requests, and Internet relay chat (IRC) traffic generated by specific ports. 

However, a skillful attacker leveraging different anti-malware and IDPS evasion techniques\footnote{Obfuscation methods, fragmentation and session splicing, application/protocol violations, and DDoS attacks \cite{marpaung2012survey} are among the most common techniques used by the adversaries to decrease the attack detection probability or to increase the chances of attack prosperity.} is capable of minimizing the detection possibilities and therefore reducing the chances of leaking attack information at each adversarial move by sneaking through the defensive system. This skillfulness can provide the adversary more time to play the game as each attack sample has a lower probability of being discovered and in extreme cases, it can ideally be different for each adversarial move making the defender's job surely difficult.
For instance, an attacker taking advantage of a polymorphic or metamorphic malware (in contrast with a monomorphic one) will disclose minimum information by encrypting the content and obfuscating the instruction sequences for each connection respectively leading to more propagation time available to the attacker. 
Therefore, dealing with a skillful adversary, if the defense system captures an attack sample, this property intuitively leads to maximizing the time and effort to push out a solution to stop the attack and generate an attack signature. More importantly, it means that only a few samples are not enough for attack signature generation. Note that this property helps to minimize the information leakage for the suspicious traffic flow detection, signature generation, malware analysis, and reverse engineering processes.

%We consider an atomic move for the adversary (or its agents) and that is the combined set of actions it takes at each time step based on the attack strategy which can take it one step closer to the attack objective. For instance, in a malware propagation game, the target discovery and compromise in addition to the malware delivery and activation can be considered as an adversarial move.  This enables us to represent the adversarial move in a single transition in the Markov model which will be explained in section \ref{ss.markovModel}. Based on this definition of an adversarial move, an attacker agent's endeavor to infect a new node for sure includes an attack sample. In addition, we assume the adversary is given the knowledge if its current state in the game $(k,)$ but he does not know the $l$.

%Moreover, let's assume the adversary is \emph{skillful}, meaning that it leverages different anti-malware and IDPS evasion techniques and is capable of sneaking through the defensive system. Note that this property helps to minimize the information leakage for the suspicious traffic flow detection, signature generation, malware analysis and reverse engineering processes. For instance, a polymorphic or metamorphic worm (in contrast with monomorphic malware) will disclose minimum information by encrypting the content and obfuscating the instruction sequences for each connection respectively. Therefore, for a skillful adversary taking advantage of a polymorphic worm, each worm sample is ideally different from other samples which makes the signature generation task surely difficult.
%Therefore, if the defense system captures a malware sample, this property intuitively leads to maximizing the time and effort to push out a solution to stop the malware and generate a universal signature for that specific class of malware. More importantly, it means that only a few samples are not enough for the purpose of signature generation.


%\noindent
%{\bf [Attacker's Move]} 
%
%
%
%\noindent
%{\bf [Defender's Move]} 
%
%
%\noindent
%{\bf [Game/System State]} 
%
%\noindent
%{\bf [Attack Objective or Winning State]} 

%We combine the multiple steps an adversary agent needs to take in order to infect a new machine into a single one and call it an adversarial move. These steps include target discovery and compromise, malware delivery and activation. Note that this is a practical assumption as the most common form of a self-replicating code found in the wild is a \emph{self-carried}\footnote{The malware payload is transferred in a packet by itself.} malware which, regardless of the transmission scheme (TCP or UDP) utilizes a blind scan strategy as its target discovery (see Table 1 in \cite{li2008survey}). First, this allows us not to be concerned about more stealthier propagation schemes (e.g., second channel delivery) which are usually more robust against anomaly-based detection systems, as they will not trigger any events during the propagation. Moreover, this enables us to represent the adversarial move in a single transition in the Markov model which will be explained in section \ref{ss.markovModel}. Based on this definition of an adversarial move, an agent's endeavor to infect a new node for sure includes a malware sample. 
%On the same lines, agent to agent and C\&C communications are not needed to be considered in the model. First, such communications are not essential during the propagation and zombie army construction phase. Second, such packets do not include any information regarding the malware payload for the purpose of signature generation. However, we give the adversary the knowledge of the total number of infected machines at each time step for free (without the extra cost of revealing any information about the attack/malware technology). Hence, at each time step, with a random scan strategy, the probability that an agent hits a vulnerable target would be $p_i = (K-i)/(N-i)$, considering that $i$ nodes from the $K$ population are already compromised.



%Since we are only concerned with payload-based detection schemes at the network level, we combine the multiple steps an adversary agent needs to take in order to infect a new machine into a single one and call it an adversarial move. These steps include target discovery and compromise, malware delivery, and activation. First, this lets us not to be concerned about more stealthier propagation schemes which are usually very robust against anomaly-based detection systems, as they will not trigger any events during the propagation. These methods include second channel delivery and embedded propagation schemes \cite{li2008survey}.

%Moreover, this enables us not to worry about the transmission scheme used in the malware delivery phase. As in the case of \emph{latency-limited} TCP worms, a \textit{syn} packet is usually sent to check if the vulnerable service is available on the target, in contrast to \emph{bandwidth-limited} UDP worms for which the whole worm sample is sent in a single packet regardless of the availability/vulnerability of the target\footnote{The famous SQL slammer is a great example for such scenarios in which the whole worm sample fits into a single UDP packet.}. Based on this definition of the adversarial move, an agent's endeavor to infect a new node for sure includes a malware sample. On the same lines, 
%%as we are not concerned about the behavioral-based detections, and we are only interested in the malware payload, 
%agent to agent and C\&C communications are not needed to be considered in the model. First, such communications are not essential during the propagation and zombie army construction phase. Second, such packets do not include any information regarding the malware payload for the purpose of signature generation. However, we give the adversary the knowledge of the total number of infected machines at each time step for free (without the extra cost of revealing any information about the attack/malware signatures). 
%%This means we do not need to consider fully connected agents who act in an organized fashion (e.g., through a C\&C structure).
%
%Let us consider the most common form of a self-replicating code found in the wild (see Table 1 in \cite{li2008survey}) i.e., a self-carried\footnote{The malware payload is included in each single packet.}
%%	 {it is also possible to deliver the payload via a second channel (e.g. a previously infected machine or the Internet in general)} 
% malware which, regardless of the transmission scheme
%\footnote{For simplicity, we prefer to consider a transmission protocol independent scheme as separating the analysis for TCP and UDP schemes makes the model more complicated without adding interesting insights. Even though a TCP-based transmission scheme relies on a three-way handshaking process and makes the propagation latency-dependent.} (TCP or UDP),                                                                                                                                                                                                                                                                                                                                                                                                                          utilizes a blind scan as the target discovery scheme. Note that this scanning scheme is the most favorable choice for the malware designers (e.g. Morris, CodeRed, Nimda, Slammer). Later we explain how the model can potentially capture other target discovery schemes, including the hit-list strategy.
%%Being self-carried means that the malware payload is included in each worm packet. 

%Moreover, let's assume the adversary is \emph{skillful}, meaning that it leverages different anti-malware and IDPS evasion techniques and is capable of sneaking through the defensive system. Note that this property helps to minimize the information leakage for the suspicious traffic flow detection, signature generation, malware analysis and reverse engineering processes. For instance, a polymorphic or metamorphic worm (in contrast with monomorphic malware) will disclose minimum information by encrypting the content and obfuscating the instruction sequences for each connection respectively. Therefore, for a skillful adversary taking advantage of a polymorphic worm, each worm sample is ideally different from other samples which makes the signature generation task surely difficult.
%Therefore, if the defense system captures a malware sample, this property intuitively leads to maximizing the time and effort to push out a solution to stop the malware and generate a universal signature for that specific class of malware. More importantly, it means that only a few samples are not enough for the purpose of signature generation.

%\begin{figure}%[h!]
%	\begin{center}
%		\scalebox{0.5}
%		{\includegraphics{IDPS_detectionSchemeFull.pdf}}
%		\caption{Defense system architecture}
%		\label{fig.ids_scenario}
%	\end{center}
%\end{figure}

\begin{figure}%[h!]
	\begin{center}
		\scalebox{0.60}
%		
%    \includegraphics[natwidth=305,natheight=467]{IDPS_detectionScheme_v2.pdf}
		{\includegraphics{IDPS_detectionScheme_v2.pdf}}
		\caption{Defense system architecture}
		\label{fig.ids_scenario}
	\end{center}
\end{figure}

\noindent
{\bf [Defender]} 
The defender's objective is to learn more and more regarding the attack technology and methodologies to be able to cease a next incoming adversarial move. In this regard, it monitors the environment for attack detection and prevention purposes via common security tools and technologies. Intrusion detection (and possibly prevention) systems are amongst the most common type of defense technologies used for monitoring, incident identification, attack detection, and prevention on both host and network levels\footnote{The first one is known as host-based intrusion detection system (HIDS), and the latter is known as network intrusion detection system (NIDS).}. Virtual and physical sensors are a common component of such systems used for data collection and analysis. Also, the defender can take advantage of electronic decoys known as honeypots for attack information assembly.

We give the defender the opportunity to learn from observed adversarial moves and actions.
The idea is that in the early phases of the game, the defender's knowledge of the attack is limited (almost non-existent). As the game proceeds, the defender's detection rates will be enhanced by witnessing enough number of attack samples. In order to study the learning rate of the defender or the time that the system is finally trained and is able to detect the adversary's actions with probability almost $1$, we consider a cumulative time-varying function $0\leq f(.) \leq 1$ as the detection rate, which is a function of the total number of times an adversary agent's activity is captured or in other words, an attack sample is given to the defender. The function $f$ indicates the probability that given $l$ samples so far, the system detects and halts a new incoming adversarial move. The idea is the more samples are given to the defender, the more accurate would be its attack signatures which immediately reflects in the detection rate which is used by the system to filter future adversarial moves. 

In this regard, we assume that all incoming traffic passes through an inline NIDS implementation\footnote{Meaning that network traffic directly passes through the IDPS sensors, and the system is capable of session snipping, dropping/rejecting suspicious network activities and altering and sanitizing the malicious content within a packet.} which gives the defender the ability to be able to block an adversarial move with some probability $f(l)$ in which $l$ represents the current realization of the attack by the defender (i.e., based on so far observed and collected adversarial moves and attack information). Moreover, we assume that a copy of all incoming traffic is given to the defender’s traffic analysis and classification engine via a network tap or a spanning port which provides the opportunity of detecting suspicious flows with some probability. For simplicity, however, we model this offline analysis as a probabilistic sampling process \cite{sperotto2010overview} in which each incoming adversarial move can be correctly sampled/labeled as suspicious with probability $\gamma$ (therefore $l = l +1$), and with $1-\gamma$, the defender misses the adversarial move or it falsely labels it as benign. Note that $\gamma$ reflects the classifier's accuracy in which it is the probability that an incoming packet will be marked as suspicious traffic conditioned on the fact that it is indeed malicious.
If the defender fails in bringing an adversarial move to a halt and therefore the attacker proceeds within the system with probability $1-f(l)$, the defender still has the opportunity to learn (i.e., $l = l +1$) regarding the attack technology with probability $h$ via the defense agents (e.g., HPs, HIDS) implemented in the environment. Hence, if the adversary deals with an electronic decoy, or as a consequence of attack activities, on an endpoint device equipped with a HIDS, the defender can learn regarding the attack meaning that $l = l+1$.

In summary, a progressive move by the defender ($l = l+1$) leads to an increase in its future detection rates $f$. This function gets updated in two different manners: $(1)$ if the attack traffic is correctly labeled as suspicious on the network level with probability $\gamma$ or $(2)$ if the attack activity leaks information on host levels with probability $h$ (whether via a honeypot or a host-based intrusion detection system installed on a fraction of defender systems\footnote{Notice that, in case of a honeypot, any adversarial move will lead to an increase in the defender's knowledge of the attack $l$ since all incoming communications with an HP is suspicious, while for a HIDS, not all the adversarial moves might be observed by the defense system. For simplicity, we use a single parameter $h$ as the probability of gaining information on host levels (mainly HPs). However, one can easily separate the learning from HPs and the HIDS agents by considering another parameter for HIDS agents $h'$ or in general, a cumulative function $f_{h'}$  for the host-level attack information and signatures (observed and gained from HIDS agents).}). This incremental learning of the attack enables the defender to be able to bring a new incoming adversarial move to a halt with probability $f(l+1)$.
Notice that the adversary's chance of making a progressive move in the future time steps decreases as the $f$ function's value increases over time.

\subsection{Markov Model of the  Game}\label{ss.markovModel}

The above description of the adversary-defender interactions can immediately be translated into a Markov model.  In summary, at each time step, the state of the system can be identified with a tuple $(i,l)$ in which $i$ represents the adversary's progress in the game, and $l$ delineates the defender's knowledge of the attack methodologies and technology. The adversary (or one of its agents) makes a move associated with a success probability $p_i$. Note that $p_i$ is indeed the attack success probability while there exists no opponent player in the environment (i.e., the defender). In the meantime, the defender can block an adversarial move, if it can detect it correctly or it can learn the attack technology if the attack is observed via the defense system or the attacker is in touch with a defense system agent (e.g., a honeypot) implemented in the environment.
% If the packet does not get filtered and the target is indeed a vulnerable node, it becomes infected and the botnet size increases by one. 

\begin{figure}
	\centering
	\begin{tikzpicture}
	\tikzset{
		>=stealth',
		node distance=3.2cm and 3.2cm ,on grid,
		every text node part/.style={align=center},
		state/.style={minimum width=2.00cm,
			%    		font=\small,
			draw,
			circle},
	}
	% Add the states
	\node[state]             (c) {$i,l$};
	\node[state, right=of c] (r) {$i+1,l$};
	%	\node[state, left=of c] (lose) {0};
	\node[state, above=of c] (b) {$i,l+1$};
	\node[state, above=of r] (rr) {$i+1,l+1$};
	% Connect the states with arrows
	\draw[every loop]
	(c) edge[auto=left]  node {$m_{2}(i,l)$} (r)
	%(r) edge[bend left, auto=right] node {0.7} (s)
	%(c) edge[loop above]             node {($1-p_i-f(.)$)} (c)
	(c) edge[ auto=right] node {$m_3(i,l)$} (rr)
	(c) edge[auto=left] node {$m_4(i,l)$} (b)
	(c) edge[loop left]             node {$m_1(i,l)$} (c);
	%(d) edge[loop above]             node {} (d);
	\end{tikzpicture}
	\caption{Possible transition probabilities at each state $(i,l)$ in the Markov model of the game}
	\label{markovModel}
\end{figure}
%
%Any adversarial move can change the state of the game in one of the following manners: (1) if the adversary's endeavors come to a halt by the defense system with probability $f(l)$, no progress is made in the horizontal axis (the Markov chain remains in the current state or it transits to higher levels $l$, i.e., no progress from the attacker's perspective). We denote the occurance of the event that an adversarial move comes to a halt with $F$. (2) The adversary might 
Let us denote the occurrence of the event that an adversarial move comes to a halt by the defense system with $\emph{F}$ and the occurrence of the event that it gets sampled (or labeled as suspicious) by the defense system with $\emph{S}$. Notice that these two events are independent, as we are assuming that the straining and filtering happens online for each detected incident whereas sampling deals with a copy of the actual traffic for attack analysis and classification.
Therefore the following outcomes are possible at each timestep:
\begin{itemize}
	\item $(F\wedge \widebar{S})$: meaning that the adversasry's move comes to a standstill by the defender (based on current knowledge of the attack technology) but not sampled which happens with probability $f(l)(1-\gamma)$, as a result, the Markov chain stays at state $(i,l)$ 
	\item  $(\widebar{F}\wedge \widebar{S})$: The adversasry's move gets neither filtered nor sampled, there exist three possible scenarios for this case:
	\begin{itemize}
		\item[$-$] if the adversary is dealing with an electronic decoy (i.e., a  honeypot), the defender has the oppurtunity to learn from this interaction meaning that the Markov model transits from state $(i,l)$ to $(i,l+1)$ with probability $(1-f(l))(1-\gamma)h$
		\item[$-$]  if the attacker makes a progressive move with probability $p_i$ then the Markov chain transits to state $(i+1,l)$ with probability $(1-f(l))(1-\gamma)p_i$.  Note that this is a ``perfect move'' for the adversary as in which the attacker gets one step closer to the attack objective while the defensive system was not able to detect and locate the adversary's activities or it falsely labeled the activity as benign (false negative) meaning that no information and knowledge regarding the attack technology is leaked to the defender
		\item[$-$] and if the attacker is not dealing with a defensive agent and not also make a progressive move with probability $(1-p_i-h)$ the Markov chain stays at the current state with probability $(1-f(l))(1-\gamma)(1-p_i-h)$
	\end{itemize}
	\item $(F\wedge S)$: If the attacker's move gets both filtered and sampled, the chain transits to the state $(i,l+1)$ with probability $\gamma f(l)$
	\item $(\widebar{F}\wedge S)$:  If the attacker's action does not get filtered but it gets sampled
	\begin{itemize}
		\item[$-$] for a successful move with probability $p_i$, the Markov chain transits to the state $(i+1,l+1)$ with probability $(1-f(l))\gamma p_i$
		\item[$-$] and for an unsuccessful move with probability $(1-p_i)$, the Markov chain transits to the state $(i,l+1)$ with probability $(1-f(l))\gamma (1-p_i)$
	\end{itemize}
\end{itemize}
In summary, the transition probabilities can be expressed by:
%\begin{equation}
\begin{eqnarray}\label{eq.transitions}
m_1(i,l) &=& Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i,l\mytiny{)})=f(l)(1-\gamma)+\nonumber\\ & &
(1-f(l))(1-\gamma)(1-p_i-h)\\ 
m_2(i,l) &=& Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i+1,l\mytiny{)}) = \nonumber\\ & & (1-f(l))(1-\gamma)p_i \\
m_3(i,l) &=& Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i+1,l+1\mytiny{)}) = \nonumber\\ & & (1-f(l))\gamma p_i\\
m_4(i,l)&=& Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i,l+1\mytiny{)}) = \nonumber\\ & & (1-f(l))(1-\gamma)h+  f(l)\gamma +\nonumber\\ & &  (1-f(l))\gamma (1-p_i)
\end{eqnarray}

%	$$
%\begin{aligned}
%Prob(\mbox{horizontal~transition}) &= Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i+1,l\mytiny{)}|\mbox{no~self-loop})\\
%&= \frac{m_2(l)}{1-m_1(l)},\\
%m_2(i,l)  &= Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i+1,l+1\mytiny{)}|\mbox{no~self-loop})\\
%&= \frac{m_3(l)}{1-m_1(l)},~\mbox{and}\\
%Prob(\mbox{vertical~transition}) &= Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i,l+1\mytiny{)}|\mbox{no~self-loop})\\
%&= \frac{m_4(l)}{1-m_1(l)}.\\
%\end{aligned}
%$$
Fig. \ref{markovModel} depicts the possible transitions at each state of the Markov model. The initial state of the game is $(0,0)$ which it shows the starting point of the attacker in the game, and the zero knowledge of the defender at the beginning (e.g., a zero-day vulnerability/exploit). As the game evolves, reaching state $k$ is in favor of the adversary which can happen via horizontal $m_2$ or diagonal $m_3$ transitions. In the meantime, the defender's knowledge of the attack technology and signatures improves through transitions via $m_3$ and $m_4$ in which the number of attack samples provided to the defender, i.e., $l$ increases and the function $f$ gets updated consequently.

%\subsection{Game Extensions}\label{subsec.gameExtentions}
%
%In this section, we briefly investigate some possible game scenarios which can be modeled and analyzed through the same methodology presented in this work. We also provide general guidance for the curious reader on how different scenarios can be modeled with a similar approach and only a few modifications.
% 
%\textbf{An adaptive adversary with multiple exploits:}
%After observing no progress in the game (i.e., being contained with some limited number of agents $k_c$), an adaptive adversary might decide to improve and update its attack technology. For instance, a bot herder can update the malware binary on its bots for different purposes. This includes enhancing and extending attack vectors and technologies by adding new functionalities or evasion techniques, migrating to different C\&C servers, and considering recent and revised exploits. Our framework, can also capture such strong and possibly well-funded adversaries by considering the composition of the introduced network security game. 
%From the attacker's perspective, each new exploit $\varepsilon_j$ (or in other words an enhanced attack technology) should be associated with some probability $p_j$ (as each exploit might refer to a different set of vulnerable nodes within the network). From the defender's perspective, the signature generator, if it cannot generate a single universal signature which matches all the malware's instances, must be able to generate multiple signatures each of which matches some subset of flows in the suspicious flow pool. Therefore, multiple detection rate functions and learning rates $f_j$ should be considered for each class of malware (in every single level of the composed game). In that case, the game terminates when the number of infected machines in each game/level sums up to $k$.
%
%\textbf{Host-level detection and prevention:} As explained in section \ref{bg.botDetection}, when the malware resides on a machine, it surely exhibits abnormal and erratic behavior (both externals such as unusual port usage \cite{inoue2009automated} and internals such as irregular system call sequences \cite{kolosnjaji2016deep}) on that machine. Therefore, one possibility is taking the knowledge gained at the host-level into consideration for the purpose of attack/malware signature generation by means of monitoring events on endpoint devices through a HIDS. Such signatures can be generated based on the malware residual activity on the target machine or the specific exploit/vulnerability used by the adversary during the infection. Hence, a cumulative function $f_h$ can be considered for the host-level signatures which depends on the total number of so far infected machines. Therefore, one can easily fine-tune the model to capture such defensive scenarios by multiplying the adversary's probability of success at each time step $p_i$ with $1-f_h(i)$ meaning that not only it must hit the right target (i.e., a vulnerable host), the malware should not be neutralized too at the host level. The $f_h$ function gets updated once a new node becomes infected. 
%There exist proposals for combined detection methods, i.e., taking both host-level and network-level information into consideration to fight against a worm/bot malware. For example, \cite{zeng2010detection} introduced a C\&C protocol-independent detection framework based on the combination of information gained from both host and network level bot activities. We decided not to count such strategies, since considering a universal host-level defense system installed on all the network devices is an unrealistic assumption in almost any practical situation.
%
%
%\textbf{Considering a rate of play for both parties:}
%The adversary's rate of play could play a significant factor in its success, and the time it takes to reach its objective. For instance, an adversary might decide not to issue a move for a long period, as it happens in case of advanced persistent threats (APT) \cite{tankard2011advanced} in which the smaller the rate of play is, the lesser is the probability of being detected. On the contrary, a self-replicating code (e.g., a worm malware) desires to propagate itself swiftly by utilizing a high-frequency scan mechanism. Therefore, it is possible to consider the scan rate for the adversary by defining a new rate of play parameter (for instance $\mu$) and then model the adversary by a probabilistic algorithm ${\mathcal{A}}$ which uses previously learned information in order to select a new future time step at which the adversary will issue its next move (or not to issue a move by probability $(1-\mu)$).  Previously learned information could include an immediate update of agents list (a successful infection of a new node or losing control of an agent), the usability of the current attack technology (for instance if an attack sample keeps getting filtered at the network level, the adversary might deduce that the defender probably has a high-quality signature and the attack traffic is detectable for the used attack technology; therefore, it might want to hold its army and update its attack vector), etc. The model can be easily modified to capture such scenarios by defining $m_1 = \mu m_1+(1-\mu)$ and multiply all other transition probabilities with the adversary's rate of play, i.e., $m_i = \mu m_i,~ for~ 2\leq i \leq 4$. Notice that $\sum_{i=1}^{4} m_i=1$. Similarly,  the defender can also be modeled by a probabilistic algorithm ${\mathcal{D}}$  who at each timestep issues a move with probability $\lambda$. This move is indeed monitoring network activities for data collection and analysis. Note that $\lambda$ determines the dynamicity or staticity of the performed analysis by the defender. Discrete modeling of IDPS here may reflect a periodic static analysis in which the system periodically takes a snapshot of the environment and analyzes this snapshot. However, if $\lambda$ tends to $1$, the model can be thought of as continuous monitoring, i.e., an online detection with possibly negligible detection delay (infinite Bandwidth,  zero communication, and processing latency). Moreover, notice that $\lambda$ is a measure of cost for the defender since the larger it is, the more costly is the intrusion detection process from both processing time and transporting the audits data perspective. 
%However, for simplicity and in order to not to introduce extra parameters in the model, we decided not to consider a rate of play in our modeling (even though as mentioned earlier, the model can potentially capture such scenarios). We discuss how the Markov model's transitions can be easily translated into actual time measured in seconds in section \ref{Real_Time}.


==> General_paper_S&P_Eprint/sections/intro.tex <==
Cyber attacks targeting individuals or enterprises have become a predominant part of the computer/information age. Such attacks are becoming more sophisticated (qualitative aspects) and prevalent (quantitative aspects) on a daily basis \cite{cisco:Misc}. The exponential growth of cyber plays and cyber players necessitate the inauguration of new methods and research for better understanding the ``\emph{cyber kill chain}'', particularly with the rise of advanced and novel malware (e.g., Stuxnet \cite{jin2018snapshotter}, WannaCry ransomware crypto worm \cite{cisco:Misc}, the Mirai \cite{bertino2017botnets} and its variants \cite{mirVar:Misc}) and the extraordinary growth in the population of Internet residents, especially connected Internet of Things (IoT) devices.

%The never-ending battle between adversaries and system defenders drives both parties to improve their methods and technologies to enhance their chances of prosperity. On the one hand, attackers and network penetrators come up with new attack methods and evasion techniques to bypass (or even deny) defensive systems in any possible manner. Code obfuscation, session splicing, fragmentation attacks, string matching and DDoS attacks \cite{marpaung2012survey} are among the most common techniques used by the adversaries to decrease the attack detection probability or to increase the chances of attack prosperity.
%An armored malware (e.g., a metamorphic or polymorphic worm) buys itself more propagation time by being hard to identify and disassemble. 
%On the other hand,  a large number of studies on malware detection/prevention techniques, Intrusion Detection and Prevention Systems (IDPSes), and Honeypot (HP) technologies have been carried out to present more effective methods and designs to reach better accuracy and performance \cite{idika2007survey,bhuyan2014network,chen2006survey}.
%For instance, fast and automatic signature generation schemes are introduced to fight against even the mightiest type of malware \cite{kim2004autograph,newsome2005polygraph,kreibich2004honeycomb,singh2004automated,li2006hamsa,tang2011signature,wang2010thwarting}. Some claim that they can generate high-quality signatures (with negligible false alarm rates) based on only a few malware samples\footnote{E.g., see Hamsa \cite{li2006hamsa} which only requires 100-500 malware samples in the suspecious flow pool to reach a \%5 false negative rate, even for a previously unknown worm} usually captured via honeypots or a heuristic flow classifier.

%However, the question unanswered here is \emph{how and why does the malware spread, especially the kinds targeting a broad audience, if it is the case that we can generate high quality and reliable signatures, even for an armored malware? Also, why do we see exponential growth in the number of botnets found in the wild \cite{Spamhaus}?} This work is an attempt to find an answer to such questions. 
Mathematical models can help the security research community to better understand the threat and therefore being able to analyze the attacker's conducts during the lifetime of a cyber attack. The sparse amount of research on modeling and evaluating a defensive systems' efficiency (especially from a security perspective), however, warrants the need for constructing a proper \emph{theoretical framework}. Such a framework allows the community to be able to evaluate the defensive technologies' effectiveness from a security standpoint.
% as a further matter to be explored by the community.
In this regard, a proper model is needed to capture the interactions between the two famous players of network security games i.e., a defender (taking advantage of common security tools and technologies such as Intrusion Detection and Prevention Systems (IDPSes), Firewalls, and Honeypots (HPs)) and an attacker (and possibly its agents) who takes actions to reach its attack objective(s) in the game. Modeling only one player by itself (e.g., opportunistic/targeted attacks, or a defensive system such as an IDPS) without acknowledging the other party's capabilities, set of actions, and strategies would be unjustifiable. Hence, a realistic model should take both parties' characteristics, objectives, and actions into consideration, as they are typically oppositional. 
Game theoretic methods have been proposed to model the interactions between an attacker and a defender in a network environment \cite{lye2005game,van2013flipit,chen2009game,alpcan2006intrusion,carroll2011game}. Although insightful, as figuring out the best attack-response strategy is in the focal point of a game-theoretic analysis, such models suffer from a lack of general applicability due to the case-specific assumptions made to reduce the complexity of the problem leading to a case-specific game with a corresponding  set of players' actions and payoffs. 
% and being too busy defining a proper set of players' actions and payoffs in the game. 
 Therefore, the developed models become ineffective in the representation of general settings. %reality. 

\noindent
{\bf Our Approach.} 
%In this article, 
We introduce a Markov Game (MG) framework and methodology for modeling various computer security scenarios prevailing today, including opportunistic, targeted and multi-stage attacks. We are particularly interested in situations in which each players' progress in the game can be viewed and modeled as an incremental process. From the viewpoint of the attacker, a progressive adversarial move associated with a probability distribution can bring it one step closer to its desired winning state (i.e., the attack objective). Similarly, by monitoring the system and capturing the adversarial moves, the defender can also get one step closer to its objective which could be different based on various attack/defense scenarios. For instance, the defender's goal could be generating a detection signal that indicates the presence of a coordinated set of activities that are part of an Advanced Persistent Threat (APT) campaign \cite{milajerdi2018holmes}, developing a signature for a malware attack to halt next adversarial moves \cite{newsome2005polygraph}, or shuffling its resources after enough number of samples (evidence) is obtained as in a Moving Target Defense strategy (MTD) \cite{saeed2016markov}.

\noindent
{\bf Contributions \& Results.} Our contributions are summarized as follows:

\begin{itemize}
	\item We introduce the notion of learning in cybersecurity games and describe a general ``game of consequences'' meaning that each player’s (mainly the attacker) chances of making a progressive move in the game depends on its previous actions. More specifically, as a consequence of the adversarial imperfect moves in the game, the other party, i.e., the defender has the opportunity to incrementally learn more and more about the attack technology. This learning enables the defender to be able to seize and halt following adversarial moves in the game, in other words, containing the attackers’ progress in the game.
	We argue that such learning is possible since the actions that need to be taken by an adversary in each cycle of a cyber attack's life inevitably entails abnormal and suspicious events and activities on both host and network levels. 
	
	
	\item Unlike game theoretic methods which commonly focus on finding the best attack-response strategies for the players, we, however, with a cryptographic mindset, mainly focus on the most significant and tangible aspects of sophisticated cyber attacks: (1) the amount of time it takes for the adversary to accomplish its mission and (2) the success probabilities of fulfilling the attack objectives.
    Therefore, our goal is to translate attacker-defender interactions into a well-defined game so that we can provide rigorous cryptographic security guarantees for a system given both players' tactics and strategies. We generalize the basic notion of computational security of a cryptographic scheme \cite{lindell2014introduction} to a \emph{system} which must be defended and introduce a \emph{computationally secure system} in which a ``given \emph{system} is $(T_{bud},k,\epsilon)$\emph{-secure} (for $T_{bud},k > 0$, and $\epsilon \leq 1$), if any adversary limited with a (time) budget at most $T_{bud}$ succeeds in reaching the attack objective $k$, with probability at most $\epsilon$''.  We study under which circumstances the defense system can provide an effective response that makes $\epsilon = poly(T_{bud})negl(k)$.
    
	
	 \item By modeling the learning rate of the defender as a function $f(l)$ (which is the probability of detecting and halting a next adversarial move) where $l$ represents the number of adversarial moves and actions so far observed and collected, we present the following results:
	\begin{itemize}
		\item[$-$] If $f(l)$ does not converge to $1$, then we call such a learning rate stagnating, and the adversary can reach its winning state (attack objective) $k$ within $poly(k)$ time budget.
		\item[$-$] If $f(l)\rightarrow 1$ and more specifically $1-f(l) = O(l^{-2})$, then the probability of the adversary winning the game is proven to be polynomial in the attacker's time budget and negligible in $k$. 
%		Our analytical results show that this property is even satisfied for $1-f\mytiny{(}l\mytiny{)} = O(l^{-a})$ for some $0.6\leq a \leq 1$.
		\item[$-$] The above results hold for time budget measured in logical Markov model transitions or physical time (seconds), and also hold for learning rates that remain equal to $f(l)=0$ until a certain number $l=L^*$ adversarial moves have been collected after which learning starts.
		\item[$-$] The adversary may not reach its desired winning state of $k$, but will reach  a  much smaller $k_c$ (called containment parameter) of the order $O(L^* + \log T_{bud})$, where $T_{bud}$ is the attacker's time budget, for $1-f(l) \rightarrow 0$.
		
		\item[$-$] We conclude that at a metalevel the adversary needs to find one attack exploit/vector for which the defender cannot find a fast enough increasing learning rate and the defender needs to have a learning system/methodology in place which should be able to reach fast enough learning rates for any possible attack exploit/vector. In practice infrastructures are being compromised and this means that, as given by our general framework, and presented theoretical and numerical analysis, effort is needed in order to understand associated learning rates and why these are $\leq 1-\Omega(l^{-a})$ for some `$a$' too small  or have $L^*=O(k)$ (i.e., learning starts too late).
	\end{itemize}
	
	\item The presented adversarial/defender game in terms of a Markov model is general and fits most practical scenarios as our extensive overview shows. We walk through different case studies to show how the presented modeling can be applied to real-world cyber attacks. 
 
\end{itemize}

%Unlike game theoretic methods which commonly focus on finding the best attack-response strategies for the players, we, however, with a cryptographic mindset, mainly focus on the most important and tangible aspects in sophisticated cyber attacks: (1) the amount of time it takes for the adversary to accomplish its mission and (2) the success probabilities of fulfilling the attack objectives.
%Therefore, the final objective of this manuscript is to translate attacker-defender interactions into a well-defined game so that to be able to provide rigorous cryptographic security gurantees on both players tactics and strategies. We generalize the basic notion of computational security of a cryptographic scheme \cite{lindell2014introduction} to a \emph{system} which must be defended and introduce a \emph{computationally secure system} in which a ``given (\emph{system}) is $(T_{bud},\epsilon)$\emph{-secure} (for $T_{bud} > 0$, and $\epsilon \leq 1$), if every adversary running for the time budget at most $T_{bud}$ succeeds in breaking\footnote{The notion of breaking the system however could mean different in different scenarios.} the (\emph{system}) with probability at most $\epsilon$''.  

%By analysing a worm’s behaviour and the factors that influence its spread, we can have insights into effectively detecting and containing a fast spreading worm. In this regard, by knowing the 


%A direct consequence of the over-specialization of MTD techniques is the lack of shared metrics to assess their effectiveness. In fact, most of the proposed techniques tend to measure their effective- ness in different and often incompatible ways. Thus, despite the huge amount of work done in this area, gaps still exist with respect to the analysis and quantification of MTDs.

%We notice that in many attacker-defender based games the interplay of the players could be summarized in one of the following states: (1) The attacker might have a fruitless effort, meaning that no progress in the game, but it got lucky and no information was leaked to the defender.
%(2) As a result of adversary's action, it might make a progress in the game meaning that getting one step closer to its final attack objective without revealing/leaking any information regarding the attack technology to the defender. This move is an ideal and perfect move for the attacker. However, it is also possible that (3) in spite of making progress in the game, the defender observes that adversarial moves meaning that both players get one step closer to their objective. And finally, (4) there might be the case in which the attacker gains nothing after its move but the defender observes the attack as a result of attack information leakage during the adversarial move.

%We introduce the notion of learning in cybersecurity games and introduce a general game of consequences meaning that each player’s (especially the attacker) chances of making a progressive move in the game depends on its previous actions. More specifically, as a consequence of the adversarial imperfect moves in the game, the other party, i.e., the defender has the opportunity to incrementally learn more and more regarding the attack technology and therefore, being able to seize and halt  next adversarial moves in the game, in other words, containing the attackers’ progress in the game.
%We argue that such learning is possible since the actions need to be taken by an adversay in each cycle of a cyber attack's life inevitably involves abnormal and suspicious activities on both host and network levels. 

Based on our theoretical analysis and its applicability to practical scenarios we understand when an adversary with time budget $T_{bud}$ can be contained and prevented from reaching its attack objective $k$  with probability $\geq 1- poly(T_{bud})negl(k)$. As a consequence, if such containment is in place, then this allows one to trust cryptographic protocols/systems which assume (for proving their security) attackers that have not reached $k$ (and have a key renewal / refresh operation that can be called every $T_{bud}$ seconds in order to push adversaries back to their initial state).


To the best knowledge of the authors, there has been no work so far considering the notion of learning in adversarial games and its impact on players chances of prosperity in the game. Moreover,  through this presented framework, we are able to extend the idea of security capacity introduced in \cite{saeed2016markov} and provide the definition of a \emph{security capacity region} as a metric for gauging a defensive system’s efficiency from a security perspective (by presenting rigorous cryptographic security guarantees in terms of the security capacity region). 



%Any advarsarial action causes effects which are observable by the defender and vice versa.


%This work is an attempt to find an answer to such questions. The sparse amount of research on modeling and evaluating the defensive systems' efficiency (especially from a security perspective) warrants the need for constructing a proper \emph{theoretical framework}. Such a framework allows the community to be able to evaluate the defensive technologies' effectiveness from a security standpoint.
%% as a further matter to be explored by the community.
%In this regard, a proper model is needed to capture the interactions between the two famous players of network security games i.e., a defender (taking advantage of an IDPS and HPs) and an attacker (and its agents) who eventually wants to make a zombie army of a specific size. 

























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%%%%%%%%%%%%%%%%%%%%%OLD INTRO%%%%%%%%%%%%%%%%%%%%%%%%5

%With the rise of advanced and novel malware (e.g., Stuxnet worm, WannaCry ransomware cryptoworm) and the extraordinary growth in the population of Internet residents, especially connected Internet of Things (IoT) devices, new methods, and research for understanding malware behaviors and jousting with sophisticated botnets seem to be crucial.
%Of specific interest to us are two types of malware, worms \cite{weaver2003taxonomy}, and autonomous bots \cite{complexbot:Misc} especially due to their large-scale audience, and self-propagating characteristics. These types of malware execute a ``seek-and-infect'' mission strategy. For instance, a scanning worm usually infects a target by utilizing vulnerability exploitation, and it automatically probes the environment to \emph{independently} propagate itself (or modified copies of itself) from the infected machine to other vulnerable hosts in the network. Consequently, a straightforward way of assembling an army of infected hosts is spreading the malicious code in the form of a scanning worm. This zombie army which is also known as a botnet is indeed a collection of compromised machines distributed over a network (usually the Internet) and controlled by a central/distributed entity known as the botmaster through a command and control (C\&C) structure \cite{feily2009survey}. 
%Afterward, these infiltrated workstations (bots) can be managed for different malicious purposes including but not limited to ransom campaigns, massive spam-marketing, large-scale information harvesting and processing, click fraud, pay-per installation, and, distributed denial-of-service (DDoS) attacks. 

%The botmaster renders a semi brood-parasitic behavior during its zombie army construction.  Similar to the brood parasites who rely on other hosts to nurse their offspring (e.g., the cuckoo bird who puts her eggs within the nest of other bird species), the botmaster lays its eggs (which in this case is a piece of malicious code) in other hosts for different mischievous purposes. Interestingly, the strategies used by both the parasites and the malware propagator are similar in many ways. For instance, in order to decrease the chances of egg loss, brood parasites commonly have a host selection mechanism \cite{teuschl1998cuckoos} in addition to distributing the eggs amongst different hosts \cite{attenborough1998life}  (comparable to the botmaster who propagates the malware to a broad audience and tries to select/locate the vulnerable hosts). Even though the poor victim animal usually will not detect such intrusions and malicious intents, in case of the botmaster, this wretched activity can be potentially detected through available security tools and technologies. This is because such malware's life cycle (from the execution of the malware binary on a target to scanning for other victims within the network during the construction phase, or agent-to-agent and agent-to-C\&C servers' communications during the botnet maintenance and application phases), unquestionably comprises abnormal and malicious behaviors leading to unusual events on the endpoint devices in addition to suspicious network traffic and activities. Current solutions for detecting and preventing intrusions and malicious behaviors on the host or network levels are HPs and IDPSes\footnote{Even though there exist various security technologies which can be used in conjunction with or as a complementary add-on to these systems, we only stick to IDPSes and HPs for our modeling since they play the primary role in bot/worm type malware detections and preventions. These technologies include firewalls, routers, network forensic analysis tools (NFAT), and anti-malware.}. These defensive systems have become an inseparable part of today's network security contrivances.  
%On one hand, system administrators and security architects crave to take advantage of such systems to protect their assets. On the other hand, network penetrators and attackers desire to bypass (or even deny) such systems in any possible manner in order to increase their chance of attack prosperity or to decrease the probability of being detected.  Therefore, on account of the existence of such defensive systems in network environments, attackers (e.g. botmaster(s) who are constructing and maintaining botnets) are  forced to find ways in order to elude these electronic decoys and defensive tools \cite{wang2010honeypot}. 
%For instance, honeypots can potentially attract botnet agents and become snoops in revealing botnet memberships and botmasters behaviors due to their sensational nature to malicious adversaries. In this regard, they are one of the most widely used security tools by security defenders for botnet defense purposes. 

%The never-ending battle between adversaries and system defenders drives both parties to improve their methods and technologies to enhance their chances of prosperity. On the one hand, attackers and network penetrators come up with new attack methods and evasion techniques to bypass (or even deny) defensive systems in any possible manner. Code obfuscation, session splicing, fragmentation attacks, string matching and DDoS attacks \cite{marpaung2012survey} are among the most common techniques used by the adversaries to decrease the attack detection probability or to increase the chances of attack prosperity.
%An armored malware (e.g., a metamorphic or polymorphic worm) buys itself more propagation time by being hard to identify and disassemble. 
%On the other hand,  a large number of studies on malware detection/prevention techniques, IDPSes, and HP technologies have been carried out to present more effective methods and designs to reach better accuracy and performance \cite{idika2007survey,bhuyan2014network,chen2006survey}.
%For instance, fast and automatic signature generation schemes are introduced to fight against even the mightiest type of malware \cite{kim2004autograph,newsome2005polygraph,kreibich2004honeycomb,singh2004automated,li2006hamsa,tang2011signature,wang2010thwarting}. Some claim that they can generate high-quality signatures (with negligible false alarm rates) based on only a few malware samples\footnote{E.g., see Hamsa \cite{li2006hamsa} which only requires 100-500 malware samples in the suspecious flow pool to reach a \%5 false negative rate, even for a previously unknown worm} usually captured via honeypots or a heuristic flow classifier.
%
%However, the question unanswered here is \emph{how and why does the malware spread, especially the kinds targeting a broad audience, if it is the case that we can generate high quality and reliable signatures, even for an armored malware? Also, why do we see exponential growth in the number of botnets found in the wild \cite{Spamhaus}?} This work is an attempt to find an answer to such questions. The sparse amount of research on modeling and evaluating the defensive systems' efficiency (especially from a security perspective) warrants the need for constructing a proper \emph{theoretical framework}. Such a framework allows the community to be able to evaluate the defensive technologies' effectiveness from a security standpoint.
%% as a further matter to be explored by the community.
%In this regard, a proper model is needed to capture the interactions between the two famous players of network security games i.e., a defender (taking advantage of an IDPS and HPs) and an attacker (and its agents) who eventually wants to make a zombie army of a specific size. 




%botmasters show the same behavior by putting their agents known as bots into other hosts.


%However, we encounter an interesting problem here and that is these cyber deception tools/techniques should satisfy two contradictory properties: first, they should be specious enough (deceptively appealing) in order to attract the malicious parties and satisfy their functionality; second, they should not diffuse obvious suspicious behavior to estrange the adversaries, since as soon as these shady environments have been detected by adversary agent(s), they can be evaded and attacker can continue his job in a lighthearted manner consequently.
% Interestingly, most of the available research in malware propagation modeling, only consider the adversary's tactics and strategies (e.g., the scanning rates) in model development regardless of the defender's reactions and maneuverings \cite{chen2009information,sellke2008modeling,rohloff2005stochastic}. A few consider a removal/cleaning rate of the malware within the model, although it is not explicit where this removal process comes from \cite{zou2002code,chen2003modeling,dagon2006modeling}. Nevertheless, we believe modeling only one player by itself (e.g., a worm/bot malware, or a defensive system such as an IDPS) without acknowledging the other party's capabilities, set of actions, and strategies would be unjustifiable. Hence, a realistic model should take both parties' characteristics, objectives, and actions into consideration, as they are typically oppositional. 
% Game theoretic methods have been introduced to model the interactions between an attacker and a defender in a network environment \cite{lye2005game,chen2007modeling,chen2009game,alpcan2006intrusion,carroll2011game}. Such models, however, suffer from a lack of practicability due to the simplifying assumptions made to reduce the complexity of the problem and to define a proper set of players' actions and payoffs. Therefore, the developed models become ineffective in the representation of reality.
%%%Fix the following

%Furthermore, by switching to smart and Software Defined Networking (SDN) \cite{kreutz2015software}, in which the entire network infrastructure can be controlled from a centralized software controller, new generations of traditional cyber defense technologies (e.g. HPs, IDPSes, firewalls, etc.), which are more capable, scalable and secure, are already being introduced \cite{giotis2014combining,zanna2014adaptive,hu2014flowguard,han2016honeymix,fan2017novel,jin2018snapshotter}. However, before a complete migration, such defensive tools and technologies' effectiveness should be studied effectively from a security standpoint.
%For instance, in an SDN environment, IDPS and HP logs can be used by the network controllers in order to update flow tables or firewall rules. An SDN-enabled host-based intrusion detection and mitigation framework called IoT-IDM is proposed in \cite{nobakht2016host} to protect IoT devices deployed in a smart home along the same lines of \cite{mehdi2011revisiting} which revisits traffic anomaly detection using SDN in small home and office networks. 
%However, before a complete migration, such defensive tools and technologies' effectiveness should be studied effectively from a security standpoint.
%These challenges altogether raise the urgent need for finding a proper model that could determine the role and importance of deception in network players' probability of success in addition to the effectiveness of defender's agents itself in protecting the system. Most of the available works in this area, focus on using game theoretic methods \cite{cceker2016deception,lye2005game,carroll2011game} in order to model an attacker-defender interaction in such environments. Even though use of game theory methods seems to be captivating, the models can not capture the real states of a network environment due to simplified assumptions made in order to find proper set of players actions, payoffs, cost and rewards. Therefore, the developed models through these studies are merely toy examples.

% Moreover, we believe modeling an adversary itself or self-propagating malware (such as bots, worms, etc.) without considering another party who acts in an opposite manner by detecting and seizing the other parties agents and activities would be useless. Therefore, a realisitc model indeed should take into account  both parties objectives, characterestics and set of availble action. This inherently leads us to a game in which

% Moreover,  This inherently leads us to a network security game who its players are 
 

%These challenges altogether raise the urgent need for finding a proper model that could capture the interactions between the two famous players of network security games i.e. a defender (taking advantage of IDPS and HPs in the network and endpoint devices) and an attacker (and its agents who eventually wants to make a zombie army of a specific size). Modeling only one player by itself (e.g. a self propagating worm or a botnet, or an IDPS) without considering another party's capabilities, set of actions, and strategies (which are usually in opposing directions) would be unjustifiable. Therefore, a realisitc model indeed should take into account both parties' characterestics, objectives, and set of availble actions. In addition, such model should be capable of determining the effectiveness of security tools, policies, and strategies in both players' probability of success. Most of the available works in this area, focus on using game theoretic methods \cite{roy2010survey,manshaei2013game,lye2005game,alpcan2003game,chen2009game,alpcan2006intrusion,patcha2004game,poongothai2008noncooperative,reddy2009game,cceker2016deception,carroll2011game} in order to model an attacker-defender interaction in such environments. Even though the use of game theoretic-based methods seems to be captivating, the models can not capture the real states of a network environment due to simplifying assumptions made in order to reduce the complexity of the problem and finding a proper set of players actions, payoffs, costs and rewards. Therefore, the developed models through these studies are merely toy examples.


% A large number of studies on IDPS and HP technologies only focus on presenting new architectures or detection/prevention methods and techniques, or proper feature selection of audit data in order to reach better accuracy and performance \cite{bhuyan2014network,chen2006survey}. However, there exist very few research presenting a proper \emph{theoretical framework} for evaluating such technologies' effectiveness from a security perspective. 
% To the best of our knowledge, this presented work is one of the first research studies which aims at providing a rigorous security language and diligent cryptographic security guarantees for IDPS technologies (more specifically any automatic signature generation scheme used by the defense system).  In this regard, we utilize the security capacity concept introduced in \cite{saeed2016markov}, as a measure of the effectiveness of an IDPS. An IDPS has a security capacity of $c$ such that the attackers' probability of winning the introduced network security game within $2^t$ steps is at most $2^{-s}$ where $c=s+t$. We show how the IDPS accuracy and completeness in addition to adversary's mastery project into security capacity of the system. 

%We model the interaction between these deceitful parties i.e. adversary owned hosts and defender agents as a deception game between different network hosts.  As a consequence of adversary's deception strategy, there exist an error for defender to find the real identity of adversary agents (such as bots). On the same line, due to defender's deception strategy, the adversary-owned hosts can determine the real identity of a defender agent with some error. 
%We borrow the general concepts of a famous discussion based game called ``Mafia'' and expand it to a network-based game. We show how the new game can capture and represent a real network scenario. 

%In addition, we study different players objectives, strategies and probability of winning the game through Markov modeling and simulation. This paper looks into Intrusion Detection Systems especially HIDs from a very different perspective. To the best of our knowledge, this is the first time one models such systems ... The purpose of this work is not to present a new IDS architecture or a new detection method. However, we model the very common agent-based intusion detection systems and present a theoretical framework for evaluating their performance and effectiveness as a traditional security tool.
 
%The hosts set is a triad and it includes three different type of players each with different capabilities and objectives: the adversary-owned hosts (malicious/infected); the defender agents\footnote{We do not consider Network Intrusion Detection Systems (NIDS) here since based on their placement in the network they usually have access to the traffic to/from all devices which is out of scope of our introduced game} (e.g. HPs, Host-based Intrusion Detection System (HIDS), etc.)  which we call them privileged hosts since they have the ability to somehow find the other parties role and finally regular hosts which are the normal users in the network. We are interested in understanding different groups' objectives and strategies, their probability of success or failure in the game. At first glance,
%adversary-owned hosts evidently desire to find the suspicious host(s) (privileged hosts). We notice that this is not essentially the final objective of an intruder in a network; however, this objective can clearly leads to a maximum profit which is attack prosperity while keeping anonymity (not being detected/identified).  The defender agents' objective could be defined as detecting all the malicious hosts in addition to informing known/trusted regular hosts of the existence of detected malicious/untrusted hosts. Regular hosts basically have the same goal as the privileged host(s). A collaboration between them can increase their probability of success.

%We notice that from a practical point of view, most of defensive systems (especially honeypots) work in a passive way. For instance, most of the existing implementations of Honeypots are server-based i.e. they listen to the incoming communications toward them. However, this is not a problem in our modeling at all. We believe by switching to smart networks and SDNs, smart honeypots are more likely to be introduced which take advantage of network infrastructure. For example in an Software Defined Network environment, IDS or HPs logs can be used to generate flow toward network controllers in order to update flow tables or firewall rules.  \saeed{client based HPs! need to be more clear}

%We believe this type of study can provide network security researchers and system administrators an intuitive overview and a more solid understanding of how large-scale self-propagating malware could behave in the wild and how effective current security solutions are.

% In this regard, the rest of this paper is organized as follows:
%In section \ref{sec:backg} we provide the motivation and background on this work specifically IDPS, HPs and malware propagation models. In section \ref{sec:gameModel&Analysis}, we describe the network security game and then present different players objectives and strategies. The security analysis of the game is presented in section \ref{sec:secAna.sim} following by simulation results. We finally conclude the paper and present future works in section \ref{sec:con}. 

%
%\noindent
%{\bf Our Approach.} 
%In this paper, instead of presenting \emph{yet another malware detection/prevention methodology}, we model the interactions of an adversary and its agents with the defensive system during the early phases of a zombie army construction as an incremental online learning game. Unlike an adversary who usually follows a passive attack strategy for the propagation of malware with a large audience (eg. worms/bots), meaning that the attack technology usually remains the same after unleashing the first few samples of the malware, the defender has the opportunity to incrementally learn regarding the attack technology (specifically, from more malware payloads). As time elapses, and more attack data is captured by the defender,
%it can reach better detection rates and accuracy. This learning rate indeed reflects into higher quality malware signatures which can be used for online malicious traffic filtering and hence malware containment purposes.

% By modeling the learning rate of the defender as a function $f\mytiny{(}l\mytiny{)}$ (which is the probability of detecting and halting a next adversarial move) where $l$ represents the number of adversarial moves and actions so far observed and collected, we present the following results:
%\begin{itemize}
%	\item If $f\mytiny{(}l\mytiny{)}$ does not converge to $1$, then we call such a learning rate stagnating and the adversary is able to reach its winning state $k$ within $poly(k)$ time budget.
%	\item If $f\mytiny{(}l\mytiny{)}\rightarrow 1$ and more specifically $1-f\mytiny{(}l\mytiny{)} = O(l^{-2})$, then the probability of the adversary winning the game is proven to be polynomial in the attacker's time budget and negligible in $k$. Our analytical results show that this property is even satisfied for $1-f\mytiny{(}l\mytiny{)} = O(l^{-a})$ for some $0.6\leq a \leq 1$.
%	\item The above results hold for time budget measured in logical Markov model transitions or real time (seconds), and also hold for learning rates that remain equal to $f(l)=0$ until a certain number $l=L^*$ adversarial moves have been collected after which learning starts.
%	\item The presented adversarial/defender game in terms of a Markov model is general and fits most practical scenarios as our extensive overview shows.
%\end{itemize}
%The adversary may not reach its desired winning state of $k$, but will reach to a satisfying though much smaller $k_c$ of the order $O(L^* + \log T_{bud})$, where $T_{bud}$ is the attacker's time budget, for $1-f(l) \rightarrow 0$. We conclude that at a meta level the adversary needs to find  one exploit for which the defender cannot find a fast enough increasing learning rate and the defender needs to have a learning system/methodology in place which should be able to reach fast enough learning rates for any possible exploit. In practice infrastructures are being compromised and this means that, as given by our general framework, its thorough analysis, and numerical analysis, effort is needed in order to understand associated learning rates and why these are $\leq 1-O(l^{-a})$ for some $a\geq 0.6$ or have $L^*=O(k)$ (i.e., learning starts too late).

% To the best of our knowledge, this presented work is one of the first research studies which aims at providing a rigorous security language and diligent cryptographic security guarantees for IDPS technologies (more specifically any automatic signature generation scheme used by the defense system).  In this regard, we utilize the security capacity concept introduced in \cite{saeed2016markov}, as a measure of the effectiveness of an IDPS. An IDPS has a security capacity of $c$ such that the attackers' probability of winning the introduced network security game within $2^t$ steps is at most $2^{-s}$ where $c=s+t$. We show how the IDPS accuracy and completeness in addition to adversary's mastery project into security capacity of the system. 
% We analyze the outcomes and
%evolution of an example game numerically for various game parameters.


\noindent
{\bf Paper Organization.}
The rest of this paper is organized as follows:
Section \ref{sec:backg} briefly reviews  related work, especially modeling cyber attacks as a game between an attacker and a defender.
The interactions of the defender and the adversary are
described as a stochastic network security game in section \ref{sec:gameModel&Analysis}.
The security analysis of the introduced game is presented in section \ref{sec:secAna.sim} followed by the corresponding parametric analysis of the game for various learning functions and system parameters to explore the effects of such variables on attack-defense objectives. In Section \ref{CaseStdy}, we walk through a few attack-defense scenarios to show how our presented framework can be applied to real-world examples. We finally conclude the paper and present future work in section \ref{sec:con}. 

%\noindent
%{\bf Paper Organization.}
%The rest of this paper is organized as follows.
%%Section \ref{sec:backg}, after presenting the motivation, briefly reviews the most common worm/bot type malware defense technologies, in addition to such malware's detection techniques and propagation models.
%Section \ref{sec:backg} briefly reviews the related work on this manuscript, especially modeling cyberattacks as a game between an attacker and a defender.
%%In section \ref{sec:backg} after presenting the motivation, we breifly review the background and related work on this work specifically IDPSes, HPs and malware propagation models. 
%The interactions of the defender and the adversary are
%described as a stochastic network security game in section \ref{sec:gameModel&Analysis}.
%%In section \ref{sec:gameModel&Analysis}, we describe the network security game and then present different players objectives and strategies. 
%The security analysis of the introduced game is presented in section \ref{sec:secAna.sim} followed by the corresponding parametric analysis of the game for various learning functions and system parameters to explore the effects of such variables on attack-defense objectives in section \ref{sec:sim}. In Section \ref{CaseStdy}, we walk trough some attack-defense scenarios to show how our presented framework can be applied to this real world examples. We finally conclude the paper and present future works in section \ref{sec:con}. 

==> General_paper_S&P_Eprint/sections/security-summary.tex <==

\section{Adversarial Containment}

The goal of the adversary is to reach a winning state $(k,l)$ for some $l\geq 0$ within a limited time budget $T_{bud}$. Here, $k$ represents the total number of nodes which the adversary wishes to compromise before using the collective of these nodes in the next attack phases (e.g. botnet applications). Time budget $T_{bud}$ represents the number of transitions in the Markov model, i.e., the total number of adversarial moves. 

The objective of the defender is to learn more and more regarding the attack technologies, specifically more malicious attack payloads in order to be able to recognize and halt future moves by the attacker. That is, the defender hopes to push level $l$ -- the number of detected malicious payloads so far -- higher and higher, leading to a higher probability $f(l)$ of successfully detecting a next malicious payload. The ultimate goal of the defender is to have a good enough learning mechanism in place such that the probability of reaching $k$ is negligible in $k$ and only polynomial in $T_{bud}$. In other words, the adversary cannot reach a winning state in practice.

We define $w(k,T_{bud})$ as the probability of the adversary to reach a state $(k,l)$ for some $l\geq 0$ within time budget $T_{bud}$. In the next subsections we analyse this probability. We want to find a tight upper bound and determine for which model parameters $\gamma$, $h$, $p$, and learning rate $f(l)$ the upper bound proves the desired asymptotic 
\begin{equation} w(k,T_{bud})=poly(T_bud) negl(k). \label{eq:as} \end{equation}
 We notice that in this case, even though the adversary cannot reach a large $k$ because $w(k,T_{bud})$ is negligible in $k$, the adversary may reach a (much) smaller $k$. We are interested in the order of magnitude of the number of compromised nodes the adversary is able to reach. For this reason we define $k_c$ as the solution of
$$ w(k_c, T_{bud}) =1/2.$$
This  $k_c$ reflects the order of magnitude of the number of compromised nodes to which the adversary is {\em contained}. By using $w(k,T_{bud})=poly(T_bud) negl(k)$ we can show that $k_c= O(\log T_{bud})$. 

Our analysis will show that for a stagnating learning rate (i.e., $1-f(l)$ remains larger than some constant $\tau>0$) the adversary is not contained since $w(k,T_{bud})$ does not follow the desired asymptotic. For a learning rate $f(l)\geq 1-O(1/l^2)$ approaching $1$ fast enough, we are able to prove the desired asymptotic. The next section evaluates other learning rates by using a dynamic programming approach developed in subsection \cite{AC-dp}. 

\subsection{Time budget measured in real time}

We first discuss the effect of translating the time budget $T_{bud}$, measured in Markov model transitions, to a time budget which is measured in real time (seconds) as this makes sense in practice. If the adversary wins as soon as $k$ nodes are compromised and if each Markov model transition takes $\Delta$ seconds, then at most $k$ moves can be made by each of the compromised nodes {\em in parallel} in $\Delta$ secconds. With a time budget of $T$ seconds, this implies $T_{bud}\leq T k/\Delta$. This means that the desired asymptotic (\ref{eq:as}) translates into
$$ w(k,T_{bud})\leq poly(T k/ \Delta) negl(k),$$
which is $poly(T)negl(k)$, which again implies that in practice  the adversary cannot reach $k$ since the probability of reaching $k$ is negligible in $k$ and only polynomial in real time budget $T$. 

\subsection{Stagnating learning rate} \label{stagnating}

Suppose that the learning rate stagnates in that $1-f(l)\geq \tau$ for some $\tau>0$. This means that $f(l)\leq 1-\tau$ and as a result at least a fraction $\tau$ goes undetected. In order to prove a lower bound on $w(k,T_{bud})$ we give a benefit to the defender and assume $1-f(l)=\tau$ with equality.

If $1-f(l) = \tau$, then $m_1,m_2,m_3$ and $m_4$ are independent of $l$ and the Markov model reduces to Fig. \ref{fig.reducedMarkovModel} where each  state $i$ represents the set of states $(i,l)$ for $l\geq 0$ in the original Markov model.

\begin{figure}[t]
	\centering
	\begin{tikzpicture}
	\tikzset{
		>=stealth',
		node distance=3cm and 3cm ,on grid,
		every text node part/.style={align=center},
		state/.style={minimum width=1.5cm,
			%    		font=\small,
			draw,
			circle},
	}
	% Add the states
	\node[state]             (c) {i};
	\node[state, right=of c] (r) {i\pp};
	%	\node[state, left=of c] (lose) {0};
	% Connect the states with arrows
	\draw[every loop]
	(c) edge[auto=left]  node {$m_{2}+m_3$} (r)
	%(r) edge[bend left, auto=right] node {0.7} (s)
	%(c) edge[loop above]             node {($1-p_i-f(.)$)} (c)
%	(c) edge[ auto=left] node {$m_3$} (rr)
%	(c) edge[auto=right] node {$m_4$} (b)
	(c) edge[loop above]             node {$m_1+m_4$} (c);
	%(d) edge[loop above]             node {} (d);
	\end{tikzpicture}
	\caption{Reduced Markov model of the game for a constant $1-f(l)=\tau>0$}
	\label{fig.reducedMarkovModel}
\end{figure}

Within time budget $T_{bud}$ we reach $i=k$ with probability 
$$ w(k,T_{bud})=  \sum_{T=0}^{T_{bud}-k} {\sum_{\substack{f_0,\dots,f_{k-1} s.t.\\ \sum f_j=T}}
\prod_{j} (m_1+m_4)^{f_j}(m_2+m_3)^{k}
},
$$
where the time budget is distributed over $k$ steps from each state to the next until state $k$ is reached and  $T\leq T_{bud}-k$ transitions consists of $f_i$ self-loops in state $i$ for $0\leq i\leq k-1$.
This probability is equal to
%
%\begin{eqnarray}
%\lefteqn{ \sum_{T=k}^{T_{bud}} {T-1 \choose k-1}(m_1+m_4)^{(T-1)-(k-1)}(m_2+m_3)^{k-1+1} =} \nonumber\\
% & & \sum_{T=k}^{T_{bud}} {T-1 \choose k-1}(m_1+m_4)^{T-k}(m_2+m_3)^{k}\nonumber\\
%&=& \sum_{T-k=0}^{T_{bud}-k} {(T-k)+(k-1) \choose (T-k)}(m_1+m_4)^{T-k}(m_2+m_3)^{k} \nonumber\\
%&=&  \sum_{i=0}^{T_{bud}-k} {i+(k-1) \choose i}(m_1+m_4)^{i}(m_2+m_3)^{k} \label{eq.7}
%\end{eqnarray}
%
%A lower bound on (\ref{eq.7}) can be derived as follows:
%
\begin{eqnarray*}
%  \sum_{i=0}^{T_{bud}-k}
%{\sum_{\substack{f_1,\dots,f_k s.t.\\ 
%		\sum f_j=i}}
%\prod_{j} (m_1+m_4)^{f_j}(m_2+m_3)^{k}
%}\\
%&=& 
\sum_{\substack{f_0,\dots,f_{k-1} s.t.\\ \sum f_j\leq T_{bud}-k}}
\prod_{j} (m_1+m_4)^{f_j}(m_2+m_3)^{k}
&\geq& \sum_{f_0=0}^{(T_{bud}-k)/k}\dots\sum_{f_{k-1}=0}^{(T_{bud}-k)/k}\prod_{j}(m_1+m_4)^{f_j}(m_2+m_3)^{k}\\
&=& \prod_{j=0}^{k-1}\sum_{f_j=0}^{(T_{bud}-k)/k}(m_1+m_4)^{f_j}(m_2+m_3)^{k}\\
&=& \prod_{j=0}^{k-1}\frac{1-(m_1+m_4)^{T_{bud}/k}}{1-(m_1+m_3)}(m_2+m_3)^{k}\\
&=& [1-(m_1+m_4)^{T_{bud}/k}]^{k} \geq 1-k(m_1+m_4)^{T_{bud}/k}.
\end{eqnarray*}
This shows that $w(k, T_{bud})\approx 1$ for relatively small $T_{bud}$ because $1-w(k,T_{bud}) \leq k(m_1+m_4)^{T_{bud}/k}$ which is exponentially small in $T_{bud}$. 
%For example, $T_{bud}=lambda k ln k$ to get >=1- x^{-lambda} for some small x
% REAL TIME: Use f_i/(i+1) in the formula -- i.e. sum f_i/(i+1) is real time, take f_i = T_real / ln k, hence T_real = lambda (ln k)^2 is sufficient
In order to have the desired asymptotics (\ref{eq:as}), the learning rate should not stagnate, i.e., we need $1-f(l)\rightarrow 0$ for $l\rightarrow \infty$ .

\subsection{Formula for $w(k,T_{bud})$}

Before proving any bounds on $w(k,T_{bud})$ we first provide a closed form for $w(k,T_{bud})$ itself. To this purpose we introduce $p(k-1,L,T_{bud})$ defined as the probability that the adversary reaches state $(k-1,L)$ and is ready to leave state $(k-1,L)$ (after zero or more self-loops at state $(k-1,L)$) within time budget $T_{bud}$. Any possible path from state $(0,0)$ to state $(k-1,L)$ in the Markov model with self-loops along the way in each of the visited state (including $(k-1,L)$) contributes to this probability. (We use $k-1$ rather than $k$ because after a path to $(k-1,L)$ for some $L\geq 0$ only a single horizontal or diagonal move is needed to reach $(k,L)$ for the first time, and this probability is what we will need for $w(k,T_{bud})$.) 

A path to $(k-1,L)$ till the moment it is ready to leave $(k-1,L)$ is uniquely represented by 
\begin{itemize}
\item $g_l$ is the number of states on the path that have the same level $l$,
\item $b_l$; if level $l$ is entered via a vertical transition, then $b_l=0$; if level $l$ is entered via a horizontal transition, then $b_l=1$,
\item $t(i,l)$ counts the number of self-loops on the path in state $(i,l)$.
\end{itemize}
(Notice that $b_0$ is undefined and $g_l\geq 1$ for all $0\leq l \leq L$.)
By using induction one can prove that the probability of having the Markov model transition along a path represented by these numbers is equal to
\begin{subequations}
\begin{eqnarray}
&& \prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg) \cdot \label{path-a}\\
&& \prod_{l=0}^{L} \bigg( \frac{m_2(l)}{1-m_1(l)}\bigg)^{g_l-1}\cdot \label{path-b}\\
&& \prod_{l=0}^{L}\prod_{i=0}^{g_l-1}m_1(l)^{t(i_l+i,l)}(1-m_1(l)) \label{path-c}
\end{eqnarray}
\end{subequations}
(the induction hypothesis is that the above statement holds for $(i,l)$, $0\leq i\leq k-1$ and $0\leq l\leq L$ such that $(i,l)\neq (k-1,L)$).
The length of the path, i.e., total number of transitions without self-loops,  is equal to 
$$(k-1) + L -B, \mbox{ where } B=\sum_{l=1}^L b_l$$
is the total number of diagonal transitions.  The total number of vertical transitions is equal to $L-B$ and the number of horizontal transitions is equal to $\sum_{l=0}^L (g_l-1) = (k-1)-B$.

Summing the above probability over all possible combinations of $g_l$, $b_l$, and $t(.,.)$ for paths that reach state $(k-1,L)$  and are ready to leave $(k-1,L)$ such that the number of self-loops is equal to $T$ and the total number of transitions including self-loops is equal to $(k-1)+L-B + T\leq T_{bud}$ leads to an expression for $p(k-1,L,T_{bud})$:
	\begin{subequations}
		\begin{eqnarray}
		p(k-1,L,T_{bud}) &= &
		\sum_{\substack{B,T s.t.\\
				(k-1)+L-B+T\leq T_{bud}}}\nonumber\\& &
		{ 
			\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ \label{p-a}
					\sum_{l=1}^{L}b_l=B}}
%			\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
(\ref{path-a})
		}\\& &
		{	\sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\ \label{p-b}
					\sum_{l=0}^{L}(g_l-1)=(k-1)-B}}
%			\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
(\ref{path-b})
		}\\& &
		{
			\sum_{\substack{t_0,\dots,t_L s.t.\\ \label{p-c}
					\sum_{l=0}^{L}t_l=T}}
			\sum_{\substack{t(i_l,l),\dots,t(i_l+g_l-1,l) \\
						s.t.\sum_{i=0}^{g_l-1}t(i_l+i,l)=t_l}}
%			\prod_{l=0}^{L} 
%			{	
%				\prod_{i=0}^{g_l-1} 
%				m_1(l)^{t(i_l+i,l)}(1-m_1(l))
%			}
(\ref{path-c})
		}
		\end{eqnarray}
	\end{subequations}
	
The formula for $w(k,T_{bud})$ considers all the possible paths towards a state $(k-1,L)$ within $T_{bud} -1$ transitions and a single final horizontal or diagonal transition (via $m_2(L)$ or $m_3(L)$) towards the winning state $(k,L)$. We are interested in the probability of entering state $(k,L)$ for some $L\geq 0$ and the time it takes to reach there \emph{for the first time}. Appropriately summing over probabilities $p(k-1,L,T_{bud}-1)$ gives
	\begin{subequations}
\begin{eqnarray}
 w(k, T_{bud})&=&	\sum_{L\geq 0} p(k-1,L,T_{bud}-1) \cdot	 \bigg( \frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\bigg) \nonumber \\
&=& \sum_{L=0}^{T_{bud}-1}\sum_{B=0}^{\min\{L,(k-1)\}}\bigg( \frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\bigg)\cdot (\ref{p-a})\cdot (\ref{p-b})\cdot \label{w-a} \\
 \sum_{T=0}^{(T_{bud}-1)-[(k-1)+L-B]} (\ref{p-c}).  \label{w-b}
\end{eqnarray}
\end{subequations}
This is a closed form of the probability we are interested in. 

\subsection{Upper and lower bound on $w(k, T_{bud})$}

By noticing that (\ref{w-b}) for $T_{bud}=\infty$ is equal to 1, a straightforward upper bound on $w(k,T_{bud})$ is given by just formula (\ref{w-a}): We have $w(k,T_{bud})$ is at most equal to 
\begin{equation}
\bar{w}(k,T_{bud}) = (\ref{w-a}) =
\sum_{L=0}^{T_{bud}-1}\sum_{B=0}^{\min\{L,(k-1)\}}\bigg( \frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\bigg)\cdot (\ref{p-a})\cdot (\ref{p-b}).
\label{UB}
\end{equation}

%By using a proof strategy similar to the one used in Section \ref{stagnating} 
We may lower bound (\ref{w-b}) as follows.
 For $e\leq T_{bud}/(L+1)$, we can show that
$$ (\ref{w-b}) \geq 1- \sum_{l=0}^{(T_{bud}/e)-1} k \cdot m_1(l)^{e/k}\geq 1- T_{bud} \frac{k}{e} (1-\gamma)^{\frac{e}{k}},$$
where the first inequality follows from a proof strategy similar to the one used in Section \ref{stagnating}, and the second inequality follows from $m_1(l)\leq 1-\gamma$.
This lower bound on (\ref{w-b})  is independent of any of the other summing variables used in (\ref{w-a}) but requires $L< T_{bud}/e$. By restricting $L$ to be $<T_{bud}/e$ in (\ref{w-a}) (i.e., we substitute $T_{bud}$ by $T_{bud}/e$) we obtain a lower bound on $w(k,T_{bud})$:
\begin{equation} w(k,T_{bud}) \geq \bar{w}(k,T_{bud}/e)\cdot (1- T_{bud} \frac{k}{e} (1-\gamma)^{\frac{e}{k}}). 
\label{LB}
\end{equation}
In particular for $e= k \ln (T_{bud}k/\epsilon) / \ln (1/(1-\gamma))$, we have $w(k,T_{bud}) \geq \bar{w}(k,T_{bud}/e)\cdot (1-\epsilon)$. 

Upper bound  (\ref{UB}) proves that if $\bar{w}(k,T_{bud})$ has desired complexity $\bar{w}(k,T_{bud})=poly(T_bud) negl(k)$, then $w(k,T_{bud})$ inherits this desired complexity. And vice versa, lower bound (\ref{LB}) for the special choice of $e$ proves that if $w(k,T_{bud})$ has desired complexity $w(k,T_{bud})=poly(T_bud) negl(k)$, then also $\bar{w}(k,T_{bud}) \leq w(k, T_{bud}\cdot e)/(1-\epsilon) = poly(T_bud \cdot e)\cdot negl(k) = poly(T_{bud})negl(k)$. We conclude that in order to find out which learning rates lead to the desired complexity for the defender, we only need to study which learning rates lead to the same desired complexity for $\bar{w}(k,T_{bud})$.

The advantage of studying $\bar{w}(k,T_{bud})$ is having eliminated expression (\ref{w-b}) which represents the effect of self-loops (and turns out to be very inefficient to evaluate as an exact expression). Probability $\bar{w}(k,T_{bud})$ corresponds to the Markov model in Figure \ref{???} without any self-loops and with horizontal transition probabilities $m_2(l)/(1-m_1(l))=(1-\gamma)\alpha(l)$, diagonal transition probabilities $m_3(l)/(1-m_1(l))=\gamma \alpha(l)$, and vertical transition probabilities $m_4(l)/(1-m_1(l))=1-\alpha(l)$, where 
$$ \alpha(l) = \frac{p(1-f(l))}{\gamma + (1-\gamma)(p+h)(1-f(l))}.$$
 Figure \ref{???}  shows that $\bar{w}(k,T_{bud})$ can be computed in $O(k\cdot T_{bud})$ time using dynamic programming -- and this is what we use in the next section to evaluate $\bar{w}(k,T_{bud})$ for different learning rates.


\subsection{Analyzing learning rate $1-f(l)=d/(l+2)^2$}

We will further upper bound $\bar{w}(k, T_{bud})$ and prove small enough learning rates $f(l)\geq 1- d/(l+1)^2$ attain our desired asymptotic.
Later we will discuss what happens if there is an intial period during which the adversary already starts compromising nodes without the defender being aware or not having learning anything, i.e., $f(l)=0$ for $l\leq L^*$ and $f(l)\geq 1-d/(l-L^*)$ for $l>L^*$. Here,  $L^*$ represents this initial period; only after a suffcient level $L^*$ is reached the learning rate increases.

For now we only assume, for all $l\geq 0$,
$1-f(l)\leq d$
for some small $d$. Equivalently,
$$\beta(l)=\sqrt{\frac{1-f(l)}{d}}\leq 1,$$
  hence, $\beta(l)^2\leq \beta(l)$.
This allows us to bound 
\begin{equation*}
\begin{aligned}
\frac{m_2(l)}{1-m_1(l)} = (1-\gamma)\alpha(l) \leq \frac{(1-\gamma)pd}{\gamma} \beta(l)^2 \leq \frac{(1-\gamma)pd}{\gamma} \beta(l),\\
\frac{m_3(l)}{1-m_1(l)} \leq  pd \beta(l)^2, \mbox{ and}\\
\frac{m_4(l)}{1-m_1(l)} \leq 1- pd \beta(l)^2.
\end{aligned}
\end{equation*}

Plugging the above bounds in the expression for $\bar{w}(k,T_{bud})$ with $\frac{m_2(L)}{1-m_1(L)}\leq \frac{(1-\gamma)pd}{\gamma} \beta(L)^2$ and $(1-\gamma)/\gamma\leq \theta$ yields
\begin{subequations}
 \begin{eqnarray}
\bar{w}(k,T_{bud}) &\leq &
\sum_{L=0}^{T_{bud}-1} (1+ \theta)pd \beta(L)^2 \nonumber \\ 
& &	
\sum_{B=0}^{\min{(L,k-1)}} { \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}pd \beta(l)^2 + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
} \label{ub-a} \\
& &
{	\sum_{\substack{g_0,\dots,g_L\geq 1 s.t.\\ 
			\sum_{l=0}^{L} (g_l-1)=(k-1)-B}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{g_l-1} 
} \label{ub-b}
\end{eqnarray}
\end{subequations}

Let $b_{L+1}=0$ and define
$$ Z = \prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{b_{l+1}}.$$
We will multiply (\ref{ub-b}) with $Z$ and show an upper bound of the product which is independent of $b_l$ and $B$. We will multiply (\ref{ub-a}) with $Z^{-1}$ and show that it behaves like a sum of products of the $\beta(l)$, which remains `small enough': We choose $d$ such that $\theta\leq 1/(pd)$. Then, since $B=\sum_{l=0}^{L}b_{l+1}$,
$$(\ref{ub-b})\cdot Z = \sum_{\substack{g_0,\dots,g_L\geq 1 s.t.\\ 
			\sum_{l=0}^{L} (g_l-1)+b_{l+1}=(k-1)}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{(g_l-1)+b_{l+1}} 
	\leq \sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L} g'_l=(k-1)}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{g'_l} \leq
	(\theta pd)^{k-1}  \sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L} g'_l=(k-1)}}
	\prod_{l=0}^{L} \beta(l)^{g'_l}
	 \leq  (\theta pd)^{k-1} \prod_{l=0}^{L} \sum_{g'_l\geq 0} \beta(l)^{g'_l} 
	=(\theta pd)^{k-1}  \prod_{l=0}^{L} \frac{1}{1-\beta(l)}.$$
We derive (notice that each $b_{l+1}$ is either equal to $0$ or $1$)
$$ (\ref{ub-a})\cdot Z^{-1} 
\leq 
\sum_{B=0}^{L} \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{ \beta(l)}{\theta} + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
=
 \sum_{b_1,\dots,b_L\in\{0,1\} }
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{ \beta(l)}{\theta} + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
	= 
\prod_{l=0}^{L-1} \sum_{b_{l+1}\in \{0,1\}} \bigg( b_{l+1}\frac{ \beta(l)}{\theta} + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
=
\prod_{l=0}^{L-1} \bigg( \frac{\beta(l)}{\theta} + (1-pd \beta(l)^2) \bigg)
\leq \prod_{l=0}^{L-1} \bigg( \frac{\beta(l)}{\theta} + 1 \bigg).
$$
Combination of the above results proves
\begin{eqnarray*}
	\bar{w}(k,T_{bud}) &\leq &\nonumber
	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k-1}(1+\frac{1}{\theta})\frac{\beta(L)^2}{1-\beta(L)}\prod_{l=0}^{L-1} \frac{1+\beta(l)/\theta}{1-\beta(l)}\\
	&\leq&  	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k}(1+\frac{1}{\theta})\prod_{l=0}^{L} \frac{1+\beta(l)/\theta}{1-\beta(l)}.
\end{eqnarray*}
The argument in the product is equal to $(1+\beta(l)/\theta)/(1-\beta(l)) = 1+(1+1/\theta)\beta(l)/(1-\beta(l))$. For differentiable continuous functions $B(.)$, we can prove a useful lemma which states that if $B'(l)\geq 0$ and $B''(l)\leq 0$ for $l\geq 0$, then for $y\geq 0$
$$\prod_{l=0}^L (1+ yB'(l))\leq e^{y(B'(0)-B(0)+B(L))}.$$
For $B(l) =\beta(l)/(1-\beta(l))$ and $y=(1+1/\theta)$, application of this inequality to our upper bound yields 
\begin{eqnarray*}
	\bar{w}(k,T_{bud}) &\leq&
	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k-1}(1+\frac{1}{\theta}). e^{(1+1/\theta)(B'(0)-B(0)+B(L))} \\
	&\leq& T_{bud}\cdot [\theta p d]^{k-1}(1+\frac{1}{\theta})e^{(1+1/\theta)(B'(0)-B(0)+B(L))} .
\end{eqnarray*}
Minimizing this upper bound with respect to $\theta\geq (1-\gamma)/\gamma$ gives ($e$ denotes the natural number)
\begin{align}\label{eq.conditions}
\bar{w}(k,T_{bud}) \leq
\begin{cases}
T_{bud} [epd (B(T_{bud})-B(0)+B'(0))/(k-1)]^{k-1}(1+ (k-1)/(B(T_{bud}-1)-B(0)+B'(0))) e^{B(T_{bud}-1)-B(0)+B'(0)}, & \text{if}\ B(T_{bud}-1)-B(0)+B'(0)\geq \frac{(k-1)(1-\gamma)}{\gamma} \\
T_{bud} [\frac{1-\gamma}{\gamma}pd]^{k-1}\frac{1}{1-\gamma}e^{(B(T_{bud}-1)-B(0)+B'(0))/(1-\gamma)}, & \text{otherwise}
\end{cases}
\end{align}
The second condition is  the case $\theta=(1-\gamma)/\gamma$.

As an example, assume that $B'(l)=\frac{\beta(l)}{1-\beta(l)} \leq \frac{1}{l+1}$, then $B(T_{bud}-1) \leq \ln(T_{bud})$ and for 
$$T_{bud} \leq e^{(k-1)(1-\gamma)/\gamma -1}$$
the probability of winning for the adversary (the second case)
$$w(k,T_{bud}) \leq \bar{w}(k,T_{bud}) \leq 
T_{bud}^{1+1/(1-\gamma)} [\frac{1-\gamma}{\gamma}pd]^{k-1}\frac{e^{1/(1-\gamma)}}{1-\gamma}.
%(\frac{1-\gamma}{\gamma}pd)^{k}\frac{1}{1-\gamma}e^{C/(1-\gamma)}T_{bud}^{1+1/(1-\gamma)}$,
$$
The condition $B'(l)=\frac{\beta(l)}{1-\beta(l)} \leq \frac{1}{l+1}$ translates into 
$$1-f(l)\leq \frac{d}{(l+2)^2}$$
where $d$ should be chosen such that $d< \gamma / [p(1-\gamma)]$. For this learning rate $w(k,T_{bud})$ satisfies the desired asymptotics.


\subsection{Delayed learning}

In practice learning only start afyer a sufficient number of suspicious looking network packets are seen. That is, $f(l)=0$ for $l\leq L^*$ for some $L^*$.




 
For $(1-f(l)) \approxeq 1$, we have:


\begin{equation*}
\begin{aligned}
m_1(l) &= (1-\gamma)(1-(p+h))\\ 
m_2(l) &= (1-\gamma)p\\
m_3(l) &= \gamma p\\
m_4(l) &= [h-\gamma(h+p)]+\gamma=(1-\gamma)h+\gamma(1-p)\\
\end{aligned}
\end{equation*}

We are interested in $k^*$ as a function of $\epsilon$ for which 
\begin{eqnarray}\label{eq.k}
\sum_{k=0}^{k^{*}-1} p(k,L^{*}-1,T_{bud}-1)(\frac{m_4(l)}{1-m_1(l)}+\frac{m_3(l)}{1-m_1(l)}) +\\ p(k^*,L^{*}-1,T_{bud}-1)\frac{m_4(l)}{1-m_1(l)} \geq 1- \epsilon \nonumber
\end{eqnarray}

Then the probability of winning is 
\begin{equation}\label{eq.deta}
\leq \epsilon + (1-\epsilon)w(k-k^{*}(\epsilon),T_{bud})
\end{equation}

Notice that during phase one an $i>k^{*}(\epsilon)$  is reached ($\epsilon$ term in the above formula) and during phase two, another $k-k^{*}(\epsilon)$ horizontal or diagonal moves are needed in order to win (the second term).

We generalize the analysis of (\ref{eq.6}) for $(1-f(l))=1$ (without any constraint on $T_{bud}$):

\begin{eqnarray}\label{eq.delta}
(\ref{eq.k}) = \sum_{B=0}^{\infty}\sum_{k=B+1}^{k^{*}-1}(\ref{eq.a})(\ref{eq.b})(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)}) 
\end{eqnarray}

\saeed{Check \ref{eq.a} I guess the above should be L not l}
Notice that 

\begin{eqnarray*}
	\sum_{k=B+1}^{k^{*}-1}(\ref{eq.b}) &=& 
	\sum_{k=B+1}^{k^{*}-1}
		{	\sum_{\substack{g_0\geq 1,\dots,g_L^{*}\geq 1 s.t.\\
				\sum_{l=0}^{L^{*}}(g_l-1)=k-1-B}}
		\prod_{l=0}^{L^{*}} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
	}\\
	&=& \sum_{\substack{g'_0,\dots,g'_{L^*}\geq 0 s.t.\\
		\sum_{l=0}^{L^*-1}{g'_l \leq k^*-2-B}}}\prod_{l=0}^{L^*} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l}\\
	&\geq& \sum_{g'_0=0}^{(k^*-2-B)/L^*+1} \dots \sum_{g'_{L^*}=0}^{(k^*-2-B)/L^*+1} (\prod \dots)\\
	&=&  \prod_{l=0}^{L^*} \sum_{g'_l\geq 0}^{(k^*-2-B)/L^*+1}\bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l} \\
	&=&	 \prod_{l=0}^{L^*}\frac{1}{1-\frac{m_2(l)}{1-m_1(l)}}\big(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \big)^{L^*+1} \\
	&=& \prod_{l=0}^{L^*} \frac{1-m_1(l)}{1-m_1(l)-m_2(l)}\bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \bigg)^{L^*+1}\\
	&=& \prod_{l=0}^{L^*} \frac{1-m_1(l)}{m_3(l)+m_4(l)}\bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \bigg)^{L^*+1}
\end{eqnarray*}

\saeed{Missing part from the notes: Since $B\leq L^* \geq \bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-1}{L^*+1}}\bigg)^{L^*+1}$}

And 

\begin{eqnarray*}
	\lefteqn{\sum_{B=0}^{\infty}(\ref{eq.a})(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)}) =} \\ & & 
	{ \sum_{\substack{b_1,\dots,b_L^*\in\{0,1\} s.t.\\ 
				\sum_{l=1}^{L^*}b_l=B}}
		\prod_{l=0}^{L^*-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)  (\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})}\\
& =&	{ \sum_{b_1,\dots,b_L^*\in\{0,1\}}\prod_{l=0}^{L^*-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})
}\\
&=&\prod_{l=0}^{L^*}(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})
\end{eqnarray*}

\saeed{Note From Marten's: In the write up we can refer in parts to the analysis of \ref{eq.6} in order to save space}

So we get 
\begin{eqnarray*}
(\ref{eq.k}) &\geq& \bigg(1-(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}} \bigg)^{L^*+1}\\
&\geq& 1 - (L^*+1)(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}}
\end{eqnarray*}

We want to solve $L\geq 1-\epsilon$

\begin{equation}\label{eq.star}
(L^*+1)(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}} = (L^*+1)[\frac{(1-\gamma)p}{1-(1-\gamma)(1-(p+h))}]^{\frac{k^*-1}{L^*+1}} \leq \epsilon
\end{equation}

Notice that $p \leq 1-h$, we have:
\begin{equation}
[\frac{(1-\gamma)p}{1-(1-\gamma)(1-(p+h))}] \leq (1-\gamma)(1-h).
\end{equation}

So, Equation (\ref{eq.star}) is satisfied for $k^*$ such that 

\begin{equation}
(L^*+1)[(1-\gamma)(1-h)]^{\frac{k^*-1}{L^*+1}} \leq \epsilon.
\end{equation}

\saeed{check equation delta \ref{eq.delta} reference, there are two of them deta and delta!}

Applying (\ref{eq.delta}) gives
probability of winning for 
\begin{equation*}
1-\tilde{f}(l)=\begin{cases}
1, & \text{if $l<L^*$}.\\
1-f(l-L^*), & \text{if $l \geq L^*$}.
\end{cases}
\end{equation*}
is 
\begin{equation}\label{eq.delta.1}
\leq (L^*+1)[(1-\gamma)(1-h)]^{\frac{k^*-1}{L^*+1}} + \bar{w}(k-k^*,T_{bud}), 
\end{equation}

where $\bar{w}$ can be computed through simulation or $\bar{w}$ has the special form as derived for $(1-f(x)) = \frac{d}{(1+x)^2}$.

We want to minimize Equation \ref{eq.delta.1} for $k^*$.
\saeed{Note: Need to do this}
This shows how $h$ plays a role as wel!? It is important in phase one.

We get some function $g(k,T_{bud})\geq Prob(win)$.







============================
============================
============================
\noindent

{\bf Contributions.} By modeling the learning rate of the defender as a function $f(l)$ ($f(l)$ is the probability of detecting a next malicious payload) where $l$ represents the number of malicious payloads for a specific exploit so far collected we have the following results:
\begin{itemize}
\item If $f(l)$ does not converge to $1$, then we call such a learning rate stagnating and the adversary is able to reach his goal of $k$ compromised nodes within $poly(k)$ time budget.
\item If $f(l)\rightarrow 1$ and more specifically $1-f(l) = O(l^{-2})$, then the probability of the adversary affecting $k$ nodes (i.e., the probability of winning) is proven to be polynomial in the attacker's time budget and negligible in $k$. Simulations show that this property is even satisfied for $1-f(l) = O(l^{-???})$.
\item The above results hold for time budget measured in logical Markov model transition or real time (seconds), and also hold for learning rates that remain equal to $f(l)=0$ until a certain number $l=L^*$ malicious payloads have been collected after which learning starts.
\item The presented adversarial/defender game in terms of a Markov model is general and fits most practical ... scenarios as our extensive overview shows.
\end{itemize}
The adversary may not reach his goal of $k$ compromised nodes, but will reach a much smaller number $k_c$ compromised nodes of the order log of the time budget for $1-f(l) = O(l^{-2})$. Therefore, we conclude that at a meta level the adversary needs to find  one exploit for which the defender cannot find a fast enough increasing learning rate and the defender needs to have a learning system/methodology in place which should be able to reach fast enough learning rates for any possible exploit. In practice infrastructures are being compromised and this means that effort is needed in order to understand associated learning rates and why these are $\leq 1-O(l^{-???})$ as given by our general framework, its thorough analysis, and simulations.

%take T_bud = 2k is already sufficient. constant real time.

%We are interested in probability $w(k,T_{bud})$ of achieving $i=k$
%goal: Let w(k,T_bud) be the probability ....

%real time transfer

%We want to find a tight upper bounds and deterimine for which p,h, gamma, f(l) we can show   asymptotics 

%w = poly(T_bud) negl(k)

%Such a  result will imply containment.

%w=1/2 gives k_c = O( log poly(T_bud) )

%call this k_c

also: w=2^{-s}, T_bud=2^t gives k<= c1 s + c2 t + c3 a sort of capacity region

%(0) we start with a negative result: constant f(l)
%we conclude we need 1-f(l) --> 0
How fast does it need to converge to 0 in order to be in the above class?
In other words, what learning rate is needed? And how soon does this learning rate need to take effect?

%(1) model, probability of a path (induction), gives formula for w (can be verified)
%this gives an expression for w

%(2) observe that T_bud part is close to 1, more precisely w without the self-loop part turns out to be a tight approximation:
%define wbar, we prove
%LB / UB
%(use the same type of thinking which proves (0))
%This can be used to study the asymptotics of w

%(3) UB on wbar for d/(l+1)^2

%(4) note that wbar corresponds to the model (also define alpha) without self-loops and that a dynamic program ...

Conclusion capacity region is lower bounded by ... and UB ...
In the next section we use the dynamic program to investigate intermediate values ..

(5) Late start of learning: does the initial convergence of the learning rate matter?

phase 1 and 2

k_c inclreases

apply to  (3)




\section{Appendix}
\label{sec:proofs}

%\vspace{-1mm}
This appendix provides the analysis of the Markov model depicted in Fig. \ref{markovModel}. The goal of the adversary is to reach a winning state $(k,l)$ for some $l\geq 0$. Here, $k$ represents the total number of nodes which the adversary wishes to compromise before using the collective of these nodes in the next attack phases (e.g. botnet applications). On the other hand, the objective of the defender is to learn more and more regarding the attack technologies, more specifically the malicious attack payloads in order to be able to recognize and halt future moves by the attacker. That is, the defender hopes to push level $l$ -the number of detected malicious payloads so far- higher and higher leading to a higher probability $f\mytiny{(}l\mytiny{)}$ of successfully detecting a next malicious payload. The ultimate goal of the defender is to have a good enough learning mechanism in place to limit the probability of reaching $k$ negligible. In other words, the adversary cannot reach a winning state in practice.

Fig. \ref{markovModel}, as explained in section \ref{ss.markovModel} shows several possible transitions from state to (another) states. The corresponding probabilities can be rewritten as follows:

\begin{equation}\label{eq.transitions.rewritten}
\begin{aligned}
m_1 &= f\mytiny{(}l\mytiny{)}(1-\gamma)+(1-f\mytiny{(}l\mytiny{)})(1-\gamma)(1-p-h)\\
	&= (1-\gamma)(1-(p+h)(1-f\mytiny{(}l\mytiny{)}))\\
m_2 &= (1-f\mytiny{(}l\mytiny{)})(1-\gamma)p \\
m_3 &= (1-f\mytiny{(}l\mytiny{)})\gamma p\\
m_4 &= (1-f\mytiny{(}l\mytiny{)})(1-\gamma)h+f\mytiny{(}l\mytiny{)}\gamma + (1-f\mytiny{(}l\mytiny{)})\gamma (1-p)\\
	&= (1-f\mytiny{(}l\mytiny{)})[(1-\gamma)h+\gamma(1-p)] + f\mytiny{(}l\mytiny{)}\gamma\\
	&= (1-f\mytiny{(}l\mytiny{)})[h-\gamma(h+p)] + \gamma
\end{aligned}
\end{equation}

where
\begin{align*}
h &= \frac{H}{N}, & p_i &= \frac{(K-i)}{N} \approx p
\end{align*}

Notice that in these transition probabilities we take $p$ to be a constant and not depending on $i$. This is a reasonable assumption if 
\begin{align*}
 p_i &= \frac{(K-i)}{N}
\end{align*}
where $K$ is the total number of vulnerable nodes out of a total number of $N$ nodes, and $p_i$ is the probability of a \emph{memoryless adversary} picking a random node in the hope to hit one of the $(K-i)$ remaining vulnerable nodes (which it has not yet compromised). Since $k \ll K $ therefore, 

\begin{align*}
 p_i &\approx \frac{K}{N} = p
\end{align*}

This means we are dealing with a constant vulnerability density function.
A smarter adversary, however, may use a hitlist target locating strategy and this would make $p_i$ not a constant. In this case, we assume a worst-case scenario for the adversary meaning that $p_i \leq p$.

We will analyze to what extent our bounds on the probability of reaching a winning state ($i=k$) are sensitive to the choice of $p$. It turns out that this sensitivity is limited, therefore, our bounds cannot be much improved when assuming non-constant (i.e., non-worst-case) $p_i$.

In the next sections, we first give a complex formula for the probability of winning $w$ (i.e., the probability of reaching a winning state). Next, we simplify the formula by upper bounding. We analyze two class of learning functions:

\begin{enumerate}
	\item $(1-f\mytiny{(}l\mytiny{)})\leq d/l$, and
	\item $ \tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up}$.
\end{enumerate}

We show how these two functions can be combined into 

%\begin{equation}
%(1-f\mytiny{(}l\mytiny{)})\leq d/l  \mbox{ for }l \leq L^*,
%\end{equation}
%\begin{equation}
%	\tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up} = (1-f\mytiny{(}L^*\mytiny{)})  \mbox{ for }l > L^* .
%\end{equation}
\begin{equation}\label{eq.(1)}
(1-f\mytiny{(}l\mytiny{)})\leq d/l  \mbox{ for }l \leq L^*,~and~\\
\tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up} = (1-f\mytiny{(}L^*\mytiny{)})  \mbox{ for }l > L^* .
\end{equation}

%\begin{eqnarray}
%(1-f\mytiny{(}l\mytiny{)})\leq d/l  \mbox{ for }l \leq L^*,~and~\\
%\tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up} = (1-f\mytiny{(}L^*\mytiny{)})  \mbox{ for }l > L^* .
%\end{eqnarray}
%$$
%(1-f\mytiny{(}l\mytiny{)})\leq d/l  \mbox{ for }l \leq L^*,
%$$
%and
%$$
%\tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up} = (1-f\mytiny{(}L^*\mytiny{)})  \mbox{ for }l > L^* .
%$$

%\begin{enumerate}
%	\item $(1-f\mytiny{(}l\mytiny{)})\leq d/l$ for $l \leq L^*$, and
%	\item $ \tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up} = (1-f\mytiny{(}L^*\mytiny{)})$ for $l > L^*$.
%\end{enumerate}

For this function with suitably chosen parameters, the probability of winning is exponentially decreasing in $k$ and is only linearly proportional to the total time budget $T_{bud}$ which is measured in the total number of transitions given to the adversary.
We represent this result in the form of a ``security capacity function'' $g\mytiny{(}k,t\mytiny{)}$ that is:
For $T_{bud} \leq 2^t$, if $(s+t)\leq g\mytiny{(}k,t\mytiny{)}$, then the probability of winning is $w \leq 2^{-s}$.
We show that for $f\mytiny{(}l\mytiny{)}$ in (\ref{eq.(1)}) with suitably chosen parameters $d,L^*,\tau_{low},\tau_{up},\gamma,h,$ and $p$,

\begin{equation*}
\begin{aligned}
g\mytiny{(}k,t\mytiny{)} = \Theta(k)
\end{aligned}
\end{equation*}
and if we measure $T_{bud}$ in terms of seconds, then $g\mytiny{(}k,t\mytiny{)}$ needs to be replaced by $[g\mytiny{(}k,t\mytiny{)} - \log k]$ which maintains the $\Theta(k)$ asymptotics. 

The analysis in this appendix teaches that if an adversary is successful in practice, then either the defender initially learns too slowly or it cannot reach a large enough probability of successful detection $f\mytiny{(}l\mytiny{)}$ no matter how many malicious payloads are known and can be learned from.

%%%%%% CHECKED: SO FAR SO GOOD %%%%%%

\subsection{Probability of Winning}

In order to analyze the probaility of winning, i.e., the adversary reaching a state $(k,L)$ for some $L$, we investigate the shape of a typical sequence of transitions (i.e., a path) through the Markov model. We define $t(i,l)$ as the total number of self-loops, i.e., transitions with probability $m_1(l)$ from the state $(i,l)$ back to itself. We notice that


\begin{equation}\label{eq.pois}
\begin{aligned}
Prob(t(i,l)=u) = m_1(l)^{u}(1-m_1(l))
\end{aligned}
\end{equation}

%is defined as a Poisson process. Fig. \ref{fig.samplePath} depicts a typical path from $(0,0)$ to $(k,L)$ without showing any self-loops where in this example $(k=18,L=22)$.
is defined as a Poisson process. Fig. \ref{fig.samplePath} depicts a typical path from $(0,0)$ to $(k,L)$ without showing any self-loops.
 	\begin{figure}[h!]
	\begin{center}
		\scalebox{0.50}
		{\includegraphics{samplePath}}%Transf
%		\caption{A sample path toward the winning state in which $k=18$ and the maximum level reached by the adversary is $L =22$}
		\caption{A sample path toward the winning state without depicting the self-loops at each state $(i,l)$ in the path}
		\label{fig.samplePath}
	\end{center}
\end{figure}
%\saeed{Missing figure: a typical path}

Along with a typical path, we see horizontal, diagonal, and vertical transitions toward the winning state. For $(i,l) \in~ path$ we have $t(i,l)$ self-loops after which the path exits $(i,l)$ along with a horizontal, diagonal or vertical transition (see (\ref{eq.pois})).
Given that $(i,l)$ does not continue with anothoer self-loop we have 

\begin{equation}
\begin{aligned}
	Prob(horizontal~transition) &= Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i+1,l\mytiny{)}|no~self\mymathhyphen loop)\\
	&= \frac{m_2(l)}{1-m_1(l)}\\
	Prob(diagonal~transition) &= Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i+1,l+1\mytiny{)}|no~self\mymathhyphen loop)\\
&= \frac{m_3(l)}{1-m_1(l)},~and\\
	Prob(vertical~transition) &= Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i,l+1\mytiny{)}|no~self\mymathhyphen loop)\\
&= \frac{m_4(l)}{1-m_1(l)}.\\
\end{aligned}
\end{equation}

Let us define $g_l$ as the number of states at each level $l$ (i.e., the number of states within the path with the same level) $(i,l) \in ~ path$, and
  \begin{equation}
b_l=
\begin{cases}
0, & \text{if}\ level~ l~ is~ entered~ via~ a~ vertical~ transition \\
1, & \text{if}\ level ~l ~is~ entered ~via~ a ~diagonal~ transition
\end{cases}
\end{equation}
This does not define $b_0$. In general $g_l \geq 1$ for all $0 \leq l \leq L$.
Note that the length of the path, i.e., the total number of transitions without self-loops, is equal to

%\begin{equation*}
%\begin{aligned}
%k+L- \sum_{a=1}^{L} b_a,
%\end{aligned}
%\end{equation*}
\begin{equation*}
\begin{aligned}
k+L- B,
\end{aligned}
\end{equation*}
where $ B = \sum_{a=1}^{L} b_a$ is the total number of diagonal transitions. Therefore, the total number of vertical transitions is equal to $(L-B)$, and the number of horizontal transitions is equal to
\begin{equation}\label{eq.4}
\begin{aligned}
\sum_{a=0}^{L} (g_a-1)= k - B,
\end{aligned}
\end{equation}
\saeed{Did we start from k=1 or 0, if from 0, the above is correct but you need to check all the following summations' bounds and change it from $k-B-1$ to $k-B$!}
and, 
\begin{equation*}
\begin{aligned}
k =  \sum_{a=0}^{L-1} (g_a-1 + b_{a+1})+(g_L-1),
\end{aligned}
\end{equation*}

%in which the number of horizontal transitions is equal to




%and the total number of vertical transitions is
%\begin{equation*}
%\begin{aligned}
%L - \sum_{a=1}^{L} b_a,
%\end{aligned}
%\end{equation*}

%and the number of diagonal transitions is 
% \begin{equation*}
% \begin{aligned}
% \sum_{a=1}^{L} b_a.
% \end{aligned}
% \end{equation*}
 
 Finally, the path enters level $l$ at $i =i_l$ with 
 
  \begin{equation*}
 \begin{aligned}
 i_l = \sum_{a=0}^{l-1} (g_a-1 + b_{a+1})
 \end{aligned}
 \end{equation*}
 where $i_L + g_L = k$ by  (\ref{eq.4}).
 
 \saeed{if we are counting from 0 the above should be $i_L +g_L =k+1$}
 
\begin{lemma}
 The probability of a path from $(0,0)$ toward $(k,L)$ with self-loops at $(k,L)$ till the moment the path is ready to leave $(k,L)$, in which the path is represented by $g_0,\dots,g_L,b_1,\dots,b_L$, and the function $t(i,l)$ is 

\begin{eqnarray}\label{eq.5}
Pr(path)&=& \prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg).\nonumber\\
&& \prod_{l=0}^{L} \bigg( \frac{m_2(l)}{1-m_1(l)}\bigg)^{g_l-1}.\nonumber\\
& & \prod_{l=0}^{L}\prod_{i=0}^{g_l-1}m_1(l)^{t(i_l+i,l)}(1-m_1(l))
\end{eqnarray}
\end{lemma}

 
%\saeed{i should start from 1 not 0}
\begin{proof}
\textbf{(Base case)}
For  $(k,L)$ = (0,0), we have $g_0 =1$ and (\ref{eq.5}) would be $m_1(0)^{t(0,0)}(1-m_1(0))$ which it holds trivially.
 
\textbf{(Hypothesis)} Suppose the claim holds for paths to $(k',L')$ where $0\leq k'\leq k$ and $0\leq L'\leq L$ such that $(k',L') \neq (k,L)$. Consider a path to (k,L). This path will first enter $(k',L') = (k-1,L)$, $(k',L')=(k-1,L-1)$, or $(k',L')=(k,L-1)$ before transitioning to $(k,L)$. Let the subpath to $(k',L')$ be represented by $b_l',g_l',i_l'$ and $t'(i,l) = t(i,l)$, where $i'_{L'} + g'_{L'} = k'$.

\textbf{Case $(k',L')=(k-1,L)$:} We multiply (\ref{eq.5}) for $(k-1,L)$ with the probability of  a self-loop in $(k-1,L)$ and the transition probability from $(k-1,L)$ toward $(k,L)$:


\begin{eqnarray*}
	m_1(L)^{t(k-1,L)}.m_2(L)
&=& [m_1(L)^{t(k-1,L)}.(1-m_1(L))].(\frac{m_2(L)}{1-m_1(L)})\\
&=& [m_1(L)^{t(i'_{L}+g'_L,L)}.(1-m_1(L))].(\frac{m_2(L)}{1-m_1(L)})
\end{eqnarray*}
Notice that $b_l=b'_l$ and $g_l = g'_l$ for $0\leq l \leq L-1$, and,
$b_L = b'_L$, $g_L = g'_L+1$, i.e., $i'_{L}+g'_{L} = i_L + g_L -1$.
Hence, (\ref{eq.5}) holds for the path to $(k,L)$.

\textbf{Case $(k',L')=(k-1,L-1)$:} Now (\ref{eq.5}) is multiplied with a self-loop in $(k-1,L-1)$ and a transition $(k-1,L-1)$ toward $(k,L)$. We have 

\begin{eqnarray*}
	m_1(L-1)^{t(k-1,L-1)}.m_3(L-1)
	&=& [m_1(L-1)^{t(k-1,L-1)}.(1-m_1(L-1))].\\& &
	(\frac{m_3(L-1)}{1-m_1(L-1)})\\
	&=& [m_1(L-1)^{t(i'_{L-1}+g'_{L-1},L-1)}.(1-m_1(L-1))].\\& &
	[b_L\frac{m_3(L-1)}{1-m_1(L-1)} + (1-b_L)\frac{m_4(L-1)}{1-m_1(L-1)}]
\end{eqnarray*}

with $b_L=1$, $g_L =0$, $g_{L-1}=g'_{L-1}+1$ and all other $b_l = b'_l$, $g_l=g'_l$. Hence, $i'_{L-1} + g'{L-1} = i_{L-1} + g_{L-1} - 1$.
Hence, (\ref{eq.5}) holds for the path to $(k,L)$.
%\saeed{Unclear equation see page 5, analysis 3}

\textbf{Case $(k',L')=(k,L-1)$:} Now, (\ref{eq.5}) is multiplied with a self-loop in $(k,L-1)$ and a transition from $(k,L-1)$ to $(k,L)$:
\begin{eqnarray*}
	m_1(L-1)^{t(k,L-1)}.m_4(L-1)
	&=& [m_1(L-1)^{t(k,L-1)}.(1-m_1(L-1))].\\& &
	(\frac{m_4(L-1)}{1-m_1(L-1)})\\
	&=& [m_1(L-1)^{t(i'_{L-1}+g'_{L-1},L-1)}.(1-m_1(L-1))].\\& &
	[b_L\frac{m_3(L-1)}{1-m_1(L-1)} + (1-b_L)\frac{m_4(L-1)}{1-m_1(L-1)}]
\end{eqnarray*}

with $b_L = 0$, $g_L = 0$, $g_{L-1} = g'_{L-1}+1$ and all other $b_l=b'_l$, $g_l=g'_l$. Hence, $i'_{L-1}+g'_{L-1} = i_{L-1} + g_{L-1}-1$. Therefore, (\ref{eq.5}) holds for the path to $(k,L)$.
\qed
\end{proof}



\saeed{analysis4 starts from here}

%As noted above, the length of the path toward $(k,L)$ is equal to 
%\begin{equation*}
%\begin{aligned}
%k+L-B,
%\end{aligned}
%\end{equation*}
%where $B = \sum_{l=1}^{L} b_{l}$. 

Suppose there is a limited number of transitions $T_{bud}$ one can use to reach $(k,L)$. Then the probability of reaching $(k,L)$ within that time budget is equal to the sum of $Prob(path~to~(k,L))$ over all possible paths satisfying 

\begin{equation*}
\begin{aligned}
k+L-B+T \leq T_{bud}.
\end{aligned}
\end{equation*}
where $T$ represents the total number of self-loops in the path and is defined as $T = \sum_{l=0}^{L}t_l$ in which $t_l = \sum_{i=0}^{g_l-1} t(i_l+i,l)$ is the number of self-loops happening at a fixed level $l$.

In order to analyze this probability, we introduce $p(k,L,T_b)$ as the probability of the Markov model reaches state $(k,L)$ within $T_b$ transitions and after -possibly zero- self-loops, it is ready to transit away from $(k,L)$.
Now notice that the probability $w$ of reaching any winning state $(k,L)$ for some $L\geq 0$ within $T_{bud}$ transitions is equal to:

\begin{eqnarray} \label{eq.w}
 w(k, . ,T_{bud})&=&	\sum_{L\geq 0} p(k-1,L,T_{bud}-1).	 \{\frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\}
\end{eqnarray}

This formula corresponds to Fig. \ref{fig.LthTerm}.

 	\begin{figure}[h!]
	\begin{center}
		\scalebox{0.50}
		{\includegraphics{Lth_term.pdf}}%Transf
		%		\caption{A sample path toward the winning state in which $k=18$ and the maximum level reached by the adversary is $L =22$}
		\caption{???}
		\label{fig.LthTerm}
	\end{center}
\end{figure}

The formula for $w$ simply considers all the possible paths toward the state $(k-1,L)$ within $(T_{bud} -1)$ transitions and a single final transition via $m_2(L)$ or $m_3(L)$ toward the winning state. This enables us to avoid counting self-loops in states $(k,L)$ and transitions from $(k,L-1)$ to $(k,L)$ (since state $i=k$ was already reached). Notice that we are interested in the probability of entering state $(k,L)$  and the time it takes to reach there \emph{for the first time} and that is why we are not interested in counting self-loops or vertical moves at $(k,L)$.

\begin{claim}
	Given our analysis for $Prob(path)$ (see (\ref{eq.5})) and bearing in mind that $k,L,$ and $T_b$ are fixed, we need to consider all the possible $B$ and $T$. Therefore, we get:
	\begin{subequations}
		\begin{eqnarray}\label{eq.ABC}
		p(k,L,T_b) &= &
		\sum_{\substack{B,T s.t.\\
				k+L-B+T\leq T_b}}\nonumber\\& &
		{ 
			\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ \label{eq.a}
					\sum_{l=1}^{L}b_l=B}}
			\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
		}\\& &
		{	\sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\ \label{eq.b}
					\sum_{l=0}^{L}(g_l-1)=k-1-B}}
			\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
		}\\& &
		{
			\sum_{\substack{t_0,\dots,t_L s.t.\\ \label{eq.c}
					\sum_{l=0}^{L}t_l=T}}
			\prod_{l=0}^{L} 
			{	\sum_{\substack{t(i_l,l),\dots,t(i_l+g_l-1,l) \\
						s.t.\sum_{i=0}^{g_l-1}t(i_l+i,l)=t_l}}
				\prod_{i=0}^{g_l-1} 
				m_1(l)^{t(i_l+i,l)}(1-m_1(l))
			}
		}
		\end{eqnarray}
	\end{subequations}
\end{claim}

\begin{proof}
	\textbf{(Base case)}
	For  $(k,L,T_{bud})$ = (0,0,0), we have $g_0 =1$ and we have $m_1(0)^{t(0,0)}(1-m_1(0))$ since the time budget is $0$ we get $(1-m_1(0))$ which it holds trivially.
	
	\textbf{(Hypothesis)}  Suppose the claim holds for paths to $(k',L')$ within $T'_{b})$ steps where $0\leq k'\leq k$, $0\leq L'\leq L$, and $0\leq T'_{b}\leq T_{b}-1$. Note that since there exist a limited time budget available for the adversary to reach the final state and it takes at least one transition for the adversary from $(k',L')$ to $(k,L)$, such that $(k',L') \leq (k,L)$ therefore we have $T'_b \leq T_b -1$.
	Consider a path to $(k,L)$ within $T'_b = T_b -1$ transitions. This path will first enter $(k',L') = (k-1,L)$, $(k',L')=(k-1,L-1)$, $(k',L')=(k,L-1)$, or $(k,L)=(k,L)$ in $T_b -1$ transitions before transitioning to $(k,L)$. Let the subpath to $(k',L')$ be represented by $b'_l,g'_l,i'_l$ and $t'(i,l) = t(i,l)$, where $i'_{L'} + g'_{L'} = k'$.
	
	\textbf{Case $(k',L',T'_b)=(k-1,L,T_b-1)$:} We multiply the above expression for $(k-1,L,T_b-1)$ with the probability of a transition from $(k-1,L)$ toward $(k,L)$ in a single step (i.e., a horizontal transition) conditiong on the fact that no more self-loops happen:
	\begin{eqnarray*}
(\frac{m_2(L)}{1-m_1(L)})
	\end{eqnarray*}
	Notice that $b_l=b'_l$ and $g_l = g'_l$ for $0\leq l \leq L-1$, and,
	$b_L = b'_L$, $g_L = g'_L+1$, i.e., $i'_{L}+g'_{L} = i_L + g_L -1$.
	Hence, the expression holds for the path to $(k,L)$.

\textbf{Case $(k',L',T'_b)=(k-1,L-1,T_b-1)$:} We multiply the above expression for $(k-1,L-1,T_b-1)$ with the probability of a transition from $(k-1,L-1)$ toward $(k,L)$ in a single step (i.e., a diagonal transition) conditiong on the fact that no more self-loops happen:
\begin{eqnarray*}
	(\frac{m_3(L-1)}{1-m_1(L-1)})=[b_L\frac{m_3(L-1)}{1-m_1(L-1)} + (1-b_L)\frac{m_4(L-1)}{1-m_1(L-1)}]
\end{eqnarray*}

with $b_L=1$, $g_L =0$, $g_{L-1}=g'_{L-1}+1$ and all other $b_l = b'_l$, $g_l=g'_l$. Hence, $i'_{L-1} + g'{L-1} = i_{L-1} + g_{L-1} - 1$.
Hence, the expression holds for the path to $(k,L)$.
	
\textbf{Case $(k',L',T'_b)=(k,L-1,T_b-1)$:} We multiply the above expression for $(k,L-1,T_b-1)$ with the probability of a transition from $(k,L-1)$ toward $(k,L)$ in a single step (i.e., a vertical transition) conditiong on the fact that no more self-loops happen:
\begin{eqnarray*}
	(\frac{m_4(L-1)}{1-m_1(L-1)})=
	[b_L\frac{m_3(L-1)}{1-m_1(L-1)} + (1-b_L)\frac{m_4(L-1)}{1-m_1(L-1)}]
\end{eqnarray*}

with $b_L = 0$, $g_L = 0$, $g_{L-1} = g'_{L-1}+1$ and all other $b_l=b'_l$, $g_l=g'_l$. Hence, $i'_{L-1}+g'_{L-1} = i_{L-1} + g_{L-1}-1$. Therefore, the expression holds for the path to $(k,L)$.

\textbf{Case $(k',L',T'_b)=(k,L,T_b-1)$:} We multiply the above expression for $(k,L,T_b-1)$ with the probability of a single self-loop at $(k,L)$:
\begin{eqnarray*}
?
\end{eqnarray*}
with???
	\qed
\end{proof}
%\begin{subequations}
%\begin{eqnarray}\label{eq.ABC}
%p(k,L,T_b) &= &\nonumber\\& &
%\sum_{\substack{B,T s.t.\\
%		k+L-B+T\leq T_b}}\nonumber\\& &
%{ 
%	\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\
%			\sum_{l=1}^{L}b_l=B}}
%				\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
%			}\\& &
%				{	\sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\
%						\sum_{l=0}^{L}(g_l-1)=k-1-B}}
%				\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
%}\\& &
%{
%	\sum_{\substack{t_0,\dots,t_L s.t.\\
%		\sum_{l=0}^{L}(t_l)=T}}
%\prod_{l=0}^{L} 
%{	\sum_{\substack{t(i_l,l),\dots,t(i_l+g_l-1,l) \\
%		s.t.\sum_{i=0}^{g_l-1}t(i_l+i,l)=t_l}}
%\prod_{i=0}^{g_l-1} 
%m_1(l)^{t(i_l+i,l)}(1-m_1(l))
%}
%}
%\end{eqnarray}
%\end{subequations}




Notice that (\ref{eq.c}) is equal to\footnote{This simply can be noticed by representing each self-loop at a fixed level by $0$ and the event that the path exits the $(i,l)$ state but remains on the same level, i.e., $(i+1,l)$, by a $1$. The problem then can be translated into choosing $(g_l-1)$ ones (as the total number of states at the same level) out of the total number of zeros and ones $(t_l+g_l-1)$ where $t_l$ is the total number of self-loops happen at the same level} 

	\begin{eqnarray*}
{
	\sum_{\substack{t_0,\dots,t_L s.t.\\ 
			\sum_{l=0}^{L}t_l=T}}
	\prod_{l=0}^{L} 
	{{t_l+g_l-1 \choose g_l-1} m_1(l)^{t_l}(1-m_1(l))^{g_l}
	}
}
\end{eqnarray*}

As a check, if we sum  (\ref{eq.c}) for $T=0$ to $T= \infty$, then this sums to $1$ (since (\ref{eq.c}) models self-loops as a Poisson process at each $(i_l+i,l)$).

So, for $L\geq1$, 

	\begin{eqnarray}
	\lefteqn{\sum_{k\geq 0}p(k,L,\infty)(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)}) = }\nonumber\\ & & \sum_{k\geq 1}p(k,L,\infty)(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})  \nonumber\\
	&=& \sum_{k\geq 1}{\sum_{B}(\ref{eq.a})(\ref{eq.b})(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})} \nonumber\\
	&=& \sum_{k\geq 1}{\sum_{B=0}^{k-1}(\ref{eq.a})(\ref{eq.b})(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})} \nonumber\\
	&=& \sum_{B=0}^{\infty}{\sum_{k=B+1}^{\infty}(\ref{eq.a})(\ref{eq.b})(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})} \label{eq.6}
	\end{eqnarray}

Notice that

	\begin{eqnarray*}
	\sum_{k=B+1}^{\infty}{(\ref{eq.b})} &=&
	\sum_{k=B+1}^{\infty}
		{	\sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\
				\sum_{l=0}^{L}(g_l-1)=k-1-B}}
		\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
	}\\
&=& \sum_{g'_0,\dots,g'_L \geq 0}\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l}\\
&=&	\prod_{l=0}^{L} \sum_{g'_l\geq 0}\bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l} 
= \prod_{l=0}^{L}\frac{1}{1-\frac{m_2(l)}{1-m_1(l)}} = \prod_{l=0}^{L} \frac{1-m_1(l)}{1-m_1(l)-m_2(l)}\\
&=& \prod_{l=0}^{L} \frac{1-m_1(l)}{m_3(l)+m_4(l)}
	\end{eqnarray*}
And 
	\begin{eqnarray*}
\lefteqn{\sum_{B=0}^{\infty}{(\ref{eq.a})\{\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)}\}} = }	 \\
& &	\sum_{B=0}^{\infty}  
{ 
	\sum_{\substack{b_1,\dots,b_L\in\{0,1\}\\ 
			s.t.\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
}
\{\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)}\}\\
&=& { 
	\sum_{b_1,\dots,b_L\in\{0,1\}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
}
\{\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)}\}\\
&=& \prod_{l=0}^{L} \bigg(\frac{m_3(l)}{1-m_1(l)} + \frac{m_4(l)}{1-m_1(l)} \bigg)
\end{eqnarray*}


%\begin{align*}
%	\sum_{B=0}^{\infty}{(\ref{eq.a})(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})} &= 
%	\sum_{B=0}^{\infty} 
%	{ 
%		\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
%				\sum_{l=1}^{L}b_l=B}}
%		\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
%	}.\\
%	(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})\\
%	&= { 
%		\sum_{b_1,\dots,b_L\in\{0,1\}}
%		\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
%	}.\\
%	(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})\\
%	&= \prod_{l=0}^{L} \bigg(\frac{m_3(l)}{1-m_1(l)} + \frac{m_4(l)}{1-m_1(l)} \bigg)
%\end{align*}
Therefore, we get (\ref{eq.6}) equals $1$ which fits Fig. \ref{fig.LthTerm}.


We are not able to easily verify that $w(k,\infty) =1$, in a similar way. This needs to be done by induction.
If $m_1,m_2,m_3,m_4$ are independent of $l_i$, an easy verification of $w(k,\infty)=1$ is possible.

\begin{eqnarray*}
\sum_{L\geq 0}p(k-1,L,\infty)(\frac{m_2(L)}{1-m_1(L)} + \frac{m_3(L)}{1-m_1(L)})&= & 
\sum_{L\geq 0}\sum_{B}(\ref{eq.a})(\ref{eq.b})(\frac{m_2(L)}{1-m_1(L)} + \frac{m_3(L)}{1-m_1(L)})\\
&=& \sum_{B=0}^{k-1}\sum_{L\geq B}(\ref{eq.a})(\ref{eq.b})(\frac{m_2(l)}{1-m_1(l)} + \frac{m_3(l)}{1-m_1(l)})\\
\end{eqnarray*}

Notice that

\begin{eqnarray*}
	(\ref{eq.b}) &=& {	
		\sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\ 
				\sum_{l=0}^{L}(g_l-1)=k-1-B}}
		\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
	}\\
&=& \sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\ 
		\sum_{l=0}^{L}(g_l-1)=k-1-B}}
 \bigg(\frac{m_2}{1-m_1} \bigg)^{k-1-B}\\
&=& {k-1-B+L \choose L}\bigg(\frac{m_2}{1-m_1} \bigg)^{k-1-B}
\end{eqnarray*}
%\saeed{check the above formula more specifically $m_2,m_3$}
moreover, 
\begin{eqnarray*}
	(\ref{eq.a}) &=& {	
	\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
}\\
&=& \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
		\sum_{l=1}^{L}b_l=B}}  \bigg( \frac{m_3}{1-m_1}\bigg)^{B} \bigg(\frac{m_4}{1-m_1} \bigg)^{(L-B)}\\
	&=& {L \choose B}\bigg( \frac{m_3}{1-m_1}\bigg)^{B}  \bigg(\frac{m_4}{1-m_1} \bigg)^{L-B}
\end{eqnarray*}
%\begin{eqnarray}\label{eq.5}
%&=& \prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg).\nonumber\\
%&& \prod_{l=0}^{L} \bigg( \frac{m_2(l)}{1-m_1(l)}\bigg)^{g_l-1}.\nonumber\\
%& & \prod_{l=0}^{L}\prod_{i=0}^{g_l-1}m_1(l)^{t(i_l+i,l)}(1-m_1(l))\nonumber
%\end{eqnarray}

Notice that
\begin{equation*}
	{k-1-B+L \choose L}{L \choose B} = {k-1+L-B \choose L-B}{k-1 \choose B}
\end{equation*}

By substituting $F=L-B$ we have:

\begin{equation*}
\sum_{L\geq B}(\ref{eq.a})(\ref{eq.b})=\sum_{F\geq 0}{k-1+F \choose F}\bigg(\frac{m_4}{1-m_1} \bigg)^{F}{k-1 \choose B}\bigg( \frac{m_2}{1-m_1}\bigg)^{k-1-B}\bigg( \frac{m_3}{1-m_1}\bigg)^{B}
\end{equation*}

Therefore,

\begin{eqnarray*}
\sum_{B=0}^{k-1}\sum_{L\geq B}(\ref{eq.a})(\ref{eq.b})&=&
\sum_{F\geq 0}{k-1+F \choose F}\bigg(\frac{m_4}{1-m_1} \bigg)^{F}\bigg( \frac{m_2+m_3}{1-m_1}\bigg)^{k-1} \\
&=& {
	\sum_{F\geq 0} 
	\sum_{\substack{f_1,\dots,f_k s.t.\\ 
			\sum f_i=F}}
		 \prod_{i=1}^{k} \bigg(\frac{m_4}{1-m_1}\bigg)^{f_i} \bigg(\frac{m_2+m_3}{1-m_1} \bigg)^{k-1}
	}\\
&=& \bigg( \prod_{i=1}^{k} \sum_{f_i=0}^{\infty}(\frac{m_4}{1-m_1})^{f_i} \bigg)(\frac{m_2+m_3}{1-m_1})^{k-1}\\
&=& \bigg(\frac{1}{1-\frac{m_4}{1-m_1}}\bigg)^{k} \bigg(\frac{m_2+m_3}{1-m_1}\bigg)^{k-1} = \frac{1-m_1}{m_2+m_3}
\end{eqnarray*}

and after multipling with $(\frac{m_2}{1-m_1} + \frac{m_3}{1-m_1})$ we get indeed $1$.

Note that if $(1-f(l)) = \tau$, then $m_1,m_2,m_3$ and $m_4$ are independent of $l$. In fact, the Markov model reduces to Fig. \ref{fig.reducedMarkovModel}.

\begin{figure}[t]
	\centering
	\begin{tikzpicture}
	\tikzset{
		>=stealth',
		node distance=3cm and 3cm ,on grid,
		every text node part/.style={align=center},
		state/.style={minimum width=1.5cm,
			%    		font=\small,
			draw,
			circle},
	}
	% Add the states
	\node[state]             (c) {i};
	\node[state, right=of c] (r) {i\pp};
	%	\node[state, left=of c] (lose) {0};
	% Connect the states with arrows
	\draw[every loop]
	(c) edge[auto=left]  node {$m_{2}+m_3$} (r)
	%(r) edge[bend left, auto=right] node {0.7} (s)
	%(c) edge[loop above]             node {($1-p_i-f(.)$)} (c)
%	(c) edge[ auto=left] node {$m_3$} (rr)
%	(c) edge[auto=right] node {$m_4$} (b)
	(c) edge[loop above]             node {$m_1+m_4$} (c);
	%(d) edge[loop above]             node {} (d);
	\end{tikzpicture}
	\caption{Reduced Markov model of the game for a constant $(1-f(l))=\tau$}
	\label{fig.reducedMarkovModel}
\end{figure}

Within a budget $T_{bud}$ we reach $i=k$ with probability 

\begin{eqnarray}
\lefteqn{ \sum_{T=k}^{T_{bud}} {T-1 \choose k-1}(m_1+m_4)^{(T-1)-(k-1)}(m_2+m_3)^{k-1+1} =} \nonumber\\
 & & \sum_{T=k}^{T_{bud}} {T-1 \choose k-1}(m_1+m_4)^{T-k}(m_2+m_3)^{k}\nonumber\\
&=& \sum_{T-k=0}^{T_{bud}-k} {(T-k)+(k-1) \choose (T-k)}(m_1+m_4)^{T-k}(m_2+m_3)^{k} \nonumber\\
&=&  \sum_{i=0}^{T_{bud}-k} {i+(k-1) \choose i}(m_1+m_4)^{i}(m_2+m_3)^{k} \label{eq.7}
\end{eqnarray}

A lower bound on (\ref{eq.7}) can be derived as follows:

\begin{eqnarray*}
(\ref{eq.7}) &=&  \sum_{i=0}^{T_{bud}-k}
{\sum_{\substack{f_1,\dots,f_k s.t.\\ 
		\sum f_j=i}}
\prod_{j} (m_1+m_4)^{f_j}(m_2+m_3)^{k}
}\\
&=& \sum_{\substack{f_1,\dots,f_k s.t.\\ 
		\sum f_j\leq T_{bud}-k}}
\prod_{j} (m_1+m_4)^{f_j}(m_2+m_3)^{k}\\
&\geq& \sum_{f_1=0}^{(T_{bud}-k)/k}\dots\sum_{f_k=0}^{(T_{bud}-k)/k}\prod_{j}(m_1+m_4)^{f_j}(m_2+m_3)^{k}\\
&=& \prod_{j}\sum_{f_j=0}^{(T_{bud}-k)/k}(m_1+m_4)^{f_j}(m_2+m_3)^{k}\\
&=& \prod_{j=1}^{k}\frac{1-(m_1+m_4)^{T_{bud}/k}}{1-(m_1+m_3)}(m_2+m_3)^{k}\\
&=& [1-(m_1+m_4)^{T_{bud}/k}]^{k}\\
&\geq& 1-k(m_1+m_4)^{T_{bud}/k}
\end{eqnarray*}

This shows that $w\approx 1$ for relatively small $T_{bud}$ because $1-w \leq k(m_1+m_4)^{T_{bud}/k}$ which is exponentially small in $T_{bud}$. To push $w$ down to $0$, we need $(1-f(l))\rightarrow 0$ for $l\rightarrow \infty$.

%\saeed{check if $g_l \leftarrow g_l -1 ?$ in the folloing equations}

Let us analyze $w(k,T_{bud})$

%\begin{subequations}
%\end{subequations}
	\begin{eqnarray}
	w(k,T_{bud}) &= &\nonumber
	\sum_{\substack{L,B,T s.t.\\
			k+L-B+T\leq T_{bud}-1\\
		B\leq L,B\leq k-1}}\nonumber\\& &
	{ 
		\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
				\sum_{l=1}^{L}b_l=B}}
		\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
	} \nonumber\\& &
	{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
				\sum_{l=0}^{L}g_l=k-1-B}}
		\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l}
	}\nonumber\\& &
	{\sum_{\substack{t_0,\dots,t_L s.t.\\ 
				\sum_{l=0}^{L}t_l=T}}
		\prod_{l=0}^{L} 
	 {t_l + g_l \choose g_l}m_1(l)^{t_l}(1-m_1(l))^{g_l+1}.
	 	}\label{eq.cc}\\ & &
	 \{\frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\}
\nonumber
	\end{eqnarray}
	
Notice that  $k+L-B+T \leq T_{bud}-1, B\leq L, B\leq k-1$, therefore we have
\begin{equation}\label{eq.9}
L\leq T_{bud}-1 , B\leq L, B\leq k-1, T\geq 0
\end{equation}

We define 
\begin{eqnarray}
\bar{w}(k,T_{bud}) &= &\nonumber
\sum_{L=0}^{T_{bud}-1}\sum_{B=0}^{\min{(L,k-1)}}\{\frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\}.\nonumber\\ & &	
{ \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
} \nonumber\\& &
{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g_l=k-1-B}}
	\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l} \label{eq.10}
}
\end{eqnarray}

By (\ref{eq.9}) and $\sum_{T\geq 0}{(\ref{eq.cc})}=1$,
we have $w(k,T_{bud}) \leq \bar{w}(k,T_{bud})$. 
Also notice that,  $k+L-B+T \leq T_{bud}-1, B\leq L, B\leq k-1$, 
$L+1 \leq \frac{T_{bud}}{e}$, $T\leq T_{bud}-(\frac{T_{bud}}{e})-k$,
$B\leq L$, $B\leq k-1$.
So, $w(k,T_{bud}) \geq \bar{w}(k,T_{bud}/e)$ with the sum terms multiplied with $\sum_{T=0}^{T_{bud}-(T_{bud}/e)-k}(\ref{eq.cc})$.

Remeber $e \leq T_{bud}/(L+1)$ (see line 3 of the following; also for line 5 see analysis for (\ref{eq.7}), for line 6 since $g_l \leq k-1$), so Note that 

\begin{eqnarray*}
\sum_{T=0}^{T_{bud}-(T_{bud}/e)-k}(\ref{eq.cc}) &=& 
\sum_{T=0}^{T_{bud}-(T_{bud}/e)-k}{ \sum_{\substack{t_0,\dots,t_L s.t.\\ 
			\sum t_l=T}}
	\prod_{l=0}^{L} 
	{t_l + g_l \choose g_l}m_1(l)^{t_l}(1-m_1(l))^{g_l+1}
}\\
&=& { \sum_{\substack{t_0,\dots,t_L s.t.\\ 
			\sum t_l\leq T_{bud}-(T_{bud}/e)-k}}
	\prod_{l=0}^{L} 
	{t_l + g_l \choose g_l}m_1(l)^{t_l}(1-m_1(l))^{g_l+1}
}\\
&\geq& \sum_{t_0=0}^{e-1-k}\dots\sum_{t_L=0}^{e-1-k}	\prod_{l=0}^{L} 
{t_l + g_l \choose g_l}m_1(l)^{t_l}(1-m_1(l))^{g_l+1}\\
&=& \prod_{l=0}^{L} \sum_{t_l=0}^{e-1-k} {t_l+g_l \choose g_l} m_1(l)^{t_l}(1-m_1(l))^{g_l}\\
&\geq& \prod_{l=0}^{L} \bigg( 1-(g_l+1)m_1(l)^{1+\frac{e-1-k}{1+g_l}} \bigg)\\ %see analysis for eq.7
&\geq& \prod_{l=0}^{L} \bigg( 1-(g_l+1)m_1(l)^{1+\frac{e-1-k}{k}} \bigg)\\ %g_l \leq k-1
&\geq& \prod_{l=0}^{L} \bigg( 1-k m_1(l)^{\frac{e-1}{k}} \bigg)\\ %g_l \leq k-1
&=& \prod_{l=0}^{T_{bud}/(e-1)} \bigg( 1-k m_1(l)^{\frac{e-1}{k}} \bigg)\\ 
&\geq&1- \sum_{l=0}^{T_{bud}/(e-1)}k m_1(l)^{\frac{e-1}{k}}\\
&=& 1- \sum_{l=0}^{T_{bud}/(e-1)}k [(1-\gamma)(1-(p+h)(1-f(l)))]^{\frac{e-1}{k}}\\
\end{eqnarray*}

Assuming $(1-f(l)) \rightarrow 0$ for $l \rightarrow \infty$, we can tightly lower bound this to

\begin{eqnarray*}
&\geq& 1- \sum_{l=0}^{T_{bud}/(e-1)}k (1-\gamma)^{\frac{e-1}{k}}\\
&=& 1- T_{bud}.\frac{k}{e}(1-\gamma)^{\frac{e-1}{k}}
\end{eqnarray*}
This proves that  $ \forall e, w(k,T_{bud})\geq \bar{w}(k,T_{bud}/e)(1- T_{bud}.\frac{k}{e}(1-\gamma)^{\frac{e-1}{k}})$.
 
As an example, $e= 1+ \frac{k\ln(T_{bud}.k/\epsilon)}{-\ln(1-\gamma)}$ gives $w(k,T_{bud})\geq \bar{w}(k,T_{bud}/e)(1-\epsilon)$. This shows that for an asymptotic analysis, which proves a statement like
$w(k,T_{bud}=k^{b})=p(k).\Theta(2^{-k})$ for some $p(k)\geq poly(k)$, it suffices to prove this statement for $\bar{w}$.
As we will now explain computation of $\bar{w}(k,T_{bud})$, it can be done in $\Theta(kT_{bud})$ time:

Essentially $\bar{w}(k,T_{bud})$ corresponds to Fig. \ref{fig.LthTerm} with $m_1'(l)=0,m_2'(l)=\frac{m_2(l)}{1-m_1(l)},m_3'(l)=\frac{m_3(l)}{1-m_1(l)}$, and $m_4'(l) = \frac{m_4(l)}{1-m_1(l)}$ which eliminates self-loops.

 	\begin{figure}[h!]
	\begin{center}
		\scalebox{0.40}
		{\includegraphics{SS_Tbud}}%Transf
		%		\caption{A sample path toward the winning state in which $k=18$ and the maximum level reached by the adversary is $L =22$}
		\caption{???}
		\label{fig.marten}
	\end{center}
\end{figure}


The figure shows that $\bar{w}(k,T_{bud})$ can be computed in $\Theta(kT_{bud})$ iterations. This allows fast simulation of the Markov model for various functions $(1-f(l))$, and parameters $p,\gamma$, and $h$.

In definition (\ref{eq.10}) of $\bar{w}(k,T_{bud})$ we use 

\begin{equation*}
\begin{aligned}
\frac{m_2(l)}{1-m_1(l)} &= \frac{(1-\gamma)p(1-f(l))}{\gamma+(1-\gamma)(p+h)(1-f(l))}=(1-\gamma)\alpha(l),\\
\frac{m_3(l)}{1-m_1(l)} &=  \frac{\gamma p (1-f(l))}{\gamma+(1-\gamma)(p+h)(1-f(l))} = \gamma \alpha(l),~and\\
\frac{m_4(l)}{1-m_1(l)} &= \frac{\gamma+(1-f(l))[h-\gamma(h+p)]}{\gamma+(1-\gamma)(p+h)(1-f(l))}\\
&= 1 - \frac{(1-f(l))[(1-\gamma)(p+h)-(h-\gamma(h+p))]}{\gamma+(1-\gamma)(p+h)(1-f(l))}\\
&= 1 - \frac{p(1-f(l))}{\gamma+(1-\gamma)(p+h)(1-f(l))} = 1 - \alpha(l),
\end{aligned}
\end{equation*}
where $\alpha(l) = \frac{p(1-f(l))}{\gamma+(1-\gamma)(p+h)(1-f(l))}$. The above form can be used in a dynamic program which takes $\alpha(l)$ as input rather than the separate $f(l),p,h,$ and $\gamma$. 

Notice that 
\begin{equation*}
\frac{m_2(l)}{1-m_1(l)} \leq \frac{(1-\gamma)pd}{\gamma} (\frac{1-f(l)}{d}) \leq \frac{(1-\gamma)pd}{\gamma} \sqrt{\frac{1-f(l)}{d}}
\end{equation*}

for $d$ such that $\forall l, (1-f(l))\leq d$.
Also,
\begin{equation*}
\begin{aligned}
\frac{m_3(l)}{1-m_1(l)} \leq  pd \sqrt{\frac{1-f(l)}{d}}^2, ~ and\\
\frac{m_4(l)}{1-m_1(l)} \leq 1- pd \sqrt{\frac{1-f(l)}{d}}^2.
\end{aligned}
\end{equation*}

We define $\beta_(l) = \sqrt{\frac{1-f(l)}{d}}$ and upperbound (\ref{eq.10}) as follows:

\begin{eqnarray*}
\bar{w}(k,T_{bud}) &\leq &\nonumber
\sum_{L=0}^{T_{bud}-1}\sum_{B=0}^{\min{(L,k-1)}} (1+ \frac{1-\gamma}{\gamma})pd \beta(L)^2\\ & &	
{ \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}pd \beta(l)^2 + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
} \nonumber\\& &
{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g_l=k-1-B}}
	\prod_{l=0}^{L} \bigg(\frac{1-\gamma}{\gamma} pd \beta(l)\bigg)^{g_l} 
}
\end{eqnarray*}

\saeed{From Marten's notes: Notice that this bounding eliminates the role of h. Simulations are needed to find out the effect of $h$.}

Define $\theta \geq \frac{1-\gamma}{\gamma}$. Considering that $\sum{b_l}=B$ (for line 3 of the following) and by defining $b_{L+1}=0$ (for line 2) we have,

\begin{eqnarray*}
	{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
				\sum_{l=0}^{L}g_l=k-1-B}}
		\prod_{l=0}^{L} \bigg(\frac{1-\gamma}{\gamma} pd \beta(l)\bigg)^{g_l} 
	} &\leq &
	{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g_l=k-1-B}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{g_l} 
} \\
&\leq &
	{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g_l=k-1-B}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{g_l + b_{l+1}}\prod_{l=0}^{L-1} \bigg(\theta pd \beta(l)\bigg)^{-b_{l+1}}
} \\
&\leq &
	{	\sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g'_l=k-1}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{g'_l}\prod_{l=0}^{L-1} \bigg(\theta pd \beta(l)\bigg)^{-b_{l+1}}
} \\
&=& (\theta p d )^{k-1}{\sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g'_l=k-1}}
	\prod_{l=0}^{L} \beta(l)^{g'_l}\prod_{l=0}^{L-1} \bigg(\theta pd \beta(l)\bigg)^{-b_{l+1}}
} \\
\end{eqnarray*}

We derive


\begin{eqnarray*}
& & \sum_{B=0}^{L}{ \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}pd \beta(l)^2 + (1-b_{l+1})(1-pd \beta(l)^2) \bigg) \prod_{l=0}^{L-1} \bigg(\theta pd \beta(l)\bigg)^{-b_{l+1}}
} \\
&= &\sum_{B=0}^{L}{ \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{\beta(l)}{\theta} + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
} \\
&= &  	\prod_{l=0}^{L-1} \bigg( \frac{\beta(l)}{\theta} + (1-pd \beta(l)^2) \bigg)\\
&= & 	\prod_{l=0}^{L-1} \bigg( 1+\beta(l) (\frac{1}{\theta} - pd \beta(l)) \bigg)\\
&\leq &  	\prod_{l=0}^{L-1} \bigg( 1+\beta(l)/\theta \bigg)
\end{eqnarray*}

We also derive that 

\begin{eqnarray*}
{	\sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
				\sum_{l=0}^{L}g'_l=k-1}}
		\prod_{l=0}^{L} \beta(l)^{g'_l}
	}
&= & {	\sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g'_l=k-1}}
	\prod_{l=0}^{L} \bigg( c_l \beta(l)^{g'_l} + (1-c_l) \bigg)
}\\
&\leq & {	\sum_{\substack{c_0,\dots,c_L\in \{0,1\} 1 s.t.\\ 
			\sum_{l=0}^{L}(c_l)=k-1}}
	\prod_{l=0}^{L} \bigg( c_l \sum_{g=1}^{\infty}{\beta(l)^{g}} + (1-c_l) \bigg)
}\\
&= & {	\sum_{\substack{c_0,\dots,c_L\in \{0,1\} 1 s.t.\\ 
			\sum_{l=0}^{L} c_l=k-1}}
	\prod_{l=0}^{L} \bigg( c_l \frac{\beta(l)}{1-\beta(l)} + (1-c_l) \bigg)
}\\
&\leq & \prod_{l=0}^{L} \bigg( \frac{\beta(l)}{1-\beta(l)} + 1 \bigg) = \prod_{l=0}^{L} \bigg( \frac{1}{1-\beta(l)}\bigg)
\end{eqnarray*}
where $c_l =1$ if $g'_l \neq 0 $ and $c_l =0$ if $g'_l = 0$.

Combining all the equations gives for $\frac{1-\gamma}{\gamma} \leq \theta$ and $\frac{1-f(l)}{d} = \beta(l) < 1$,

\begin{eqnarray*}
	\bar{w}(k,T_{bud}) &\leq &\nonumber
	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k}(1+\frac{1}{\theta})\frac{\beta(L)^2}{1-\beta(L)}\prod_{l=0}^{L-1} \frac{(1+\beta(l)/\theta)}{(1-\beta(l))}\\
	&\leq&  	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k}(1+\frac{1}{\theta})\prod_{l=0}^{L-1} \frac{(1+\beta(l)/\theta)}{(1-\beta(l))}\\
\end{eqnarray*}
We derive:

\begin{eqnarray*}
\prod_{l=0}^{L-1} \frac{(1+\beta(l)/\theta)}{(1-\beta(l))} &=& \sum_{l=0}^{L}[1+(1+\frac{1}{\theta})\frac{\beta(l)}{1-\beta(l)}]
\end{eqnarray*}

%\lemma{ $\prod_{a=0}^{A}(1+yB'(a)) \leq e^{y[B'(0)-B(0)+B(A-1)}$ for $B'(a)\geq 0$ and $B''(a)\leq 0$}
%\proof

\begin{lemma}\label{lemma.diri}
$\prod_{a=0}^{A}(1+yB'(a)) \leq e^{y[B'(0)-B(0)+B(A-1)]}$ for $B'(a)\geq 0$ and $B''(a)\leq 0$.
\end{lemma}
\begin{proof}
We find an upperbound of $\ln \prod_{a=0}^{A}(1+yB'(a)) = \sum_{a=0}^{A}\ln(1+yB'(a))$. Differentiating w.r.t. $y$ gives
\begin{eqnarray*}
	\sum_{a=0}^{A} \frac{1}{1+yB'(a)}. B'(a) &\leq& \sum_{a=0}^{A}B'(a) = B'(0)+\sum_{a=1}^{A}B'(a)\\
	&\leq& B'(0) + \int_{a=0}^{A-1} B'(a) da\\
	&=& B'(0) + B(A-1) - B(0)
\end{eqnarray*}
Also $\sum_{a=0}^{A}\ln(1+yB'(a))|_{y=0}=0=y.[B'(0)-B(0)+B(A-1)]|_{y=0}$. We conclude that $\sum_{a=0}^{A}\ln(1+yB'(a)) \leq y.[B'(0)-B(0)+B(A-1)]$. \qed
\end{proof}

We get:
\begin{eqnarray*}
	\bar{w}(k,T_{bud}) &\leq&
	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k}(1+\frac{1}{\theta}). e^{(\frac{1+\theta}{\theta})(B(L-1)+C)} \\
	&\leq& [\theta p d]^{k}(1+\frac{1}{\theta})e^{(\frac{1+\theta}{\theta})(B(T_{bud})+C)}. T_{bud}
\end{eqnarray*}
where, $C = B'(0)-B(0)$ and $\frac{\mathrm{d}B(x)}{\mathrm{d}x}=\frac{\beta(x)}{1-\beta(x)}$. Notice that the conditions of the lemma \ref{lemma.diri} are satisfied for a decreasing $\beta(x) = \sqrt{\frac{a-f(x)}{d}} \leq 1$.

Minimizing this upperbound with respect to $\theta \geq (1-\gamma)/\gamma$:

\begin{equation*}
\theta^{k} e^{(1/\theta).B[T_{bud}]} = e^{[k\ln{\theta}]+B[T_{bud}]/\theta}
\end{equation*}

Differentiating $k\ln{\theta} + B[T_{bud}]/\theta$ with respect to $\theta$:
\begin{equation*}
\frac{k}{\theta} - \frac{B[T_{bud}]}{\theta^2} = 0 \implies \theta = \frac{B[T_{bud}]}{k}
\end{equation*}

We obtain 

\begin{align}\label{eq.conditions}
\bar{w}(k,T_{bud}) \leq
\begin{cases}
[pd]^{k}e^{k\ln(\frac{B[T_{bud}]}{k})+k+B[T_{bud}]+kC/B[T_{bud}]+C}, & \text{if}\ B[T_{bud}]\geq \frac{k(1-\gamma)}{\gamma} \\
[\frac{1-\gamma}{\gamma}pd]^{k}\frac{1}{1-\gamma}e^{(B[T_{bud}]+d)/(1-\gamma)}.T_{bud}, & \text{otherwise}
\end{cases}
\end{align}


%\begin{numcases}{$\bar{w}(k,T_{bud}) \leq$}
%	$[pd]^{k}e^{k\ln(\frac{B[T_{bud}]}{k})+k+B[T_{bud}]+kC/B[T_{bud}]+C}$, & if $B[T_{bud}]\geq \frac{k(1-\gamma)}{\gamma}$\\
%	$[\frac{1-\gamma}{\gamma}pd]^{k}\frac{1}{1-\gamma}e^{(B[T_{bud}]+d)/(1-\gamma)}.T_{bud}$, & otherwise
%\end{numcases}


For $\gamma$ not too small $k(1-\gamma)/\gamma$ is a function of k. Usually $(1-f(l))$ is designed such that $B[T_{bud}] = \Theta (\ln T_{bud})$ in which case $B[T_{bud}]\geq \frac{k(1-\gamma)}{\gamma}$ for $T_{bud}$ exponentially large in $k$. 
This means that in general, we only need to consider the second condition of (\ref{eq.conditions}) i.e., $B[T_{bud}] < \frac{k(1-\gamma)}{\gamma}$.

As an example, assume that $\frac{\beta(l)}{1-\beta(l)} \leq \frac{1}{l}$, then $B(T_{bud}) = \ln(T_{bud})$ and
$\bar{w}(k,T_{bud}) \leq (\frac{1-\gamma}{\gamma}pd)^{k}\frac{1}{1-\gamma}e^{C/(1-\gamma)}T_{bud}^{1+1/(1-\gamma)}$, for $T_{bud} \leq e^{k(1-\gamma)/\gamma}$. The probability of winning for the adversary is exponentially small in $k$.

\begin{equation*}
\frac{\beta(l)}{1-\beta(l)} \leq \frac{1}{l} \iff \beta(l) \leq \frac{1}{l+1} \iff \sqrt{\frac{1-f(l)}{d}} \leq \frac{1}{l+1} \iff 1-f(l) \leq \frac{d}{(l+1)^2}
\end{equation*}

\saeed{From Marten notes: Still wish to do additional induction proof for $p(k,lT_{bud})$ Exercise for me!}

\saeed{analysis 5 starts here}

In practice, we may not immediately start learning at a rate $(1-f(l)) \approx d/(l+1)^2$. This will only happen after reaching for example $L^*$ samples. During such a first phase $(1-f(l)) \approxeq 1$ and the adversary tries to compromise as many, say $k^*$, nodes as possible before reaching $L^*$ levels.

For $(1-f(l)) \approxeq 1$, we have:


\begin{equation*}
\begin{aligned}
m_1(l) &= (1-\gamma)(1-(p+h))\\ 
m_2(l) &= (1-\gamma)p\\
m_3(l) &= \gamma p\\
m_4(l) &= [h-\gamma(h+p)]+\gamma=(1-\gamma)h+\gamma(1-p)\\
\end{aligned}
\end{equation*}

We are interested in $k^*$ as a function of $\epsilon$ for which 
\begin{eqnarray}\label{eq.k}
\sum_{k=0}^{k^{*}-1} p(k,L^{*}-1,T_{bud}-1)(\frac{m_4(l)}{1-m_1(l)}+\frac{m_3(l)}{1-m_1(l)}) +\\ p(k^*,L^{*}-1,T_{bud}-1)\frac{m_4(l)}{1-m_1(l)} \geq 1- \epsilon \nonumber
\end{eqnarray}

Then the probability of winning is 
\begin{equation}\label{eq.deta}
\leq \epsilon + (1-\epsilon)w(k-k^{*}(\epsilon),T_{bud})
\end{equation}

Notice that during phase one an $i>k^{*}(\epsilon)$  is reached ($\epsilon$ term in the above formula) and during phase two, another $k-k^{*}(\epsilon)$ horizontal or diagonal moves are needed in order to win (the second term).

We generalize the analysis of (\ref{eq.6}) for $(1-f(l))=1$ (without any constraint on $T_{bud}$):

\begin{eqnarray}\label{eq.delta}
(\ref{eq.k}) = \sum_{B=0}^{\infty}\sum_{k=B+1}^{k^{*}-1}(\ref{eq.a})(\ref{eq.b})(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)}) 
\end{eqnarray}

\saeed{Check \ref{eq.a} I guess the above should be L not l}
Notice that 

\begin{eqnarray*}
	\sum_{k=B+1}^{k^{*}-1}(\ref{eq.b}) &=& 
	\sum_{k=B+1}^{k^{*}-1}
		{	\sum_{\substack{g_0\geq 1,\dots,g_L^{*}\geq 1 s.t.\\
				\sum_{l=0}^{L^{*}}(g_l-1)=k-1-B}}
		\prod_{l=0}^{L^{*}} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
	}\\
	&=& \sum_{\substack{g'_0,\dots,g'_{L^*}\geq 0 s.t.\\
		\sum_{l=0}^{L^*-1}{g'_l \leq k^*-2-B}}}\prod_{l=0}^{L^*} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l}\\
	&\geq& \sum_{g'_0=0}^{(k^*-2-B)/L^*+1} \dots \sum_{g'_{L^*}=0}^{(k^*-2-B)/L^*+1} (\prod \dots)\\
	&=&  \prod_{l=0}^{L^*} \sum_{g'_l\geq 0}^{(k^*-2-B)/L^*+1}\bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l} \\
	&=&	 \prod_{l=0}^{L^*}\frac{1}{1-\frac{m_2(l)}{1-m_1(l)}}\big(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \big)^{L^*+1} \\
	&=& \prod_{l=0}^{L^*} \frac{1-m_1(l)}{1-m_1(l)-m_2(l)}\bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \bigg)^{L^*+1}\\
	&=& \prod_{l=0}^{L^*} \frac{1-m_1(l)}{m_3(l)+m_4(l)}\bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \bigg)^{L^*+1}
\end{eqnarray*}

\saeed{Missing part from the notes: Since $B\leq L^* \geq \bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-1}{L^*+1}}\bigg)^{L^*+1}$}

And 

\begin{eqnarray*}
	\lefteqn{\sum_{B=0}^{\infty}(\ref{eq.a})(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)}) =} \\ & & 
	{ \sum_{\substack{b_1,\dots,b_L^*\in\{0,1\} s.t.\\ 
				\sum_{l=1}^{L^*}b_l=B}}
		\prod_{l=0}^{L^*-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)  (\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})}\\
& =&	{ \sum_{b_1,\dots,b_L^*\in\{0,1\}}\prod_{l=0}^{L^*-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})
}\\
&=&\prod_{l=0}^{L^*}(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})
\end{eqnarray*}

\saeed{Note From Marten's: In the write up we can refer in parts to the analysis of \ref{eq.6} in order to save space}

So we get 
\begin{eqnarray*}
(\ref{eq.k}) &\geq& \bigg(1-(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}} \bigg)^{L^*+1}\\
&\geq& 1 - (L^*+1)(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}}
\end{eqnarray*}

We want to solve $L\geq 1-\epsilon$

\begin{equation}\label{eq.star}
(L^*+1)(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}} = (L^*+1)[\frac{(1-\gamma)p}{1-(1-\gamma)(1-(p+h))}]^{\frac{k^*-1}{L^*+1}} \leq \epsilon
\end{equation}

Notice that $p \leq 1-h$, we have:
\begin{equation}
[\frac{(1-\gamma)p}{1-(1-\gamma)(1-(p+h))}] \leq (1-\gamma)(1-h).
\end{equation}

So, Equation (\ref{eq.star}) is satisfied for $k^*$ such that 

\begin{equation}
(L^*+1)[(1-\gamma)(1-h)]^{\frac{k^*-1}{L^*+1}} \leq \epsilon.
\end{equation}

\saeed{check equation delta \ref{eq.delta} reference, there are two of them deta and delta!}

Applying (\ref{eq.delta}) gives
probability of winning for 
\begin{equation*}
1-\tilde{f}(l)=\begin{cases}
1, & \text{if $l<L^*$}.\\
1-f(l-L^*), & \text{if $l \geq L^*$}.
\end{cases}
\end{equation*}
is 
\begin{equation}\label{eq.delta.1}
\leq (L^*+1)[(1-\gamma)(1-h)]^{\frac{k^*-1}{L^*+1}} + \bar{w}(k-k^*,T_{bud}), 
\end{equation}

where $\bar{w}$ can be computed through simulation or $\bar{w}$ has the special form as derived for $(1-f(x)) = \frac{d}{(1+x)^2}$.

We want to minimize Equation \ref{eq.delta.1} for $k^*$.
\saeed{Note: Need to do this}
This shows how $h$ plays a role as wel!? It is important in phase one.

We get some function $g(k,T_{bud})\geq Prob(win)$.


\subsection{Security Capacity}

$T_{bud} \leq 2^t$, and $Prob(win) \leq 2^{-s}$ is implied by $\hat{g}(k,2^t) \leq 2^{-s}$. After taking the logarithm in base 2 we get
\begin{eqnarray} \label{eq.secCap}
s \leq -\log\hat{g}(k,2^t)
\end{eqnarray}

We need to figure out what equation \ref{eq.delta.1} gives.
\ref{??} should lead to a bound of the form $\delta . s + \eta t \leq g(k,t)$, where $g(k,t)= \Theta(k)$ behaving like $\zeta k $ for large $k$.

Then, the triples $(\delta , \eta , \zeta)$ defines a \emph{security capacity region}:

For $T_{bud} \leq 2^t$ the probability of reaching state $k$ is at most $2^{-s}$ if $\delta s + \eta t \leq g(k,t) \approx \zeta k$.

We can show in a paths (graphs?) how this behaves for several parameter settings (our simulations etc)
\saeed{can we compute actually examples?}

Take $s=t=128$ For different $p,\gamma,h$ we can plot for which minimal $k$ the above bound holds. Larger $k$ cannot be achieved in $2^{128}$ time budget and winning prob $\geq 2^{-128}$!

\saeed{General lemma: Nice for eprint: we donot make use of it in our bounds}

\textbf{Composition}

Suppose for fixed $h,p,\gamma$ we have:
$s+t \leq g_1(k,t)$ for $f_1(l)$, assume $g_1(k,t)$ is an increasing function,
$s+t \leq g_2(k,t)$ for $f_2(l+L^*)$ (we start at level $L^*$ rather than $0$), assume $g_2(k,t)$ is an increasing function.

Let 

\begin{equation*}
f(l)=\begin{cases}
f_1(l), & \text{if $l \leq L^*$}.\\
f_2(l), & \text{if $l > L^*$}.
\end{cases}
\end{equation*}

Given $2^t$ timesteps then with $prob \leq 2^{-s}$ we achieve $k$, for $s+t \leq g_1(k)$ or $g_1^{-1}(s+t) \leq k_1$ if we use $f_1(l)$.
So within $2^t$ timesteps before $l=L^*$ is reached (another restriction) we have with $prob \leq 2^{-s}$ we achieve $k_1 = g_1^{-1}(s+t)$,
or with $prob \geq (1-2^{-s})$ we have $k_1 \leq g_1^{-1}(s+t)$.
We give the adversary an advantage with $prob\geq (1-2^{-s})$, if we upgrade him to position $k_1= g_1^{-1}(s+t)$ once $L^*$ is achieved. And we again give him $2^t$ timesteps. Now $f_2(l+L^*)$ is being used for $l\geq 0$. With $prob \leq 2^{-s}$ another 
$k_2 \geq g_2^{-1}(s+t)$ positions are gained.

So, given  $2^t$ time steps, with $prob \leq 2^{-s} + 2^{-s} = 2^{-(s-1)}$, $k \geq g_1{-1}(s+t) + g_2{-1}(s+t)$ is reached.
Define $g(g_1{-1}(s+t)+g_2^{-1}(s+t)) = s+ t$. Then for $f(l): s'+t \leq g(k) -1$ where $s'=s-1$. 
The above shows how $(1-f_1(l)) \leq d/l$ for $l \leq L^*$ and $\tau_{low} \leq 1-f_2(l) \leq \tau_{up} < 1$ for $l > L^*$ compose.
Note that this also holds for $(1-f_2(l+L^*))$, independent of the level.

So we have $s+t \leq g_1(k)$ of Th1 and $s+t \leq g_2(k)$ of Th2.
\saeed{Th? Theorem 1 and 2?}

and we obtain for the composed $f$:
$s+t \leq g(k) -1$, where $g^{-1}(x) = g_1^{-1}(x) + g_2^{-1}(x)$.

Assymptotics: $g_1(k) \sim \alpha_1.k$ and $g_2(k) \sim \alpha_2.k$, therefore, $g(k) = \frac{\alpha_1 \alpha_2}{\alpha_1 + \alpha_2}.k$ worse than $g_2(k)$: $1-f(l) \geq 1-f_2(l)$ for $l \leq L^*$, so $f$ is worse than $f_2$!

In our (???) case $\alpha_1 \gg \alpha_2$ we get $g(k) \sim \alpha_2 k$. Hence, the effect of $f_2(l)$ really matters. It does not matter how one learns $ \tau_{low} \leq (1-f_2(l)) \leq \tau_{up}$ after $L^*$ levels.


\textbf{Important for eprint/paper:}
Rate of play:
Suppose $s+t \leq g(k)$. Suppose 1 adversarial move (i.e., one transition in the Markov model) takes $\Delta$ time. Suppose we have $T$ time step budget. If $k$ nodes are infected after $T$ time, then at most $\frac{T}{\Delta k}$ moves have been made.
If $s + \log(\frac{T}{\Delta k}) \leq g(k)$, then with probbaility $\leq 2^{-s}$ state $k$ is reached. Hence, $s+ t' \leq g(k) + \log k$ gives $prob_{win} \leq 2^{-s}$ where $t' = \log(\frac{T}{\Delta})$.

Notice if the time budget $T \leq \Delta. 2^{t'}$, then with $prob \leq 2^{-s}$, a state $k$ with $s+t' \leq g(k) + \log k$ can be reached.
Now if $g(k) = \Theta(k)$, then we get pretty much the same secrecy capacity. So ``real time with parallel adversarial moves" can be interchanged with ``Total number of moves/transition steps/time steps" good news!

\saeed{Analysis 6 starts from here: Sort of TODS and FUTURE WORKS}

1 - Given a model on rate of adversarial play (see also $T_{bud} \rightleftarrows time$ analysis, can a defender estimate how many nodes have been compromised given when $l$ got incremented?

We can estimate function $1-f(l)$ and extrapolate; leads to a bound on reaching $k$.
This could be very helpful. The defender knows when to invest resources w.r.t. a certain type of attack in order to get a better curve for $1-f(l)$!?

2 - Given our Markov model, suppose the defender can prove that he invest resources to reach a certain $1-f(l),h,\gamma$. Then the adversary believes in the bound dictated by the secrecy capacity and will be discuraged to move at all (econimically motivated adversay). How do we design such a proof.

3 -  FlipIt: Show the equilibrium game and also analyze how both parties can profit more if D can prove its strategy to A.

In general, can 2kp be used to change games for mutual additional gain?
(Did Micali do this stuff? Prof at CSAIL? Silvio Micali? )

4 - Current paper and TODO 1 can lead to a webtool? What about other Markov models and their analysis?

5 - Cheers!
%\begin{eqnarray} \label{eq.w}
%&=&	\sum_{L=0}^{w(k,T_{bud})} p(k-1,L,T_{bud}-1).	 [\frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}]\\
%\end{eqnarray}


% \RandomWalk {number = 50,length = 4pt, angles = {0,45,90}, degree}
 
 
%The winning state for the adversary is state $k \ll K$. 
%\saeed{Missing: a Figure for sample path l based on i} 
%
%Suppose we arrived at level $l$ in state $i_l$. Suppose we enter at level $l+1$ in state $i_{l+1}$.
%
%\textbf{Case 1: $i_{l+1}=i_l$} Lets denote the number of times the adversary stays in state $(i_l,l)$ by $T_l$ and after that it makes a transition to the state $(i_{l+1}=i_l,l+1)$. This can happen in $T_{l}+1$ time steps with probability $m_1(l)^{T_l}. m_4(l)$
%
%\textbf{Case 2: $i_{l+1}>i_l$} \\
%\textit{(2-a):}
%Consider the following sample path which can happen in $T_{l}+i_{l+1}-i_{l}+1$ time steps with probability $m_1(l)^{T_l}.m_2(l)^{i_{l+1}-i_{l}} .m_4(l)$ where $T_l = t(i_l)+\dots+t(i_{l+1})$.
%\saeed{Missing: a Figure for sample path l based on i} 
%
%\textit{(2-b):}
%Consider the following sample path which can happen in $T_{l}+i_{l+1}-i_{l}$ time steps with probability $m_1(l)^{T_l}.m_2(l)^{i_{l+1}-1-i_{l}} .m_3(l)$ where $T_l = t(i_l)+\dots+t(i_{l+1})$.
%\saeed{Missing: a Figure for sample path l based on i} 
%
%\textbf{Case 3: We have arrived at the highest level $L$ before entering the winning state $(i_L < k)$:} \\
%\textit{(3-a):}
%Define $T_L = t(i_L)+\dots+t(k-1)$
%This sample path happens with probability $m_1(L)^{T_L}.m_2(L)^{k-i_L}$ in $T_L+k-i_L$ time steps.\\
%\textit{(3-b):}
%Define $T_L = t(i_L)+\dots+t(k-1)$
%This sample path happens with probability $m_1(L)^{T_L}.m_2(L)^{k-1-i_L}m_3(L)$ in $T_L+k-i_L$ time steps.\\
%
%Path towards a winning state:
%$0=i_1 \leq i_2 \leq \dots \leq i_L <k$
%We use the following notaion:
%$0=j_1 \leq j_2 \leq \dots \leq i_R <k$,
%$\sum_{n=1}^{R} r_n = L$ with $r_1,\dots,r_R \geq 1$. Therefore,\\
%$j_1=(0=i_1=\dots=i_{r_1}) < j_2 =(i_{r_1+1}=\dots=i_{r_1+r_2}) < j_3 = (i_{r_1+r_2+1}=\dots=i_{r_1+r_2+r_3}) < \dots$





%We prove Theorem \ref{Theorem.Cost}:
% Let $A_{i,j}$ represent the probability the adversary moves in state $i$ and reaches state $j$ as a consequence of the move. Let the real number $c_{i,j}\geq 0$ indicate the adversarial cost associated to $A_{i,j}$. Then 
%\begin{equation}\label{eq.rho}
%\alpha = \sum_{i,j}{\pi_i  A_{i,j}  c_{i,j}}  
%\end{equation}
% is a convex combination of costs $c_{i,j}$ (since $\sum_{i,j} \pi_i  A_{i,j} \leq \sum_{i,j} \pi_i  M_{i,j}= \sum_j \pi_j =1$). We need to prove that
%the probability  the attacker wins the $M$-MTD game by paying at most $C$ is
%	$$\leq \frac{C\cdot \pi_{k}}{\sum_{i,j}{\pi_i  A_{i,j}  c_{i,j}} }. $$
%
%
%	We first introduce a mapping of matrix $M$ to a new matrix $M^{*}$ which we can analyze using our theorem but has all the necessary cost information embedded:
%	
%	First, we split each transition from state $i$ to state $j$ with probability $M_{i,j}$ into two transitions. One from $i$ to $j$ with probability $A_{i,j}$ and the other from $i$ to $j$ with probability $D_{i,j}=M_{i,j}-A_{i,j}$: $A_{i,j}$ represents the probability that the adversary moves in state $i$ and reaches state $j$ as a consequence of that move, while $D_{i,j}$ represents the probability of a defender's move or no move (if $i=j$) from state $i$ to state $j$.
%	
%	Second, let $c_{i,j}\geq 0$ be a real number representing the cost for the adversary if he moves from $i$ to $j$ with probability $A_{i,j}$. Let $\epsilon \geq 0$ (later in the proof we will take the limit $\epsilon \rightarrow 0$) and define	
%	\begin{equation*} \label{eq.Int.Cost}
%	C_{i,j} = \lceil \frac {c_{i,j}}{\epsilon} \rceil \in \mathbb{N}
%	\end{equation*}
%	
%	We transform each edge from $i\rightarrow j$ with probability $A_{i,j}$ into a path $i\rightarrow (i,j;1)\rightarrow (i,j;2)\rightarrow \ldots \rightarrow (i,j;C_{i,j})\rightarrow j$ with probabilities as depicted in Figure~\ref{fig.Transfer}. The transition  $i\rightarrow (i,j;1)$ has probability $A_{i,j}$. If $C_{i,j}=0$, then $i$ is directly connected to $j$ without intermediary nodes and $i\rightarrow j$ is transitioned with probability $A_{i,j}$ by the adversary. We denote the transformed matrix by $M^{*}$.
%	
%	
%	\begin{figure}[h!]
%		\begin{center}
%			\scalebox{0.60}
%			{\includegraphics{Transf2.pdf}}%Transf
%			\caption{Each transition $M_{i,j}$ from $i\rightarrow j$ will be replaced with above transition from state $i$ to $j$}
%			\label{fig.Transfer}
%		\end{center}
%	\end{figure}
%	
%	
%	
%	\begin{lemma} \label{lem:cost} If $M$ has an stationary probability distribution $\pi$, then $M^{*}$ has an stationary distribution $\pi^{*}$ defined by:
%		\begin{eqnarray}
%		\pi^{*}_{i}&=&\frac{\pi_{i}}{1+\alpha} \mbox{ and } \nonumber \\ %\label{eq.piStar}\\ 
%		\pi^{*}_{i,j;h}&=&\frac{\pi_{i} \cdot A_{i,j}}{1+\alpha} \mbox{ for } 1\leq h \leq C_{i,j}.	\nonumber
%		\end{eqnarray}
%	\end{lemma}
%	
%	
%	\noindent
%	{\bf Proof.} From $\pi^{*}=\pi^{*} M^{*}$ and the definition of $M^{*}$ we infer the following equations:
%	\begin{eqnarray*}
%		\pi^{*}_{i,j;1}&=&{\pi^{*}_{i}}\cdot A_{i,j}, \hspace{1cm} \mbox{    if } C_{i,j}\geq 1, \\  	
%		\pi^{*}_{i,j;h+1}&=&\pi^{*}_{i,j;h}, \hspace{1.3cm} \mbox{         for } 1\leq h \leq C_{i,j},  	\\
%		%\begin{equation}
%		\pi^{*}_{j} &=& \sum_{i} \pi^{*}_i D_{i,j} + \sum_{\substack{i \\ C_{i,j}\neq 0}} \pi^{*}_{i,j;C_{i,j}} + \sum_{\substack{i \\ C_{i,j}= 0}} {\pi^{*}_{i}}\cdot A_{i,j}.
%		%\end{equation}
%	\end{eqnarray*}
%	By combining the above equations we have,
%	\begin{eqnarray*}
%		\pi^{*}_{j}&=& \sum_{i} \pi^{*}_i D_{i,j} + \sum_{\substack{i \\ C_{i,j}\neq 0}} \pi^{*}_{i,j;1} + \sum_{\substack{i \\ C_{i,j}= 0}} {\pi^{*}_{i}}\cdot A_{i,j}\\
%		&=& \sum_{i} \pi^{*}_i D_{i,j} + \sum_{\substack{i}} {\pi^{*}_{i}}\cdot A_{i,j}
%		= \sum_{i} \pi^{*}_i M_{i,j}
%	\end{eqnarray*}
%	We conclude that the vector $(\pi^{*}_1,\pi^{*}_2,...)$ is proportional to vector $\pi$ and this proves $\pi^*_i=\pi_i/\rho$ for some $\rho$. 
%	%the form of (\ref{eq.piStar}).
%	As a result
%	$$
%	\pi^{*}_{i,j;h}= \pi^{*}_{i,j;1}= \pi^{*}_i \cdot A_{i,j} = \frac {\pi_i \cdot A_{i,j}}{\rho}  \mbox{ for } 1\leq h \leq C_{i,j}.
%	$$
%	
%	The proportionality factor $\rho$ satisfies
%	\begin{eqnarray*}
%		1&=& \sum_{i}{\pi^{*}_i} + \sum_{\substack{i,j,h \\ C_{i,j}\neq 0\\1\leq h \leq C_{i,j}}} {\pi^{*}_{i,j;h}} \\
%		&=& \sum_{i}{\frac{\pi_i}{\rho}} + \sum_{\substack{i,j,h \\ C_{i,j}\neq 0\\1\leq h \leq C_{i,j}}}{\frac {\pi_i \cdot A_{i,j}}{\rho}} \\
%		&=& \sum_{i} \frac{\pi_i}{\rho} + \sum_{i,j}{\frac{\pi_i \cdot A_{i,j} \cdot C_{i,j}}{\rho}}
%	\end{eqnarray*}
%	Together with $\sum_{i} {\pi_i}=1$ and (\ref{eq.rho}), this proves $\rho=1+\alpha$  and the lemma follows.
%	
%	In order to prove the theorem we introduce new random variables:
%	%
%	Let $T_{M}$ be the random variable indicating the number of transitions $i\xrightarrow{D_{i,j}}j$, $i\xrightarrow{A_{i,j}}(i,j;1)$ (if $C_{i,j}\geq 1$) and $i\xrightarrow{A_{i,j}}j$ (if $C_{i;j}=0$), made before the adversary wins the MTD-game corresponding to $M^{*}$. 
%	
%	Let $T_{C}=\sum_{i,j}{N_{i,j}\cdot C_{i,j}}$ be the random variable indicating the number of all other transitions where $N_{i,j}$ represents the random variable counting the number of times the path$(i,j;1)\xrightarrow{1}(i,j;2)\xrightarrow{1}\ldots\xrightarrow{1}(i,j;C_{i,j})$ is traversed.
%	Notice that $T=T_M + \sum_{i,j}{N_{i,j}}$ is the random variable representing the number of transitions in the $M$-MTD game before the attacker wins the game.
%	
%	Let the random variable $C_R$ represent the real cost of the adversary before he wins the MTD-game corresponding to $M$. Notice that,  for  random variables $N_{i,j}$ in the MTD-game corresponding to $M^{*}$,
%%	\begin{eqnarray}
%$$	C_R = \sum_{i,j}{N_{i,j}\cdot c_{i,j}}. $$
%%	\end{eqnarray}
%	This  shows how the MTD games based on $M$ and $M^*$ are related.
%	
%	We derive
%	\begin{eqnarray}
%	T_C &=& \sum_{i,j}{N_{i,j}\cdot C_{i,j}} = \sum_{i,j}{N_{i,j}\cdot \lceil \frac{c_{i,j}}{\epsilon} \rceil} \nonumber \\
%	&=& \frac{1}{\epsilon} \sum_{i,j}{N_{i,j}\cdot (\lceil  \frac{c_{i,j}}{\epsilon} \rceil \cdot \epsilon )} \nonumber \\
%	&=& \frac{1}{\epsilon} \sum_{i,j}{N_{i,j}\cdot c_{i,j}} + \frac{1}{\epsilon} \sum_{i,j}{N_{i,j}\cdot (\lceil \frac{c_{i,j}}{\epsilon} \rceil \cdot \epsilon - c_{i,j})} \nonumber \\
%	&=& \frac{C_R}{\epsilon} + E 
%	\mbox{ where } 
%	0\leq E \leq \sum_{i,j}{N_{i,j}} \label{eq.error}
%	\end{eqnarray}
%	
%	Since $T=T_M + \sum_{i,j}{N_{i,j}}$ represents the number of transitions in the $M$-MTD game before the attacker wins the game, we can use Theorem \ref{theo-single} in combination with (\ref{eq.error}) and derive for all $t$:
%	\begin{eqnarray}
%	&& \frac{C\cdot \pi^*_{k}}{\epsilon}  \label{Eq.c} \\
%	&\geq & Prob(T_M+T_C \leq \frac {C}{\epsilon}) 
%	= Prob(T_M+\frac{C_R}{\epsilon}+E \leq \frac {C}{\epsilon}) \nonumber \\
%	&=& Prob(C_R\leq C-\epsilon(T_M+E)) \nonumber \\
%	&\geq&Prob(C_R\leq C-\epsilon t | T_M+E\leq t)Prob(T_M+E\leq t) \nonumber \\
%	&=&Prob(C_R\leq C-\epsilon t)- \nonumber \\& &
%	Prob(C_R\leq C-\epsilon t | T_M+E \geq t)Prob(T_M+E \geq t) \nonumber \\
%	&\geq&Prob(C_R\leq C-\epsilon t) - Prob(T_M+E\geq t) \nonumber \\
%	&\geq&Prob(C_R\leq C-\epsilon t) - Prob(T_M+ \sum_{i,j}{N_{i,j}}\geq t) \nonumber \\
%	&=& Prob(C_R\leq C-\epsilon t) - Prob(T\geq t). \label{Eq.5}
%	\end{eqnarray}
%	If we choose $\epsilon=\frac{1}{t^{2}}$ and let $t\rightarrow \infty$ then (\ref{Eq.5}) tends to $Prob(C_R \leq C)$.
%	
%	We now analyse upper bound (\ref{Eq.c}) by using Lemma \ref{lem:cost}:
%	$$
%	\frac{C\cdot \pi^*_{k}}{\epsilon}= \frac{C\cdot \pi_{k}}{\epsilon (1+\alpha)}, \mbox{ where}
%	$$
%%	where
%	\begin{eqnarray*}
%		\epsilon (1+\alpha) &=& \epsilon + \sum_{i,j}{\pi_i A_{i,j}  C_{i,j} \cdot \epsilon}
%		= \epsilon +  \sum_{i,j}{\pi_i  A_{i,j} 
%			\lceil \frac{c_{i,j}}{\epsilon}\rceil  \epsilon}\\
%		&=& \epsilon +  \sum_{i,j}{\pi_i A_{i,j}  c_{i,j}}  + \sum_{i,j}{\pi_i  A_{i,j} 
%			(\lceil \frac{c_{i,j}}{\epsilon} \rceil  \epsilon - c_{i,j})}
%	\end{eqnarray*}
%	Hence,
%	\begin{eqnarray*}
%	&&	\epsilon (1+\alpha) -  \sum_{i,j}{\pi_i A_{i,j} c_{i,j}} \leq \epsilon + \sum_{i,j}{\pi_i  A_{i,j} 
%			(\lceil \frac{c_{i,j}}{\epsilon} \rceil  \epsilon - c_{i,j})}\\
% &&\leq \epsilon + \sum_{i,j}{\pi_i  M_{i,j} 
%			\epsilon}
%		= \epsilon +  \sum_{j}{\pi_j  
%			\epsilon} = 2\epsilon.
%	\end{eqnarray*}
%	This proves that,
%	for $\epsilon=\frac{1}{t^{2}}$ and $t\rightarrow \infty$,  $\epsilon (1+\alpha) \rightarrow \sum_{i,j}{\pi_i A_{i,j} c_{i,j}}=\alpha$ and the theorem follows:
%	\begin{equation}
%	Prob(C_R \leq C) \leq C\cdot \pi_k /\alpha. \nonumber %\frac{C\cdot \pi_{k}}{\sum_{i,j}{\pi_i  A_{i,j}  c_{i,j}} }. \nonumber
%	\end{equation}


==> General_paper_S&P_Eprint/sections/sim.tex <==
%Fig. \ref{fig.wbar} depicts $\bar{w}(k,T_{bud})$ as a function of $k$  with $T_{bud}=10,000$ for several $\gamma$ and  several learning rates represented by $\alpha(l)= (l+1)^{-a}$, see (\ref{eq-alpha}). 
%%based on $k$ for different $\gamma$ values while the adversary has $T_{bud)=10,000$ logical timesteps available to it in order to construct its zombie army. Four different  polynomial learning functions are considered for the defender for four different $\gamma$. 
%This plot shows the importance of having a proper defense learning mechanism in order to be able to contain the adversary. Clearly, $k$ remains small $<100$ with high probability for sufficiently fast converging learning rates and large enough $\gamma$.
%Fig. \ref{fig.kc} depicts how the containment parameter $k_c$ (computed using $\bar{w}(k,T_{bud})$) depends on $\alpha(l)= (l+1)^{-a}$. For $a\geq 0.9$, $k_c\leq 20$ is very small making it impossible for the adversary to construct its zombie army.
%
%\begin{figure*}%[h!]
%	\begin{center}
%		\scalebox{0.65}
%		{\includegraphics{figure2k50_gammaED}}
%		\caption{$\bar{w}(k,T_{bud})$ based on different values of $\gamma$ and learning functions $\alpha(l) = (l+1)^{-a}$ where $T_{bud} = 10,000$ logical timesteps}
%		\label{fig.wbar}
%	\end{center}
%\end{figure*}
%
%\begin{figure}%[h!]
%	\begin{center}
%		\scalebox{0.43}
%		{\includegraphics{kc}}
%		\caption{$k_c$ for different classes of learning functions $\alpha(l) = (l+1)^{-a}$ where $T_{bud} = 10,000$ logical timesteps}
%		\label{fig.kc}
%	\end{center}
%\end{figure}
%
%Fig. \ref{fig.roleOfp} depicts that even in the extreme cases that $\%10$ of the population is vulnerable, with $\gamma = 0.5$ meaning that half of the adversary's packets will be marked as suspicious on the flow classifier level, and while $\%0.1$ of the address space are honeypots, the adversary's probability of success (even for a small size botnet) is negligible with a good defense mechanism in place. In the same figure, $p =1$ represents the case of the strongest adversary equipped with a precompiled list of vulnerable nodes, i.e., a hitlist, meaning that it does not require to probe the network environment which gives the defender the minimum number of malware samples. Notice that in this case, at each time step, the adversary only hits a vulnerable node ($p=1, h= 0$). Even for such a strong adversary, the simulation shows that with a proper learning rate mechanism in place, chances of constructing a botnet for the attacker are minimal.
%\begin{figure}%[h!]
%	\begin{center}
%		\scalebox{0.43}
%		{\includegraphics{figureP_hitlist}}
%		\caption{$\bar{w}(k,10000)$ for extreme cases $p=0.10$ and $p=1$ with $\gamma=0.5$ and learning function $1-f(l) = (l+1)^{-a}$ where $a=0.6$ and $a=1$ respectively.}
%		\label{fig.roleOfp}
%	\end{center}
%\end{figure}
%%\begin{algorithm}
%%	\caption{$\bar{w}$ Computation}
%%	\label{alg:wbar}
%%	\begin{algorithmic}[1]
%%		\Function{$\bar{w}$}{$k,l,\gamma$}
%%		\State {$A \gets prob(k-1,l,\gamma)[k-1,...]$}
%%		\State{$\bar{w}\gets 0$}
%%		\For{$i\gets 0,l$}
%%		\State{$\bar{w} \gets \bar{w}+\alpha(i)A[i]$}
%%		\EndFor{;}
%%		\Return{$\bar{w}$;}
%%		\EndFunction
%%		\Statex
%%		\Function{$prob$}{$k,l,\gamma$}
%%		\State{$pr \gets zeros[k,l]$}
%%		\For{$i\gets 0,l$}
%%		\If{$i == 0$}\State{$pr[0,i]\gets 1$}
%%		\Else \State{$pr[0,i]\gets(1-\alpha(i-1))pr[0,i-1]$}
%%		\EndIf
%%		\For{$j \gets 1,k$}
%%		\If{$i==0$}\State{$pr[j,i]\gets [(1-\gamma)\alpha(0)]^{j}$}
%%		\Else \State{$pr[j,i]\gets (1 - \gamma)\alpha(i)pr[j-1,i] + \gamma \alpha(i - 1) pr[j-1,i-1] + (
%%			1 - \alpha(i - 1))pr[j,i-1]$}
%%		\EndIf
%%		\EndFor
%%		\EndFor{;}
%%		\Return{$pr$;}
%%		\EndFunction
%%		\Statex
%%		\Function{$\alpha$}{$l,a$}
%%		\Return{$(l+1)^{-a}$}
%%		\EndFunction
%%	\end{algorithmic}
%%\end{algorithm}
%
%Fig. \ref{fig.delayed} shows the importance of learning the adversarial moves as soon as possible. It compares the value of $k_c$ as the adversarial containment parameter for two different cases. In the first scenario the learning starts immidiately and with no delay (i.e., $L^{*}=0$) and in the second case the defeder misses only the first 100 malware samples (i.e., $L^*=100$). 
%
%%means_a0 = (100, 29, 11)
%%means_a1 = (300, 228, 210)
%\begin{figure}%[h!]
%	\begin{center}
%		\scalebox{0.43}
%		{\includegraphics{delayedLearning}}
%		\caption{The impact of delayed learning on $k_c$ for different classes of learning functions $\alpha(l) = (l+1)^{-a}$ where $T_{bud} = 10,000$ logical timesteps}
%		\label{fig.delayed}
%	\end{center}
%\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%% New simulations
Taking the CodeRed1v2 worm as an example, we apply our model to answer the following questions. First, we want to see how practical is the assumption of giving the adversary the advantage of $p= \sup_i p_i$ in our analysis. 
Second, with comparison to the well-accepted deterministic simple epidemic model (see equation \ref{eq.DE}, with no removal rates), we want to see how the simulations based on the Algorithm \ref{alg:sim} behave with and without learning rates. Third, based on these results, we want to see how the proposed learning functions and the analytical analysis in the previous sections perform while plugging in the codeRed worm actual parameters and converting the Markov model logical time steps to actual time (measured in seconds).

In the codeRed1v2 epidemic, we consider the address space to be $N = 2^{32}$ (the entire IPv4 address space), the approximate number of nodes susceptible to the malware to be $K=350,000$ (i.e., $p=8.15 \times 10^{-5}$), and the number of scans performed by an infected machine to be $10188$ scans per hour, and an initially one infected machine at time zero. 

This figure shows ...
\begin{figure}%[h!]
	\begin{center}
		\scalebox{0.45}
		{\includegraphics{simulation1_fv.eps}}
		\caption{$(a)$ Depicts the plot for the solution of the differential equation \ref{eq.DE} with the actual codeRed1v2 parameters. $(b)$ Depicts the simulation of the codeRed1v2 with the same parameters while the learning function is of the form $f(l)= 1- 1/(l/10000 +1)$ and $\gamma = 0.01$ as the classifier's accuracy}
		\label{fig.comparison}
	\end{center}
\end{figure}

%% missing plot simulation of codeRED for different cases
\begin{figure}%[h!]
	\begin{center}
		\scalebox{0.45}
		{\includegraphics{simulations.eps}}
		\caption{No learning, vs learning}
		\label{fig.Sim_ODE_Learning}
	\end{center}
\end{figure}


Fig. \ref{fig.lastOne} depicts $\bar{w}(k,T_{bud})$ for a fixed learning function of the form $f(l)= 1- 1/(l/1000 +1)$, while $p=8.15 \times 10^{-5}$, and $\gamma = 0.05$ as the classifier's accuracy. By doing  a simple extrapolation, we notice that for a time window of a month (i.e., $T_{bud} \leq 31 * 24 * 10188$ adversarial moves for the CodeRed example), and $\bar{w}$ set to $2^{-128}$, the value of $k$ would be almost 130 infected nodes. This means that in practice, with this attack-defense parameters, the probability that the attacker constructs an army of 130 infected nodes wihtin a one-month time window would be at most $2^{-128}$ which depicts how important the learning function is when it comes to containing the adversary.

\begin{figure}%[h!]
	\begin{center}
		\scalebox{0.45}
		{\includegraphics{Lastfig.eps}}
		\caption{$\bar{w}(k,T_{bud})$ for different values of $T_{bud} = 2^{t}, 8\leq t \leq 14$ with a fixed learning function of the form $f(l)= 1- 1/(l/1000 +1)$, $p=8.15 \times 10^{-5}$, and $\gamma = 0.05$ as the classifier's accuracy}
		\label{fig.lastOne}
	\end{center}
\end{figure}

==> sections/security-summary.tex <==

\section{Adversarial Containment}

The goal of the adversary is to reach a winning state $(k,l)$ for some $l\geq 0$ within a limited time budget $T_{bud}$. Here, $k$ represents the total number of nodes which the adversary wishes to compromise before using the collective of these nodes in the next attack phases (e.g. botnet applications). Time budget $T_{bud}$ represents the number of transitions in the Markov model, i.e., the total number of adversarial moves. 

The objective of the defender is to learn more and more regarding the attack technologies, specifically more malicious attack payloads in order to be able to recognize and halt future moves by the attacker. That is, the defender hopes to push level $l$ -- the number of detected malicious payloads so far -- higher and higher, leading to a higher probability $f(l)$ of successfully detecting a next malicious payload. The ultimate goal of the defender is to have a good enough learning mechanism in place such that the probability of reaching $k$ is negligible in $k$ and only polynomial in $T_{bud}$. In other words, the adversary cannot reach a winning state in practice.

We define $w(k,T_{bud})$ as the probability of the adversary to reach a state $(k,l)$ for some $l\geq 0$ within time budget $T_{bud}$. In the next subsections we analyse this probability. We want to find a tight upper bound and determine for which model parameters $\gamma$, $h$, $p$, and learning rate $f(l)$ the upper bound proves the desired asymptotic 
\begin{equation} w(k,T_{bud})=poly(T_bud) negl(k). \label{eq:as} \end{equation}
 We notice that in this case, even though the adversary cannot reach a large $k$ because $w(k,T_{bud})$ is negligible in $k$, the adversary may reach a (much) smaller $k$. We are interested in the order of magnitude of the number of compromised nodes the adversary is able to reach. For this reason we define $k_c$ as the solution of
$$ w(k_c, T_{bud}) =1/2.$$
This  $k_c$ reflects the order of magnitude of the number of compromised nodes to which the adversary is {\em contained}. By using $w(k,T_{bud})=poly(T_bud) negl(k)$ we can show that $k_c= O(\log T_{bud})$. 

Our analysis will show that for a stagnating learning rate (i.e., $1-f(l)$ remains larger than some constant $\tau>0$) the adversary is not contained since $w(k,T_{bud})$ does not follow the desired asymptotic. For a learning rate $f(l)\geq 1-O(1/l^2)$ approaching $1$ fast enough, we are able to prove the desired asymptotic. The next section evaluates other learning rates by using a dynamic programming approach developed in subsection \cite{AC-dp}. 

\subsection{Time budget measured in real time}

We first discuss the effect of translating the time budget $T_{bud}$, measured in Markov model transitions, to a time budget which is measured in real time (seconds) as this makes sense in practice. If the adversary wins as soon as $k$ nodes are compromised and if each Markov model transition takes $\Delta$ seconds, then at most $k$ moves can be made by each of the compromised nodes {\em in parallel} in $\Delta$ secconds. With a time budget of $T$ seconds, this implies $T_{bud}\leq T k/\Delta$. This means that the desired asymptotic (\ref{eq:as}) translates into
$$ w(k,T_{bud})\leq poly(T k/ \Delta) negl(k),$$
which is $poly(T)negl(k)$, which again implies that in practice  the adversary cannot reach $k$ since the probability of reaching $k$ is negligible in $k$ and only polynomial in real time budget $T$. 

\subsection{Stagnating learning rate} \label{stagnating}

Suppose that the learning rate stagnates in that $1-f(l)\geq \tau$ for some $\tau>0$. This means that $f(l)\leq 1-\tau$ and as a result at least a fraction $\tau$ goes undetected. In order to prove a lower bound on $w(k,T_{bud})$ we give a benefit to the defender and assume $1-f(l)=\tau$ with equality.

If $1-f(l) = \tau$, then $m_1,m_2,m_3$ and $m_4$ are independent of $l$ and the Markov model reduces to Fig. \ref{fig.reducedMarkovModel} where each  state $i$ represents the set of states $(i,l)$ for $l\geq 0$ in the original Markov model.

\begin{figure}[t]
	\centering
	\begin{tikzpicture}
	\tikzset{
		>=stealth',
		node distance=3cm and 3cm ,on grid,
		every text node part/.style={align=center},
		state/.style={minimum width=1.5cm,
			%    		font=\small,
			draw,
			circle},
	}
	% Add the states
	\node[state]             (c) {i};
	\node[state, right=of c] (r) {i\pp};
	%	\node[state, left=of c] (lose) {0};
	% Connect the states with arrows
	\draw[every loop]
	(c) edge[auto=left]  node {$m_{2}+m_3$} (r)
	%(r) edge[bend left, auto=right] node {0.7} (s)
	%(c) edge[loop above]             node {($1-p_i-f(.)$)} (c)
%	(c) edge[ auto=left] node {$m_3$} (rr)
%	(c) edge[auto=right] node {$m_4$} (b)
	(c) edge[loop above]             node {$m_1+m_4$} (c);
	%(d) edge[loop above]             node {} (d);
	\end{tikzpicture}
	\caption{Reduced Markov model of the game for a constant $1-f(l)=\tau>0$}
	\label{fig.reducedMarkovModel}
\end{figure}

Within time budget $T_{bud}$ we reach $i=k$ with probability 
$$ w(k,T_{bud})=  \sum_{T=0}^{T_{bud}-k} {\sum_{\substack{f_0,\dots,f_{k-1} s.t.\\ \sum f_j=T}}
\prod_{j} (m_1+m_4)^{f_j}(m_2+m_3)^{k}
},
$$
where the time budget is distributed over $k$ steps from each state to the next until state $k$ is reached and  $T\leq T_{bud}-k$ transitions consists of $f_i$ self-loops in state $i$ for $0\leq i\leq k-1$.
This probability is equal to
%
%\begin{eqnarray}
%\lefteqn{ \sum_{T=k}^{T_{bud}} {T-1 \choose k-1}(m_1+m_4)^{(T-1)-(k-1)}(m_2+m_3)^{k-1+1} =} \nonumber\\
% & & \sum_{T=k}^{T_{bud}} {T-1 \choose k-1}(m_1+m_4)^{T-k}(m_2+m_3)^{k}\nonumber\\
%&=& \sum_{T-k=0}^{T_{bud}-k} {(T-k)+(k-1) \choose (T-k)}(m_1+m_4)^{T-k}(m_2+m_3)^{k} \nonumber\\
%&=&  \sum_{i=0}^{T_{bud}-k} {i+(k-1) \choose i}(m_1+m_4)^{i}(m_2+m_3)^{k} \label{eq.7}
%\end{eqnarray}
%
%A lower bound on (\ref{eq.7}) can be derived as follows:
%
\begin{eqnarray*}
%  \sum_{i=0}^{T_{bud}-k}
%{\sum_{\substack{f_1,\dots,f_k s.t.\\ 
%		\sum f_j=i}}
%\prod_{j} (m_1+m_4)^{f_j}(m_2+m_3)^{k}
%}\\
%&=& 
\sum_{\substack{f_0,\dots,f_{k-1} s.t.\\ \sum f_j\leq T_{bud}-k}}
\prod_{j} (m_1+m_4)^{f_j}(m_2+m_3)^{k}
&\geq& \sum_{f_0=0}^{(T_{bud}-k)/k}\dots\sum_{f_{k-1}=0}^{(T_{bud}-k)/k}\prod_{j}(m_1+m_4)^{f_j}(m_2+m_3)^{k}\\
&=& \prod_{j=0}^{k-1}\sum_{f_j=0}^{(T_{bud}-k)/k}(m_1+m_4)^{f_j}(m_2+m_3)^{k}\\
&=& \prod_{j=0}^{k-1}\frac{1-(m_1+m_4)^{T_{bud}/k}}{1-(m_1+m_3)}(m_2+m_3)^{k}\\
&=& [1-(m_1+m_4)^{T_{bud}/k}]^{k} \geq 1-k(m_1+m_4)^{T_{bud}/k}.
\end{eqnarray*}
This shows that $w(k, T_{bud})\approx 1$ for relatively small $T_{bud}$ because $1-w(k,T_{bud}) \leq k(m_1+m_4)^{T_{bud}/k}$ which is exponentially small in $T_{bud}$. 
%For example, $T_{bud}=lambda k ln k$ to get >=1- x^{-lambda} for some small x
% REAL TIME: Use f_i/(i+1) in the formula -- i.e. sum f_i/(i+1) is real time, take f_i = T_real / ln k, hence T_real = lambda (ln k)^2 is sufficient
In order to have the desired asymptotics (\ref{eq:as}), the learning rate should not stagnate, i.e., we need $1-f(l)\rightarrow 0$ for $l\rightarrow \infty$ .

\subsection{Formula for $w(k,T_{bud})$}

Before proving any bounds on $w(k,T_{bud})$ we first provide a closed form for $w(k,T_{bud})$ itself. To this purpose we introduce $p(k-1,L,T_{bud})$ defined as the probability that the adversary reaches state $(k-1,L)$ and is ready to leave state $(k-1,L)$ (after zero or more self-loops at state $(k-1,L)$) within time budget $T_{bud}$. Any possible path from state $(0,0)$ to state $(k-1,L)$ in the Markov model with self-loops along the way in each of the visited state (including $(k-1,L)$) contributes to this probability. (We use $k-1$ rather than $k$ because after a path to $(k-1,L)$ for some $L\geq 0$ only a single horizontal or diagonal move is needed to reach $(k,L)$ for the first time, and this probability is what we will need for $w(k,T_{bud})$.) 

A path to $(k-1,L)$ till the moment it is ready to leave $(k-1,L)$ is uniquely represented by 
\begin{itemize}
\item $g_l$ is the number of states on the path that have the same level $l$,
\item $b_l$; if level $l$ is entered via a vertical transition, then $b_l=0$; if level $l$ is entered via a horizontal transition, then $b_l=1$,
\item $t(i,l)$ counts the number of self-loops on the path in state $(i,l)$.
\end{itemize}
(Notice that $b_0$ is undefined and $g_l\geq 1$ for all $0\leq l \leq L$.)
By using induction one can prove that the probability of having the Markov model transition along a path represented by these numbers is equal to
\begin{subequations}
\begin{eqnarray}
&& \prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg) \cdot \label{path-a}\\
&& \prod_{l=0}^{L} \bigg( \frac{m_2(l)}{1-m_1(l)}\bigg)^{g_l-1}\cdot \label{path-b}\\
&& \prod_{l=0}^{L}\prod_{i=0}^{g_l-1}m_1(l)^{t(i_l+i,l)}(1-m_1(l)) \label{path-c}
\end{eqnarray}
\end{subequations}
(the induction hypothesis is that the above statement holds for $(i,l)$, $0\leq i\leq k-1$ and $0\leq l\leq L$ such that $(i,l)\neq (k-1,L)$).
The length of the path, i.e., total number of transitions without self-loops,  is equal to 
$$(k-1) + L -B, \mbox{ where } B=\sum_{l=1}^L b_l$$
is the total number of diagonal transitions.  The total number of vertical transitions is equal to $L-B$ and the number of horizontal transitions is equal to $\sum_{l=0}^L (g_l-1) = (k-1)-B$.

Summing the above probability over all possible combinations of $g_l$, $b_l$, and $t(.,.)$ for paths that reach state $(k-1,L)$  and are ready to leave $(k-1,L)$ such that the number of self-loops is equal to $T$ and the total number of transitions including self-loops is equal to $(k-1)+L-B + T\leq T_{bud}$ leads to an expression for $p(k-1,L,T_{bud})$:
	\begin{subequations}
		\begin{eqnarray}
		p(k-1,L,T_{bud}) &= &
		\sum_{\substack{B,T s.t.\\
				(k-1)+L-B+T\leq T_{bud}}}\nonumber\\& &
		{ 
			\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ \label{p-a}
					\sum_{l=1}^{L}b_l=B}}
%			\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
(\ref{path-a})
		}\\& &
		{	\sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\ \label{p-b}
					\sum_{l=0}^{L}(g_l-1)=(k-1)-B}}
%			\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
(\ref{path-b})
		}\\& &
		{
			\sum_{\substack{t_0,\dots,t_L s.t.\\ \label{p-c}
					\sum_{l=0}^{L}t_l=T}}
			\sum_{\substack{t(i_l,l),\dots,t(i_l+g_l-1,l) \\
						s.t.\sum_{i=0}^{g_l-1}t(i_l+i,l)=t_l}}
%			\prod_{l=0}^{L} 
%			{	
%				\prod_{i=0}^{g_l-1} 
%				m_1(l)^{t(i_l+i,l)}(1-m_1(l))
%			}
(\ref{path-c})
		}
		\end{eqnarray}
	\end{subequations}
	
The formula for $w(k,T_{bud})$ considers all the possible paths towards a state $(k-1,L)$ within $T_{bud} -1$ transitions and a single final horizontal or diagonal transition (via $m_2(L)$ or $m_3(L)$) towards the winning state $(k,L)$. We are interested in the probability of entering state $(k,L)$ for some $L\geq 0$ and the time it takes to reach there \emph{for the first time}. Appropriately summing over probabilities $p(k-1,L,T_{bud}-1)$ gives
	\begin{subequations}
\begin{eqnarray}
 w(k, T_{bud})&=&	\sum_{L\geq 0} p(k-1,L,T_{bud}-1) \cdot	 \bigg( \frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\bigg) \nonumber \\
&=& \sum_{L=0}^{T_{bud}-1}\sum_{B=0}^{\min\{L,(k-1)\}}\bigg( \frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\bigg)\cdot (\ref{p-a})\cdot (\ref{p-b})\cdot \label{w-a} \\
 \sum_{T=0}^{(T_{bud}-1)-[(k-1)+L-B]} (\ref{p-c}).  \label{w-b}
\end{eqnarray}
\end{subequations}
This is a closed form of the probability we are interested in. 

\subsection{Upper and lower bound on $w(k, T_{bud})$}

By noticing that (\ref{w-b}) for $T_{bud}=\infty$ is equal to 1, a straightforward upper bound on $w(k,T_{bud})$ is given by just formula (\ref{w-a}): We have $w(k,T_{bud})$ is at most equal to 
\begin{equation}
\bar{w}(k,T_{bud}) = (\ref{w-a}) =
\sum_{L=0}^{T_{bud}-1}\sum_{B=0}^{\min\{L,(k-1)\}}\bigg( \frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\bigg)\cdot (\ref{p-a})\cdot (\ref{p-b}).
\label{UB}
\end{equation}

%By using a proof strategy similar to the one used in Section \ref{stagnating} 
We may lower bound (\ref{w-b}) as follows.
 For $e\leq T_{bud}/(L+1)$, we can show that
$$ (\ref{w-b}) \geq 1- \sum_{l=0}^{(T_{bud}/e)-1} k \cdot m_1(l)^{e/k}\geq 1- T_{bud} \frac{k}{e} (1-\gamma)^{\frac{e}{k}},$$
where the first inequality follows from a proof strategy similar to the one used in Section \ref{stagnating}, and the second inequality follows from $m_1(l)\leq 1-\gamma$.
This lower bound on (\ref{w-b})  is independent of any of the other summing variables used in (\ref{w-a}) but requires $L< T_{bud}/e$. By restricting $L$ to be $<T_{bud}/e$ in (\ref{w-a}) (i.e., we substitute $T_{bud}$ by $T_{bud}/e$) we obtain a lower bound on $w(k,T_{bud})$:
\begin{equation} w(k,T_{bud}) \geq \bar{w}(k,T_{bud}/e)\cdot (1- T_{bud} \frac{k}{e} (1-\gamma)^{\frac{e}{k}}). 
\label{LB}
\end{equation}
In particular for $e= k \ln (T_{bud}k/\epsilon) / \ln (1/(1-\gamma))$, we have $w(k,T_{bud}) \geq \bar{w}(k,T_{bud}/e)\cdot (1-\epsilon)$. 

Upper bound  (\ref{UB}) proves that if $\bar{w}(k,T_{bud})$ has desired complexity $\bar{w}(k,T_{bud})=poly(T_bud) negl(k)$, then $w(k,T_{bud})$ inherits this desired complexity. And vice versa, lower bound (\ref{LB}) for the special choice of $e$ proves that if $w(k,T_{bud})$ has desired complexity $w(k,T_{bud})=poly(T_bud) negl(k)$, then also $\bar{w}(k,T_{bud}) \leq w(k, T_{bud}\cdot e)/(1-\epsilon) = poly(T_bud \cdot e)\cdot negl(k) = poly(T_{bud})negl(k)$. We conclude that in order to find out which learning rates lead to the desired complexity for the defender, we only need to study which learning rates lead to the same desired complexity for $\bar{w}(k,T_{bud})$.

The advantage of studying $\bar{w}(k,T_{bud})$ is having eliminated expression (\ref{w-b}) which represents the effect of self-loops (and turns out to be very inefficient to evaluate as an exact expression). Probability $\bar{w}(k,T_{bud})$ corresponds to the Markov model in Figure \ref{???} without any self-loops and with horizontal transition probabilities $m_2(l)/(1-m_1(l))=(1-\gamma)\alpha(l)$, diagonal transition probabilities $m_3(l)/(1-m_1(l))=\gamma \alpha(l)$, and vertical transition probabilities $m_4(l)/(1-m_1(l))=1-\alpha(l)$, where 
$$ \alpha(l) = \frac{p(1-f(l))}{\gamma + (1-\gamma)(p+h)(1-f(l))}.$$
 Figure \ref{???}  shows that $\bar{w}(k,T_{bud})$ can be computed in $O(k\cdot T_{bud})$ time using dynamic programming -- and this is what we use in the next section to evaluate $\bar{w}(k,T_{bud})$ for different learning rates.


\subsection{Analyzing learning rate $1-f(l)=d/(l+2)^2$}

We will further upper bound $\bar{w}(k, T_{bud})$ and prove small enough learning rates $f(l)\geq 1- d/(l+1)^2$ attain our desired asymptotic.
Later we will discuss what happens if there is an intial period during which the adversary already starts compromising nodes without the defender being aware or not having learning anything, i.e., $f(l)=0$ for $l\leq L^*$ and $f(l)\geq 1-d/(l-L^*)$ for $l>L^*$. Here,  $L^*$ represents this initial period; only after a suffcient level $L^*$ is reached the learning rate increases.

For now we only assume, for all $l\geq 0$,
$1-f(l)\leq d$
for some small $d$. Equivalently,
$$\beta(l)=\sqrt{\frac{1-f(l)}{d}}\leq 1,$$
  hence, $\beta(l)^2\leq \beta(l)$.
This allows us to bound 
\begin{equation*}
\begin{aligned}
\frac{m_2(l)}{1-m_1(l)} = (1-\gamma)\alpha(l) \leq \frac{(1-\gamma)pd}{\gamma} \beta(l)^2 \leq \frac{(1-\gamma)pd}{\gamma} \beta(l),\\
\frac{m_3(l)}{1-m_1(l)} \leq  pd \beta(l)^2, \mbox{ and}\\
\frac{m_4(l)}{1-m_1(l)} \leq 1- pd \beta(l)^2.
\end{aligned}
\end{equation*}

Plugging the above bounds in the expression for $\bar{w}(k,T_{bud})$ with $\frac{m_2(L)}{1-m_1(L)}\leq \frac{(1-\gamma)pd}{\gamma} \beta(L)^2$ and $(1-\gamma)/\gamma\leq \theta$ yields
\begin{subequations}
 \begin{eqnarray}
\bar{w}(k,T_{bud}) &\leq &
\sum_{L=0}^{T_{bud}-1} (1+ \theta)pd \beta(L)^2 \nonumber \\ 
& &	
\sum_{B=0}^{\min{(L,k-1)}} { \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}pd \beta(l)^2 + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
} \label{ub-a} \\
& &
{	\sum_{\substack{g_0,\dots,g_L\geq 1 s.t.\\ 
			\sum_{l=0}^{L} (g_l-1)=(k-1)-B}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{g_l-1} 
} \label{ub-b}
\end{eqnarray}
\end{subequations}

Let $b_{L+1}=0$ and define
$$ Z = \prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{b_{l+1}}.$$
We will multiply (\ref{ub-b}) with $Z$ and show an upper bound of the product which is independent of $b_l$ and $B$. We will multiply (\ref{ub-a}) with $Z^{-1}$ and show that it behaves like a sum of products of the $\beta(l)$, which remains `small enough': We choose $d$ such that $\theta\leq 1/(pd)$. Then, since $B=\sum_{l=0}^{L}b_{l+1}$,
$$(\ref{ub-b})\cdot Z = \sum_{\substack{g_0,\dots,g_L\geq 1 s.t.\\ 
			\sum_{l=0}^{L} (g_l-1)+b_{l+1}=(k-1)}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{(g_l-1)+b_{l+1}} 
	\leq \sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L} g'_l=(k-1)}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{g'_l} \leq
	(\theta pd)^{k-1}  \sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L} g'_l=(k-1)}}
	\prod_{l=0}^{L} \beta(l)^{g'_l}
	 \leq  (\theta pd)^{k-1} \prod_{l=0}^{L} \sum_{g'_l\geq 0} \beta(l)^{g'_l} 
	=(\theta pd)^{k-1}  \prod_{l=0}^{L} \frac{1}{1-\beta(l)}.$$
We derive (notice that each $b_{l+1}$ is either equal to $0$ or $1$)
$$ (\ref{ub-a})\cdot Z^{-1} 
\leq 
\sum_{B=0}^{L} \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{ \beta(l)}{\theta} + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
=
 \sum_{b_1,\dots,b_L\in\{0,1\} }
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{ \beta(l)}{\theta} + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
	= 
\prod_{l=0}^{L-1} \sum_{b_{l+1}\in \{0,1\}} \bigg( b_{l+1}\frac{ \beta(l)}{\theta} + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
=
\prod_{l=0}^{L-1} \bigg( \frac{\beta(l)}{\theta} + (1-pd \beta(l)^2) \bigg)
\leq \prod_{l=0}^{L-1} \bigg( \frac{\beta(l)}{\theta} + 1 \bigg).
$$
Combination of the above results proves
\begin{eqnarray*}
	\bar{w}(k,T_{bud}) &\leq &\nonumber
	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k-1}(1+\frac{1}{\theta})\frac{\beta(L)^2}{1-\beta(L)}\prod_{l=0}^{L-1} \frac{1+\beta(l)/\theta}{1-\beta(l)}\\
	&\leq&  	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k}(1+\frac{1}{\theta})\prod_{l=0}^{L} \frac{1+\beta(l)/\theta}{1-\beta(l)}.
\end{eqnarray*}
The argument in the product is equal to $(1+\beta(l)/\theta)/(1-\beta(l)) = 1+(1+1/\theta)\beta(l)/(1-\beta(l))$. For differentiable continuous functions $B(.)$, we can prove a useful lemma which states that if $B'(l)\geq 0$ and $B''(l)\leq 0$ for $l\geq 0$, then for $y\geq 0$
$$\prod_{l=0}^L (1+ yB'(l))\leq e^{y(B'(0)-B(0)+B(L))}.$$
For $B(l) =\beta(l)/(1-\beta(l))$ and $y=(1+1/\theta)$, application of this inequality to our upper bound yields 
\begin{eqnarray*}
	\bar{w}(k,T_{bud}) &\leq&
	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k-1}(1+\frac{1}{\theta}). e^{(1+1/\theta)(B'(0)-B(0)+B(L))} \\
	&\leq& T_{bud}\cdot [\theta p d]^{k-1}(1+\frac{1}{\theta})e^{(1+1/\theta)(B'(0)-B(0)+B(L))} .
\end{eqnarray*}
Minimizing this upper bound with respect to $\theta\geq (1-\gamma)/\gamma$ gives ($e$ denotes the natural number)
\begin{align}\label{eq.conditions}
\bar{w}(k,T_{bud}) \leq
\begin{cases}
T_{bud} [epd (B(T_{bud})-B(0)+B'(0))/(k-1)]^{k-1}(1+ (k-1)/(B(T_{bud}-1)-B(0)+B'(0))) e^{B(T_{bud}-1)-B(0)+B'(0)}, & \text{if}\ B(T_{bud}-1)-B(0)+B'(0)\geq \frac{(k-1)(1-\gamma)}{\gamma} \\
T_{bud} [\frac{1-\gamma}{\gamma}pd]^{k-1}\frac{1}{1-\gamma}e^{(B(T_{bud}-1)-B(0)+B'(0))/(1-\gamma)}, & \text{otherwise}
\end{cases}
\end{align}
The second condition is  the case $\theta=(1-\gamma)/\gamma$.

As an example, assume that $B'(l)=\frac{\beta(l)}{1-\beta(l)} \leq \frac{1}{l+1}$, then $B(T_{bud}-1) \leq \ln(T_{bud})$ and for 
$$T_{bud} \leq e^{(k-1)(1-\gamma)/\gamma -1}$$
the probability of winning for the adversary (the second case)
$$w(k,T_{bud}) \leq \bar{w}(k,T_{bud}) \leq 
T_{bud}^{1+1/(1-\gamma)} [\frac{1-\gamma}{\gamma}pd]^{k-1}\frac{e^{1/(1-\gamma)}}{1-\gamma}.
%(\frac{1-\gamma}{\gamma}pd)^{k}\frac{1}{1-\gamma}e^{C/(1-\gamma)}T_{bud}^{1+1/(1-\gamma)}$,
$$
The condition $B'(l)=\frac{\beta(l)}{1-\beta(l)} \leq \frac{1}{l+1}$ translates into 
$$1-f(l)\leq \frac{d}{(l+2)^2}$$
where $d$ should be chosen such that $d< \gamma / [p(1-\gamma)]$. For this learning rate $w(k,T_{bud})$ satisfies the desired asymptotics.


\subsection{Delayed learning}

In practice learning only start afyer a sufficient number of suspicious looking network packets are seen. That is, $f(l)=0$ for $l\leq L^*$ for some $L^*$.




 
For $(1-f(l)) \approxeq 1$, we have:


\begin{equation*}
\begin{aligned}
m_1(l) &= (1-\gamma)(1-(p+h))\\ 
m_2(l) &= (1-\gamma)p\\
m_3(l) &= \gamma p\\
m_4(l) &= [h-\gamma(h+p)]+\gamma=(1-\gamma)h+\gamma(1-p)\\
\end{aligned}
\end{equation*}

We are interested in $k^*$ as a function of $\epsilon$ for which 
\begin{eqnarray}\label{eq.k}
\sum_{k=0}^{k^{*}-1} p(k,L^{*}-1,T_{bud}-1)(\frac{m_4(l)}{1-m_1(l)}+\frac{m_3(l)}{1-m_1(l)}) +\\ p(k^*,L^{*}-1,T_{bud}-1)\frac{m_4(l)}{1-m_1(l)} \geq 1- \epsilon \nonumber
\end{eqnarray}

Then the probability of winning is 
\begin{equation}\label{eq.deta}
\leq \epsilon + (1-\epsilon)w(k-k^{*}(\epsilon),T_{bud})
\end{equation}

Notice that during phase one an $i>k^{*}(\epsilon)$  is reached ($\epsilon$ term in the above formula) and during phase two, another $k-k^{*}(\epsilon)$ horizontal or diagonal moves are needed in order to win (the second term).

We generalize the analysis of (\ref{eq.6}) for $(1-f(l))=1$ (without any constraint on $T_{bud}$):

\begin{eqnarray}\label{eq.delta}
(\ref{eq.k}) = \sum_{B=0}^{\infty}\sum_{k=B+1}^{k^{*}-1}(\ref{eq.a})(\ref{eq.b})(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)}) 
\end{eqnarray}

\saeed{Check \ref{eq.a} I guess the above should be L not l}
Notice that 

\begin{eqnarray*}
	\sum_{k=B+1}^{k^{*}-1}(\ref{eq.b}) &=& 
	\sum_{k=B+1}^{k^{*}-1}
		{	\sum_{\substack{g_0\geq 1,\dots,g_L^{*}\geq 1 s.t.\\
				\sum_{l=0}^{L^{*}}(g_l-1)=k-1-B}}
		\prod_{l=0}^{L^{*}} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
	}\\
	&=& \sum_{\substack{g'_0,\dots,g'_{L^*}\geq 0 s.t.\\
		\sum_{l=0}^{L^*-1}{g'_l \leq k^*-2-B}}}\prod_{l=0}^{L^*} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l}\\
	&\geq& \sum_{g'_0=0}^{(k^*-2-B)/L^*+1} \dots \sum_{g'_{L^*}=0}^{(k^*-2-B)/L^*+1} (\prod \dots)\\
	&=&  \prod_{l=0}^{L^*} \sum_{g'_l\geq 0}^{(k^*-2-B)/L^*+1}\bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l} \\
	&=&	 \prod_{l=0}^{L^*}\frac{1}{1-\frac{m_2(l)}{1-m_1(l)}}\big(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \big)^{L^*+1} \\
	&=& \prod_{l=0}^{L^*} \frac{1-m_1(l)}{1-m_1(l)-m_2(l)}\bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \bigg)^{L^*+1}\\
	&=& \prod_{l=0}^{L^*} \frac{1-m_1(l)}{m_3(l)+m_4(l)}\bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \bigg)^{L^*+1}
\end{eqnarray*}

\saeed{Missing part from the notes: Since $B\leq L^* \geq \bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-1}{L^*+1}}\bigg)^{L^*+1}$}

And 

\begin{eqnarray*}
	\lefteqn{\sum_{B=0}^{\infty}(\ref{eq.a})(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)}) =} \\ & & 
	{ \sum_{\substack{b_1,\dots,b_L^*\in\{0,1\} s.t.\\ 
				\sum_{l=1}^{L^*}b_l=B}}
		\prod_{l=0}^{L^*-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)  (\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})}\\
& =&	{ \sum_{b_1,\dots,b_L^*\in\{0,1\}}\prod_{l=0}^{L^*-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})
}\\
&=&\prod_{l=0}^{L^*}(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})
\end{eqnarray*}

\saeed{Note From Marten's: In the write up we can refer in parts to the analysis of \ref{eq.6} in order to save space}

So we get 
\begin{eqnarray*}
(\ref{eq.k}) &\geq& \bigg(1-(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}} \bigg)^{L^*+1}\\
&\geq& 1 - (L^*+1)(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}}
\end{eqnarray*}

We want to solve $L\geq 1-\epsilon$

\begin{equation}\label{eq.star}
(L^*+1)(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}} = (L^*+1)[\frac{(1-\gamma)p}{1-(1-\gamma)(1-(p+h))}]^{\frac{k^*-1}{L^*+1}} \leq \epsilon
\end{equation}

Notice that $p \leq 1-h$, we have:
\begin{equation}
[\frac{(1-\gamma)p}{1-(1-\gamma)(1-(p+h))}] \leq (1-\gamma)(1-h).
\end{equation}

So, Equation (\ref{eq.star}) is satisfied for $k^*$ such that 

\begin{equation}
(L^*+1)[(1-\gamma)(1-h)]^{\frac{k^*-1}{L^*+1}} \leq \epsilon.
\end{equation}

\saeed{check equation delta \ref{eq.delta} reference, there are two of them deta and delta!}

Applying (\ref{eq.delta}) gives
probability of winning for 
\begin{equation*}
1-\tilde{f}(l)=\begin{cases}
1, & \text{if $l<L^*$}.\\
1-f(l-L^*), & \text{if $l \geq L^*$}.
\end{cases}
\end{equation*}
is 
\begin{equation}\label{eq.delta.1}
\leq (L^*+1)[(1-\gamma)(1-h)]^{\frac{k^*-1}{L^*+1}} + \bar{w}(k-k^*,T_{bud}), 
\end{equation}

where $\bar{w}$ can be computed through simulation or $\bar{w}$ has the special form as derived for $(1-f(x)) = \frac{d}{(1+x)^2}$.

We want to minimize Equation \ref{eq.delta.1} for $k^*$.
\saeed{Note: Need to do this}
This shows how $h$ plays a role as wel!? It is important in phase one.

We get some function $g(k,T_{bud})\geq Prob(win)$.







============================
============================
============================
\noindent

{\bf Contributions.} By modeling the learning rate of the defender as a function $f(l)$ ($f(l)$ is the probability of detecting a next malicious payload) where $l$ represents the number of malicious payloads for a specific exploit so far collected we have the following results:
\begin{itemize}
\item If $f(l)$ does not converge to $1$, then we call such a learning rate stagnating and the adversary is able to reach his goal of $k$ compromised nodes within $poly(k)$ time budget.
\item If $f(l)\rightarrow 1$ and more specifically $1-f(l) = O(l^{-2})$, then the probability of the adversary affecting $k$ nodes (i.e., the probability of winning) is proven to be polynomial in the attacker's time budget and negligible in $k$. Simulations show that this property is even satisfied for $1-f(l) = O(l^{-???})$.
\item The above results hold for time budget measured in logical Markov model transition or real time (seconds), and also hold for learning rates that remain equal to $f(l)=0$ until a certain number $l=L^*$ malicious payloads have been collected after which learning starts.
\item The presented adversarial/defender game in terms of a Markov model is general and fits most practical ... scenarios as our extensive overview shows.
\end{itemize}
The adversary may not reach his goal of $k$ compromised nodes, but will reach a much smaller number $k_c$ compromised nodes of the order log of the time budget for $1-f(l) = O(l^{-2})$. Therefore, we conclude that at a meta level the adversary needs to find  one exploit for which the defender cannot find a fast enough increasing learning rate and the defender needs to have a learning system/methodology in place which should be able to reach fast enough learning rates for any possible exploit. In practice infrastructures are being compromised and this means that effort is needed in order to understand associated learning rates and why these are $\leq 1-O(l^{-???})$ as given by our general framework, its thorough analysis, and simulations.

%take T_bud = 2k is already sufficient. constant real time.

%We are interested in probability $w(k,T_{bud})$ of achieving $i=k$
%goal: Let w(k,T_bud) be the probability ....

%real time transfer

%We want to find a tight upper bounds and deterimine for which p,h, gamma, f(l) we can show   asymptotics 

%w = poly(T_bud) negl(k)

%Such a  result will imply containment.

%w=1/2 gives k_c = O( log poly(T_bud) )

%call this k_c

also: w=2^{-s}, T_bud=2^t gives k<= c1 s + c2 t + c3 a sort of capacity region

%(0) we start with a negative result: constant f(l)
%we conclude we need 1-f(l) --> 0
How fast does it need to converge to 0 in order to be in the above class?
In other words, what learning rate is needed? And how soon does this learning rate need to take effect?

%(1) model, probability of a path (induction), gives formula for w (can be verified)
%this gives an expression for w

%(2) observe that T_bud part is close to 1, more precisely w without the self-loop part turns out to be a tight approximation:
%define wbar, we prove
%LB / UB
%(use the same type of thinking which proves (0))
%This can be used to study the asymptotics of w

%(3) UB on wbar for d/(l+1)^2

%(4) note that wbar corresponds to the model (also define alpha) without self-loops and that a dynamic program ...

Conclusion capacity region is lower bounded by ... and UB ...
In the next section we use the dynamic program to investigate intermediate values ..

(5) Late start of learning: does the initial convergence of the learning rate matter?

phase 1 and 2

k_c inclreases

apply to  (3)




\section{Appendix}
\label{sec:proofs}

%\vspace{-1mm}
This appendix provides the analysis of the Markov model depicted in Fig. \ref{markovModel}. The goal of the adversary is to reach a winning state $(k,l)$ for some $l\geq 0$. Here, $k$ represents the total number of nodes which the adversary wishes to compromise before using the collective of these nodes in the next attack phases (e.g. botnet applications). On the other hand, the objective of the defender is to learn more and more regarding the attack technologies, more specifically the malicious attack payloads in order to be able to recognize and halt future moves by the attacker. That is, the defender hopes to push level $l$ -the number of detected malicious payloads so far- higher and higher leading to a higher probability $f\mytiny{(}l\mytiny{)}$ of successfully detecting a next malicious payload. The ultimate goal of the defender is to have a good enough learning mechanism in place to limit the probability of reaching $k$ negligible. In other words, the adversary cannot reach a winning state in practice.

Fig. \ref{markovModel}, as explained in section \ref{ss.markovModel} shows several possible transitions from state to (another) states. The corresponding probabilities can be rewritten as follows:

\begin{equation}\label{eq.transitions.rewritten}
\begin{aligned}
m_1 &= f\mytiny{(}l\mytiny{)}(1-\gamma)+(1-f\mytiny{(}l\mytiny{)})(1-\gamma)(1-p-h)\\
	&= (1-\gamma)(1-(p+h)(1-f\mytiny{(}l\mytiny{)}))\\
m_2 &= (1-f\mytiny{(}l\mytiny{)})(1-\gamma)p \\
m_3 &= (1-f\mytiny{(}l\mytiny{)})\gamma p\\
m_4 &= (1-f\mytiny{(}l\mytiny{)})(1-\gamma)h+f\mytiny{(}l\mytiny{)}\gamma + (1-f\mytiny{(}l\mytiny{)})\gamma (1-p)\\
	&= (1-f\mytiny{(}l\mytiny{)})[(1-\gamma)h+\gamma(1-p)] + f\mytiny{(}l\mytiny{)}\gamma\\
	&= (1-f\mytiny{(}l\mytiny{)})[h-\gamma(h+p)] + \gamma
\end{aligned}
\end{equation}

where
\begin{align*}
h &= \frac{H}{N}, & p_i &= \frac{(K-i)}{N} \approx p
\end{align*}

Notice that in these transition probabilities we take $p$ to be a constant and not depending on $i$. This is a reasonable assumption if 
\begin{align*}
 p_i &= \frac{(K-i)}{N}
\end{align*}
where $K$ is the total number of vulnerable nodes out of a total number of $N$ nodes, and $p_i$ is the probability of a \emph{memoryless adversary} picking a random node in the hope to hit one of the $(K-i)$ remaining vulnerable nodes (which it has not yet compromised). Since $k \ll K $ therefore, 

\begin{align*}
 p_i &\approx \frac{K}{N} = p
\end{align*}

This means we are dealing with a constant vulnerability density function.
A smarter adversary, however, may use a hitlist target locating strategy and this would make $p_i$ not a constant. In this case, we assume a worst-case scenario for the adversary meaning that $p_i \leq p$.

We will analyze to what extent our bounds on the probability of reaching a winning state ($i=k$) are sensitive to the choice of $p$. It turns out that this sensitivity is limited, therefore, our bounds cannot be much improved when assuming non-constant (i.e., non-worst-case) $p_i$.

In the next sections, we first give a complex formula for the probability of winning $w$ (i.e., the probability of reaching a winning state). Next, we simplify the formula by upper bounding. We analyze two class of learning functions:

\begin{enumerate}
	\item $(1-f\mytiny{(}l\mytiny{)})\leq d/l$, and
	\item $ \tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up}$.
\end{enumerate}

We show how these two functions can be combined into 

%\begin{equation}
%(1-f\mytiny{(}l\mytiny{)})\leq d/l  \mbox{ for }l \leq L^*,
%\end{equation}
%\begin{equation}
%	\tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up} = (1-f\mytiny{(}L^*\mytiny{)})  \mbox{ for }l > L^* .
%\end{equation}
\begin{equation}\label{eq.(1)}
(1-f\mytiny{(}l\mytiny{)})\leq d/l  \mbox{ for }l \leq L^*,~and~\\
\tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up} = (1-f\mytiny{(}L^*\mytiny{)})  \mbox{ for }l > L^* .
\end{equation}

%\begin{eqnarray}
%(1-f\mytiny{(}l\mytiny{)})\leq d/l  \mbox{ for }l \leq L^*,~and~\\
%\tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up} = (1-f\mytiny{(}L^*\mytiny{)})  \mbox{ for }l > L^* .
%\end{eqnarray}
%$$
%(1-f\mytiny{(}l\mytiny{)})\leq d/l  \mbox{ for }l \leq L^*,
%$$
%and
%$$
%\tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up} = (1-f\mytiny{(}L^*\mytiny{)})  \mbox{ for }l > L^* .
%$$

%\begin{enumerate}
%	\item $(1-f\mytiny{(}l\mytiny{)})\leq d/l$ for $l \leq L^*$, and
%	\item $ \tau_{low}\leq (1-f\mytiny{(}l\mytiny{)})\leq \tau_{up} = (1-f\mytiny{(}L^*\mytiny{)})$ for $l > L^*$.
%\end{enumerate}

For this function with suitably chosen parameters, the probability of winning is exponentially decreasing in $k$ and is only linearly proportional to the total time budget $T_{bud}$ which is measured in the total number of transitions given to the adversary.
We represent this result in the form of a ``security capacity function'' $g\mytiny{(}k,t\mytiny{)}$ that is:
For $T_{bud} \leq 2^t$, if $(s+t)\leq g\mytiny{(}k,t\mytiny{)}$, then the probability of winning is $w \leq 2^{-s}$.
We show that for $f\mytiny{(}l\mytiny{)}$ in (\ref{eq.(1)}) with suitably chosen parameters $d,L^*,\tau_{low},\tau_{up},\gamma,h,$ and $p$,

\begin{equation*}
\begin{aligned}
g\mytiny{(}k,t\mytiny{)} = \Theta(k)
\end{aligned}
\end{equation*}
and if we measure $T_{bud}$ in terms of seconds, then $g\mytiny{(}k,t\mytiny{)}$ needs to be replaced by $[g\mytiny{(}k,t\mytiny{)} - \log k]$ which maintains the $\Theta(k)$ asymptotics. 

The analysis in this appendix teaches that if an adversary is successful in practice, then either the defender initially learns too slowly or it cannot reach a large enough probability of successful detection $f\mytiny{(}l\mytiny{)}$ no matter how many malicious payloads are known and can be learned from.

%%%%%% CHECKED: SO FAR SO GOOD %%%%%%

\subsection{Probability of Winning}

In order to analyze the probaility of winning, i.e., the adversary reaching a state $(k,L)$ for some $L$, we investigate the shape of a typical sequence of transitions (i.e., a path) through the Markov model. We define $t(i,l)$ as the total number of self-loops, i.e., transitions with probability $m_1(l)$ from the state $(i,l)$ back to itself. We notice that


\begin{equation}\label{eq.pois}
\begin{aligned}
Prob(t(i,l)=u) = m_1(l)^{u}(1-m_1(l))
\end{aligned}
\end{equation}

%is defined as a Poisson process. Fig. \ref{fig.samplePath} depicts a typical path from $(0,0)$ to $(k,L)$ without showing any self-loops where in this example $(k=18,L=22)$.
is defined as a Poisson process. Fig. \ref{fig.samplePath} depicts a typical path from $(0,0)$ to $(k,L)$ without showing any self-loops.
 	\begin{figure}[h!]
	\begin{center}
		\scalebox{0.50}
		{\includegraphics{samplePath}}%Transf
%		\caption{A sample path toward the winning state in which $k=18$ and the maximum level reached by the adversary is $L =22$}
		\caption{A sample path toward the winning state without depicting the self-loops at each state $(i,l)$ in the path}
		\label{fig.samplePath}
	\end{center}
\end{figure}
%\saeed{Missing figure: a typical path}

Along with a typical path, we see horizontal, diagonal, and vertical transitions toward the winning state. For $(i,l) \in~ path$ we have $t(i,l)$ self-loops after which the path exits $(i,l)$ along with a horizontal, diagonal or vertical transition (see (\ref{eq.pois})).
Given that $(i,l)$ does not continue with anothoer self-loop we have 

\begin{equation}
\begin{aligned}
	Prob(horizontal~transition) &= Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i+1,l\mytiny{)}|no~self\mymathhyphen loop)\\
	&= \frac{m_2(l)}{1-m_1(l)}\\
	Prob(diagonal~transition) &= Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i+1,l+1\mytiny{)}|no~self\mymathhyphen loop)\\
&= \frac{m_3(l)}{1-m_1(l)},~and\\
	Prob(vertical~transition) &= Prob(\mytiny{(}i,l\mytiny{)}\rightarrow\mytiny{(}i,l+1\mytiny{)}|no~self\mymathhyphen loop)\\
&= \frac{m_4(l)}{1-m_1(l)}.\\
\end{aligned}
\end{equation}

Let us define $g_l$ as the number of states at each level $l$ (i.e., the number of states within the path with the same level) $(i,l) \in ~ path$, and
  \begin{equation}
b_l=
\begin{cases}
0, & \text{if}\ level~ l~ is~ entered~ via~ a~ vertical~ transition \\
1, & \text{if}\ level ~l ~is~ entered ~via~ a ~diagonal~ transition
\end{cases}
\end{equation}
This does not define $b_0$. In general $g_l \geq 1$ for all $0 \leq l \leq L$.
Note that the length of the path, i.e., the total number of transitions without self-loops, is equal to

%\begin{equation*}
%\begin{aligned}
%k+L- \sum_{a=1}^{L} b_a,
%\end{aligned}
%\end{equation*}
\begin{equation*}
\begin{aligned}
k+L- B,
\end{aligned}
\end{equation*}
where $ B = \sum_{a=1}^{L} b_a$ is the total number of diagonal transitions. Therefore, the total number of vertical transitions is equal to $(L-B)$, and the number of horizontal transitions is equal to
\begin{equation}\label{eq.4}
\begin{aligned}
\sum_{a=0}^{L} (g_a-1)= k - B,
\end{aligned}
\end{equation}
\saeed{Did we start from k=1 or 0, if from 0, the above is correct but you need to check all the following summations' bounds and change it from $k-B-1$ to $k-B$!}
and, 
\begin{equation*}
\begin{aligned}
k =  \sum_{a=0}^{L-1} (g_a-1 + b_{a+1})+(g_L-1),
\end{aligned}
\end{equation*}

%in which the number of horizontal transitions is equal to




%and the total number of vertical transitions is
%\begin{equation*}
%\begin{aligned}
%L - \sum_{a=1}^{L} b_a,
%\end{aligned}
%\end{equation*}

%and the number of diagonal transitions is 
% \begin{equation*}
% \begin{aligned}
% \sum_{a=1}^{L} b_a.
% \end{aligned}
% \end{equation*}
 
 Finally, the path enters level $l$ at $i =i_l$ with 
 
  \begin{equation*}
 \begin{aligned}
 i_l = \sum_{a=0}^{l-1} (g_a-1 + b_{a+1})
 \end{aligned}
 \end{equation*}
 where $i_L + g_L = k$ by  (\ref{eq.4}).
 
 \saeed{if we are counting from 0 the above should be $i_L +g_L =k+1$}
 
\begin{lemma}
 The probability of a path from $(0,0)$ toward $(k,L)$ with self-loops at $(k,L)$ till the moment the path is ready to leave $(k,L)$, in which the path is represented by $g_0,\dots,g_L,b_1,\dots,b_L$, and the function $t(i,l)$ is 

\begin{eqnarray}\label{eq.5}
Pr(path)&=& \prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg).\nonumber\\
&& \prod_{l=0}^{L} \bigg( \frac{m_2(l)}{1-m_1(l)}\bigg)^{g_l-1}.\nonumber\\
& & \prod_{l=0}^{L}\prod_{i=0}^{g_l-1}m_1(l)^{t(i_l+i,l)}(1-m_1(l))
\end{eqnarray}
\end{lemma}

 
%\saeed{i should start from 1 not 0}
\begin{proof}
\textbf{(Base case)}
For  $(k,L)$ = (0,0), we have $g_0 =1$ and (\ref{eq.5}) would be $m_1(0)^{t(0,0)}(1-m_1(0))$ which it holds trivially.
 
\textbf{(Hypothesis)} Suppose the claim holds for paths to $(k',L')$ where $0\leq k'\leq k$ and $0\leq L'\leq L$ such that $(k',L') \neq (k,L)$. Consider a path to (k,L). This path will first enter $(k',L') = (k-1,L)$, $(k',L')=(k-1,L-1)$, or $(k',L')=(k,L-1)$ before transitioning to $(k,L)$. Let the subpath to $(k',L')$ be represented by $b_l',g_l',i_l'$ and $t'(i,l) = t(i,l)$, where $i'_{L'} + g'_{L'} = k'$.

\textbf{Case $(k',L')=(k-1,L)$:} We multiply (\ref{eq.5}) for $(k-1,L)$ with the probability of  a self-loop in $(k-1,L)$ and the transition probability from $(k-1,L)$ toward $(k,L)$:


\begin{eqnarray*}
	m_1(L)^{t(k-1,L)}.m_2(L)
&=& [m_1(L)^{t(k-1,L)}.(1-m_1(L))].(\frac{m_2(L)}{1-m_1(L)})\\
&=& [m_1(L)^{t(i'_{L}+g'_L,L)}.(1-m_1(L))].(\frac{m_2(L)}{1-m_1(L)})
\end{eqnarray*}
Notice that $b_l=b'_l$ and $g_l = g'_l$ for $0\leq l \leq L-1$, and,
$b_L = b'_L$, $g_L = g'_L+1$, i.e., $i'_{L}+g'_{L} = i_L + g_L -1$.
Hence, (\ref{eq.5}) holds for the path to $(k,L)$.

\textbf{Case $(k',L')=(k-1,L-1)$:} Now (\ref{eq.5}) is multiplied with a self-loop in $(k-1,L-1)$ and a transition $(k-1,L-1)$ toward $(k,L)$. We have 

\begin{eqnarray*}
	m_1(L-1)^{t(k-1,L-1)}.m_3(L-1)
	&=& [m_1(L-1)^{t(k-1,L-1)}.(1-m_1(L-1))].\\& &
	(\frac{m_3(L-1)}{1-m_1(L-1)})\\
	&=& [m_1(L-1)^{t(i'_{L-1}+g'_{L-1},L-1)}.(1-m_1(L-1))].\\& &
	[b_L\frac{m_3(L-1)}{1-m_1(L-1)} + (1-b_L)\frac{m_4(L-1)}{1-m_1(L-1)}]
\end{eqnarray*}

with $b_L=1$, $g_L =0$, $g_{L-1}=g'_{L-1}+1$ and all other $b_l = b'_l$, $g_l=g'_l$. Hence, $i'_{L-1} + g'{L-1} = i_{L-1} + g_{L-1} - 1$.
Hence, (\ref{eq.5}) holds for the path to $(k,L)$.
%\saeed{Unclear equation see page 5, analysis 3}

\textbf{Case $(k',L')=(k,L-1)$:} Now, (\ref{eq.5}) is multiplied with a self-loop in $(k,L-1)$ and a transition from $(k,L-1)$ to $(k,L)$:
\begin{eqnarray*}
	m_1(L-1)^{t(k,L-1)}.m_4(L-1)
	&=& [m_1(L-1)^{t(k,L-1)}.(1-m_1(L-1))].\\& &
	(\frac{m_4(L-1)}{1-m_1(L-1)})\\
	&=& [m_1(L-1)^{t(i'_{L-1}+g'_{L-1},L-1)}.(1-m_1(L-1))].\\& &
	[b_L\frac{m_3(L-1)}{1-m_1(L-1)} + (1-b_L)\frac{m_4(L-1)}{1-m_1(L-1)}]
\end{eqnarray*}

with $b_L = 0$, $g_L = 0$, $g_{L-1} = g'_{L-1}+1$ and all other $b_l=b'_l$, $g_l=g'_l$. Hence, $i'_{L-1}+g'_{L-1} = i_{L-1} + g_{L-1}-1$. Therefore, (\ref{eq.5}) holds for the path to $(k,L)$.
\qed
\end{proof}



\saeed{analysis4 starts from here}

%As noted above, the length of the path toward $(k,L)$ is equal to 
%\begin{equation*}
%\begin{aligned}
%k+L-B,
%\end{aligned}
%\end{equation*}
%where $B = \sum_{l=1}^{L} b_{l}$. 

Suppose there is a limited number of transitions $T_{bud}$ one can use to reach $(k,L)$. Then the probability of reaching $(k,L)$ within that time budget is equal to the sum of $Prob(path~to~(k,L))$ over all possible paths satisfying 

\begin{equation*}
\begin{aligned}
k+L-B+T \leq T_{bud}.
\end{aligned}
\end{equation*}
where $T$ represents the total number of self-loops in the path and is defined as $T = \sum_{l=0}^{L}t_l$ in which $t_l = \sum_{i=0}^{g_l-1} t(i_l+i,l)$ is the number of self-loops happening at a fixed level $l$.

In order to analyze this probability, we introduce $p(k,L,T_b)$ as the probability of the Markov model reaches state $(k,L)$ within $T_b$ transitions and after -possibly zero- self-loops, it is ready to transit away from $(k,L)$.
Now notice that the probability $w$ of reaching any winning state $(k,L)$ for some $L\geq 0$ within $T_{bud}$ transitions is equal to:

\begin{eqnarray} \label{eq.w}
 w(k, . ,T_{bud})&=&	\sum_{L\geq 0} p(k-1,L,T_{bud}-1).	 \{\frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\}
\end{eqnarray}

This formula corresponds to Fig. \ref{fig.LthTerm}.

 	\begin{figure}[h!]
	\begin{center}
		\scalebox{0.50}
		{\includegraphics{Lth_term.pdf}}%Transf
		%		\caption{A sample path toward the winning state in which $k=18$ and the maximum level reached by the adversary is $L =22$}
		\caption{???}
		\label{fig.LthTerm}
	\end{center}
\end{figure}

The formula for $w$ simply considers all the possible paths toward the state $(k-1,L)$ within $(T_{bud} -1)$ transitions and a single final transition via $m_2(L)$ or $m_3(L)$ toward the winning state. This enables us to avoid counting self-loops in states $(k,L)$ and transitions from $(k,L-1)$ to $(k,L)$ (since state $i=k$ was already reached). Notice that we are interested in the probability of entering state $(k,L)$  and the time it takes to reach there \emph{for the first time} and that is why we are not interested in counting self-loops or vertical moves at $(k,L)$.

\begin{claim}
	Given our analysis for $Prob(path)$ (see (\ref{eq.5})) and bearing in mind that $k,L,$ and $T_b$ are fixed, we need to consider all the possible $B$ and $T$. Therefore, we get:
	\begin{subequations}
		\begin{eqnarray}\label{eq.ABC}
		p(k,L,T_b) &= &
		\sum_{\substack{B,T s.t.\\
				k+L-B+T\leq T_b}}\nonumber\\& &
		{ 
			\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ \label{eq.a}
					\sum_{l=1}^{L}b_l=B}}
			\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
		}\\& &
		{	\sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\ \label{eq.b}
					\sum_{l=0}^{L}(g_l-1)=k-1-B}}
			\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
		}\\& &
		{
			\sum_{\substack{t_0,\dots,t_L s.t.\\ \label{eq.c}
					\sum_{l=0}^{L}t_l=T}}
			\prod_{l=0}^{L} 
			{	\sum_{\substack{t(i_l,l),\dots,t(i_l+g_l-1,l) \\
						s.t.\sum_{i=0}^{g_l-1}t(i_l+i,l)=t_l}}
				\prod_{i=0}^{g_l-1} 
				m_1(l)^{t(i_l+i,l)}(1-m_1(l))
			}
		}
		\end{eqnarray}
	\end{subequations}
\end{claim}

\begin{proof}
	\textbf{(Base case)}
	For  $(k,L,T_{bud})$ = (0,0,0), we have $g_0 =1$ and we have $m_1(0)^{t(0,0)}(1-m_1(0))$ since the time budget is $0$ we get $(1-m_1(0))$ which it holds trivially.
	
	\textbf{(Hypothesis)}  Suppose the claim holds for paths to $(k',L')$ within $T'_{b})$ steps where $0\leq k'\leq k$, $0\leq L'\leq L$, and $0\leq T'_{b}\leq T_{b}-1$. Note that since there exist a limited time budget available for the adversary to reach the final state and it takes at least one transition for the adversary from $(k',L')$ to $(k,L)$, such that $(k',L') \leq (k,L)$ therefore we have $T'_b \leq T_b -1$.
	Consider a path to $(k,L)$ within $T'_b = T_b -1$ transitions. This path will first enter $(k',L') = (k-1,L)$, $(k',L')=(k-1,L-1)$, $(k',L')=(k,L-1)$, or $(k,L)=(k,L)$ in $T_b -1$ transitions before transitioning to $(k,L)$. Let the subpath to $(k',L')$ be represented by $b'_l,g'_l,i'_l$ and $t'(i,l) = t(i,l)$, where $i'_{L'} + g'_{L'} = k'$.
	
	\textbf{Case $(k',L',T'_b)=(k-1,L,T_b-1)$:} We multiply the above expression for $(k-1,L,T_b-1)$ with the probability of a transition from $(k-1,L)$ toward $(k,L)$ in a single step (i.e., a horizontal transition) conditiong on the fact that no more self-loops happen:
	\begin{eqnarray*}
(\frac{m_2(L)}{1-m_1(L)})
	\end{eqnarray*}
	Notice that $b_l=b'_l$ and $g_l = g'_l$ for $0\leq l \leq L-1$, and,
	$b_L = b'_L$, $g_L = g'_L+1$, i.e., $i'_{L}+g'_{L} = i_L + g_L -1$.
	Hence, the expression holds for the path to $(k,L)$.

\textbf{Case $(k',L',T'_b)=(k-1,L-1,T_b-1)$:} We multiply the above expression for $(k-1,L-1,T_b-1)$ with the probability of a transition from $(k-1,L-1)$ toward $(k,L)$ in a single step (i.e., a diagonal transition) conditiong on the fact that no more self-loops happen:
\begin{eqnarray*}
	(\frac{m_3(L-1)}{1-m_1(L-1)})=[b_L\frac{m_3(L-1)}{1-m_1(L-1)} + (1-b_L)\frac{m_4(L-1)}{1-m_1(L-1)}]
\end{eqnarray*}

with $b_L=1$, $g_L =0$, $g_{L-1}=g'_{L-1}+1$ and all other $b_l = b'_l$, $g_l=g'_l$. Hence, $i'_{L-1} + g'{L-1} = i_{L-1} + g_{L-1} - 1$.
Hence, the expression holds for the path to $(k,L)$.
	
\textbf{Case $(k',L',T'_b)=(k,L-1,T_b-1)$:} We multiply the above expression for $(k,L-1,T_b-1)$ with the probability of a transition from $(k,L-1)$ toward $(k,L)$ in a single step (i.e., a vertical transition) conditiong on the fact that no more self-loops happen:
\begin{eqnarray*}
	(\frac{m_4(L-1)}{1-m_1(L-1)})=
	[b_L\frac{m_3(L-1)}{1-m_1(L-1)} + (1-b_L)\frac{m_4(L-1)}{1-m_1(L-1)}]
\end{eqnarray*}

with $b_L = 0$, $g_L = 0$, $g_{L-1} = g'_{L-1}+1$ and all other $b_l=b'_l$, $g_l=g'_l$. Hence, $i'_{L-1}+g'_{L-1} = i_{L-1} + g_{L-1}-1$. Therefore, the expression holds for the path to $(k,L)$.

\textbf{Case $(k',L',T'_b)=(k,L,T_b-1)$:} We multiply the above expression for $(k,L,T_b-1)$ with the probability of a single self-loop at $(k,L)$:
\begin{eqnarray*}
?
\end{eqnarray*}
with???
	\qed
\end{proof}
%\begin{subequations}
%\begin{eqnarray}\label{eq.ABC}
%p(k,L,T_b) &= &\nonumber\\& &
%\sum_{\substack{B,T s.t.\\
%		k+L-B+T\leq T_b}}\nonumber\\& &
%{ 
%	\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\
%			\sum_{l=1}^{L}b_l=B}}
%				\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
%			}\\& &
%				{	\sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\
%						\sum_{l=0}^{L}(g_l-1)=k-1-B}}
%				\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
%}\\& &
%{
%	\sum_{\substack{t_0,\dots,t_L s.t.\\
%		\sum_{l=0}^{L}(t_l)=T}}
%\prod_{l=0}^{L} 
%{	\sum_{\substack{t(i_l,l),\dots,t(i_l+g_l-1,l) \\
%		s.t.\sum_{i=0}^{g_l-1}t(i_l+i,l)=t_l}}
%\prod_{i=0}^{g_l-1} 
%m_1(l)^{t(i_l+i,l)}(1-m_1(l))
%}
%}
%\end{eqnarray}
%\end{subequations}




Notice that (\ref{eq.c}) is equal to\footnote{This simply can be noticed by representing each self-loop at a fixed level by $0$ and the event that the path exits the $(i,l)$ state but remains on the same level, i.e., $(i+1,l)$, by a $1$. The problem then can be translated into choosing $(g_l-1)$ ones (as the total number of states at the same level) out of the total number of zeros and ones $(t_l+g_l-1)$ where $t_l$ is the total number of self-loops happen at the same level} 

	\begin{eqnarray*}
{
	\sum_{\substack{t_0,\dots,t_L s.t.\\ 
			\sum_{l=0}^{L}t_l=T}}
	\prod_{l=0}^{L} 
	{{t_l+g_l-1 \choose g_l-1} m_1(l)^{t_l}(1-m_1(l))^{g_l}
	}
}
\end{eqnarray*}

As a check, if we sum  (\ref{eq.c}) for $T=0$ to $T= \infty$, then this sums to $1$ (since (\ref{eq.c}) models self-loops as a Poisson process at each $(i_l+i,l)$).

So, for $L\geq1$, 

	\begin{eqnarray}
	\lefteqn{\sum_{k\geq 0}p(k,L,\infty)(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)}) = }\nonumber\\ & & \sum_{k\geq 1}p(k,L,\infty)(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})  \nonumber\\
	&=& \sum_{k\geq 1}{\sum_{B}(\ref{eq.a})(\ref{eq.b})(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})} \nonumber\\
	&=& \sum_{k\geq 1}{\sum_{B=0}^{k-1}(\ref{eq.a})(\ref{eq.b})(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})} \nonumber\\
	&=& \sum_{B=0}^{\infty}{\sum_{k=B+1}^{\infty}(\ref{eq.a})(\ref{eq.b})(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})} \label{eq.6}
	\end{eqnarray}

Notice that

	\begin{eqnarray*}
	\sum_{k=B+1}^{\infty}{(\ref{eq.b})} &=&
	\sum_{k=B+1}^{\infty}
		{	\sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\
				\sum_{l=0}^{L}(g_l-1)=k-1-B}}
		\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
	}\\
&=& \sum_{g'_0,\dots,g'_L \geq 0}\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l}\\
&=&	\prod_{l=0}^{L} \sum_{g'_l\geq 0}\bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l} 
= \prod_{l=0}^{L}\frac{1}{1-\frac{m_2(l)}{1-m_1(l)}} = \prod_{l=0}^{L} \frac{1-m_1(l)}{1-m_1(l)-m_2(l)}\\
&=& \prod_{l=0}^{L} \frac{1-m_1(l)}{m_3(l)+m_4(l)}
	\end{eqnarray*}
And 
	\begin{eqnarray*}
\lefteqn{\sum_{B=0}^{\infty}{(\ref{eq.a})\{\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)}\}} = }	 \\
& &	\sum_{B=0}^{\infty}  
{ 
	\sum_{\substack{b_1,\dots,b_L\in\{0,1\}\\ 
			s.t.\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
}
\{\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)}\}\\
&=& { 
	\sum_{b_1,\dots,b_L\in\{0,1\}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
}
\{\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)}\}\\
&=& \prod_{l=0}^{L} \bigg(\frac{m_3(l)}{1-m_1(l)} + \frac{m_4(l)}{1-m_1(l)} \bigg)
\end{eqnarray*}


%\begin{align*}
%	\sum_{B=0}^{\infty}{(\ref{eq.a})(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})} &= 
%	\sum_{B=0}^{\infty} 
%	{ 
%		\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
%				\sum_{l=1}^{L}b_l=B}}
%		\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
%	}.\\
%	(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})\\
%	&= { 
%		\sum_{b_1,\dots,b_L\in\{0,1\}}
%		\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
%	}.\\
%	(\frac{m_3(L)}{1-m_1(L)} + \frac{m_4(L)}{1-m_1(L)})\\
%	&= \prod_{l=0}^{L} \bigg(\frac{m_3(l)}{1-m_1(l)} + \frac{m_4(l)}{1-m_1(l)} \bigg)
%\end{align*}
Therefore, we get (\ref{eq.6}) equals $1$ which fits Fig. \ref{fig.LthTerm}.


We are not able to easily verify that $w(k,\infty) =1$, in a similar way. This needs to be done by induction.
If $m_1,m_2,m_3,m_4$ are independent of $l_i$, an easy verification of $w(k,\infty)=1$ is possible.

\begin{eqnarray*}
\sum_{L\geq 0}p(k-1,L,\infty)(\frac{m_2(L)}{1-m_1(L)} + \frac{m_3(L)}{1-m_1(L)})&= & 
\sum_{L\geq 0}\sum_{B}(\ref{eq.a})(\ref{eq.b})(\frac{m_2(L)}{1-m_1(L)} + \frac{m_3(L)}{1-m_1(L)})\\
&=& \sum_{B=0}^{k-1}\sum_{L\geq B}(\ref{eq.a})(\ref{eq.b})(\frac{m_2(l)}{1-m_1(l)} + \frac{m_3(l)}{1-m_1(l)})\\
\end{eqnarray*}

Notice that

\begin{eqnarray*}
	(\ref{eq.b}) &=& {	
		\sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\ 
				\sum_{l=0}^{L}(g_l-1)=k-1-B}}
		\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
	}\\
&=& \sum_{\substack{g_0\geq 1,\dots,g_L\geq 1 s.t.\\ 
		\sum_{l=0}^{L}(g_l-1)=k-1-B}}
 \bigg(\frac{m_2}{1-m_1} \bigg)^{k-1-B}\\
&=& {k-1-B+L \choose L}\bigg(\frac{m_2}{1-m_1} \bigg)^{k-1-B}
\end{eqnarray*}
%\saeed{check the above formula more specifically $m_2,m_3$}
moreover, 
\begin{eqnarray*}
	(\ref{eq.a}) &=& {	
	\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
}\\
&=& \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
		\sum_{l=1}^{L}b_l=B}}  \bigg( \frac{m_3}{1-m_1}\bigg)^{B} \bigg(\frac{m_4}{1-m_1} \bigg)^{(L-B)}\\
	&=& {L \choose B}\bigg( \frac{m_3}{1-m_1}\bigg)^{B}  \bigg(\frac{m_4}{1-m_1} \bigg)^{L-B}
\end{eqnarray*}
%\begin{eqnarray}\label{eq.5}
%&=& \prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg).\nonumber\\
%&& \prod_{l=0}^{L} \bigg( \frac{m_2(l)}{1-m_1(l)}\bigg)^{g_l-1}.\nonumber\\
%& & \prod_{l=0}^{L}\prod_{i=0}^{g_l-1}m_1(l)^{t(i_l+i,l)}(1-m_1(l))\nonumber
%\end{eqnarray}

Notice that
\begin{equation*}
	{k-1-B+L \choose L}{L \choose B} = {k-1+L-B \choose L-B}{k-1 \choose B}
\end{equation*}

By substituting $F=L-B$ we have:

\begin{equation*}
\sum_{L\geq B}(\ref{eq.a})(\ref{eq.b})=\sum_{F\geq 0}{k-1+F \choose F}\bigg(\frac{m_4}{1-m_1} \bigg)^{F}{k-1 \choose B}\bigg( \frac{m_2}{1-m_1}\bigg)^{k-1-B}\bigg( \frac{m_3}{1-m_1}\bigg)^{B}
\end{equation*}

Therefore,

\begin{eqnarray*}
\sum_{B=0}^{k-1}\sum_{L\geq B}(\ref{eq.a})(\ref{eq.b})&=&
\sum_{F\geq 0}{k-1+F \choose F}\bigg(\frac{m_4}{1-m_1} \bigg)^{F}\bigg( \frac{m_2+m_3}{1-m_1}\bigg)^{k-1} \\
&=& {
	\sum_{F\geq 0} 
	\sum_{\substack{f_1,\dots,f_k s.t.\\ 
			\sum f_i=F}}
		 \prod_{i=1}^{k} \bigg(\frac{m_4}{1-m_1}\bigg)^{f_i} \bigg(\frac{m_2+m_3}{1-m_1} \bigg)^{k-1}
	}\\
&=& \bigg( \prod_{i=1}^{k} \sum_{f_i=0}^{\infty}(\frac{m_4}{1-m_1})^{f_i} \bigg)(\frac{m_2+m_3}{1-m_1})^{k-1}\\
&=& \bigg(\frac{1}{1-\frac{m_4}{1-m_1}}\bigg)^{k} \bigg(\frac{m_2+m_3}{1-m_1}\bigg)^{k-1} = \frac{1-m_1}{m_2+m_3}
\end{eqnarray*}

and after multipling with $(\frac{m_2}{1-m_1} + \frac{m_3}{1-m_1})$ we get indeed $1$.

Note that if $(1-f(l)) = \tau$, then $m_1,m_2,m_3$ and $m_4$ are independent of $l$. In fact, the Markov model reduces to Fig. \ref{fig.reducedMarkovModel}.

\begin{figure}[t]
	\centering
	\begin{tikzpicture}
	\tikzset{
		>=stealth',
		node distance=3cm and 3cm ,on grid,
		every text node part/.style={align=center},
		state/.style={minimum width=1.5cm,
			%    		font=\small,
			draw,
			circle},
	}
	% Add the states
	\node[state]             (c) {i};
	\node[state, right=of c] (r) {i\pp};
	%	\node[state, left=of c] (lose) {0};
	% Connect the states with arrows
	\draw[every loop]
	(c) edge[auto=left]  node {$m_{2}+m_3$} (r)
	%(r) edge[bend left, auto=right] node {0.7} (s)
	%(c) edge[loop above]             node {($1-p_i-f(.)$)} (c)
%	(c) edge[ auto=left] node {$m_3$} (rr)
%	(c) edge[auto=right] node {$m_4$} (b)
	(c) edge[loop above]             node {$m_1+m_4$} (c);
	%(d) edge[loop above]             node {} (d);
	\end{tikzpicture}
	\caption{Reduced Markov model of the game for a constant $(1-f(l))=\tau$}
	\label{fig.reducedMarkovModel}
\end{figure}

Within a budget $T_{bud}$ we reach $i=k$ with probability 

\begin{eqnarray}
\lefteqn{ \sum_{T=k}^{T_{bud}} {T-1 \choose k-1}(m_1+m_4)^{(T-1)-(k-1)}(m_2+m_3)^{k-1+1} =} \nonumber\\
 & & \sum_{T=k}^{T_{bud}} {T-1 \choose k-1}(m_1+m_4)^{T-k}(m_2+m_3)^{k}\nonumber\\
&=& \sum_{T-k=0}^{T_{bud}-k} {(T-k)+(k-1) \choose (T-k)}(m_1+m_4)^{T-k}(m_2+m_3)^{k} \nonumber\\
&=&  \sum_{i=0}^{T_{bud}-k} {i+(k-1) \choose i}(m_1+m_4)^{i}(m_2+m_3)^{k} \label{eq.7}
\end{eqnarray}

A lower bound on (\ref{eq.7}) can be derived as follows:

\begin{eqnarray*}
(\ref{eq.7}) &=&  \sum_{i=0}^{T_{bud}-k}
{\sum_{\substack{f_1,\dots,f_k s.t.\\ 
		\sum f_j=i}}
\prod_{j} (m_1+m_4)^{f_j}(m_2+m_3)^{k}
}\\
&=& \sum_{\substack{f_1,\dots,f_k s.t.\\ 
		\sum f_j\leq T_{bud}-k}}
\prod_{j} (m_1+m_4)^{f_j}(m_2+m_3)^{k}\\
&\geq& \sum_{f_1=0}^{(T_{bud}-k)/k}\dots\sum_{f_k=0}^{(T_{bud}-k)/k}\prod_{j}(m_1+m_4)^{f_j}(m_2+m_3)^{k}\\
&=& \prod_{j}\sum_{f_j=0}^{(T_{bud}-k)/k}(m_1+m_4)^{f_j}(m_2+m_3)^{k}\\
&=& \prod_{j=1}^{k}\frac{1-(m_1+m_4)^{T_{bud}/k}}{1-(m_1+m_3)}(m_2+m_3)^{k}\\
&=& [1-(m_1+m_4)^{T_{bud}/k}]^{k}\\
&\geq& 1-k(m_1+m_4)^{T_{bud}/k}
\end{eqnarray*}

This shows that $w\approx 1$ for relatively small $T_{bud}$ because $1-w \leq k(m_1+m_4)^{T_{bud}/k}$ which is exponentially small in $T_{bud}$. To push $w$ down to $0$, we need $(1-f(l))\rightarrow 0$ for $l\rightarrow \infty$.

%\saeed{check if $g_l \leftarrow g_l -1 ?$ in the folloing equations}

Let us analyze $w(k,T_{bud})$

%\begin{subequations}
%\end{subequations}
	\begin{eqnarray}
	w(k,T_{bud}) &= &\nonumber
	\sum_{\substack{L,B,T s.t.\\
			k+L-B+T\leq T_{bud}-1\\
		B\leq L,B\leq k-1}}\nonumber\\& &
	{ 
		\sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
				\sum_{l=1}^{L}b_l=B}}
		\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
	} \nonumber\\& &
	{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
				\sum_{l=0}^{L}g_l=k-1-B}}
		\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l}
	}\nonumber\\& &
	{\sum_{\substack{t_0,\dots,t_L s.t.\\ 
				\sum_{l=0}^{L}t_l=T}}
		\prod_{l=0}^{L} 
	 {t_l + g_l \choose g_l}m_1(l)^{t_l}(1-m_1(l))^{g_l+1}.
	 	}\label{eq.cc}\\ & &
	 \{\frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\}
\nonumber
	\end{eqnarray}
	
Notice that  $k+L-B+T \leq T_{bud}-1, B\leq L, B\leq k-1$, therefore we have
\begin{equation}\label{eq.9}
L\leq T_{bud}-1 , B\leq L, B\leq k-1, T\geq 0
\end{equation}

We define 
\begin{eqnarray}
\bar{w}(k,T_{bud}) &= &\nonumber
\sum_{L=0}^{T_{bud}-1}\sum_{B=0}^{\min{(L,k-1)}}\{\frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}\}.\nonumber\\ & &	
{ \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)
} \nonumber\\& &
{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g_l=k-1-B}}
	\prod_{l=0}^{L} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l} \label{eq.10}
}
\end{eqnarray}

By (\ref{eq.9}) and $\sum_{T\geq 0}{(\ref{eq.cc})}=1$,
we have $w(k,T_{bud}) \leq \bar{w}(k,T_{bud})$. 
Also notice that,  $k+L-B+T \leq T_{bud}-1, B\leq L, B\leq k-1$, 
$L+1 \leq \frac{T_{bud}}{e}$, $T\leq T_{bud}-(\frac{T_{bud}}{e})-k$,
$B\leq L$, $B\leq k-1$.
So, $w(k,T_{bud}) \geq \bar{w}(k,T_{bud}/e)$ with the sum terms multiplied with $\sum_{T=0}^{T_{bud}-(T_{bud}/e)-k}(\ref{eq.cc})$.

Remeber $e \leq T_{bud}/(L+1)$ (see line 3 of the following; also for line 5 see analysis for (\ref{eq.7}), for line 6 since $g_l \leq k-1$), so Note that 

\begin{eqnarray*}
\sum_{T=0}^{T_{bud}-(T_{bud}/e)-k}(\ref{eq.cc}) &=& 
\sum_{T=0}^{T_{bud}-(T_{bud}/e)-k}{ \sum_{\substack{t_0,\dots,t_L s.t.\\ 
			\sum t_l=T}}
	\prod_{l=0}^{L} 
	{t_l + g_l \choose g_l}m_1(l)^{t_l}(1-m_1(l))^{g_l+1}
}\\
&=& { \sum_{\substack{t_0,\dots,t_L s.t.\\ 
			\sum t_l\leq T_{bud}-(T_{bud}/e)-k}}
	\prod_{l=0}^{L} 
	{t_l + g_l \choose g_l}m_1(l)^{t_l}(1-m_1(l))^{g_l+1}
}\\
&\geq& \sum_{t_0=0}^{e-1-k}\dots\sum_{t_L=0}^{e-1-k}	\prod_{l=0}^{L} 
{t_l + g_l \choose g_l}m_1(l)^{t_l}(1-m_1(l))^{g_l+1}\\
&=& \prod_{l=0}^{L} \sum_{t_l=0}^{e-1-k} {t_l+g_l \choose g_l} m_1(l)^{t_l}(1-m_1(l))^{g_l}\\
&\geq& \prod_{l=0}^{L} \bigg( 1-(g_l+1)m_1(l)^{1+\frac{e-1-k}{1+g_l}} \bigg)\\ %see analysis for eq.7
&\geq& \prod_{l=0}^{L} \bigg( 1-(g_l+1)m_1(l)^{1+\frac{e-1-k}{k}} \bigg)\\ %g_l \leq k-1
&\geq& \prod_{l=0}^{L} \bigg( 1-k m_1(l)^{\frac{e-1}{k}} \bigg)\\ %g_l \leq k-1
&=& \prod_{l=0}^{T_{bud}/(e-1)} \bigg( 1-k m_1(l)^{\frac{e-1}{k}} \bigg)\\ 
&\geq&1- \sum_{l=0}^{T_{bud}/(e-1)}k m_1(l)^{\frac{e-1}{k}}\\
&=& 1- \sum_{l=0}^{T_{bud}/(e-1)}k [(1-\gamma)(1-(p+h)(1-f(l)))]^{\frac{e-1}{k}}\\
\end{eqnarray*}

Assuming $(1-f(l)) \rightarrow 0$ for $l \rightarrow \infty$, we can tightly lower bound this to

\begin{eqnarray*}
&\geq& 1- \sum_{l=0}^{T_{bud}/(e-1)}k (1-\gamma)^{\frac{e-1}{k}}\\
&=& 1- T_{bud}.\frac{k}{e}(1-\gamma)^{\frac{e-1}{k}}
\end{eqnarray*}
This proves that  $ \forall e, w(k,T_{bud})\geq \bar{w}(k,T_{bud}/e)(1- T_{bud}.\frac{k}{e}(1-\gamma)^{\frac{e-1}{k}})$.
 
As an example, $e= 1+ \frac{k\ln(T_{bud}.k/\epsilon)}{-\ln(1-\gamma)}$ gives $w(k,T_{bud})\geq \bar{w}(k,T_{bud}/e)(1-\epsilon)$. This shows that for an asymptotic analysis, which proves a statement like
$w(k,T_{bud}=k^{b})=p(k).\Theta(2^{-k})$ for some $p(k)\geq poly(k)$, it suffices to prove this statement for $\bar{w}$.
As we will now explain computation of $\bar{w}(k,T_{bud})$, it can be done in $\Theta(kT_{bud})$ time:

Essentially $\bar{w}(k,T_{bud})$ corresponds to Fig. \ref{fig.LthTerm} with $m_1'(l)=0,m_2'(l)=\frac{m_2(l)}{1-m_1(l)},m_3'(l)=\frac{m_3(l)}{1-m_1(l)}$, and $m_4'(l) = \frac{m_4(l)}{1-m_1(l)}$ which eliminates self-loops.

 	\begin{figure}[h!]
	\begin{center}
		\scalebox{0.40}
		{\includegraphics{SS_Tbud}}%Transf
		%		\caption{A sample path toward the winning state in which $k=18$ and the maximum level reached by the adversary is $L =22$}
		\caption{???}
		\label{fig.marten}
	\end{center}
\end{figure}


The figure shows that $\bar{w}(k,T_{bud})$ can be computed in $\Theta(kT_{bud})$ iterations. This allows fast simulation of the Markov model for various functions $(1-f(l))$, and parameters $p,\gamma$, and $h$.

In definition (\ref{eq.10}) of $\bar{w}(k,T_{bud})$ we use 

\begin{equation*}
\begin{aligned}
\frac{m_2(l)}{1-m_1(l)} &= \frac{(1-\gamma)p(1-f(l))}{\gamma+(1-\gamma)(p+h)(1-f(l))}=(1-\gamma)\alpha(l),\\
\frac{m_3(l)}{1-m_1(l)} &=  \frac{\gamma p (1-f(l))}{\gamma+(1-\gamma)(p+h)(1-f(l))} = \gamma \alpha(l),~and\\
\frac{m_4(l)}{1-m_1(l)} &= \frac{\gamma+(1-f(l))[h-\gamma(h+p)]}{\gamma+(1-\gamma)(p+h)(1-f(l))}\\
&= 1 - \frac{(1-f(l))[(1-\gamma)(p+h)-(h-\gamma(h+p))]}{\gamma+(1-\gamma)(p+h)(1-f(l))}\\
&= 1 - \frac{p(1-f(l))}{\gamma+(1-\gamma)(p+h)(1-f(l))} = 1 - \alpha(l),
\end{aligned}
\end{equation*}
where $\alpha(l) = \frac{p(1-f(l))}{\gamma+(1-\gamma)(p+h)(1-f(l))}$. The above form can be used in a dynamic program which takes $\alpha(l)$ as input rather than the separate $f(l),p,h,$ and $\gamma$. 

Notice that 
\begin{equation*}
\frac{m_2(l)}{1-m_1(l)} \leq \frac{(1-\gamma)pd}{\gamma} (\frac{1-f(l)}{d}) \leq \frac{(1-\gamma)pd}{\gamma} \sqrt{\frac{1-f(l)}{d}}
\end{equation*}

for $d$ such that $\forall l, (1-f(l))\leq d$.
Also,
\begin{equation*}
\begin{aligned}
\frac{m_3(l)}{1-m_1(l)} \leq  pd \sqrt{\frac{1-f(l)}{d}}^2, ~ and\\
\frac{m_4(l)}{1-m_1(l)} \leq 1- pd \sqrt{\frac{1-f(l)}{d}}^2.
\end{aligned}
\end{equation*}

We define $\beta_(l) = \sqrt{\frac{1-f(l)}{d}}$ and upperbound (\ref{eq.10}) as follows:

\begin{eqnarray*}
\bar{w}(k,T_{bud}) &\leq &\nonumber
\sum_{L=0}^{T_{bud}-1}\sum_{B=0}^{\min{(L,k-1)}} (1+ \frac{1-\gamma}{\gamma})pd \beta(L)^2\\ & &	
{ \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}pd \beta(l)^2 + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
} \nonumber\\& &
{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g_l=k-1-B}}
	\prod_{l=0}^{L} \bigg(\frac{1-\gamma}{\gamma} pd \beta(l)\bigg)^{g_l} 
}
\end{eqnarray*}

\saeed{From Marten's notes: Notice that this bounding eliminates the role of h. Simulations are needed to find out the effect of $h$.}

Define $\theta \geq \frac{1-\gamma}{\gamma}$. Considering that $\sum{b_l}=B$ (for line 3 of the following) and by defining $b_{L+1}=0$ (for line 2) we have,

\begin{eqnarray*}
	{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
				\sum_{l=0}^{L}g_l=k-1-B}}
		\prod_{l=0}^{L} \bigg(\frac{1-\gamma}{\gamma} pd \beta(l)\bigg)^{g_l} 
	} &\leq &
	{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g_l=k-1-B}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{g_l} 
} \\
&\leq &
	{	\sum_{\substack{g_0,\dots,g_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g_l=k-1-B}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{g_l + b_{l+1}}\prod_{l=0}^{L-1} \bigg(\theta pd \beta(l)\bigg)^{-b_{l+1}}
} \\
&\leq &
	{	\sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g'_l=k-1}}
	\prod_{l=0}^{L} \bigg(\theta pd \beta(l)\bigg)^{g'_l}\prod_{l=0}^{L-1} \bigg(\theta pd \beta(l)\bigg)^{-b_{l+1}}
} \\
&=& (\theta p d )^{k-1}{\sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g'_l=k-1}}
	\prod_{l=0}^{L} \beta(l)^{g'_l}\prod_{l=0}^{L-1} \bigg(\theta pd \beta(l)\bigg)^{-b_{l+1}}
} \\
\end{eqnarray*}

We derive


\begin{eqnarray*}
& & \sum_{B=0}^{L}{ \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}pd \beta(l)^2 + (1-b_{l+1})(1-pd \beta(l)^2) \bigg) \prod_{l=0}^{L-1} \bigg(\theta pd \beta(l)\bigg)^{-b_{l+1}}
} \\
&= &\sum_{B=0}^{L}{ \sum_{\substack{b_1,\dots,b_L\in\{0,1\} s.t.\\ 
			\sum_{l=1}^{L}b_l=B}}
	\prod_{l=0}^{L-1} \bigg( b_{l+1}\frac{\beta(l)}{\theta} + (1-b_{l+1})(1-pd \beta(l)^2) \bigg)
} \\
&= &  	\prod_{l=0}^{L-1} \bigg( \frac{\beta(l)}{\theta} + (1-pd \beta(l)^2) \bigg)\\
&= & 	\prod_{l=0}^{L-1} \bigg( 1+\beta(l) (\frac{1}{\theta} - pd \beta(l)) \bigg)\\
&\leq &  	\prod_{l=0}^{L-1} \bigg( 1+\beta(l)/\theta \bigg)
\end{eqnarray*}

We also derive that 

\begin{eqnarray*}
{	\sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
				\sum_{l=0}^{L}g'_l=k-1}}
		\prod_{l=0}^{L} \beta(l)^{g'_l}
	}
&= & {	\sum_{\substack{g'_0,\dots,g'_L\geq 0 s.t.\\ 
			\sum_{l=0}^{L}g'_l=k-1}}
	\prod_{l=0}^{L} \bigg( c_l \beta(l)^{g'_l} + (1-c_l) \bigg)
}\\
&\leq & {	\sum_{\substack{c_0,\dots,c_L\in \{0,1\} 1 s.t.\\ 
			\sum_{l=0}^{L}(c_l)=k-1}}
	\prod_{l=0}^{L} \bigg( c_l \sum_{g=1}^{\infty}{\beta(l)^{g}} + (1-c_l) \bigg)
}\\
&= & {	\sum_{\substack{c_0,\dots,c_L\in \{0,1\} 1 s.t.\\ 
			\sum_{l=0}^{L} c_l=k-1}}
	\prod_{l=0}^{L} \bigg( c_l \frac{\beta(l)}{1-\beta(l)} + (1-c_l) \bigg)
}\\
&\leq & \prod_{l=0}^{L} \bigg( \frac{\beta(l)}{1-\beta(l)} + 1 \bigg) = \prod_{l=0}^{L} \bigg( \frac{1}{1-\beta(l)}\bigg)
\end{eqnarray*}
where $c_l =1$ if $g'_l \neq 0 $ and $c_l =0$ if $g'_l = 0$.

Combining all the equations gives for $\frac{1-\gamma}{\gamma} \leq \theta$ and $\frac{1-f(l)}{d} = \beta(l) < 1$,

\begin{eqnarray*}
	\bar{w}(k,T_{bud}) &\leq &\nonumber
	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k}(1+\frac{1}{\theta})\frac{\beta(L)^2}{1-\beta(L)}\prod_{l=0}^{L-1} \frac{(1+\beta(l)/\theta)}{(1-\beta(l))}\\
	&\leq&  	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k}(1+\frac{1}{\theta})\prod_{l=0}^{L-1} \frac{(1+\beta(l)/\theta)}{(1-\beta(l))}\\
\end{eqnarray*}
We derive:

\begin{eqnarray*}
\prod_{l=0}^{L-1} \frac{(1+\beta(l)/\theta)}{(1-\beta(l))} &=& \sum_{l=0}^{L}[1+(1+\frac{1}{\theta})\frac{\beta(l)}{1-\beta(l)}]
\end{eqnarray*}

%\lemma{ $\prod_{a=0}^{A}(1+yB'(a)) \leq e^{y[B'(0)-B(0)+B(A-1)}$ for $B'(a)\geq 0$ and $B''(a)\leq 0$}
%\proof

\begin{lemma}\label{lemma.diri}
$\prod_{a=0}^{A}(1+yB'(a)) \leq e^{y[B'(0)-B(0)+B(A-1)]}$ for $B'(a)\geq 0$ and $B''(a)\leq 0$.
\end{lemma}
\begin{proof}
We find an upperbound of $\ln \prod_{a=0}^{A}(1+yB'(a)) = \sum_{a=0}^{A}\ln(1+yB'(a))$. Differentiating w.r.t. $y$ gives
\begin{eqnarray*}
	\sum_{a=0}^{A} \frac{1}{1+yB'(a)}. B'(a) &\leq& \sum_{a=0}^{A}B'(a) = B'(0)+\sum_{a=1}^{A}B'(a)\\
	&\leq& B'(0) + \int_{a=0}^{A-1} B'(a) da\\
	&=& B'(0) + B(A-1) - B(0)
\end{eqnarray*}
Also $\sum_{a=0}^{A}\ln(1+yB'(a))|_{y=0}=0=y.[B'(0)-B(0)+B(A-1)]|_{y=0}$. We conclude that $\sum_{a=0}^{A}\ln(1+yB'(a)) \leq y.[B'(0)-B(0)+B(A-1)]$. \qed
\end{proof}

We get:
\begin{eqnarray*}
	\bar{w}(k,T_{bud}) &\leq&
	\sum_{L=0}^{T_{bud}-1} [\theta p d]^{k}(1+\frac{1}{\theta}). e^{(\frac{1+\theta}{\theta})(B(L-1)+C)} \\
	&\leq& [\theta p d]^{k}(1+\frac{1}{\theta})e^{(\frac{1+\theta}{\theta})(B(T_{bud})+C)}. T_{bud}
\end{eqnarray*}
where, $C = B'(0)-B(0)$ and $\frac{\mathrm{d}B(x)}{\mathrm{d}x}=\frac{\beta(x)}{1-\beta(x)}$. Notice that the conditions of the lemma \ref{lemma.diri} are satisfied for a decreasing $\beta(x) = \sqrt{\frac{a-f(x)}{d}} \leq 1$.

Minimizing this upperbound with respect to $\theta \geq (1-\gamma)/\gamma$:

\begin{equation*}
\theta^{k} e^{(1/\theta).B[T_{bud}]} = e^{[k\ln{\theta}]+B[T_{bud}]/\theta}
\end{equation*}

Differentiating $k\ln{\theta} + B[T_{bud}]/\theta$ with respect to $\theta$:
\begin{equation*}
\frac{k}{\theta} - \frac{B[T_{bud}]}{\theta^2} = 0 \implies \theta = \frac{B[T_{bud}]}{k}
\end{equation*}

We obtain 

\begin{align}\label{eq.conditions}
\bar{w}(k,T_{bud}) \leq
\begin{cases}
[pd]^{k}e^{k\ln(\frac{B[T_{bud}]}{k})+k+B[T_{bud}]+kC/B[T_{bud}]+C}, & \text{if}\ B[T_{bud}]\geq \frac{k(1-\gamma)}{\gamma} \\
[\frac{1-\gamma}{\gamma}pd]^{k}\frac{1}{1-\gamma}e^{(B[T_{bud}]+d)/(1-\gamma)}.T_{bud}, & \text{otherwise}
\end{cases}
\end{align}


%\begin{numcases}{$\bar{w}(k,T_{bud}) \leq$}
%	$[pd]^{k}e^{k\ln(\frac{B[T_{bud}]}{k})+k+B[T_{bud}]+kC/B[T_{bud}]+C}$, & if $B[T_{bud}]\geq \frac{k(1-\gamma)}{\gamma}$\\
%	$[\frac{1-\gamma}{\gamma}pd]^{k}\frac{1}{1-\gamma}e^{(B[T_{bud}]+d)/(1-\gamma)}.T_{bud}$, & otherwise
%\end{numcases}


For $\gamma$ not too small $k(1-\gamma)/\gamma$ is a function of k. Usually $(1-f(l))$ is designed such that $B[T_{bud}] = \Theta (\ln T_{bud})$ in which case $B[T_{bud}]\geq \frac{k(1-\gamma)}{\gamma}$ for $T_{bud}$ exponentially large in $k$. 
This means that in general, we only need to consider the second condition of (\ref{eq.conditions}) i.e., $B[T_{bud}] < \frac{k(1-\gamma)}{\gamma}$.

As an example, assume that $\frac{\beta(l)}{1-\beta(l)} \leq \frac{1}{l}$, then $B(T_{bud}) = \ln(T_{bud})$ and
$\bar{w}(k,T_{bud}) \leq (\frac{1-\gamma}{\gamma}pd)^{k}\frac{1}{1-\gamma}e^{C/(1-\gamma)}T_{bud}^{1+1/(1-\gamma)}$, for $T_{bud} \leq e^{k(1-\gamma)/\gamma}$. The probability of winning for the adversary is exponentially small in $k$.

\begin{equation*}
\frac{\beta(l)}{1-\beta(l)} \leq \frac{1}{l} \iff \beta(l) \leq \frac{1}{l+1} \iff \sqrt{\frac{1-f(l)}{d}} \leq \frac{1}{l+1} \iff 1-f(l) \leq \frac{d}{(l+1)^2}
\end{equation*}

\saeed{From Marten notes: Still wish to do additional induction proof for $p(k,lT_{bud})$ Exercise for me!}

\saeed{analysis 5 starts here}

In practice, we may not immediately start learning at a rate $(1-f(l)) \approx d/(l+1)^2$. This will only happen after reaching for example $L^*$ samples. During such a first phase $(1-f(l)) \approxeq 1$ and the adversary tries to compromise as many, say $k^*$, nodes as possible before reaching $L^*$ levels.

For $(1-f(l)) \approxeq 1$, we have:


\begin{equation*}
\begin{aligned}
m_1(l) &= (1-\gamma)(1-(p+h))\\ 
m_2(l) &= (1-\gamma)p\\
m_3(l) &= \gamma p\\
m_4(l) &= [h-\gamma(h+p)]+\gamma=(1-\gamma)h+\gamma(1-p)\\
\end{aligned}
\end{equation*}

We are interested in $k^*$ as a function of $\epsilon$ for which 
\begin{eqnarray}\label{eq.k}
\sum_{k=0}^{k^{*}-1} p(k,L^{*}-1,T_{bud}-1)(\frac{m_4(l)}{1-m_1(l)}+\frac{m_3(l)}{1-m_1(l)}) +\\ p(k^*,L^{*}-1,T_{bud}-1)\frac{m_4(l)}{1-m_1(l)} \geq 1- \epsilon \nonumber
\end{eqnarray}

Then the probability of winning is 
\begin{equation}\label{eq.deta}
\leq \epsilon + (1-\epsilon)w(k-k^{*}(\epsilon),T_{bud})
\end{equation}

Notice that during phase one an $i>k^{*}(\epsilon)$  is reached ($\epsilon$ term in the above formula) and during phase two, another $k-k^{*}(\epsilon)$ horizontal or diagonal moves are needed in order to win (the second term).

We generalize the analysis of (\ref{eq.6}) for $(1-f(l))=1$ (without any constraint on $T_{bud}$):

\begin{eqnarray}\label{eq.delta}
(\ref{eq.k}) = \sum_{B=0}^{\infty}\sum_{k=B+1}^{k^{*}-1}(\ref{eq.a})(\ref{eq.b})(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)}) 
\end{eqnarray}

\saeed{Check \ref{eq.a} I guess the above should be L not l}
Notice that 

\begin{eqnarray*}
	\sum_{k=B+1}^{k^{*}-1}(\ref{eq.b}) &=& 
	\sum_{k=B+1}^{k^{*}-1}
		{	\sum_{\substack{g_0\geq 1,\dots,g_L^{*}\geq 1 s.t.\\
				\sum_{l=0}^{L^{*}}(g_l-1)=k-1-B}}
		\prod_{l=0}^{L^{*}} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g_l-1}
	}\\
	&=& \sum_{\substack{g'_0,\dots,g'_{L^*}\geq 0 s.t.\\
		\sum_{l=0}^{L^*-1}{g'_l \leq k^*-2-B}}}\prod_{l=0}^{L^*} \bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l}\\
	&\geq& \sum_{g'_0=0}^{(k^*-2-B)/L^*+1} \dots \sum_{g'_{L^*}=0}^{(k^*-2-B)/L^*+1} (\prod \dots)\\
	&=&  \prod_{l=0}^{L^*} \sum_{g'_l\geq 0}^{(k^*-2-B)/L^*+1}\bigg(\frac{m_2(l)}{1-m_1(l)} \bigg)^{g'_l} \\
	&=&	 \prod_{l=0}^{L^*}\frac{1}{1-\frac{m_2(l)}{1-m_1(l)}}\big(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \big)^{L^*+1} \\
	&=& \prod_{l=0}^{L^*} \frac{1-m_1(l)}{1-m_1(l)-m_2(l)}\bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \bigg)^{L^*+1}\\
	&=& \prod_{l=0}^{L^*} \frac{1-m_1(l)}{m_3(l)+m_4(l)}\bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-2-B}{L^*+1}+1} \bigg)^{L^*+1}
\end{eqnarray*}

\saeed{Missing part from the notes: Since $B\leq L^* \geq \bigg(1-(\frac{m_2(l)}{1-m_1(l)})^{\frac{k^*-1}{L^*+1}}\bigg)^{L^*+1}$}

And 

\begin{eqnarray*}
	\lefteqn{\sum_{B=0}^{\infty}(\ref{eq.a})(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)}) =} \\ & & 
	{ \sum_{\substack{b_1,\dots,b_L^*\in\{0,1\} s.t.\\ 
				\sum_{l=1}^{L^*}b_l=B}}
		\prod_{l=0}^{L^*-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)  (\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})}\\
& =&	{ \sum_{b_1,\dots,b_L^*\in\{0,1\}}\prod_{l=0}^{L^*-1} \bigg( b_{l+1}\frac{m_3(l)}{1-m_1(l)} + (1-b_{l+1})\frac{m_4(l)}{1-m_1(l)} \bigg)(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})
}\\
&=&\prod_{l=0}^{L^*}(\frac{m_3(l)}{1-m_1(l)}+\frac{m_4(l)}{1-m_1(l)})
\end{eqnarray*}

\saeed{Note From Marten's: In the write up we can refer in parts to the analysis of \ref{eq.6} in order to save space}

So we get 
\begin{eqnarray*}
(\ref{eq.k}) &\geq& \bigg(1-(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}} \bigg)^{L^*+1}\\
&\geq& 1 - (L^*+1)(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}}
\end{eqnarray*}

We want to solve $L\geq 1-\epsilon$

\begin{equation}\label{eq.star}
(L^*+1)(\frac{m_2}{1-m_1})^{\frac{k^*-1}{L^*+1}} = (L^*+1)[\frac{(1-\gamma)p}{1-(1-\gamma)(1-(p+h))}]^{\frac{k^*-1}{L^*+1}} \leq \epsilon
\end{equation}

Notice that $p \leq 1-h$, we have:
\begin{equation}
[\frac{(1-\gamma)p}{1-(1-\gamma)(1-(p+h))}] \leq (1-\gamma)(1-h).
\end{equation}

So, Equation (\ref{eq.star}) is satisfied for $k^*$ such that 

\begin{equation}
(L^*+1)[(1-\gamma)(1-h)]^{\frac{k^*-1}{L^*+1}} \leq \epsilon.
\end{equation}

\saeed{check equation delta \ref{eq.delta} reference, there are two of them deta and delta!}

Applying (\ref{eq.delta}) gives
probability of winning for 
\begin{equation*}
1-\tilde{f}(l)=\begin{cases}
1, & \text{if $l<L^*$}.\\
1-f(l-L^*), & \text{if $l \geq L^*$}.
\end{cases}
\end{equation*}
is 
\begin{equation}\label{eq.delta.1}
\leq (L^*+1)[(1-\gamma)(1-h)]^{\frac{k^*-1}{L^*+1}} + \bar{w}(k-k^*,T_{bud}), 
\end{equation}

where $\bar{w}$ can be computed through simulation or $\bar{w}$ has the special form as derived for $(1-f(x)) = \frac{d}{(1+x)^2}$.

We want to minimize Equation \ref{eq.delta.1} for $k^*$.
\saeed{Note: Need to do this}
This shows how $h$ plays a role as wel!? It is important in phase one.

We get some function $g(k,T_{bud})\geq Prob(win)$.


\subsection{Security Capacity}

$T_{bud} \leq 2^t$, and $Prob(win) \leq 2^{-s}$ is implied by $\hat{g}(k,2^t) \leq 2^{-s}$. After taking the logarithm in base 2 we get
\begin{eqnarray} \label{eq.secCap}
s \leq -\log\hat{g}(k,2^t)
\end{eqnarray}

We need to figure out what equation \ref{eq.delta.1} gives.
\ref{??} should lead to a bound of the form $\delta . s + \eta t \leq g(k,t)$, where $g(k,t)= \Theta(k)$ behaving like $\zeta k $ for large $k$.

Then, the triples $(\delta , \eta , \zeta)$ defines a \emph{security capacity region}:

For $T_{bud} \leq 2^t$ the probability of reaching state $k$ is at most $2^{-s}$ if $\delta s + \eta t \leq g(k,t) \approx \zeta k$.

We can show in a paths (graphs?) how this behaves for several parameter settings (our simulations etc)
\saeed{can we compute actually examples?}

Take $s=t=128$ For different $p,\gamma,h$ we can plot for which minimal $k$ the above bound holds. Larger $k$ cannot be achieved in $2^{128}$ time budget and winning prob $\geq 2^{-128}$!

\saeed{General lemma: Nice for eprint: we donot make use of it in our bounds}

\textbf{Composition}

Suppose for fixed $h,p,\gamma$ we have:
$s+t \leq g_1(k,t)$ for $f_1(l)$, assume $g_1(k,t)$ is an increasing function,
$s+t \leq g_2(k,t)$ for $f_2(l+L^*)$ (we start at level $L^*$ rather than $0$), assume $g_2(k,t)$ is an increasing function.

Let 

\begin{equation*}
f(l)=\begin{cases}
f_1(l), & \text{if $l \leq L^*$}.\\
f_2(l), & \text{if $l > L^*$}.
\end{cases}
\end{equation*}

Given $2^t$ timesteps then with $prob \leq 2^{-s}$ we achieve $k$, for $s+t \leq g_1(k)$ or $g_1^{-1}(s+t) \leq k_1$ if we use $f_1(l)$.
So within $2^t$ timesteps before $l=L^*$ is reached (another restriction) we have with $prob \leq 2^{-s}$ we achieve $k_1 = g_1^{-1}(s+t)$,
or with $prob \geq (1-2^{-s})$ we have $k_1 \leq g_1^{-1}(s+t)$.
We give the adversary an advantage with $prob\geq (1-2^{-s})$, if we upgrade him to position $k_1= g_1^{-1}(s+t)$ once $L^*$ is achieved. And we again give him $2^t$ timesteps. Now $f_2(l+L^*)$ is being used for $l\geq 0$. With $prob \leq 2^{-s}$ another 
$k_2 \geq g_2^{-1}(s+t)$ positions are gained.

So, given  $2^t$ time steps, with $prob \leq 2^{-s} + 2^{-s} = 2^{-(s-1)}$, $k \geq g_1{-1}(s+t) + g_2{-1}(s+t)$ is reached.
Define $g(g_1{-1}(s+t)+g_2^{-1}(s+t)) = s+ t$. Then for $f(l): s'+t \leq g(k) -1$ where $s'=s-1$. 
The above shows how $(1-f_1(l)) \leq d/l$ for $l \leq L^*$ and $\tau_{low} \leq 1-f_2(l) \leq \tau_{up} < 1$ for $l > L^*$ compose.
Note that this also holds for $(1-f_2(l+L^*))$, independent of the level.

So we have $s+t \leq g_1(k)$ of Th1 and $s+t \leq g_2(k)$ of Th2.
\saeed{Th? Theorem 1 and 2?}

and we obtain for the composed $f$:
$s+t \leq g(k) -1$, where $g^{-1}(x) = g_1^{-1}(x) + g_2^{-1}(x)$.

Assymptotics: $g_1(k) \sim \alpha_1.k$ and $g_2(k) \sim \alpha_2.k$, therefore, $g(k) = \frac{\alpha_1 \alpha_2}{\alpha_1 + \alpha_2}.k$ worse than $g_2(k)$: $1-f(l) \geq 1-f_2(l)$ for $l \leq L^*$, so $f$ is worse than $f_2$!

In our (???) case $\alpha_1 \gg \alpha_2$ we get $g(k) \sim \alpha_2 k$. Hence, the effect of $f_2(l)$ really matters. It does not matter how one learns $ \tau_{low} \leq (1-f_2(l)) \leq \tau_{up}$ after $L^*$ levels.


\textbf{Important for eprint/paper:}
Rate of play:
Suppose $s+t \leq g(k)$. Suppose 1 adversarial move (i.e., one transition in the Markov model) takes $\Delta$ time. Suppose we have $T$ time step budget. If $k$ nodes are infected after $T$ time, then at most $\frac{T}{\Delta k}$ moves have been made.
If $s + \log(\frac{T}{\Delta k}) \leq g(k)$, then with probbaility $\leq 2^{-s}$ state $k$ is reached. Hence, $s+ t' \leq g(k) + \log k$ gives $prob_{win} \leq 2^{-s}$ where $t' = \log(\frac{T}{\Delta})$.

Notice if the time budget $T \leq \Delta. 2^{t'}$, then with $prob \leq 2^{-s}$, a state $k$ with $s+t' \leq g(k) + \log k$ can be reached.
Now if $g(k) = \Theta(k)$, then we get pretty much the same secrecy capacity. So ``real time with parallel adversarial moves" can be interchanged with ``Total number of moves/transition steps/time steps" good news!

\saeed{Analysis 6 starts from here: Sort of TODS and FUTURE WORKS}

1 - Given a model on rate of adversarial play (see also $T_{bud} \rightleftarrows time$ analysis, can a defender estimate how many nodes have been compromised given when $l$ got incremented?

We can estimate function $1-f(l)$ and extrapolate; leads to a bound on reaching $k$.
This could be very helpful. The defender knows when to invest resources w.r.t. a certain type of attack in order to get a better curve for $1-f(l)$!?

2 - Given our Markov model, suppose the defender can prove that he invest resources to reach a certain $1-f(l),h,\gamma$. Then the adversary believes in the bound dictated by the secrecy capacity and will be discuraged to move at all (econimically motivated adversay). How do we design such a proof.

3 -  FlipIt: Show the equilibrium game and also analyze how both parties can profit more if D can prove its strategy to A.

In general, can 2kp be used to change games for mutual additional gain?
(Did Micali do this stuff? Prof at CSAIL? Silvio Micali? )

4 - Current paper and TODO 1 can lead to a webtool? What about other Markov models and their analysis?

5 - Cheers!
%\begin{eqnarray} \label{eq.w}
%&=&	\sum_{L=0}^{w(k,T_{bud})} p(k-1,L,T_{bud}-1).	 [\frac{m_2(L)}{1-m_1(L)}+\frac{m_3(L)}{1-m_1(L)}]\\
%\end{eqnarray}


% \RandomWalk {number = 50,length = 4pt, angles = {0,45,90}, degree}
 
 
%The winning state for the adversary is state $k \ll K$. 
%\saeed{Missing: a Figure for sample path l based on i} 
%
%Suppose we arrived at level $l$ in state $i_l$. Suppose we enter at level $l+1$ in state $i_{l+1}$.
%
%\textbf{Case 1: $i_{l+1}=i_l$} Lets denote the number of times the adversary stays in state $(i_l,l)$ by $T_l$ and after that it makes a transition to the state $(i_{l+1}=i_l,l+1)$. This can happen in $T_{l}+1$ time steps with probability $m_1(l)^{T_l}. m_4(l)$
%
%\textbf{Case 2: $i_{l+1}>i_l$} \\
%\textit{(2-a):}
%Consider the following sample path which can happen in $T_{l}+i_{l+1}-i_{l}+1$ time steps with probability $m_1(l)^{T_l}.m_2(l)^{i_{l+1}-i_{l}} .m_4(l)$ where $T_l = t(i_l)+\dots+t(i_{l+1})$.
%\saeed{Missing: a Figure for sample path l based on i} 
%
%\textit{(2-b):}
%Consider the following sample path which can happen in $T_{l}+i_{l+1}-i_{l}$ time steps with probability $m_1(l)^{T_l}.m_2(l)^{i_{l+1}-1-i_{l}} .m_3(l)$ where $T_l = t(i_l)+\dots+t(i_{l+1})$.
%\saeed{Missing: a Figure for sample path l based on i} 
%
%\textbf{Case 3: We have arrived at the highest level $L$ before entering the winning state $(i_L < k)$:} \\
%\textit{(3-a):}
%Define $T_L = t(i_L)+\dots+t(k-1)$
%This sample path happens with probability $m_1(L)^{T_L}.m_2(L)^{k-i_L}$ in $T_L+k-i_L$ time steps.\\
%\textit{(3-b):}
%Define $T_L = t(i_L)+\dots+t(k-1)$
%This sample path happens with probability $m_1(L)^{T_L}.m_2(L)^{k-1-i_L}m_3(L)$ in $T_L+k-i_L$ time steps.\\
%
%Path towards a winning state:
%$0=i_1 \leq i_2 \leq \dots \leq i_L <k$
%We use the following notaion:
%$0=j_1 \leq j_2 \leq \dots \leq i_R <k$,
%$\sum_{n=1}^{R} r_n = L$ with $r_1,\dots,r_R \geq 1$. Therefore,\\
%$j_1=(0=i_1=\dots=i_{r_1}) < j_2 =(i_{r_1+1}=\dots=i_{r_1+r_2}) < j_3 = (i_{r_1+r_2+1}=\dots=i_{r_1+r_2+r_3}) < \dots$





%We prove Theorem \ref{Theorem.Cost}:
% Let $A_{i,j}$ represent the probability the adversary moves in state $i$ and reaches state $j$ as a consequence of the move. Let the real number $c_{i,j}\geq 0$ indicate the adversarial cost associated to $A_{i,j}$. Then 
%\begin{equation}\label{eq.rho}
%\alpha = \sum_{i,j}{\pi_i  A_{i,j}  c_{i,j}}  
%\end{equation}
% is a convex combination of costs $c_{i,j}$ (since $\sum_{i,j} \pi_i  A_{i,j} \leq \sum_{i,j} \pi_i  M_{i,j}= \sum_j \pi_j =1$). We need to prove that
%the probability  the attacker wins the $M$-MTD game by paying at most $C$ is
%	$$\leq \frac{C\cdot \pi_{k}}{\sum_{i,j}{\pi_i  A_{i,j}  c_{i,j}} }. $$
%
%
%	We first introduce a mapping of matrix $M$ to a new matrix $M^{*}$ which we can analyze using our theorem but has all the necessary cost information embedded:
%	
%	First, we split each transition from state $i$ to state $j$ with probability $M_{i,j}$ into two transitions. One from $i$ to $j$ with probability $A_{i,j}$ and the other from $i$ to $j$ with probability $D_{i,j}=M_{i,j}-A_{i,j}$: $A_{i,j}$ represents the probability that the adversary moves in state $i$ and reaches state $j$ as a consequence of that move, while $D_{i,j}$ represents the probability of a defender's move or no move (if $i=j$) from state $i$ to state $j$.
%	
%	Second, let $c_{i,j}\geq 0$ be a real number representing the cost for the adversary if he moves from $i$ to $j$ with probability $A_{i,j}$. Let $\epsilon \geq 0$ (later in the proof we will take the limit $\epsilon \rightarrow 0$) and define	
%	\begin{equation*} \label{eq.Int.Cost}
%	C_{i,j} = \lceil \frac {c_{i,j}}{\epsilon} \rceil \in \mathbb{N}
%	\end{equation*}
%	
%	We transform each edge from $i\rightarrow j$ with probability $A_{i,j}$ into a path $i\rightarrow (i,j;1)\rightarrow (i,j;2)\rightarrow \ldots \rightarrow (i,j;C_{i,j})\rightarrow j$ with probabilities as depicted in Figure~\ref{fig.Transfer}. The transition  $i\rightarrow (i,j;1)$ has probability $A_{i,j}$. If $C_{i,j}=0$, then $i$ is directly connected to $j$ without intermediary nodes and $i\rightarrow j$ is transitioned with probability $A_{i,j}$ by the adversary. We denote the transformed matrix by $M^{*}$.
%	
%	
%	\begin{figure}[h!]
%		\begin{center}
%			\scalebox{0.60}
%			{\includegraphics{Transf2.pdf}}%Transf
%			\caption{Each transition $M_{i,j}$ from $i\rightarrow j$ will be replaced with above transition from state $i$ to $j$}
%			\label{fig.Transfer}
%		\end{center}
%	\end{figure}
%	
%	
%	
%	\begin{lemma} \label{lem:cost} If $M$ has an stationary probability distribution $\pi$, then $M^{*}$ has an stationary distribution $\pi^{*}$ defined by:
%		\begin{eqnarray}
%		\pi^{*}_{i}&=&\frac{\pi_{i}}{1+\alpha} \mbox{ and } \nonumber \\ %\label{eq.piStar}\\ 
%		\pi^{*}_{i,j;h}&=&\frac{\pi_{i} \cdot A_{i,j}}{1+\alpha} \mbox{ for } 1\leq h \leq C_{i,j}.	\nonumber
%		\end{eqnarray}
%	\end{lemma}
%	
%	
%	\noindent
%	{\bf Proof.} From $\pi^{*}=\pi^{*} M^{*}$ and the definition of $M^{*}$ we infer the following equations:
%	\begin{eqnarray*}
%		\pi^{*}_{i,j;1}&=&{\pi^{*}_{i}}\cdot A_{i,j}, \hspace{1cm} \mbox{    if } C_{i,j}\geq 1, \\  	
%		\pi^{*}_{i,j;h+1}&=&\pi^{*}_{i,j;h}, \hspace{1.3cm} \mbox{         for } 1\leq h \leq C_{i,j},  	\\
%		%\begin{equation}
%		\pi^{*}_{j} &=& \sum_{i} \pi^{*}_i D_{i,j} + \sum_{\substack{i \\ C_{i,j}\neq 0}} \pi^{*}_{i,j;C_{i,j}} + \sum_{\substack{i \\ C_{i,j}= 0}} {\pi^{*}_{i}}\cdot A_{i,j}.
%		%\end{equation}
%	\end{eqnarray*}
%	By combining the above equations we have,
%	\begin{eqnarray*}
%		\pi^{*}_{j}&=& \sum_{i} \pi^{*}_i D_{i,j} + \sum_{\substack{i \\ C_{i,j}\neq 0}} \pi^{*}_{i,j;1} + \sum_{\substack{i \\ C_{i,j}= 0}} {\pi^{*}_{i}}\cdot A_{i,j}\\
%		&=& \sum_{i} \pi^{*}_i D_{i,j} + \sum_{\substack{i}} {\pi^{*}_{i}}\cdot A_{i,j}
%		= \sum_{i} \pi^{*}_i M_{i,j}
%	\end{eqnarray*}
%	We conclude that the vector $(\pi^{*}_1,\pi^{*}_2,...)$ is proportional to vector $\pi$ and this proves $\pi^*_i=\pi_i/\rho$ for some $\rho$. 
%	%the form of (\ref{eq.piStar}).
%	As a result
%	$$
%	\pi^{*}_{i,j;h}= \pi^{*}_{i,j;1}= \pi^{*}_i \cdot A_{i,j} = \frac {\pi_i \cdot A_{i,j}}{\rho}  \mbox{ for } 1\leq h \leq C_{i,j}.
%	$$
%	
%	The proportionality factor $\rho$ satisfies
%	\begin{eqnarray*}
%		1&=& \sum_{i}{\pi^{*}_i} + \sum_{\substack{i,j,h \\ C_{i,j}\neq 0\\1\leq h \leq C_{i,j}}} {\pi^{*}_{i,j;h}} \\
%		&=& \sum_{i}{\frac{\pi_i}{\rho}} + \sum_{\substack{i,j,h \\ C_{i,j}\neq 0\\1\leq h \leq C_{i,j}}}{\frac {\pi_i \cdot A_{i,j}}{\rho}} \\
%		&=& \sum_{i} \frac{\pi_i}{\rho} + \sum_{i,j}{\frac{\pi_i \cdot A_{i,j} \cdot C_{i,j}}{\rho}}
%	\end{eqnarray*}
%	Together with $\sum_{i} {\pi_i}=1$ and (\ref{eq.rho}), this proves $\rho=1+\alpha$  and the lemma follows.
%	
%	In order to prove the theorem we introduce new random variables:
%	%
%	Let $T_{M}$ be the random variable indicating the number of transitions $i\xrightarrow{D_{i,j}}j$, $i\xrightarrow{A_{i,j}}(i,j;1)$ (if $C_{i,j}\geq 1$) and $i\xrightarrow{A_{i,j}}j$ (if $C_{i;j}=0$), made before the adversary wins the MTD-game corresponding to $M^{*}$. 
%	
%	Let $T_{C}=\sum_{i,j}{N_{i,j}\cdot C_{i,j}}$ be the random variable indicating the number of all other transitions where $N_{i,j}$ represents the random variable counting the number of times the path$(i,j;1)\xrightarrow{1}(i,j;2)\xrightarrow{1}\ldots\xrightarrow{1}(i,j;C_{i,j})$ is traversed.
%	Notice that $T=T_M + \sum_{i,j}{N_{i,j}}$ is the random variable representing the number of transitions in the $M$-MTD game before the attacker wins the game.
%	
%	Let the random variable $C_R$ represent the real cost of the adversary before he wins the MTD-game corresponding to $M$. Notice that,  for  random variables $N_{i,j}$ in the MTD-game corresponding to $M^{*}$,
%%	\begin{eqnarray}
%$$	C_R = \sum_{i,j}{N_{i,j}\cdot c_{i,j}}. $$
%%	\end{eqnarray}
%	This  shows how the MTD games based on $M$ and $M^*$ are related.
%	
%	We derive
%	\begin{eqnarray}
%	T_C &=& \sum_{i,j}{N_{i,j}\cdot C_{i,j}} = \sum_{i,j}{N_{i,j}\cdot \lceil \frac{c_{i,j}}{\epsilon} \rceil} \nonumber \\
%	&=& \frac{1}{\epsilon} \sum_{i,j}{N_{i,j}\cdot (\lceil  \frac{c_{i,j}}{\epsilon} \rceil \cdot \epsilon )} \nonumber \\
%	&=& \frac{1}{\epsilon} \sum_{i,j}{N_{i,j}\cdot c_{i,j}} + \frac{1}{\epsilon} \sum_{i,j}{N_{i,j}\cdot (\lceil \frac{c_{i,j}}{\epsilon} \rceil \cdot \epsilon - c_{i,j})} \nonumber \\
%	&=& \frac{C_R}{\epsilon} + E 
%	\mbox{ where } 
%	0\leq E \leq \sum_{i,j}{N_{i,j}} \label{eq.error}
%	\end{eqnarray}
%	
%	Since $T=T_M + \sum_{i,j}{N_{i,j}}$ represents the number of transitions in the $M$-MTD game before the attacker wins the game, we can use Theorem \ref{theo-single} in combination with (\ref{eq.error}) and derive for all $t$:
%	\begin{eqnarray}
%	&& \frac{C\cdot \pi^*_{k}}{\epsilon}  \label{Eq.c} \\
%	&\geq & Prob(T_M+T_C \leq \frac {C}{\epsilon}) 
%	= Prob(T_M+\frac{C_R}{\epsilon}+E \leq \frac {C}{\epsilon}) \nonumber \\
%	&=& Prob(C_R\leq C-\epsilon(T_M+E)) \nonumber \\
%	&\geq&Prob(C_R\leq C-\epsilon t | T_M+E\leq t)Prob(T_M+E\leq t) \nonumber \\
%	&=&Prob(C_R\leq C-\epsilon t)- \nonumber \\& &
%	Prob(C_R\leq C-\epsilon t | T_M+E \geq t)Prob(T_M+E \geq t) \nonumber \\
%	&\geq&Prob(C_R\leq C-\epsilon t) - Prob(T_M+E\geq t) \nonumber \\
%	&\geq&Prob(C_R\leq C-\epsilon t) - Prob(T_M+ \sum_{i,j}{N_{i,j}}\geq t) \nonumber \\
%	&=& Prob(C_R\leq C-\epsilon t) - Prob(T\geq t). \label{Eq.5}
%	\end{eqnarray}
%	If we choose $\epsilon=\frac{1}{t^{2}}$ and let $t\rightarrow \infty$ then (\ref{Eq.5}) tends to $Prob(C_R \leq C)$.
%	
%	We now analyse upper bound (\ref{Eq.c}) by using Lemma \ref{lem:cost}:
%	$$
%	\frac{C\cdot \pi^*_{k}}{\epsilon}= \frac{C\cdot \pi_{k}}{\epsilon (1+\alpha)}, \mbox{ where}
%	$$
%%	where
%	\begin{eqnarray*}
%		\epsilon (1+\alpha) &=& \epsilon + \sum_{i,j}{\pi_i A_{i,j}  C_{i,j} \cdot \epsilon}
%		= \epsilon +  \sum_{i,j}{\pi_i  A_{i,j} 
%			\lceil \frac{c_{i,j}}{\epsilon}\rceil  \epsilon}\\
%		&=& \epsilon +  \sum_{i,j}{\pi_i A_{i,j}  c_{i,j}}  + \sum_{i,j}{\pi_i  A_{i,j} 
%			(\lceil \frac{c_{i,j}}{\epsilon} \rceil  \epsilon - c_{i,j})}
%	\end{eqnarray*}
%	Hence,
%	\begin{eqnarray*}
%	&&	\epsilon (1+\alpha) -  \sum_{i,j}{\pi_i A_{i,j} c_{i,j}} \leq \epsilon + \sum_{i,j}{\pi_i  A_{i,j} 
%			(\lceil \frac{c_{i,j}}{\epsilon} \rceil  \epsilon - c_{i,j})}\\
% &&\leq \epsilon + \sum_{i,j}{\pi_i  M_{i,j} 
%			\epsilon}
%		= \epsilon +  \sum_{j}{\pi_j  
%			\epsilon} = 2\epsilon.
%	\end{eqnarray*}
%	This proves that,
%	for $\epsilon=\frac{1}{t^{2}}$ and $t\rightarrow \infty$,  $\epsilon (1+\alpha) \rightarrow \sum_{i,j}{\pi_i A_{i,j} c_{i,j}}=\alpha$ and the theorem follows:
%	\begin{equation}
%	Prob(C_R \leq C) \leq C\cdot \pi_k /\alpha. \nonumber %\frac{C\cdot \pi_{k}}{\sum_{i,j}{\pi_i  A_{i,j}  c_{i,j}} }. \nonumber
%	\end{equation}


==> sections/sim.tex <==
%Fig. \ref{fig.wbar} depicts $\bar{w}(k,T_{bud})$ as a function of $k$  with $T_{bud}=10,000$ for several $\gamma$ and  several learning rates represented by $\alpha(l)= (l+1)^{-a}$, see (\ref{eq-alpha}). 
%%based on $k$ for different $\gamma$ values while the adversary has $T_{bud)=10,000$ logical timesteps available to it in order to construct its zombie army. Four different  polynomial learning functions are considered for the defender for four different $\gamma$. 
%This plot shows the importance of having a proper defense learning mechanism in order to be able to contain the adversary. Clearly, $k$ remains small $<100$ with high probability for sufficiently fast converging learning rates and large enough $\gamma$.
%Fig. \ref{fig.kc} depicts how the containment parameter $k_c$ (computed using $\bar{w}(k,T_{bud})$) depends on $\alpha(l)= (l+1)^{-a}$. For $a\geq 0.9$, $k_c\leq 20$ is very small making it impossible for the adversary to construct its zombie army.
%
%\begin{figure*}%[h!]
%	\begin{center}
%		\scalebox{0.65}
%		{\includegraphics{figure2k50_gammaED}}
%		\caption{$\bar{w}(k,T_{bud})$ based on different values of $\gamma$ and learning functions $\alpha(l) = (l+1)^{-a}$ where $T_{bud} = 10,000$ logical timesteps}
%		\label{fig.wbar}
%	\end{center}
%\end{figure*}
%
%\begin{figure}%[h!]
%	\begin{center}
%		\scalebox{0.43}
%		{\includegraphics{kc}}
%		\caption{$k_c$ for different classes of learning functions $\alpha(l) = (l+1)^{-a}$ where $T_{bud} = 10,000$ logical timesteps}
%		\label{fig.kc}
%	\end{center}
%\end{figure}
%
%Fig. \ref{fig.roleOfp} depicts that even in the extreme cases that $\%10$ of the population is vulnerable, with $\gamma = 0.5$ meaning that half of the adversary's packets will be marked as suspicious on the flow classifier level, and while $\%0.1$ of the address space are honeypots, the adversary's probability of success (even for a small size botnet) is negligible with a good defense mechanism in place. In the same figure, $p =1$ represents the case of the strongest adversary equipped with a precompiled list of vulnerable nodes, i.e., a hitlist, meaning that it does not require to probe the network environment which gives the defender the minimum number of malware samples. Notice that in this case, at each time step, the adversary only hits a vulnerable node ($p=1, h= 0$). Even for such a strong adversary, the simulation shows that with a proper learning rate mechanism in place, chances of constructing a botnet for the attacker are minimal.
%\begin{figure}%[h!]
%	\begin{center}
%		\scalebox{0.43}
%		{\includegraphics{figureP_hitlist}}
%		\caption{$\bar{w}(k,10000)$ for extreme cases $p=0.10$ and $p=1$ with $\gamma=0.5$ and learning function $1-f(l) = (l+1)^{-a}$ where $a=0.6$ and $a=1$ respectively.}
%		\label{fig.roleOfp}
%	\end{center}
%\end{figure}
%%\begin{algorithm}
%%	\caption{$\bar{w}$ Computation}
%%	\label{alg:wbar}
%%	\begin{algorithmic}[1]
%%		\Function{$\bar{w}$}{$k,l,\gamma$}
%%		\State {$A \gets prob(k-1,l,\gamma)[k-1,...]$}
%%		\State{$\bar{w}\gets 0$}
%%		\For{$i\gets 0,l$}
%%		\State{$\bar{w} \gets \bar{w}+\alpha(i)A[i]$}
%%		\EndFor{;}
%%		\Return{$\bar{w}$;}
%%		\EndFunction
%%		\Statex
%%		\Function{$prob$}{$k,l,\gamma$}
%%		\State{$pr \gets zeros[k,l]$}
%%		\For{$i\gets 0,l$}
%%		\If{$i == 0$}\State{$pr[0,i]\gets 1$}
%%		\Else \State{$pr[0,i]\gets(1-\alpha(i-1))pr[0,i-1]$}
%%		\EndIf
%%		\For{$j \gets 1,k$}
%%		\If{$i==0$}\State{$pr[j,i]\gets [(1-\gamma)\alpha(0)]^{j}$}
%%		\Else \State{$pr[j,i]\gets (1 - \gamma)\alpha(i)pr[j-1,i] + \gamma \alpha(i - 1) pr[j-1,i-1] + (
%%			1 - \alpha(i - 1))pr[j,i-1]$}
%%		\EndIf
%%		\EndFor
%%		\EndFor{;}
%%		\Return{$pr$;}
%%		\EndFunction
%%		\Statex
%%		\Function{$\alpha$}{$l,a$}
%%		\Return{$(l+1)^{-a}$}
%%		\EndFunction
%%	\end{algorithmic}
%%\end{algorithm}
%
%Fig. \ref{fig.delayed} shows the importance of learning the adversarial moves as soon as possible. It compares the value of $k_c$ as the adversarial containment parameter for two different cases. In the first scenario the learning starts immidiately and with no delay (i.e., $L^{*}=0$) and in the second case the defeder misses only the first 100 malware samples (i.e., $L^*=100$). 
%
%%means_a0 = (100, 29, 11)
%%means_a1 = (300, 228, 210)
%\begin{figure}%[h!]
%	\begin{center}
%		\scalebox{0.43}
%		{\includegraphics{delayedLearning}}
%		\caption{The impact of delayed learning on $k_c$ for different classes of learning functions $\alpha(l) = (l+1)^{-a}$ where $T_{bud} = 10,000$ logical timesteps}
%		\label{fig.delayed}
%	\end{center}
%\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%% New simulations
Taking the CodeRed1v2 worm as an example, we apply our model to answer the following questions. First, we want to see how practical is the assumption of giving the adversary the advantage of $p= \sup_i p_i$ in our analysis. 
Second, with comparison to the well-accepted deterministic simple epidemic model (see equation \ref{eq.DE}, with no removal rates), we want to see how the simulations based on the Algorithm \ref{alg:sim} behave with and without learning rates. Third, based on these results, we want to see how the proposed learning functions and the analytical analysis in the previous sections perform while plugging in the codeRed worm actual parameters and converting the Markov model logical time steps to actual time (measured in seconds).

In the codeRed1v2 epidemic, we consider the address space to be $N = 2^{32}$ (the entire IPv4 address space), the approximate number of nodes susceptible to the malware to be $K=350,000$ (i.e., $p=8.15 \times 10^{-5}$), and the number of scans performed by an infected machine to be $10188$ scans per hour, and an initially one infected machine at time zero. 

This figure shows ...
\begin{figure}%[h!]
	\begin{center}
		\scalebox{0.45}
		{\includegraphics{simulation1_fv.eps}}
		\caption{$(a)$ Depicts the plot for the solution of the differential equation \ref{eq.DE} with the actual codeRed1v2 parameters. $(b)$ Depicts the simulation of the codeRed1v2 with the same parameters while the learning function is of the form $f(l)= 1- 1/(l/10000 +1)$ and $\gamma = 0.01$ as the classifier's accuracy}
		\label{fig.comparison}
	\end{center}
\end{figure}

%% missing plot simulation of codeRED for different cases
\begin{figure}%[h!]
	\begin{center}
		\scalebox{0.45}
		{\includegraphics{simulations.eps}}
		\caption{No learning, vs learning}
		\label{fig.Sim_ODE_Learning}
	\end{center}
\end{figure}


Fig. \ref{fig.lastOne} depicts $\bar{w}(k,T_{bud})$ for a fixed learning function of the form $f(l)= 1- 1/(l/1000 +1)$, while $p=8.15 \times 10^{-5}$, and $\gamma = 0.05$ as the classifier's accuracy. By doing  a simple extrapolation, we notice that for a time window of a month (i.e., $T_{bud} \leq 31 * 24 * 10188$ adversarial moves for the CodeRed example), and $\bar{w}$ set to $2^{-128}$, the value of $k$ would be almost 130 infected nodes. This means that in practice, with this attack-defense parameters, the probability that the attacker constructs an army of 130 infected nodes wihtin a one-month time window would be at most $2^{-128}$ which depicts how important the learning function is when it comes to containing the adversary.

\begin{figure}%[h!]
	\begin{center}
		\scalebox{0.45}
		{\includegraphics{Lastfig.eps}}
		\caption{$\bar{w}(k,T_{bud})$ for different values of $T_{bud} = 2^{t}, 8\leq t \leq 14$ with a fixed learning function of the form $f(l)= 1- 1/(l/1000 +1)$, $p=8.15 \times 10^{-5}$, and $\gamma = 0.05$ as the classifier's accuracy}
		\label{fig.lastOne}
	\end{center}
\end{figure}
